Deterministic Kalman filters for uncertain dynamical systems

The Kalman(-Bucy) filter is the natural choice for the state reconstruction of disturbed, linear dynamical systems based on flawed and incomplete measurements. Taking a deterministic viewpoint this work investigates possible extensions of the concept to systems with uncertain dynamics and noise covariances. In a theoretical analysis error bounds in terms of the variance of the uncertainties are derived. The article concludes with a numerical implementation of two example systems allowing for a comparison of the estimators.

==> Data/Oscillator/sigma01/kf_en_pos.tex <==
    \addplot[
    thick,
    dashed,
    cyan
    ]
    table {
         0    1.0000
    0.0100    0.9972
    0.0200    0.9928
    0.0300    0.9838
    0.0400    0.9791
    0.0500    0.9755
    0.0600    0.9713
    0.0700    0.9672
    0.0800    0.9638
    0.0900    0.9550
    0.1000    0.9461
    0.1100    0.9477
    0.1200    0.9491
    0.1300    0.9486
    0.1400    0.9457
    0.1500    0.9413
    0.1600    0.9382
    0.1700    0.9349
    0.1800    0.9296
    0.1900    0.9234
    0.2000    0.9188
    0.2100    0.9137
    0.2200    0.9096
    0.2300    0.9120
    0.2400    0.9096
    0.2500    0.9033
    0.2600    0.8974
    0.2700    0.8925
    0.2800    0.8938
    0.2900    0.8884
    0.3000    0.8847
    0.3100    0.8825
    0.3200    0.8762
    0.3300    0.8746
    0.3400    0.8718
    0.3500    0.8705
    0.3600    0.8736
    0.3700    0.8734
    0.3800    0.8661
    0.3900    0.8589
    0.4000    0.8534
    0.4100    0.8471
    0.4200    0.8406
    0.4300    0.8346
    0.4400    0.8336
    0.4500    0.8312
    0.4600    0.8251
    0.4700    0.8220
    0.4800    0.8207
    0.4900    0.8181
    0.5000    0.8153
    0.5100    0.8133
    0.5200    0.8093
    0.5300    0.8048
    0.5400    0.8008
    0.5500    0.7948
    0.5600    0.7901
    0.5700    0.7867
    0.5800    0.7820
    0.5900    0.7775
    0.6000    0.7744
    0.6100    0.7714
    0.6200    0.7674
    0.6300    0.7633
    0.6400    0.7592
    0.6500    0.7539
    0.6600    0.7491
    0.6700    0.7471
    0.6800    0.7430
    0.6900    0.7397
    0.7000    0.7370
    0.7100    0.7317
    0.7200    0.7261
    0.7300    0.7200
    0.7400    0.7138
    0.7500    0.7085
    0.7600    0.7057
    0.7700    0.7030
    0.7800    0.6991
    0.7900    0.6968
    0.8000    0.6909
    0.8100    0.6836
    0.8200    0.6793
    0.8300    0.6756
    0.8400    0.6705
    0.8500    0.6636
    0.8600    0.6589
    0.8700    0.6547
    0.8800    0.6503
    0.8900    0.6455
    0.9000    0.6384
    0.9100    0.6330
    0.9200    0.6298
    0.9300    0.6274
    0.9400    0.6227
    0.9500    0.6156
    0.9600    0.6088
    0.9700    0.6030
    0.9800    0.5977
    0.9900    0.5936
    1.0000    0.5890
    1.0100    0.5816
    1.0200    0.5758
    1.0300    0.5723
    1.0400    0.5679
    1.0500    0.5614
    1.0600    0.5559
    1.0700    0.5500
    1.0800    0.5440
    1.0900    0.5400
    1.1000    0.5361
    1.1100    0.5301
    1.1200    0.5237
    1.1300    0.5184
    1.1400    0.5147
    1.1500    0.5119
    1.1600    0.5074
    1.1700    0.5035
    1.1800    0.4991
    1.1900    0.4931
    1.2000    0.4891
    1.2100    0.4862
    1.2200    0.4828
    1.2300    0.4788
    1.2400    0.4738
    1.2500    0.4692
    1.2600    0.4645
    1.2700    0.4595
    1.2800    0.4553
    1.2900    0.4514
    1.3000    0.4471
    1.3100    0.4423
    1.3200    0.4386
    1.3300    0.4338
    1.3400    0.4284
    1.3500    0.4249
    1.3600    0.4212
    1.3700    0.4162
    1.3800    0.4117
    1.3900    0.4071
    1.4000    0.4025
    1.4100    0.3981
    1.4200    0.3933
    1.4300    0.3888
    1.4400    0.3852
    1.4500    0.3814
    1.4600    0.3780
    1.4700    0.3733
    1.4800    0.3671
    1.4900    0.3627
    1.5000    0.3579
    1.5100    0.3521
    1.5200    0.3472
    1.5300    0.3434
    1.5400    0.3393
    1.5500    0.3352
    1.5600    0.3304
    1.5700    0.3252
    1.5800    0.3205
    1.5900    0.3157
    1.6000    0.3109
    1.6100    0.3080
    1.6200    0.3044
    1.6300    0.3001
    1.6400    0.2954
    1.6500    0.2912
    1.6600    0.2871
    1.6700    0.2823
    1.6800    0.2779
    1.6900    0.2734
    1.7000    0.2695
    1.7100    0.2650
    1.7200    0.2622
    1.7300    0.2591
    1.7400    0.2541
    1.7500    0.2513
    1.7600    0.2478
    1.7700    0.2432
    1.7800    0.2388
    1.7900    0.2346
    1.8000    0.2311
    1.8100    0.2274
    1.8200    0.2235
    1.8300    0.2192
    1.8400    0.2160
    1.8500    0.2117
    1.8600    0.2057
    1.8700    0.2014
    1.8800    0.1974
    1.8900    0.1930
    1.9000    0.1884
    1.9100    0.1834
    1.9200    0.1790
    1.9300    0.1747
    1.9400    0.1702
    1.9500    0.1659
    1.9600    0.1614
    1.9700    0.1579
    1.9800    0.1542
    1.9900    0.1507
    2.0000    0.1477
    2.0100    0.1431
    2.0200    0.1386
    2.0300    0.1350
    2.0400    0.1322
    2.0500    0.1290
    2.0600    0.1255
    2.0700    0.1224
    2.0800    0.1184
    2.0900    0.1141
    2.1000    0.1097
    2.1100    0.1052
    2.1200    0.1020
    2.1300    0.0991
    2.1400    0.0968
    2.1500    0.0945
    2.1600    0.0900
    2.1700    0.0864
    2.1800    0.0844
    2.1900    0.0812
    2.2000    0.0776
    2.2100    0.0747
    2.2200    0.0718
    2.2300    0.0690
    2.2400    0.0660
    2.2500    0.0626
    2.2600    0.0595
    2.2700    0.0560
    2.2800    0.0531
    2.2900    0.0505
    2.3000    0.0476
    2.3100    0.0445
    2.3200    0.0406
    2.3300    0.0372
    2.3400    0.0340
    2.3500    0.0314
    2.3600    0.0290
    2.3700    0.0265
    2.3800    0.0232
    2.3900    0.0194
    2.4000    0.0163
    2.4100    0.0133
    2.4200    0.0107
    2.4300    0.0089
    2.4400    0.0063
    2.4500    0.0035
    2.4600    0.0016
    2.4700   -0.0007
    2.4800   -0.0028
    2.4900   -0.0046
    2.5000   -0.0069
    2.5100   -0.0093
    2.5200   -0.0115
    2.5300   -0.0143
    2.5400   -0.0169
    2.5500   -0.0193
    2.5600   -0.0221
    2.5700   -0.0241
    2.5800   -0.0261
    2.5900   -0.0276
    2.6000   -0.0293
    2.6100   -0.0318
    2.6200   -0.0336
    2.6300   -0.0346
    2.6400   -0.0359
    2.6500   -0.0387
    2.6600   -0.0410
    2.6700   -0.0435
    2.6800   -0.0464
    2.6900   -0.0487
    2.7000   -0.0505
    2.7100   -0.0517
    2.7200   -0.0536
    2.7300   -0.0555
    2.7400   -0.0575
    2.7500   -0.0598
    2.7600   -0.0610
    2.7700   -0.0625
    2.7800   -0.0647
    2.7900   -0.0671
    2.8000   -0.0692
    2.8100   -0.0706
    2.8200   -0.0715
    2.8300   -0.0729
    2.8400   -0.0749
    2.8500   -0.0771
    2.8600   -0.0787
    2.8700   -0.0800
    2.8800   -0.0824
    2.8900   -0.0837
    2.9000   -0.0846
    2.9100   -0.0860
    2.9200   -0.0880
    2.9300   -0.0901
    2.9400   -0.0914
    2.9500   -0.0934
    2.9600   -0.0956
    2.9700   -0.0976
    2.9800   -0.0992
    2.9900   -0.1011
    3.0000   -0.1028
    3.0100   -0.1035
    3.0200   -0.1047
    3.0300   -0.1065
    3.0400   -0.1079
    3.0500   -0.1090
    3.0600   -0.1100
    3.0700   -0.1112
    3.0800   -0.1128
    3.0900   -0.1145
    3.1000   -0.1159
    3.1100   -0.1167
    3.1200   -0.1173
    3.1300   -0.1190
    3.1400   -0.1207
    3.1500   -0.1219
    3.1600   -0.1234
    3.1700   -0.1248
    3.1800   -0.1265
    3.1900   -0.1281
    3.2000   -0.1297
    3.2100   -0.1313
    3.2200   -0.1326
    3.2300   -0.1337
    3.2400   -0.1349
    3.2500   -0.1361
    3.2600   -0.1373
    3.2700   -0.1383
    3.2800   -0.1389
    3.2900   -0.1394
    3.3000   -0.1404
    3.3100   -0.1413
    3.3200   -0.1422
    3.3300   -0.1438
    3.3400   -0.1460
    3.3500   -0.1481
    3.3600   -0.1496
    3.3700   -0.1507
    3.3800   -0.1520
    3.3900   -0.1531
    3.4000   -0.1540
    3.4100   -0.1553
    3.4200   -0.1561
    3.4300   -0.1565
    3.4400   -0.1563
    3.4500   -0.1562
    3.4600   -0.1569
    3.4700   -0.1577
    3.4800   -0.1587
    3.4900   -0.1593
    3.5000   -0.1605
    3.5100   -0.1618
    3.5200   -0.1621
    3.5300   -0.1626
    3.5400   -0.1633
    3.5500   -0.1633
    3.5600   -0.1633
    3.5700   -0.1631
    3.5800   -0.1641
    3.5900   -0.1655
    3.6000   -0.1657
    3.6100   -0.1657
    3.6200   -0.1660
    3.6300   -0.1663
    3.6400   -0.1662
    3.6500   -0.1661
    3.6600   -0.1666
    3.6700   -0.1672
    3.6800   -0.1676
    3.6900   -0.1677
    3.7000   -0.1675
    3.7100   -0.1675
    3.7200   -0.1674
    3.7300   -0.1677
    3.7400   -0.1679
    3.7500   -0.1679
    3.7600   -0.1684
    3.7700   -0.1689
    3.7800   -0.1686
    3.7900   -0.1685
    3.8000   -0.1681
    3.8100   -0.1674
    3.8200   -0.1674
    3.8300   -0.1676
    3.8400   -0.1677
    3.8500   -0.1677
    3.8600   -0.1673
    3.8700   -0.1670
    3.8800   -0.1670
    3.8900   -0.1661
    3.9000   -0.1652
    3.9100   -0.1646
    3.9200   -0.1644
    3.9300   -0.1646
    3.9400   -0.1645
    3.9500   -0.1641
    3.9600   -0.1643
    3.9700   -0.1651
    3.9800   -0.1648
    3.9900   -0.1645
    4.0000   -0.1637
    4.0100   -0.1633
    4.0200   -0.1637
    4.0300   -0.1630
    4.0400   -0.1629
    4.0500   -0.1625
    4.0600   -0.1622
    4.0700   -0.1618
    4.0800   -0.1609
    4.0900   -0.1609
    4.1000   -0.1616
    4.1100   -0.1619
    4.1200   -0.1610
    4.1300   -0.1600
    4.1400   -0.1595
    4.1500   -0.1586
    4.1600   -0.1583
    4.1700   -0.1576
    4.1800   -0.1567
    4.1900   -0.1564
    4.2000   -0.1558
    4.2100   -0.1551
    4.2200   -0.1550
    4.2300   -0.1544
    4.2400   -0.1530
    4.2500   -0.1516
    4.2600   -0.1498
    4.2700   -0.1486
    4.2800   -0.1481
    4.2900   -0.1481
    4.3000   -0.1478
    4.3100   -0.1468
    4.3200   -0.1456
    4.3300   -0.1447
    4.3400   -0.1439
    4.3500   -0.1426
    4.3600   -0.1420
    4.3700   -0.1411
    4.3800   -0.1398
    4.3900   -0.1389
    4.4000   -0.1375
    4.4100   -0.1357
    4.4200   -0.1347
    4.4300   -0.1336
    4.4400   -0.1325
    4.4500   -0.1314
    4.4600   -0.1301
    4.4700   -0.1291
    4.4800   -0.1285
    4.4900   -0.1276
    4.5000   -0.1257
    4.5100   -0.1241
    4.5200   -0.1235
    4.5300   -0.1227
    4.5400   -0.1217
    4.5500   -0.1208
    4.5600   -0.1196
    4.5700   -0.1182
    4.5800   -0.1173
    4.5900   -0.1163
    4.6000   -0.1156
    4.6100   -0.1150
    4.6200   -0.1144
    4.6300   -0.1136
    4.6400   -0.1128
    4.6500   -0.1121
    4.6600   -0.1110
    4.6700   -0.1101
    4.6800   -0.1092
    4.6900   -0.1077
    4.7000   -0.1066
    4.7100   -0.1052
    4.7200   -0.1039
    4.7300   -0.1032
    4.7400   -0.1023
    4.7500   -0.1014
    4.7600   -0.1005
    4.7700   -0.0996
    4.7800   -0.0985
    4.7900   -0.0976
    4.8000   -0.0972
    4.8100   -0.0962
    4.8200   -0.0940
    4.8300   -0.0913
    4.8400   -0.0893
    4.8500   -0.0881
    4.8600   -0.0867
    4.8700   -0.0854
    4.8800   -0.0840
    4.8900   -0.0834
    4.9000   -0.0824
    4.9100   -0.0811
    4.9200   -0.0807
    4.9300   -0.0789
    4.9400   -0.0767
    4.9500   -0.0753
    4.9600   -0.0731
    4.9700   -0.0717
    4.9800   -0.0706
    4.9900   -0.0687
    5.0000   -0.0670
    5.0100   -0.0653
    5.0200   -0.0639
    5.0300   -0.0622
    5.0400   -0.0606
    5.0500   -0.0595
    5.0600   -0.0580
    5.0700   -0.0556
    5.0800   -0.0536
    5.0900   -0.0523
    5.1000   -0.0507
    5.1100   -0.0487
    5.1200   -0.0465
    5.1300   -0.0445
    5.1400   -0.0430
    5.1500   -0.0413
    5.1600   -0.0396
    5.1700   -0.0375
    5.1800   -0.0358
    5.1900   -0.0347
    5.2000   -0.0325
    5.2100   -0.0306
    5.2200   -0.0293
    5.2300   -0.0281
    5.2400   -0.0268
    5.2500   -0.0253
    5.2600   -0.0236
    5.2700   -0.0221
    5.2800   -0.0207
    5.2900   -0.0192
    5.3000   -0.0178
    5.3100   -0.0164
    5.3200   -0.0152
    5.3300   -0.0126
    5.3400   -0.0089
    5.3500   -0.0060
    5.3600   -0.0038
    5.3700   -0.0023
    5.3800   -0.0012
    5.3900    0.0001
    5.4000    0.0017
    5.4100    0.0037
    5.4200    0.0055
    5.4300    0.0071
    5.4400    0.0084
    5.4500    0.0097
    5.4600    0.0117
    5.4700    0.0139
    5.4800    0.0156
    5.4900    0.0175
    5.5000    0.0195
    5.5100    0.0208
    5.5200    0.0219
    5.5300    0.0236
    5.5400    0.0245
    5.5500    0.0251
    5.5600    0.0262
    5.5700    0.0281
    5.5800    0.0298
    5.5900    0.0314
    5.6000    0.0329
    5.6100    0.0336
    5.6200    0.0346
    5.6300    0.0360
    5.6400    0.0375
    5.6500    0.0401
    5.6600    0.0419
    5.6700    0.0436
    5.6800    0.0459
    5.6900    0.0473
    5.7000    0.0483
    5.7100    0.0500
    5.7200    0.0517
    5.7300    0.0536
    5.7400    0.0555
    5.7500    0.0574
    5.7600    0.0590
    5.7700    0.0605
    5.7800    0.0615
    5.7900    0.0619
    5.8000    0.0635
    5.8100    0.0652
    5.8200    0.0664
    5.8300    0.0685
    5.8400    0.0701
    5.8500    0.0710
    5.8600    0.0720
    5.8700    0.0734
    5.8800    0.0750
    5.8900    0.0760
    5.9000    0.0767
    5.9100    0.0775
    5.9200    0.0788
    5.9300    0.0799
    5.9400    0.0811
    5.9500    0.0820
    5.9600    0.0833
    5.9700    0.0842
    5.9800    0.0848
    5.9900    0.0866
    6.0000    0.0878
    6.0100    0.0888
    6.0200    0.0902
    6.0300    0.0914
    6.0400    0.0924
    6.0500    0.0939
    6.0600    0.0949
    6.0700    0.0961
    6.0800    0.0979
    6.0900    0.0995
    6.1000    0.1009
    6.1100    0.1017
    6.1200    0.1027
    6.1300    0.1037
    6.1400    0.1049
    6.1500    0.1067
    6.1600    0.1080
    6.1700    0.1092
    6.1800    0.1096
    6.1900    0.1097
    6.2000    0.1105
    6.2100    0.1125
    6.2200    0.1145
    6.2300    0.1158
    6.2400    0.1168
    6.2500    0.1176
    6.2600    0.1190
    6.2700    0.1201
    6.2800    0.1217
    6.2900    0.1229
    6.3000    0.1233
    6.3100    0.1243
    6.3200    0.1247
    6.3300    0.1252
    6.3400    0.1264
    6.3500    0.1273
    6.3600    0.1284
    6.3700    0.1298
    6.3800    0.1313
    6.3900    0.1322
    6.4000    0.1328
    6.4100    0.1338
    6.4200    0.1344
    6.4300    0.1345
    6.4400    0.1349
    6.4500    0.1356
    6.4600    0.1369
    6.4700    0.1384
    6.4800    0.1392
    6.4900    0.1396
    6.5000    0.1405
    6.5100    0.1425
    6.5200    0.1440
    6.5300    0.1445
    6.5400    0.1446
    6.5500    0.1451
    6.5600    0.1461
    6.5700    0.1471
    6.5800    0.1478
    6.5900    0.1481
    6.6000    0.1485
    6.6100    0.1493
    6.6200    0.1500
    6.6300    0.1503
    6.6400    0.1507
    6.6500    0.1513
    6.6600    0.1523
    6.6700    0.1525
    6.6800    0.1525
    6.6900    0.1524
    6.7000    0.1526
    6.7100    0.1534
    6.7200    0.1534
    6.7300    0.1527
    6.7400    0.1525
    6.7500    0.1530
    6.7600    0.1536
    6.7700    0.1536
    6.7800    0.1529
    6.7900    0.1530
    6.8000    0.1535
    6.8100    0.1535
    6.8200    0.1540
    6.8300    0.1544
    6.8400    0.1543
    6.8500    0.1547
    6.8600    0.1552
    6.8700    0.1554
    6.8800    0.1552
    6.8900    0.1563
    6.9000    0.1568
    6.9100    0.1564
    6.9200    0.1566
    6.9300    0.1564
    6.9400    0.1559
    6.9500    0.1557
    6.9600    0.1567
    6.9700    0.1571
    6.9800    0.1569
    6.9900    0.1568
    7.0000    0.1571
    7.0100    0.1579
    7.0200    0.1578
    7.0300    0.1578
    7.0400    0.1578
    7.0500    0.1580
    7.0600    0.1582
    7.0700    0.1575
    7.0800    0.1570
    7.0900    0.1575
    7.1000    0.1574
    7.1100    0.1565
    7.1200    0.1567
    7.1300    0.1561
    7.1400    0.1554
    7.1500    0.1556
    7.1600    0.1555
    7.1700    0.1550
    7.1800    0.1544
    7.1900    0.1541
    7.2000    0.1540
    7.2100    0.1541
    7.2200    0.1537
    7.2300    0.1536
    7.2400    0.1537
    7.2500    0.1530
    7.2600    0.1521
    7.2700    0.1518
    7.2800    0.1516
    7.2900    0.1514
    7.3000    0.1510
    7.3100    0.1513
    7.3200    0.1510
    7.3300    0.1497
    7.3400    0.1491
    7.3500    0.1484
    7.3600    0.1482
    7.3700    0.1481
    7.3800    0.1474
    7.3900    0.1467
    7.4000    0.1463
    7.4100    0.1456
    7.4200    0.1449
    7.4300    0.1439
    7.4400    0.1426
    7.4500    0.1417
    7.4600    0.1404
    7.4700    0.1396
    7.4800    0.1386
    7.4900    0.1372
    7.5000    0.1358
    7.5100    0.1338
    7.5200    0.1323
    7.5300    0.1318
    7.5400    0.1312
    7.5500    0.1303
    7.5600    0.1289
    7.5700    0.1282
    7.5800    0.1277
    7.5900    0.1270
    7.6000    0.1266
    7.6100    0.1256
    7.6200    0.1248
    7.6300    0.1245
    7.6400    0.1237
    7.6500    0.1229
    7.6600    0.1229
    7.6700    0.1223
    7.6800    0.1211
    7.6900    0.1201
    7.7000    0.1193
    7.7100    0.1185
    7.7200    0.1176
    7.7300    0.1166
    7.7400    0.1160
    7.7500    0.1152
    7.7600    0.1142
    7.7700    0.1127
    7.7800    0.1109
    7.7900    0.1090
    7.8000    0.1071
    7.8100    0.1056
    7.8200    0.1038
    7.8300    0.1028
    7.8400    0.1026
    7.8500    0.1009
    7.8600    0.0987
    7.8700    0.0972
    7.8800    0.0955
    7.8900    0.0935
    7.9000    0.0925
    7.9100    0.0916
    7.9200    0.0902
    7.9300    0.0886
    7.9400    0.0869
    7.9500    0.0851
    7.9600    0.0835
    7.9700    0.0822
    7.9800    0.0809
    7.9900    0.0802
    8.0000    0.0795
    8.0100    0.0784
    8.0200    0.0769
    8.0300    0.0751
    8.0400    0.0733
    8.0500    0.0724
    8.0600    0.0712
    8.0700    0.0696
    8.0800    0.0683
    8.0900    0.0674
    8.1000    0.0658
    8.1100    0.0640
    8.1200    0.0628
    8.1300    0.0613
    8.1400    0.0601
    8.1500    0.0589
    8.1600    0.0571
    8.1700    0.0555
    8.1800    0.0543
    8.1900    0.0529
    8.2000    0.0517
    8.2100    0.0500
    8.2200    0.0479
    8.2300    0.0452
    8.2400    0.0430
    8.2500    0.0416
    8.2600    0.0396
    8.2700    0.0385
    8.2800    0.0373
    8.2900    0.0357
    8.3000    0.0339
    8.3100    0.0320
    8.3200    0.0308
    8.3300    0.0290
    8.3400    0.0270
    8.3500    0.0259
    8.3600    0.0241
    8.3700    0.0224
    8.3800    0.0214
    8.3900    0.0199
    8.4000    0.0176
    8.4100    0.0158
    8.4200    0.0147
    8.4300    0.0136
    8.4400    0.0125
    8.4500    0.0108
    8.4600    0.0092
    8.4700    0.0077
    8.4800    0.0059
    8.4900    0.0038
    8.5000    0.0022
    8.5100    0.0011
    8.5200   -0.0002
    8.5300   -0.0008
    8.5400   -0.0023
    8.5500   -0.0040
    8.5600   -0.0052
    8.5700   -0.0065
    8.5800   -0.0074
    8.5900   -0.0083
    8.6000   -0.0099
    8.6100   -0.0116
    8.6200   -0.0132
    8.6300   -0.0136
    8.6400   -0.0139
    8.6500   -0.0144
    8.6600   -0.0151
    8.6700   -0.0165
    8.6800   -0.0177
    8.6900   -0.0192
    8.7000   -0.0205
    8.7100   -0.0215
    8.7200   -0.0236
    8.7300   -0.0251
    8.7400   -0.0267
    8.7500   -0.0293
    8.7600   -0.0311
    8.7700   -0.0326
    8.7800   -0.0347
    8.7900   -0.0364
    8.8000   -0.0380
    8.8100   -0.0396
    8.8200   -0.0410
    8.8300   -0.0427
    8.8400   -0.0447
    8.8500   -0.0471
    8.8600   -0.0493
    8.8700   -0.0505
    8.8800   -0.0519
    8.8900   -0.0534
    8.9000   -0.0545
    8.9100   -0.0555
    8.9200   -0.0562
    8.9300   -0.0575
    8.9400   -0.0594
    8.9500   -0.0609
    8.9600   -0.0625
    8.9700   -0.0637
    8.9800   -0.0641
    8.9900   -0.0650
    9.0000   -0.0665
    9.0100   -0.0678
    9.0200   -0.0691
    9.0300   -0.0707
    9.0400   -0.0722
    9.0500   -0.0736
    9.0600   -0.0745
    9.0700   -0.0753
    9.0800   -0.0760
    9.0900   -0.0772
    9.1000   -0.0787
    9.1100   -0.0802
    9.1200   -0.0816
    9.1300   -0.0826
    9.1400   -0.0834
    9.1500   -0.0840
    9.1600   -0.0847
    9.1700   -0.0859
    9.1800   -0.0873
    9.1900   -0.0892
    9.2000   -0.0911
    9.2100   -0.0928
    9.2200   -0.0942
    9.2300   -0.0947
    9.2400   -0.0956
    9.2500   -0.0968
    9.2600   -0.0980
    9.2700   -0.0987
    9.2800   -0.0988
    9.2900   -0.0997
    9.3000   -0.1009
    9.3100   -0.1022
    9.3200   -0.1035
    9.3300   -0.1042
    9.3400   -0.1047
    9.3500   -0.1060
    9.3600   -0.1074
    9.3700   -0.1084
    9.3800   -0.1098
    9.3900   -0.1106
    9.4000   -0.1113
    9.4100   -0.1122
    9.4200   -0.1131
    9.4300   -0.1134
    9.4400   -0.1140
    9.4500   -0.1155
    9.4600   -0.1171
    9.4700   -0.1185
    9.4800   -0.1199
    9.4900   -0.1207
    9.5000   -0.1220
    9.5100   -0.1234
    9.5200   -0.1244
    9.5300   -0.1251
    9.5400   -0.1258
    9.5500   -0.1268
    9.5600   -0.1278
    9.5700   -0.1291
    9.5800   -0.1301
    9.5900   -0.1309
    9.6000   -0.1319
    9.6100   -0.1324
    9.6200   -0.1327
    9.6300   -0.1327
    9.6400   -0.1329
    9.6500   -0.1333
    9.6600   -0.1343
    9.6700   -0.1354
    9.6800   -0.1356
    9.6900   -0.1363
    9.7000   -0.1368
    9.7100   -0.1369
    9.7200   -0.1370
    9.7300   -0.1371
    9.7400   -0.1374
    9.7500   -0.1379
    9.7600   -0.1390
    9.7700   -0.1398
    9.7800   -0.1403
    9.7900   -0.1404
    9.8000   -0.1408
    9.8100   -0.1418
    9.8200   -0.1414
    9.8300   -0.1411
    9.8400   -0.1413
    9.8500   -0.1407
    9.8600   -0.1411
    9.8700   -0.1416
    9.8800   -0.1420
    9.8900   -0.1424
    9.9000   -0.1420
    9.9100   -0.1425
    9.9200   -0.1428
    9.9300   -0.1420
    9.9400   -0.1423
    9.9500   -0.1428
    9.9600   -0.1429
    9.9700   -0.1430
    9.9800   -0.1428
    9.9900   -0.1423
   10.0000   -0.1422
    };

==> Data/Oscillator/sigma01/kf_en_vel.tex <==
    \addplot[
    thick,
    dashed,
    cyan
    ]
    table {
         0         0
    0.0100   -0.0099
    0.0200   -0.0196
    0.0300   -0.0291
    0.0400   -0.0384
    0.0500   -0.0475
    0.0600   -0.0563
    0.0700   -0.0650
    0.0800   -0.0735
    0.0900   -0.0818
    0.1000   -0.0898
    0.1100   -0.0976
    0.1200   -0.1054
    0.1300   -0.1129
    0.1400   -0.1203
    0.1500   -0.1275
    0.1600   -0.1345
    0.1700   -0.1414
    0.1800   -0.1480
    0.1900   -0.1545
    0.2000   -0.1607
    0.2100   -0.1668
    0.2200   -0.1727
    0.2300   -0.1785
    0.2400   -0.1842
    0.2500   -0.1896
    0.2600   -0.1948
    0.2700   -0.1999
    0.2800   -0.2051
    0.2900   -0.2099
    0.3000   -0.2145
    0.3100   -0.2192
    0.3200   -0.2235
    0.3300   -0.2278
    0.3400   -0.2320
    0.3500   -0.2362
    0.3600   -0.2404
    0.3700   -0.2445
    0.3800   -0.2481
    0.3900   -0.2515
    0.4000   -0.2548
    0.4100   -0.2580
    0.4200   -0.2611
    0.4300   -0.2640
    0.4400   -0.2671
    0.4500   -0.2701
    0.4600   -0.2728
    0.4700   -0.2755
    0.4800   -0.2783
    0.4900   -0.2810
    0.5000   -0.2835
    0.5100   -0.2861
    0.5200   -0.2884
    0.5300   -0.2905
    0.5400   -0.2927
    0.5500   -0.2946
    0.5600   -0.2965
    0.5700   -0.2984
    0.5800   -0.3002
    0.5900   -0.3019
    0.6000   -0.3037
    0.6100   -0.3054
    0.6200   -0.3070
    0.6300   -0.3085
    0.6400   -0.3099
    0.6500   -0.3112
    0.6600   -0.3124
    0.6700   -0.3139
    0.6800   -0.3151
    0.6900   -0.3164
    0.7000   -0.3177
    0.7100   -0.3186
    0.7200   -0.3195
    0.7300   -0.3202
    0.7400   -0.3208
    0.7500   -0.3215
    0.7600   -0.3225
    0.7700   -0.3234
    0.7800   -0.3241
    0.7900   -0.3250
    0.8000   -0.3254
    0.8100   -0.3256
    0.8200   -0.3261
    0.8300   -0.3266
    0.8400   -0.3270
    0.8500   -0.3270
    0.8600   -0.3272
    0.8700   -0.3275
    0.8800   -0.3278
    0.8900   -0.3279
    0.9000   -0.3277
    0.9100   -0.3276
    0.9200   -0.3279
    0.9300   -0.3282
    0.9400   -0.3281
    0.9500   -0.3277
    0.9600   -0.3273
    0.9700   -0.3270
    0.9800   -0.3267
    0.9900   -0.3265
    1.0000   -0.3262
    1.0100   -0.3255
    1.0200   -0.3250
    1.0300   -0.3248
    1.0400   -0.3244
    1.0500   -0.3237
    1.0600   -0.3231
    1.0700   -0.3223
    1.0800   -0.3216
    1.0900   -0.3211
    1.1000   -0.3206
    1.1100   -0.3197
    1.1200   -0.3188
    1.1300   -0.3180
    1.1400   -0.3174
    1.1500   -0.3169
    1.1600   -0.3161
    1.1700   -0.3154
    1.1800   -0.3146
    1.1900   -0.3136
    1.2000   -0.3128
    1.2100   -0.3121
    1.2200   -0.3113
    1.2300   -0.3105
    1.2400   -0.3095
    1.2500   -0.3085
    1.2600   -0.3075
    1.2700   -0.3064
    1.2800   -0.3054
    1.2900   -0.3045
    1.3000   -0.3034
    1.3100   -0.3023
    1.3200   -0.3013
    1.3300   -0.3001
    1.3400   -0.2989
    1.3500   -0.2978
    1.3600   -0.2967
    1.3700   -0.2955
    1.3800   -0.2942
    1.3900   -0.2930
    1.4000   -0.2917
    1.4100   -0.2904
    1.4200   -0.2891
    1.4300   -0.2878
    1.4400   -0.2865
    1.4500   -0.2853
    1.4600   -0.2840
    1.4700   -0.2826
    1.4800   -0.2810
    1.4900   -0.2796
    1.5000   -0.2781
    1.5100   -0.2765
    1.5200   -0.2750
    1.5300   -0.2736
    1.5400   -0.2721
    1.5500   -0.2706
    1.5600   -0.2691
    1.5700   -0.2674
    1.5800   -0.2658
    1.5900   -0.2642
    1.6000   -0.2626
    1.6100   -0.2611
    1.6200   -0.2596
    1.6300   -0.2580
    1.6400   -0.2563
    1.6500   -0.2547
    1.6600   -0.2531
    1.6700   -0.2514
    1.6800   -0.2497
    1.6900   -0.2480
    1.7000   -0.2463
    1.7100   -0.2446
    1.7200   -0.2430
    1.7300   -0.2414
    1.7400   -0.2396
    1.7500   -0.2380
    1.7600   -0.2364
    1.7700   -0.2346
    1.7800   -0.2328
    1.7900   -0.2311
    1.8000   -0.2294
    1.8100   -0.2276
    1.8200   -0.2259
    1.8300   -0.2241
    1.8400   -0.2224
    1.8500   -0.2206
    1.8600   -0.2186
    1.8700   -0.2168
    1.8800   -0.2150
    1.8900   -0.2131
    1.9000   -0.2112
    1.9100   -0.2093
    1.9200   -0.2074
    1.9300   -0.2055
    1.9400   -0.2036
    1.9500   -0.2017
    1.9600   -0.1998
    1.9700   -0.1979
    1.9800   -0.1960
    1.9900   -0.1941
    2.0000   -0.1923
    2.0100   -0.1903
    2.0200   -0.1884
    2.0300   -0.1865
    2.0400   -0.1846
    2.0500   -0.1827
    2.0600   -0.1808
    2.0700   -0.1789
    2.0800   -0.1770
    2.0900   -0.1751
    2.1000   -0.1731
    2.1100   -0.1711
    2.1200   -0.1692
    2.1300   -0.1673
    2.1400   -0.1654
    2.1500   -0.1635
    2.1600   -0.1616
    2.1700   -0.1596
    2.1800   -0.1578
    2.1900   -0.1559
    2.2000   -0.1539
    2.2100   -0.1520
    2.2200   -0.1502
    2.2300   -0.1483
    2.2400   -0.1464
    2.2500   -0.1445
    2.2600   -0.1426
    2.2700   -0.1407
    2.2800   -0.1388
    2.2900   -0.1369
    2.3000   -0.1350
    2.3100   -0.1331
    2.3200   -0.1312
    2.3300   -0.1293
    2.3400   -0.1274
    2.3500   -0.1256
    2.3600   -0.1237
    2.3700   -0.1218
    2.3800   -0.1199
    2.3900   -0.1181
    2.4000   -0.1162
    2.4100   -0.1143
    2.4200   -0.1124
    2.4300   -0.1105
    2.4400   -0.1087
    2.4500   -0.1068
    2.4600   -0.1050
    2.4700   -0.1031
    2.4800   -0.1013
    2.4900   -0.0995
    2.5000   -0.0977
    2.5100   -0.0958
    2.5200   -0.0940
    2.5300   -0.0923
    2.5400   -0.0905
    2.5500   -0.0887
    2.5600   -0.0869
    2.5700   -0.0851
    2.5800   -0.0833
    2.5900   -0.0815
    2.6000   -0.0798
    2.6100   -0.0780
    2.6200   -0.0763
    2.6300   -0.0745
    2.6400   -0.0728
    2.6500   -0.0711
    2.6600   -0.0694
    2.6700   -0.0677
    2.6800   -0.0660
    2.6900   -0.0643
    2.7000   -0.0626
    2.7100   -0.0609
    2.7200   -0.0592
    2.7300   -0.0576
    2.7400   -0.0559
    2.7500   -0.0543
    2.7600   -0.0526
    2.7700   -0.0509
    2.7800   -0.0493
    2.7900   -0.0477
    2.8000   -0.0461
    2.8100   -0.0445
    2.8200   -0.0428
    2.8300   -0.0412
    2.8400   -0.0396
    2.8500   -0.0381
    2.8600   -0.0365
    2.8700   -0.0349
    2.8800   -0.0334
    2.8900   -0.0318
    2.9000   -0.0302
    2.9100   -0.0287
    2.9200   -0.0272
    2.9300   -0.0257
    2.9400   -0.0241
    2.9500   -0.0227
    2.9600   -0.0212
    2.9700   -0.0197
    2.9800   -0.0182
    2.9900   -0.0167
    3.0000   -0.0153
    3.0100   -0.0137
    3.0200   -0.0122
    3.0300   -0.0108
    3.0400   -0.0093
    3.0500   -0.0079
    3.0600   -0.0064
    3.0700   -0.0050
    3.0800   -0.0036
    3.0900   -0.0022
    3.1000   -0.0008
    3.1100    0.0007
    3.1200    0.0021
    3.1300    0.0034
    3.1400    0.0048
    3.1500    0.0061
    3.1600    0.0075
    3.1700    0.0088
    3.1800    0.0101
    3.1900    0.0114
    3.2000    0.0127
    3.2100    0.0140
    3.2200    0.0154
    3.2300    0.0167
    3.2400    0.0180
    3.2500    0.0193
    3.2600    0.0206
    3.2700    0.0219
    3.2800    0.0232
    3.2900    0.0245
    3.3000    0.0258
    3.3100    0.0270
    3.3200    0.0283
    3.3300    0.0295
    3.3400    0.0306
    3.3500    0.0317
    3.3600    0.0329
    3.3700    0.0341
    3.3800    0.0353
    3.3900    0.0365
    3.4000    0.0377
    3.4100    0.0389
    3.4200    0.0401
    3.4300    0.0413
    3.4400    0.0426
    3.4500    0.0438
    3.4600    0.0450
    3.4700    0.0461
    3.4800    0.0472
    3.4900    0.0483
    3.5000    0.0494
    3.5100    0.0504
    3.5200    0.0515
    3.5300    0.0526
    3.5400    0.0537
    3.5500    0.0548
    3.5600    0.0559
    3.5700    0.0570
    3.5800    0.0580
    3.5900    0.0589
    3.6000    0.0600
    3.6100    0.0610
    3.6200    0.0620
    3.6300    0.0630
    3.6400    0.0640
    3.6500    0.0650
    3.6600    0.0659
    3.6700    0.0668
    3.6800    0.0677
    3.6900    0.0686
    3.7000    0.0696
    3.7100    0.0705
    3.7200    0.0714
    3.7300    0.0722
    3.7400    0.0731
    3.7500    0.0739
    3.7600    0.0747
    3.7700    0.0755
    3.7800    0.0763
    3.7900    0.0771
    3.8000    0.0780
    3.8100    0.0788
    3.8200    0.0796
    3.8300    0.0803
    3.8400    0.0810
    3.8500    0.0817
    3.8600    0.0825
    3.8700    0.0832
    3.8800    0.0838
    3.8900    0.0846
    3.9000    0.0853
    3.9100    0.0860
    3.9200    0.0866
    3.9300    0.0872
    3.9400    0.0878
    3.9500    0.0884
    3.9600    0.0889
    3.9700    0.0894
    3.9800    0.0900
    3.9900    0.0905
    4.0000    0.0911
    4.0100    0.0917
    4.0200    0.0921
    4.0300    0.0927
    4.0400    0.0932
    4.0500    0.0937
    4.0600    0.0941
    4.0700    0.0946
    4.0800    0.0951
    4.0900    0.0955
    4.1000    0.0958
    4.1100    0.0962
    4.1200    0.0967
    4.1300    0.0972
    4.1400    0.0976
    4.1500    0.0980
    4.1600    0.0984
    4.1700    0.0987
    4.1800    0.0991
    4.1900    0.0995
    4.2000    0.0998
    4.2100    0.1001
    4.2200    0.1004
    4.2300    0.1007
    4.2400    0.1011
    4.2500    0.1014
    4.2600    0.1018
    4.2700    0.1021
    4.2800    0.1023
    4.2900    0.1024
    4.3000    0.1026
    4.3100    0.1028
    4.3200    0.1030
    4.3300    0.1032
    4.3400    0.1034
    4.3500    0.1036
    4.3600    0.1037
    4.3700    0.1038
    4.3800    0.1040
    4.3900    0.1041
    4.4000    0.1043
    4.4100    0.1044
    4.4200    0.1045
    4.4300    0.1045
    4.4400    0.1046
    4.4500    0.1046
    4.4600    0.1047
    4.4700    0.1047
    4.4800    0.1046
    4.4900    0.1046
    4.5000    0.1046
    4.5100    0.1046
    4.5200    0.1045
    4.5300    0.1044
    4.5400    0.1043
    4.5500    0.1042
    4.5600    0.1041
    4.5700    0.1041
    4.5800    0.1039
    4.5900    0.1038
    4.6000    0.1036
    4.6100    0.1034
    4.6200    0.1032
    4.6300    0.1030
    4.6400    0.1028
    4.6500    0.1026
    4.6600    0.1024
    4.6700    0.1022
    4.6800    0.1020
    4.6900    0.1018
    4.7000    0.1016
    4.7100    0.1014
    4.7200    0.1012
    4.7300    0.1009
    4.7400    0.1006
    4.7500    0.1004
    4.7600    0.1001
    4.7700    0.0998
    4.7800    0.0995
    4.7900    0.0992
    4.8000    0.0988
    4.8100    0.0985
    4.8200    0.0983
    4.8300    0.0982
    4.8400    0.0979
    4.8500    0.0976
    4.8600    0.0972
    4.8700    0.0969
    4.8800    0.0965
    4.8900    0.0961
    4.9000    0.0956
    4.9100    0.0953
    4.9200    0.0948
    4.9300    0.0944
    4.9400    0.0941
    4.9500    0.0937
    4.9600    0.0933
    4.9700    0.0929
    4.9800    0.0924
    4.9900    0.0920
    5.0000    0.0916
    5.0100    0.0911
    5.0200    0.0906
    5.0300    0.0901
    5.0400    0.0896
    5.0500    0.0891
    5.0600    0.0886
    5.0700    0.0881
    5.0800    0.0876
    5.0900    0.0870
    5.1000    0.0865
    5.1100    0.0860
    5.1200    0.0854
    5.1300    0.0849
    5.1400    0.0843
    5.1500    0.0836
    5.1600    0.0830
    5.1700    0.0825
    5.1800    0.0818
    5.1900    0.0811
    5.2000    0.0805
    5.2100    0.0799
    5.2200    0.0791
    5.2300    0.0784
    5.2400    0.0777
    5.2500    0.0770
    5.2600    0.0763
    5.2700    0.0755
    5.2800    0.0748
    5.2900    0.0741
    5.3000    0.0733
    5.3100    0.0726
    5.3200    0.0718
    5.3300    0.0712
    5.3400    0.0707
    5.3500    0.0700
    5.3600    0.0693
    5.3700    0.0684
    5.3800    0.0676
    5.3900    0.0667
    5.4000    0.0659
    5.4100    0.0651
    5.4200    0.0643
    5.4300    0.0635
    5.4400    0.0626
    5.4500    0.0617
    5.4600    0.0609
    5.4700    0.0601
    5.4800    0.0592
    5.4900    0.0584
    5.5000    0.0575
    5.5100    0.0566
    5.5200    0.0557
    5.5300    0.0548
    5.5400    0.0538
    5.5500    0.0528
    5.5600    0.0519
    5.5700    0.0510
    5.5800    0.0501
    5.5900    0.0492
    5.6000    0.0483
    5.6100    0.0473
    5.6200    0.0464
    5.6300    0.0455
    5.6400    0.0446
    5.6500    0.0438
    5.6600    0.0429
    5.6700    0.0420
    5.6800    0.0411
    5.6900    0.0402
    5.7000    0.0392
    5.7100    0.0383
    5.7200    0.0373
    5.7300    0.0364
    5.7400    0.0355
    5.7500    0.0346
    5.7600    0.0336
    5.7700    0.0327
    5.7800    0.0317
    5.7900    0.0306
    5.8000    0.0296
    5.8100    0.0287
    5.8200    0.0277
    5.8300    0.0268
    5.8400    0.0258
    5.8500    0.0248
    5.8600    0.0238
    5.8700    0.0228
    5.8800    0.0218
    5.8900    0.0208
    5.9000    0.0198
    5.9100    0.0187
    5.9200    0.0178
    5.9300    0.0168
    5.9400    0.0158
    5.9500    0.0148
    5.9600    0.0138
    5.9700    0.0128
    5.9800    0.0118
    5.9900    0.0109
    6.0000    0.0100
    6.0100    0.0090
    6.0200    0.0081
    6.0300    0.0071
    6.0400    0.0061
    6.0500    0.0052
    6.0600    0.0042
    6.0700    0.0033
    6.0800    0.0024
    6.0900    0.0015
    6.1000    0.0006
    6.1100   -0.0004
    6.1200   -0.0014
    6.1300   -0.0024
    6.1400   -0.0033
    6.1500   -0.0042
    6.1600   -0.0051
    6.1700   -0.0061
    6.1800   -0.0071
    6.1900   -0.0082
    6.2000   -0.0091
    6.2100   -0.0099
    6.2200   -0.0108
    6.2300   -0.0117
    6.2400   -0.0126
    6.2500   -0.0136
    6.2600   -0.0145
    6.2700   -0.0154
    6.2800   -0.0163
    6.2900   -0.0172
    6.3000   -0.0182
    6.3100   -0.0192
    6.3200   -0.0202
    6.3300   -0.0211
    6.3400   -0.0220
    6.3500   -0.0229
    6.3600   -0.0238
    6.3700   -0.0247
    6.3800   -0.0255
    6.3900   -0.0264
    6.4000   -0.0274
    6.4100   -0.0283
    6.4200   -0.0292
    6.4300   -0.0302
    6.4400   -0.0311
    6.4500   -0.0320
    6.4600   -0.0328
    6.4700   -0.0336
    6.4800   -0.0345
    6.4900   -0.0354
    6.5000   -0.0363
    6.5100   -0.0370
    6.5200   -0.0378
    6.5300   -0.0387
    6.5400   -0.0396
    6.5500   -0.0405
    6.5600   -0.0413
    6.5700   -0.0421
    6.5800   -0.0430
    6.5900   -0.0439
    6.6000   -0.0447
    6.6100   -0.0456
    6.6200   -0.0464
    6.6300   -0.0472
    6.6400   -0.0481
    6.6500   -0.0489
    6.6600   -0.0496
    6.6700   -0.0505
    6.6800   -0.0513
    6.6900   -0.0522
    6.7000   -0.0530
    6.7100   -0.0537
    6.7200   -0.0546
    6.7300   -0.0554
    6.7400   -0.0562
    6.7500   -0.0569
    6.7600   -0.0576
    6.7700   -0.0584
    6.7800   -0.0592
    6.7900   -0.0600
    6.8000   -0.0606
    6.8100   -0.0613
    6.8200   -0.0620
    6.8300   -0.0626
    6.8400   -0.0633
    6.8500   -0.0640
    6.8600   -0.0646
    6.8700   -0.0652
    6.8800   -0.0659
    6.8900   -0.0664
    6.9000   -0.0670
    6.9100   -0.0677
    6.9200   -0.0683
    6.9300   -0.0690
    6.9400   -0.0696
    6.9500   -0.0702
    6.9600   -0.0707
    6.9700   -0.0713
    6.9800   -0.0719
    6.9900   -0.0725
    7.0000   -0.0730
    7.0100   -0.0735
    7.0200   -0.0740
    7.0300   -0.0746
    7.0400   -0.0751
    7.0500   -0.0756
    7.0600   -0.0761
    7.0700   -0.0767
    7.0800   -0.0773
    7.0900   -0.0777
    7.1000   -0.0782
    7.1100   -0.0788
    7.1200   -0.0792
    7.1300   -0.0797
    7.1400   -0.0803
    7.1500   -0.0807
    7.1600   -0.0811
    7.1700   -0.0815
    7.1800   -0.0820
    7.1900   -0.0824
    7.2000   -0.0828
    7.2100   -0.0832
    7.2200   -0.0836
    7.2300   -0.0839
    7.2400   -0.0843
    7.2500   -0.0847
    7.2600   -0.0851
    7.2700   -0.0855
    7.2800   -0.0858
    7.2900   -0.0861
    7.3000   -0.0864
    7.3100   -0.0867
    7.3200   -0.0870
    7.3300   -0.0874
    7.3400   -0.0877
    7.3500   -0.0880
    7.3600   -0.0883
    7.3700   -0.0885
    7.3800   -0.0888
    7.3900   -0.0891
    7.4000   -0.0893
    7.4100   -0.0896
    7.4200   -0.0898
    7.4300   -0.0901
    7.4400   -0.0904
    7.4500   -0.0906
    7.4600   -0.0909
    7.4700   -0.0910
    7.4800   -0.0912
    7.4900   -0.0915
    7.5000   -0.0917
    7.5100   -0.0919
    7.5200   -0.0921
    7.5300   -0.0921
    7.5400   -0.0922
    7.5500   -0.0923
    7.5600   -0.0924
    7.5700   -0.0924
    7.5800   -0.0924
    7.5900   -0.0924
    7.6000   -0.0924
    7.6100   -0.0924
    7.6200   -0.0924
    7.6300   -0.0924
    7.6400   -0.0923
    7.6500   -0.0923
    7.6600   -0.0922
    7.6700   -0.0921
    7.6800   -0.0922
    7.6900   -0.0921
    7.7000   -0.0921
    7.7100   -0.0920
    7.7200   -0.0920
    7.7300   -0.0919
    7.7400   -0.0918
    7.7500   -0.0917
    7.7600   -0.0916
    7.7700   -0.0916
    7.7800   -0.0915
    7.7900   -0.0915
    7.8000   -0.0915
    7.8100   -0.0914
    7.8200   -0.0913
    7.8300   -0.0911
    7.8400   -0.0908
    7.8500   -0.0907
    7.8600   -0.0906
    7.8700   -0.0904
    7.8800   -0.0902
    7.8900   -0.0901
    7.9000   -0.0898
    7.9100   -0.0895
    7.9200   -0.0892
    7.9300   -0.0890
    7.9400   -0.0887
    7.9500   -0.0885
    7.9600   -0.0882
    7.9700   -0.0879
    7.9800   -0.0875
    7.9900   -0.0871
    8.0000   -0.0867
    8.0100   -0.0863
    8.0200   -0.0860
    8.0300   -0.0857
    8.0400   -0.0853
    8.0500   -0.0849
    8.0600   -0.0845
    8.0700   -0.0841
    8.0800   -0.0837
    8.0900   -0.0832
    8.1000   -0.0828
    8.1100   -0.0824
    8.1200   -0.0820
    8.1300   -0.0815
    8.1400   -0.0810
    8.1500   -0.0806
    8.1600   -0.0801
    8.1700   -0.0797
    8.1800   -0.0792
    8.1900   -0.0787
    8.2000   -0.0781
    8.2100   -0.0777
    8.2200   -0.0772
    8.2300   -0.0768
    8.2400   -0.0764
    8.2500   -0.0758
    8.2600   -0.0753
    8.2700   -0.0747
    8.2800   -0.0740
    8.2900   -0.0735
    8.3000   -0.0729
    8.3100   -0.0723
    8.3200   -0.0717
    8.3300   -0.0711
    8.3400   -0.0705
    8.3500   -0.0698
    8.3600   -0.0692
    8.3700   -0.0686
    8.3800   -0.0679
    8.3900   -0.0672
    8.4000   -0.0666
    8.4100   -0.0660
    8.4200   -0.0653
    8.4300   -0.0645
    8.4400   -0.0638
    8.4500   -0.0631
    8.4600   -0.0624
    8.4700   -0.0617
    8.4800   -0.0610
    8.4900   -0.0604
    8.5000   -0.0597
    8.5100   -0.0589
    8.5200   -0.0581
    8.5300   -0.0573
    8.5400   -0.0565
    8.5500   -0.0558
    8.5600   -0.0550
    8.5700   -0.0542
    8.5800   -0.0534
    8.5900   -0.0526
    8.6000   -0.0519
    8.6100   -0.0511
    8.6200   -0.0504
    8.6300   -0.0495
    8.6400   -0.0486
    8.6500   -0.0477
    8.6600   -0.0469
    8.6700   -0.0462
    8.6800   -0.0454
    8.6900   -0.0447
    8.7000   -0.0439
    8.7100   -0.0431
    8.7200   -0.0424
    8.7300   -0.0417
    8.7400   -0.0409
    8.7500   -0.0403
    8.7600   -0.0395
    8.7700   -0.0387
    8.7800   -0.0380
    8.7900   -0.0372
    8.8000   -0.0364
    8.8100   -0.0356
    8.8200   -0.0348
    8.8300   -0.0340
    8.8400   -0.0332
    8.8500   -0.0325
    8.8600   -0.0317
    8.8700   -0.0308
    8.8800   -0.0299
    8.8900   -0.0291
    8.9000   -0.0281
    8.9100   -0.0272
    8.9200   -0.0263
    8.9300   -0.0254
    8.9400   -0.0246
    8.9500   -0.0237
    8.9600   -0.0229
    8.9700   -0.0220
    8.9800   -0.0210
    8.9900   -0.0201
    9.0000   -0.0192
    9.0100   -0.0183
    9.0200   -0.0175
    9.0300   -0.0166
    9.0400   -0.0157
    9.0500   -0.0149
    9.0600   -0.0139
    9.0700   -0.0130
    9.0800   -0.0121
    9.0900   -0.0112
    9.1000   -0.0103
    9.1100   -0.0095
    9.1200   -0.0086
    9.1300   -0.0077
    9.1400   -0.0068
    9.1500   -0.0058
    9.1600   -0.0049
    9.1700   -0.0040
    9.1800   -0.0032
    9.1900   -0.0024
    9.2000   -0.0016
    9.2100   -0.0008
    9.2200    0.0001
    9.2300    0.0010
    9.2400    0.0020
    9.2500    0.0028
    9.2600    0.0037
    9.2700    0.0046
    9.2800    0.0056
    9.2900    0.0065
    9.3000    0.0073
    9.3100    0.0082
    9.3200    0.0090
    9.3300    0.0099
    9.3400    0.0108
    9.3500    0.0117
    9.3600    0.0125
    9.3700    0.0133
    9.3800    0.0141
    9.3900    0.0150
    9.4000    0.0159
    9.4100    0.0168
    9.4200    0.0176
    9.4300    0.0186
    9.4400    0.0194
    9.4500    0.0202
    9.4600    0.0210
    9.4700    0.0217
    9.4800    0.0225
    9.4900    0.0234
    9.5000    0.0242
    9.5100    0.0250
    9.5200    0.0258
    9.5300    0.0267
    9.5400    0.0275
    9.5500    0.0283
    9.5600    0.0292
    9.5700    0.0299
    9.5800    0.0308
    9.5900    0.0316
    9.6000    0.0324
    9.6100    0.0333
    9.6200    0.0342
    9.6300    0.0351
    9.6400    0.0359
    9.6500    0.0368
    9.6600    0.0375
    9.6700    0.0382
    9.6800    0.0391
    9.6900    0.0399
    9.7000    0.0407
    9.7100    0.0415
    9.7200    0.0423
    9.7300    0.0431
    9.7400    0.0439
    9.7500    0.0447
    9.7600    0.0453
    9.7700    0.0460
    9.7800    0.0468
    9.7900    0.0475
    9.8000    0.0483
    9.8100    0.0489
    9.8200    0.0498
    9.8300    0.0505
    9.8400    0.0513
    9.8500    0.0521
    9.8600    0.0527
    9.8700    0.0534
    9.8800    0.0540
    9.8900    0.0547
    9.9000    0.0554
    9.9100    0.0560
    9.9200    0.0567
    9.9300    0.0574
    9.9400    0.0580
    9.9500    0.0586
    9.9600    0.0592
    9.9700    0.0598
    9.9800    0.0605
    9.9900    0.0611
   10.0000    0.0617
    };

==> Data/Oscillator/sigma01/kf_exp_pos.tex <==
    \addplot[
    thick,
    green
    ]
    table {
         0    1.0000
    0.0100    0.9972
    0.0200    0.9928
    0.0300    0.9838
    0.0400    0.9791
    0.0500    0.9755
    0.0600    0.9713
    0.0700    0.9672
    0.0800    0.9637
    0.0900    0.9550
    0.1000    0.9460
    0.1100    0.9476
    0.1200    0.9490
    0.1300    0.9486
    0.1400    0.9456
    0.1500    0.9412
    0.1600    0.9380
    0.1700    0.9347
    0.1800    0.9293
    0.1900    0.9231
    0.2000    0.9184
    0.2100    0.9132
    0.2200    0.9091
    0.2300    0.9114
    0.2400    0.9089
    0.2500    0.9026
    0.2600    0.8965
    0.2700    0.8915
    0.2800    0.8927
    0.2900    0.8871
    0.3000    0.8833
    0.3100    0.8809
    0.3200    0.8744
    0.3300    0.8726
    0.3400    0.8697
    0.3500    0.8682
    0.3600    0.8710
    0.3700    0.8706
    0.3800    0.8631
    0.3900    0.8556
    0.4000    0.8499
    0.4100    0.8433
    0.4200    0.8366
    0.4300    0.8303
    0.4400    0.8290
    0.4500    0.8264
    0.4600    0.8199
    0.4700    0.8165
    0.4800    0.8149
    0.4900    0.8120
    0.5000    0.8089
    0.5100    0.8066
    0.5200    0.8022
    0.5300    0.7974
    0.5400    0.7931
    0.5500    0.7867
    0.5600    0.7817
    0.5700    0.7779
    0.5800    0.7728
    0.5900    0.7680
    0.6000    0.7645
    0.6100    0.7611
    0.6200    0.7567
    0.6300    0.7523
    0.6400    0.7479
    0.6500    0.7421
    0.6600    0.7370
    0.6700    0.7346
    0.6800    0.7301
    0.6900    0.7265
    0.7000    0.7234
    0.7100    0.7178
    0.7200    0.7118
    0.7300    0.7053
    0.7400    0.6988
    0.7500    0.6931
    0.7600    0.6901
    0.7700    0.6870
    0.7800    0.6827
    0.7900    0.6801
    0.8000    0.6739
    0.8100    0.6662
    0.8200    0.6616
    0.8300    0.6576
    0.8400    0.6522
    0.8500    0.6450
    0.8600    0.6400
    0.8700    0.6355
    0.8800    0.6308
    0.8900    0.6257
    0.9000    0.6184
    0.9100    0.6127
    0.9200    0.6092
    0.9300    0.6065
    0.9400    0.6016
    0.9500    0.5943
    0.9600    0.5873
    0.9700    0.5813
    0.9800    0.5758
    0.9900    0.5714
    1.0000    0.5666
    1.0100    0.5591
    1.0200    0.5531
    1.0300    0.5493
    1.0400    0.5448
    1.0500    0.5382
    1.0600    0.5325
    1.0700    0.5265
    1.0800    0.5203
    1.0900    0.5161
    1.1000    0.5121
    1.1100    0.5060
    1.1200    0.4996
    1.1300    0.4942
    1.1400    0.4903
    1.1500    0.4873
    1.1600    0.4827
    1.1700    0.4787
    1.1800    0.4741
    1.1900    0.4682
    1.2000    0.4640
    1.2100    0.4610
    1.2200    0.4574
    1.2300    0.4533
    1.2400    0.4483
    1.2500    0.4437
    1.2600    0.4389
    1.2700    0.4338
    1.2800    0.4296
    1.2900    0.4256
    1.3000    0.4213
    1.3100    0.4165
    1.3200    0.4127
    1.3300    0.4079
    1.3400    0.4026
    1.3500    0.3989
    1.3600    0.3952
    1.3700    0.3903
    1.3800    0.3857
    1.3900    0.3811
    1.4000    0.3766
    1.4100    0.3721
    1.4200    0.3674
    1.4300    0.3629
    1.4400    0.3593
    1.4500    0.3555
    1.4600    0.3521
    1.4700    0.3473
    1.4800    0.3413
    1.4900    0.3369
    1.5000    0.3322
    1.5100    0.3266
    1.5200    0.3218
    1.5300    0.3180
    1.5400    0.3139
    1.5500    0.3098
    1.5600    0.3052
    1.5700    0.3001
    1.5800    0.2955
    1.5900    0.2908
    1.6000    0.2861
    1.6100    0.2831
    1.6200    0.2796
    1.6300    0.2753
    1.6400    0.2708
    1.6500    0.2666
    1.6600    0.2626
    1.6700    0.2579
    1.6800    0.2536
    1.6900    0.2493
    1.7000    0.2454
    1.7100    0.2410
    1.7200    0.2382
    1.7300    0.2351
    1.7400    0.2303
    1.7500    0.2275
    1.7600    0.2240
    1.7700    0.2196
    1.7800    0.2153
    1.7900    0.2112
    1.8000    0.2078
    1.8100    0.2041
    1.8200    0.2003
    1.8300    0.1961
    1.8400    0.1930
    1.8500    0.1888
    1.8600    0.1831
    1.8700    0.1789
    1.8800    0.1750
    1.8900    0.1707
    1.9000    0.1663
    1.9100    0.1615
    1.9200    0.1572
    1.9300    0.1531
    1.9400    0.1487
    1.9500    0.1446
    1.9600    0.1402
    1.9700    0.1368
    1.9800    0.1332
    1.9900    0.1298
    2.0000    0.1268
    2.0100    0.1224
    2.0200    0.1180
    2.0300    0.1146
    2.0400    0.1118
    2.0500    0.1087
    2.0600    0.1052
    2.0700    0.1021
    2.0800    0.0983
    2.0900    0.0941
    2.1000    0.0899
    2.1100    0.0856
    2.1200    0.0824
    2.1300    0.0795
    2.1400    0.0772
    2.1500    0.0749
    2.1600    0.0706
    2.1700    0.0671
    2.1800    0.0650
    2.1900    0.0619
    2.2000    0.0584
    2.2100    0.0556
    2.2200    0.0527
    2.2300    0.0499
    2.2400    0.0469
    2.2500    0.0436
    2.2600    0.0406
    2.2700    0.0372
    2.2800    0.0343
    2.2900    0.0317
    2.3000    0.0288
    2.3100    0.0258
    2.3200    0.0221
    2.3300    0.0187
    2.3400    0.0156
    2.3500    0.0130
    2.3600    0.0106
    2.3700    0.0081
    2.3800    0.0049
    2.3900    0.0011
    2.4000   -0.0019
    2.4100   -0.0048
    2.4200   -0.0074
    2.4300   -0.0092
    2.4400   -0.0118
    2.4500   -0.0146
    2.4600   -0.0166
    2.4700   -0.0188
    2.4800   -0.0210
    2.4900   -0.0228
    2.5000   -0.0251
    2.5100   -0.0275
    2.5200   -0.0297
    2.5300   -0.0325
    2.5400   -0.0351
    2.5500   -0.0375
    2.5600   -0.0403
    2.5700   -0.0423
    2.5800   -0.0443
    2.5900   -0.0459
    2.6000   -0.0476
    2.6100   -0.0502
    2.6200   -0.0520
    2.6300   -0.0530
    2.6400   -0.0545
    2.6500   -0.0572
    2.6600   -0.0595
    2.6700   -0.0620
    2.6800   -0.0649
    2.6900   -0.0672
    2.7000   -0.0690
    2.7100   -0.0703
    2.7200   -0.0723
    2.7300   -0.0743
    2.7400   -0.0763
    2.7500   -0.0785
    2.7600   -0.0799
    2.7700   -0.0814
    2.7800   -0.0837
    2.7900   -0.0861
    2.8000   -0.0881
    2.8100   -0.0897
    2.8200   -0.0907
    2.8300   -0.0921
    2.8400   -0.0941
    2.8500   -0.0963
    2.8600   -0.0981
    2.8700   -0.0995
    2.8800   -0.1018
    2.8900   -0.1032
    2.9000   -0.1042
    2.9100   -0.1057
    2.9200   -0.1077
    2.9300   -0.1098
    2.9400   -0.1113
    2.9500   -0.1133
    2.9600   -0.1156
    2.9700   -0.1175
    2.9800   -0.1192
    2.9900   -0.1212
    3.0000   -0.1230
    3.0100   -0.1237
    3.0200   -0.1250
    3.0300   -0.1269
    3.0400   -0.1284
    3.0500   -0.1295
    3.0600   -0.1306
    3.0700   -0.1320
    3.0800   -0.1336
    3.0900   -0.1354
    3.1000   -0.1369
    3.1100   -0.1377
    3.1200   -0.1385
    3.1300   -0.1403
    3.1400   -0.1420
    3.1500   -0.1433
    3.1600   -0.1448
    3.1700   -0.1464
    3.1800   -0.1481
    3.1900   -0.1498
    3.2000   -0.1514
    3.2100   -0.1531
    3.2200   -0.1545
    3.2300   -0.1557
    3.2400   -0.1570
    3.2500   -0.1583
    3.2600   -0.1596
    3.2700   -0.1607
    3.2800   -0.1614
    3.2900   -0.1620
    3.3000   -0.1631
    3.3100   -0.1641
    3.3200   -0.1651
    3.3300   -0.1667
    3.3400   -0.1690
    3.3500   -0.1713
    3.3600   -0.1728
    3.3700   -0.1740
    3.3800   -0.1754
    3.3900   -0.1766
    3.4000   -0.1776
    3.4100   -0.1790
    3.4200   -0.1799
    3.4300   -0.1804
    3.4400   -0.1803
    3.4500   -0.1803
    3.4600   -0.1811
    3.4700   -0.1820
    3.4800   -0.1831
    3.4900   -0.1838
    3.5000   -0.1851
    3.5100   -0.1865
    3.5200   -0.1870
    3.5300   -0.1876
    3.5400   -0.1884
    3.5500   -0.1885
    3.5600   -0.1886
    3.5700   -0.1886
    3.5800   -0.1896
    3.5900   -0.1911
    3.6000   -0.1915
    3.6100   -0.1916
    3.6200   -0.1920
    3.6300   -0.1924
    3.6400   -0.1924
    3.6500   -0.1924
    3.6600   -0.1931
    3.6700   -0.1937
    3.6800   -0.1942
    3.6900   -0.1944
    3.7000   -0.1943
    3.7100   -0.1944
    3.7200   -0.1944
    3.7300   -0.1948
    3.7400   -0.1952
    3.7500   -0.1953
    3.7600   -0.1958
    3.7700   -0.1965
    3.7800   -0.1962
    3.7900   -0.1962
    3.8000   -0.1960
    3.8100   -0.1954
    3.8200   -0.1955
    3.8300   -0.1958
    3.8400   -0.1959
    3.8500   -0.1960
    3.8600   -0.1957
    3.8700   -0.1956
    3.8800   -0.1956
    3.8900   -0.1949
    3.9000   -0.1941
    3.9100   -0.1935
    3.9200   -0.1934
    3.9300   -0.1938
    3.9400   -0.1937
    3.9500   -0.1935
    3.9600   -0.1938
    3.9700   -0.1946
    3.9800   -0.1944
    3.9900   -0.1942
    4.0000   -0.1935
    4.0100   -0.1932
    4.0200   -0.1936
    4.0300   -0.1930
    4.0400   -0.1930
    4.0500   -0.1927
    4.0600   -0.1925
    4.0700   -0.1921
    4.0800   -0.1914
    4.0900   -0.1914
    4.1000   -0.1922
    4.1100   -0.1926
    4.1200   -0.1918
    4.1300   -0.1909
    4.1400   -0.1904
    4.1500   -0.1896
    4.1600   -0.1893
    4.1700   -0.1887
    4.1800   -0.1879
    4.1900   -0.1877
    4.2000   -0.1871
    4.2100   -0.1865
    4.2200   -0.1865
    4.2300   -0.1859
    4.2400   -0.1846
    4.2500   -0.1833
    4.2600   -0.1815
    4.2700   -0.1804
    4.2800   -0.1799
    4.2900   -0.1800
    4.3000   -0.1797
    4.3100   -0.1788
    4.3200   -0.1776
    4.3300   -0.1767
    4.3400   -0.1760
    4.3500   -0.1748
    4.3600   -0.1742
    4.3700   -0.1733
    4.3800   -0.1720
    4.3900   -0.1712
    4.4000   -0.1698
    4.4100   -0.1681
    4.4200   -0.1671
    4.4300   -0.1660
    4.4400   -0.1649
    4.4500   -0.1639
    4.4600   -0.1626
    4.4700   -0.1616
    4.4800   -0.1610
    4.4900   -0.1601
    4.5000   -0.1583
    4.5100   -0.1567
    4.5200   -0.1561
    4.5300   -0.1553
    4.5400   -0.1544
    4.5500   -0.1535
    4.5600   -0.1523
    4.5700   -0.1510
    4.5800   -0.1500
    4.5900   -0.1491
    4.6000   -0.1484
    4.6100   -0.1477
    4.6200   -0.1471
    4.6300   -0.1464
    4.6400   -0.1456
    4.6500   -0.1449
    4.6600   -0.1438
    4.6700   -0.1429
    4.6800   -0.1420
    4.6900   -0.1404
    4.7000   -0.1394
    4.7100   -0.1379
    4.7200   -0.1367
    4.7300   -0.1359
    4.7400   -0.1350
    4.7500   -0.1341
    4.7600   -0.1332
    4.7700   -0.1323
    4.7800   -0.1312
    4.7900   -0.1303
    4.8000   -0.1298
    4.8100   -0.1288
    4.8200   -0.1266
    4.8300   -0.1238
    4.8400   -0.1218
    4.8500   -0.1205
    4.8600   -0.1191
    4.8700   -0.1177
    4.8800   -0.1163
    4.8900   -0.1157
    4.9000   -0.1147
    4.9100   -0.1133
    4.9200   -0.1129
    4.9300   -0.1111
    4.9400   -0.1087
    4.9500   -0.1073
    4.9600   -0.1050
    4.9700   -0.1036
    4.9800   -0.1025
    4.9900   -0.1005
    5.0000   -0.0987
    5.0100   -0.0970
    5.0200   -0.0955
    5.0300   -0.0937
    5.0400   -0.0920
    5.0500   -0.0909
    5.0600   -0.0893
    5.0700   -0.0868
    5.0800   -0.0847
    5.0900   -0.0834
    5.1000   -0.0817
    5.1100   -0.0796
    5.1200   -0.0773
    5.1300   -0.0752
    5.1400   -0.0736
    5.1500   -0.0719
    5.1600   -0.0700
    5.1700   -0.0679
    5.1800   -0.0661
    5.1900   -0.0649
    5.2000   -0.0626
    5.2100   -0.0606
    5.2200   -0.0592
    5.2300   -0.0579
    5.2400   -0.0565
    5.2500   -0.0549
    5.2600   -0.0531
    5.2700   -0.0516
    5.2800   -0.0500
    5.2900   -0.0484
    5.3000   -0.0469
    5.3100   -0.0454
    5.3200   -0.0441
    5.3300   -0.0414
    5.3400   -0.0375
    5.3500   -0.0345
    5.3600   -0.0321
    5.3700   -0.0305
    5.3800   -0.0293
    5.3900   -0.0279
    5.4000   -0.0261
    5.4100   -0.0240
    5.4200   -0.0221
    5.4300   -0.0204
    5.4400   -0.0190
    5.4500   -0.0175
    5.4600   -0.0153
    5.4700   -0.0131
    5.4800   -0.0112
    5.4900   -0.0092
    5.5000   -0.0070
    5.5100   -0.0056
    5.5200   -0.0043
    5.5300   -0.0026
    5.5400   -0.0015
    5.5500   -0.0008
    5.5600    0.0005
    5.5700    0.0025
    5.5800    0.0044
    5.5900    0.0061
    5.6000    0.0078
    5.6100    0.0085
    5.6200    0.0097
    5.6300    0.0112
    5.6400    0.0129
    5.6500    0.0156
    5.6600    0.0177
    5.6700    0.0195
    5.6800    0.0220
    5.6900    0.0235
    5.7000    0.0247
    5.7100    0.0266
    5.7200    0.0285
    5.7300    0.0305
    5.7400    0.0325
    5.7500    0.0346
    5.7600    0.0364
    5.7700    0.0381
    5.7800    0.0393
    5.7900    0.0397
    5.8000    0.0415
    5.8100    0.0434
    5.8200    0.0448
    5.8300    0.0471
    5.8400    0.0489
    5.8500    0.0499
    5.8600    0.0511
    5.8700    0.0527
    5.8800    0.0544
    5.8900    0.0557
    5.9000    0.0565
    5.9100    0.0575
    5.9200    0.0589
    5.9300    0.0603
    5.9400    0.0616
    5.9500    0.0627
    5.9600    0.0642
    5.9700    0.0653
    5.9800    0.0660
    5.9900    0.0680
    6.0000    0.0694
    6.0100    0.0705
    6.0200    0.0722
    6.0300    0.0735
    6.0400    0.0747
    6.0500    0.0764
    6.0600    0.0777
    6.0700    0.0790
    6.0800    0.0811
    6.0900    0.0828
    6.1000    0.0844
    6.1100    0.0854
    6.1200    0.0866
    6.1300    0.0877
    6.1400    0.0892
    6.1500    0.0912
    6.1600    0.0927
    6.1700    0.0941
    6.1800    0.0947
    6.1900    0.0949
    6.2000    0.0960
    6.2100    0.0981
    6.2200    0.1004
    6.2300    0.1019
    6.2400    0.1030
    6.2500    0.1041
    6.2600    0.1057
    6.2700    0.1070
    6.2800    0.1088
    6.2900    0.1102
    6.3000    0.1108
    6.3100    0.1120
    6.3200    0.1125
    6.3300    0.1133
    6.3400    0.1147
    6.3500    0.1158
    6.3600    0.1171
    6.3700    0.1187
    6.3800    0.1204
    6.3900    0.1215
    6.4000    0.1224
    6.4100    0.1236
    6.4200    0.1244
    6.4300    0.1247
    6.4400    0.1253
    6.4500    0.1261
    6.4600    0.1276
    6.4700    0.1294
    6.4800    0.1304
    6.4900    0.1309
    6.5000    0.1320
    6.5100    0.1343
    6.5200    0.1360
    6.5300    0.1367
    6.5400    0.1370
    6.5500    0.1377
    6.5600    0.1389
    6.5700    0.1401
    6.5800    0.1410
    6.5900    0.1415
    6.6000    0.1421
    6.6100    0.1431
    6.6200    0.1441
    6.6300    0.1445
    6.6400    0.1451
    6.6500    0.1459
    6.6600    0.1471
    6.6700    0.1475
    6.6800    0.1477
    6.6900    0.1478
    6.7000    0.1482
    6.7100    0.1492
    6.7200    0.1494
    6.7300    0.1488
    6.7400    0.1488
    6.7500    0.1496
    6.7600    0.1504
    6.7700    0.1505
    6.7800    0.1500
    6.7900    0.1503
    6.8000    0.1510
    6.8100    0.1511
    6.8200    0.1519
    6.8300    0.1525
    6.8400    0.1526
    6.8500    0.1531
    6.8600    0.1539
    6.8700    0.1542
    6.8800    0.1542
    6.8900    0.1555
    6.9000    0.1562
    6.9100    0.1560
    6.9200    0.1564
    6.9300    0.1563
    6.9400    0.1560
    6.9500    0.1560
    6.9600    0.1572
    6.9700    0.1577
    6.9800    0.1577
    6.9900    0.1579
    7.0000    0.1583
    7.0100    0.1593
    7.0200    0.1594
    7.0300    0.1596
    7.0400    0.1598
    7.0500    0.1601
    7.0600    0.1605
    7.0700    0.1600
    7.0800    0.1597
    7.0900    0.1603
    7.1000    0.1604
    7.1100    0.1597
    7.1200    0.1600
    7.1300    0.1596
    7.1400    0.1590
    7.1500    0.1594
    7.1600    0.1595
    7.1700    0.1592
    7.1800    0.1587
    7.1900    0.1586
    7.2000    0.1586
    7.2100    0.1589
    7.2200    0.1587
    7.2300    0.1588
    7.2400    0.1590
    7.2500    0.1584
    7.2600    0.1577
    7.2700    0.1575
    7.2800    0.1575
    7.2900    0.1574
    7.3000    0.1572
    7.3100    0.1577
    7.3200    0.1575
    7.3300    0.1563
    7.3400    0.1559
    7.3500    0.1553
    7.3600    0.1553
    7.3700    0.1554
    7.3800    0.1548
    7.3900    0.1543
    7.4000    0.1540
    7.4100    0.1534
    7.4200    0.1528
    7.4300    0.1519
    7.4400    0.1508
    7.4500    0.1500
    7.4600    0.1488
    7.4700    0.1482
    7.4800    0.1473
    7.4900    0.1460
    7.5000    0.1446
    7.5100    0.1428
    7.5200    0.1414
    7.5300    0.1410
    7.5400    0.1406
    7.5500    0.1397
    7.5600    0.1385
    7.5700    0.1379
    7.5800    0.1375
    7.5900    0.1369
    7.6000    0.1366
    7.6100    0.1357
    7.6200    0.1351
    7.6300    0.1349
    7.6400    0.1342
    7.6500    0.1335
    7.6600    0.1336
    7.6700    0.1331
    7.6800    0.1320
    7.6900    0.1311
    7.7000    0.1304
    7.7100    0.1297
    7.7200    0.1289
    7.7300    0.1279
    7.7400    0.1275
    7.7500    0.1268
    7.7600    0.1258
    7.7700    0.1245
    7.7800    0.1227
    7.7900    0.1209
    7.8000    0.1190
    7.8100    0.1176
    7.8200    0.1159
    7.8300    0.1149
    7.8400    0.1148
    7.8500    0.1132
    7.8600    0.1110
    7.8700    0.1096
    7.8800    0.1079
    7.8900    0.1060
    7.9000    0.1051
    7.9100    0.1042
    7.9200    0.1029
    7.9300    0.1014
    7.9400    0.0997
    7.9500    0.0979
    7.9600    0.0964
    7.9700    0.0951
    7.9800    0.0939
    7.9900    0.0932
    8.0000    0.0926
    8.0100    0.0916
    8.0200    0.0901
    8.0300    0.0883
    8.0400    0.0866
    8.0500    0.0857
    8.0600    0.0845
    8.0700    0.0830
    8.0800    0.0817
    8.0900    0.0809
    8.1000    0.0793
    8.1100    0.0775
    8.1200    0.0764
    8.1300    0.0750
    8.1400    0.0738
    8.1500    0.0726
    8.1600    0.0708
    8.1700    0.0692
    8.1800    0.0681
    8.1900    0.0666
    8.2000    0.0654
    8.2100    0.0638
    8.2200    0.0617
    8.2300    0.0590
    8.2400    0.0568
    8.2500    0.0553
    8.2600    0.0534
    8.2700    0.0522
    8.2800    0.0511
    8.2900    0.0495
    8.3000    0.0476
    8.3100    0.0458
    8.3200    0.0445
    8.3300    0.0428
    8.3400    0.0407
    8.3500    0.0396
    8.3600    0.0378
    8.3700    0.0360
    8.3800    0.0351
    8.3900    0.0335
    8.4000    0.0312
    8.4100    0.0294
    8.4200    0.0283
    8.4300    0.0272
    8.4400    0.0261
    8.4500    0.0244
    8.4600    0.0227
    8.4700    0.0213
    8.4800    0.0194
    8.4900    0.0172
    8.5000    0.0156
    8.5100    0.0145
    8.5200    0.0132
    8.5300    0.0125
    8.5400    0.0110
    8.5500    0.0093
    8.5600    0.0080
    8.5700    0.0067
    8.5800    0.0057
    8.5900    0.0048
    8.6000    0.0032
    8.6100    0.0014
    8.6200   -0.0002
    8.6300   -0.0007
    8.6400   -0.0009
    8.6500   -0.0015
    8.6600   -0.0022
    8.6700   -0.0037
    8.6800   -0.0049
    8.6900   -0.0065
    8.7000   -0.0078
    8.7100   -0.0089
    8.7200   -0.0110
    8.7300   -0.0127
    8.7400   -0.0143
    8.7500   -0.0169
    8.7600   -0.0188
    8.7700   -0.0204
    8.7800   -0.0226
    8.7900   -0.0244
    8.8000   -0.0260
    8.8100   -0.0278
    8.8200   -0.0292
    8.8300   -0.0309
    8.8400   -0.0331
    8.8500   -0.0356
    8.8600   -0.0378
    8.8700   -0.0391
    8.8800   -0.0406
    8.8900   -0.0422
    8.9000   -0.0433
    8.9100   -0.0444
    8.9200   -0.0453
    8.9300   -0.0466
    8.9400   -0.0486
    8.9500   -0.0502
    8.9600   -0.0519
    8.9700   -0.0531
    8.9800   -0.0537
    8.9900   -0.0547
    9.0000   -0.0563
    9.0100   -0.0576
    9.0200   -0.0591
    9.0300   -0.0607
    9.0400   -0.0623
    9.0500   -0.0639
    9.0600   -0.0649
    9.0700   -0.0657
    9.0800   -0.0665
    9.0900   -0.0679
    9.1000   -0.0695
    9.1100   -0.0710
    9.1200   -0.0726
    9.1300   -0.0737
    9.1400   -0.0746
    9.1500   -0.0752
    9.1600   -0.0760
    9.1700   -0.0773
    9.1800   -0.0789
    9.1900   -0.0809
    9.2000   -0.0829
    9.2100   -0.0847
    9.2200   -0.0863
    9.2300   -0.0869
    9.2400   -0.0879
    9.2500   -0.0892
    9.2600   -0.0905
    9.2700   -0.0913
    9.2800   -0.0916
    9.2900   -0.0926
    9.3000   -0.0939
    9.3100   -0.0953
    9.3200   -0.0968
    9.3300   -0.0976
    9.3400   -0.0982
    9.3500   -0.0996
    9.3600   -0.1011
    9.3700   -0.1022
    9.3800   -0.1038
    9.3900   -0.1047
    9.4000   -0.1055
    9.4100   -0.1066
    9.4200   -0.1076
    9.4300   -0.1079
    9.4400   -0.1087
    9.4500   -0.1103
    9.4600   -0.1121
    9.4700   -0.1137
    9.4800   -0.1152
    9.4900   -0.1161
    9.5000   -0.1176
    9.5100   -0.1191
    9.5200   -0.1202
    9.5300   -0.1210
    9.5400   -0.1219
    9.5500   -0.1231
    9.5600   -0.1242
    9.5700   -0.1256
    9.5800   -0.1267
    9.5900   -0.1277
    9.6000   -0.1289
    9.6100   -0.1295
    9.6200   -0.1299
    9.6300   -0.1300
    9.6400   -0.1304
    9.6500   -0.1309
    9.6600   -0.1320
    9.6700   -0.1333
    9.6800   -0.1336
    9.6900   -0.1344
    9.7000   -0.1351
    9.7100   -0.1353
    9.7200   -0.1355
    9.7300   -0.1358
    9.7400   -0.1362
    9.7500   -0.1368
    9.7600   -0.1380
    9.7700   -0.1390
    9.7800   -0.1397
    9.7900   -0.1399
    9.8000   -0.1404
    9.8100   -0.1416
    9.8200   -0.1413
    9.8300   -0.1411
    9.8400   -0.1415
    9.8500   -0.1410
    9.8600   -0.1414
    9.8700   -0.1422
    9.8800   -0.1427
    9.8900   -0.1432
    9.9000   -0.1429
    9.9100   -0.1435
    9.9200   -0.1439
    9.9300   -0.1434
    9.9400   -0.1438
    9.9500   -0.1444
    9.9600   -0.1447
    9.9700   -0.1449
    9.9800   -0.1448
    9.9900   -0.1444
   10.0000   -0.1444
    };

==> Data/Oscillator/sigma01/kf_exp_vel.tex <==
    \addplot[
    thick,
    green
    ]
    table {
         0         0
    0.0100   -0.0099
    0.0200   -0.0196
    0.0300   -0.0291
    0.0400   -0.0384
    0.0500   -0.0475
    0.0600   -0.0564
    0.0700   -0.0652
    0.0800   -0.0738
    0.0900   -0.0821
    0.1000   -0.0903
    0.1100   -0.0983
    0.1200   -0.1062
    0.1300   -0.1140
    0.1400   -0.1216
    0.1500   -0.1291
    0.1600   -0.1364
    0.1700   -0.1436
    0.1800   -0.1506
    0.1900   -0.1574
    0.2000   -0.1641
    0.2100   -0.1706
    0.2200   -0.1770
    0.2300   -0.1834
    0.2400   -0.1896
    0.2500   -0.1956
    0.2600   -0.2014
    0.2700   -0.2071
    0.2800   -0.2129
    0.2900   -0.2183
    0.3000   -0.2237
    0.3100   -0.2290
    0.3200   -0.2341
    0.3300   -0.2392
    0.3400   -0.2441
    0.3500   -0.2490
    0.3600   -0.2540
    0.3700   -0.2588
    0.3800   -0.2633
    0.3900   -0.2675
    0.4000   -0.2718
    0.4100   -0.2758
    0.4200   -0.2797
    0.4300   -0.2835
    0.4400   -0.2875
    0.4500   -0.2913
    0.4600   -0.2948
    0.4700   -0.2983
    0.4800   -0.3019
    0.4900   -0.3053
    0.5000   -0.3087
    0.5100   -0.3120
    0.5200   -0.3151
    0.5300   -0.3181
    0.5400   -0.3210
    0.5500   -0.3237
    0.5600   -0.3263
    0.5700   -0.3290
    0.5800   -0.3315
    0.5900   -0.3339
    0.6000   -0.3364
    0.6100   -0.3388
    0.6200   -0.3410
    0.6300   -0.3432
    0.6400   -0.3453
    0.6500   -0.3471
    0.6600   -0.3490
    0.6700   -0.3510
    0.6800   -0.3528
    0.6900   -0.3546
    0.7000   -0.3564
    0.7100   -0.3578
    0.7200   -0.3592
    0.7300   -0.3604
    0.7400   -0.3615
    0.7500   -0.3626
    0.7600   -0.3640
    0.7700   -0.3652
    0.7800   -0.3664
    0.7900   -0.3676
    0.8000   -0.3684
    0.8100   -0.3689
    0.8200   -0.3697
    0.8300   -0.3705
    0.8400   -0.3711
    0.8500   -0.3714
    0.8600   -0.3719
    0.8700   -0.3724
    0.8800   -0.3728
    0.8900   -0.3732
    0.9000   -0.3731
    0.9100   -0.3732
    0.9200   -0.3736
    0.9300   -0.3740
    0.9400   -0.3741
    0.9500   -0.3738
    0.9600   -0.3735
    0.9700   -0.3732
    0.9800   -0.3730
    0.9900   -0.3728
    1.0000   -0.3726
    1.0100   -0.3719
    1.0200   -0.3714
    1.0300   -0.3711
    1.0400   -0.3707
    1.0500   -0.3700
    1.0600   -0.3693
    1.0700   -0.3685
    1.0800   -0.3677
    1.0900   -0.3671
    1.1000   -0.3665
    1.1100   -0.3656
    1.1200   -0.3645
    1.1300   -0.3636
    1.1400   -0.3628
    1.1500   -0.3622
    1.1600   -0.3613
    1.1700   -0.3605
    1.1800   -0.3595
    1.1900   -0.3583
    1.2000   -0.3573
    1.2100   -0.3565
    1.2200   -0.3556
    1.2300   -0.3545
    1.2400   -0.3533
    1.2500   -0.3522
    1.2600   -0.3509
    1.2700   -0.3496
    1.2800   -0.3484
    1.2900   -0.3472
    1.3000   -0.3460
    1.3100   -0.3446
    1.3200   -0.3434
    1.3300   -0.3420
    1.3400   -0.3404
    1.3500   -0.3391
    1.3600   -0.3378
    1.3700   -0.3363
    1.3800   -0.3348
    1.3900   -0.3333
    1.4000   -0.3317
    1.4100   -0.3302
    1.4200   -0.3286
    1.4300   -0.3270
    1.4400   -0.3255
    1.4500   -0.3239
    1.4600   -0.3224
    1.4700   -0.3208
    1.4800   -0.3189
    1.4900   -0.3172
    1.5000   -0.3154
    1.5100   -0.3135
    1.5200   -0.3117
    1.5300   -0.3099
    1.5400   -0.3082
    1.5500   -0.3064
    1.5600   -0.3046
    1.5700   -0.3026
    1.5800   -0.3007
    1.5900   -0.2988
    1.6000   -0.2969
    1.6100   -0.2951
    1.6200   -0.2933
    1.6300   -0.2914
    1.6400   -0.2894
    1.6500   -0.2875
    1.6600   -0.2856
    1.6700   -0.2836
    1.6800   -0.2816
    1.6900   -0.2796
    1.7000   -0.2776
    1.7100   -0.2756
    1.7200   -0.2737
    1.7300   -0.2718
    1.7400   -0.2697
    1.7500   -0.2679
    1.7600   -0.2659
    1.7700   -0.2638
    1.7800   -0.2618
    1.7900   -0.2598
    1.8000   -0.2578
    1.8100   -0.2557
    1.8200   -0.2537
    1.8300   -0.2516
    1.8400   -0.2497
    1.8500   -0.2476
    1.8600   -0.2454
    1.8700   -0.2433
    1.8800   -0.2412
    1.8900   -0.2390
    1.9000   -0.2369
    1.9100   -0.2347
    1.9200   -0.2326
    1.9300   -0.2304
    1.9400   -0.2282
    1.9500   -0.2261
    1.9600   -0.2239
    1.9700   -0.2217
    1.9800   -0.2196
    1.9900   -0.2175
    2.0000   -0.2154
    2.0100   -0.2132
    2.0200   -0.2110
    2.0300   -0.2088
    2.0400   -0.2067
    2.0500   -0.2046
    2.0600   -0.2025
    2.0700   -0.2003
    2.0800   -0.1982
    2.0900   -0.1960
    2.1000   -0.1939
    2.1100   -0.1917
    2.1200   -0.1895
    2.1300   -0.1874
    2.1400   -0.1853
    2.1500   -0.1832
    2.1600   -0.1810
    2.1700   -0.1789
    2.1800   -0.1768
    2.1900   -0.1747
    2.2000   -0.1726
    2.2100   -0.1705
    2.2200   -0.1684
    2.2300   -0.1663
    2.2400   -0.1642
    2.2500   -0.1622
    2.2600   -0.1601
    2.2700   -0.1580
    2.2800   -0.1560
    2.2900   -0.1539
    2.3000   -0.1518
    2.3100   -0.1498
    2.3200   -0.1478
    2.3300   -0.1457
    2.3400   -0.1437
    2.3500   -0.1416
    2.3600   -0.1396
    2.3700   -0.1375
    2.3800   -0.1355
    2.3900   -0.1335
    2.4000   -0.1315
    2.4100   -0.1295
    2.4200   -0.1275
    2.4300   -0.1255
    2.4400   -0.1235
    2.4500   -0.1215
    2.4600   -0.1195
    2.4700   -0.1175
    2.4800   -0.1156
    2.4900   -0.1136
    2.5000   -0.1117
    2.5100   -0.1097
    2.5200   -0.1078
    2.5300   -0.1059
    2.5400   -0.1040
    2.5500   -0.1022
    2.5600   -0.1003
    2.5700   -0.0984
    2.5800   -0.0965
    2.5900   -0.0946
    2.6000   -0.0927
    2.6100   -0.0909
    2.6200   -0.0891
    2.6300   -0.0872
    2.6400   -0.0853
    2.6500   -0.0836
    2.6600   -0.0818
    2.6700   -0.0801
    2.6800   -0.0783
    2.6900   -0.0766
    2.7000   -0.0748
    2.7100   -0.0730
    2.7200   -0.0713
    2.7300   -0.0695
    2.7400   -0.0678
    2.7500   -0.0661
    2.7600   -0.0644
    2.7700   -0.0626
    2.7800   -0.0610
    2.7900   -0.0593
    2.8000   -0.0577
    2.8100   -0.0560
    2.8200   -0.0543
    2.8300   -0.0526
    2.8400   -0.0510
    2.8500   -0.0494
    2.8600   -0.0478
    2.8700   -0.0462
    2.8800   -0.0446
    2.8900   -0.0430
    2.9000   -0.0414
    2.9100   -0.0398
    2.9200   -0.0382
    2.9300   -0.0367
    2.9400   -0.0352
    2.9500   -0.0337
    2.9600   -0.0322
    2.9700   -0.0307
    2.9800   -0.0292
    2.9900   -0.0277
    3.0000   -0.0262
    3.0100   -0.0246
    3.0200   -0.0231
    3.0300   -0.0217
    3.0400   -0.0202
    3.0500   -0.0187
    3.0600   -0.0172
    3.0700   -0.0158
    3.0800   -0.0144
    3.0900   -0.0130
    3.1000   -0.0116
    3.1100   -0.0101
    3.1200   -0.0086
    3.1300   -0.0073
    3.1400   -0.0059
    3.1500   -0.0046
    3.1600   -0.0032
    3.1700   -0.0019
    3.1800   -0.0006
    3.1900    0.0007
    3.2000    0.0020
    3.2100    0.0033
    3.2200    0.0046
    3.2300    0.0060
    3.2400    0.0073
    3.2500    0.0086
    3.2600    0.0099
    3.2700    0.0112
    3.2800    0.0125
    3.2900    0.0139
    3.3000    0.0151
    3.3100    0.0164
    3.3200    0.0176
    3.3300    0.0188
    3.3400    0.0199
    3.3500    0.0210
    3.3600    0.0222
    3.3700    0.0234
    3.3800    0.0246
    3.3900    0.0258
    3.4000    0.0270
    3.4100    0.0282
    3.4200    0.0294
    3.4300    0.0306
    3.4400    0.0319
    3.4500    0.0332
    3.4600    0.0344
    3.4700    0.0355
    3.4800    0.0366
    3.4900    0.0377
    3.5000    0.0388
    3.5100    0.0398
    3.5200    0.0410
    3.5300    0.0421
    3.5400    0.0431
    3.5500    0.0443
    3.5600    0.0454
    3.5700    0.0465
    3.5800    0.0475
    3.5900    0.0484
    3.6000    0.0495
    3.6100    0.0506
    3.6200    0.0516
    3.6300    0.0526
    3.6400    0.0536
    3.6500    0.0546
    3.6600    0.0556
    3.6700    0.0565
    3.6800    0.0574
    3.6900    0.0584
    3.7000    0.0593
    3.7100    0.0603
    3.7200    0.0612
    3.7300    0.0621
    3.7400    0.0629
    3.7500    0.0638
    3.7600    0.0646
    3.7700    0.0654
    3.7800    0.0663
    3.7900    0.0672
    3.8000    0.0680
    3.8100    0.0689
    3.8200    0.0697
    3.8300    0.0704
    3.8400    0.0712
    3.8500    0.0719
    3.8600    0.0727
    3.8700    0.0735
    3.8800    0.0742
    3.8900    0.0750
    3.9000    0.0758
    3.9100    0.0765
    3.9200    0.0772
    3.9300    0.0778
    3.9400    0.0784
    3.9500    0.0791
    3.9600    0.0796
    3.9700    0.0801
    3.9800    0.0808
    3.9900    0.0814
    4.0000    0.0820
    4.0100    0.0826
    4.0200    0.0831
    4.0300    0.0837
    4.0400    0.0843
    4.0500    0.0848
    4.0600    0.0853
    4.0700    0.0859
    4.0800    0.0864
    4.0900    0.0869
    4.1000    0.0873
    4.1100    0.0877
    4.1200    0.0882
    4.1300    0.0888
    4.1400    0.0893
    4.1500    0.0898
    4.1600    0.0902
    4.1700    0.0906
    4.1800    0.0911
    4.1900    0.0915
    4.2000    0.0919
    4.2100    0.0923
    4.2200    0.0926
    4.2300    0.0930
    4.2400    0.0934
    4.2500    0.0939
    4.2600    0.0943
    4.2700    0.0947
    4.2800    0.0950
    4.2900    0.0952
    4.3000    0.0954
    4.3100    0.0957
    4.3200    0.0961
    4.3300    0.0963
    4.3400    0.0966
    4.3500    0.0968
    4.3600    0.0970
    4.3700    0.0973
    4.3800    0.0975
    4.3900    0.0977
    4.4000    0.0979
    4.4100    0.0982
    4.4200    0.0984
    4.4300    0.0985
    4.4400    0.0986
    4.4500    0.0988
    4.4600    0.0989
    4.4700    0.0990
    4.4800    0.0990
    4.4900    0.0991
    4.5000    0.0992
    4.5100    0.0993
    4.5200    0.0993
    4.5300    0.0993
    4.5400    0.0993
    4.5500    0.0993
    4.5600    0.0993
    4.5700    0.0993
    4.5800    0.0993
    4.5900    0.0992
    4.6000    0.0992
    4.6100    0.0991
    4.6200    0.0990
    4.6300    0.0989
    4.6400    0.0988
    4.6500    0.0987
    4.6600    0.0986
    4.6700    0.0985
    4.6800    0.0984
    4.6900    0.0983
    4.7000    0.0982
    4.7100    0.0981
    4.7200    0.0980
    4.7300    0.0978
    4.7400    0.0977
    4.7500    0.0975
    4.7600    0.0973
    4.7700    0.0971
    4.7800    0.0969
    4.7900    0.0968
    4.8000    0.0965
    4.8100    0.0963
    4.8200    0.0962
    4.8300    0.0962
    4.8400    0.0961
    4.8500    0.0958
    4.8600    0.0956
    4.8700    0.0954
    4.8800    0.0951
    4.8900    0.0948
    4.9000    0.0945
    4.9100    0.0942
    4.9200    0.0938
    4.9300    0.0936
    4.9400    0.0934
    4.9500    0.0931
    4.9600    0.0929
    4.9700    0.0926
    4.9800    0.0922
    4.9900    0.0919
    5.0000    0.0916
    5.0100    0.0912
    5.0200    0.0909
    5.0300    0.0905
    5.0400    0.0901
    5.0500    0.0897
    5.0600    0.0893
    5.0700    0.0890
    5.0800    0.0886
    5.0900    0.0881
    5.1000    0.0877
    5.1100    0.0873
    5.1200    0.0869
    5.1300    0.0865
    5.1400    0.0860
    5.1500    0.0855
    5.1600    0.0850
    5.1700    0.0845
    5.1800    0.0840
    5.1900    0.0834
    5.2000    0.0829
    5.2100    0.0824
    5.2200    0.0818
    5.2300    0.0812
    5.2400    0.0806
    5.2500    0.0800
    5.2600    0.0794
    5.2700    0.0788
    5.2800    0.0782
    5.2900    0.0776
    5.3000    0.0770
    5.3100    0.0763
    5.3200    0.0757
    5.3300    0.0752
    5.3400    0.0748
    5.3500    0.0743
    5.3600    0.0737
    5.3700    0.0729
    5.3800    0.0722
    5.3900    0.0714
    5.4000    0.0707
    5.4100    0.0701
    5.4200    0.0694
    5.4300    0.0686
    5.4400    0.0679
    5.4500    0.0671
    5.4600    0.0664
    5.4700    0.0657
    5.4800    0.0650
    5.4900    0.0643
    5.5000    0.0635
    5.5100    0.0627
    5.5200    0.0619
    5.5300    0.0611
    5.5400    0.0602
    5.5500    0.0593
    5.5600    0.0585
    5.5700    0.0578
    5.5800    0.0570
    5.5900    0.0562
    5.6000    0.0554
    5.6100    0.0545
    5.6200    0.0537
    5.6300    0.0529
    5.6400    0.0521
    5.6500    0.0514
    5.6600    0.0506
    5.6700    0.0498
    5.6800    0.0491
    5.6900    0.0482
    5.7000    0.0474
    5.7100    0.0465
    5.7200    0.0457
    5.7300    0.0449
    5.7400    0.0441
    5.7500    0.0433
    5.7600    0.0424
    5.7700    0.0416
    5.7800    0.0407
    5.7900    0.0396
    5.8000    0.0388
    5.8100    0.0380
    5.8200    0.0371
    5.8300    0.0363
    5.8400    0.0354
    5.8500    0.0345
    5.8600    0.0335
    5.8700    0.0327
    5.8800    0.0318
    5.8900    0.0309
    5.9000    0.0299
    5.9100    0.0290
    5.9200    0.0281
    5.9300    0.0272
    5.9400    0.0263
    5.9500    0.0254
    5.9600    0.0245
    5.9700    0.0236
    5.9800    0.0227
    5.9900    0.0219
    6.0000    0.0210
    6.0100    0.0201
    6.0200    0.0192
    6.0300    0.0184
    6.0400    0.0175
    6.0500    0.0166
    6.0600    0.0158
    6.0700    0.0149
    6.0800    0.0141
    6.0900    0.0133
    6.1000    0.0124
    6.1100    0.0115
    6.1200    0.0106
    6.1300    0.0097
    6.1400    0.0088
    6.1500    0.0080
    6.1600    0.0072
    6.1700    0.0063
    6.1800    0.0053
    6.1900    0.0043
    6.2000    0.0034
    6.2100    0.0027
    6.2200    0.0019
    6.2300    0.0011
    6.2400    0.0002
    6.2500   -0.0007
    6.2600   -0.0015
    6.2700   -0.0024
    6.2800   -0.0032
    6.2900   -0.0041
    6.3000   -0.0050
    6.3100   -0.0059
    6.3200   -0.0069
    6.3300   -0.0078
    6.3400   -0.0086
    6.3500   -0.0095
    6.3600   -0.0103
    6.3700   -0.0111
    6.3800   -0.0119
    6.3900   -0.0128
    6.4000   -0.0137
    6.4100   -0.0145
    6.4200   -0.0154
    6.4300   -0.0163
    6.4400   -0.0172
    6.4500   -0.0181
    6.4600   -0.0189
    6.4700   -0.0196
    6.4800   -0.0204
    6.4900   -0.0213
    6.5000   -0.0222
    6.5100   -0.0228
    6.5200   -0.0236
    6.5300   -0.0245
    6.5400   -0.0254
    6.5500   -0.0262
    6.5600   -0.0270
    6.5700   -0.0278
    6.5800   -0.0286
    6.5900   -0.0295
    6.6000   -0.0303
    6.6100   -0.0311
    6.6200   -0.0319
    6.6300   -0.0328
    6.6400   -0.0336
    6.6500   -0.0344
    6.6600   -0.0351
    6.6700   -0.0359
    6.6800   -0.0368
    6.6900   -0.0376
    6.7000   -0.0384
    6.7100   -0.0391
    6.7200   -0.0399
    6.7300   -0.0408
    6.7400   -0.0416
    6.7500   -0.0423
    6.7600   -0.0430
    6.7700   -0.0438
    6.7800   -0.0446
    6.7900   -0.0453
    6.8000   -0.0459
    6.8100   -0.0467
    6.8200   -0.0473
    6.8300   -0.0480
    6.8400   -0.0487
    6.8500   -0.0493
    6.8600   -0.0499
    6.8700   -0.0506
    6.8800   -0.0513
    6.8900   -0.0518
    6.9000   -0.0524
    6.9100   -0.0531
    6.9200   -0.0537
    6.9300   -0.0544
    6.9400   -0.0551
    6.9500   -0.0557
    6.9600   -0.0562
    6.9700   -0.0567
    6.9800   -0.0574
    6.9900   -0.0580
    7.0000   -0.0585
    7.0100   -0.0590
    7.0200   -0.0596
    7.0300   -0.0602
    7.0400   -0.0607
    7.0500   -0.0613
    7.0600   -0.0618
    7.0700   -0.0624
    7.0800   -0.0630
    7.0900   -0.0635
    7.1000   -0.0640
    7.1100   -0.0646
    7.1200   -0.0651
    7.1300   -0.0656
    7.1400   -0.0662
    7.1500   -0.0666
    7.1600   -0.0671
    7.1700   -0.0676
    7.1800   -0.0681
    7.1900   -0.0686
    7.2000   -0.0690
    7.2100   -0.0694
    7.2200   -0.0698
    7.2300   -0.0702
    7.2400   -0.0706
    7.2500   -0.0711
    7.2600   -0.0716
    7.2700   -0.0720
    7.2800   -0.0723
    7.2900   -0.0727
    7.3000   -0.0731
    7.3100   -0.0734
    7.3200   -0.0737
    7.3300   -0.0742
    7.3400   -0.0746
    7.3500   -0.0750
    7.3600   -0.0753
    7.3700   -0.0755
    7.3800   -0.0759
    7.3900   -0.0762
    7.4000   -0.0765
    7.4100   -0.0769
    7.4200   -0.0772
    7.4300   -0.0775
    7.4400   -0.0779
    7.4500   -0.0782
    7.4600   -0.0785
    7.4700   -0.0787
    7.4800   -0.0790
    7.4900   -0.0793
    7.5000   -0.0796
    7.5100   -0.0799
    7.5200   -0.0802
    7.5300   -0.0803
    7.5400   -0.0804
    7.5500   -0.0806
    7.5600   -0.0808
    7.5700   -0.0809
    7.5800   -0.0809
    7.5900   -0.0810
    7.6000   -0.0811
    7.6100   -0.0812
    7.6200   -0.0813
    7.6300   -0.0813
    7.6400   -0.0814
    7.6500   -0.0814
    7.6600   -0.0814
    7.6700   -0.0814
    7.6800   -0.0815
    7.6900   -0.0816
    7.7000   -0.0816
    7.7100   -0.0816
    7.7200   -0.0816
    7.7300   -0.0817
    7.7400   -0.0816
    7.7500   -0.0816
    7.7600   -0.0817
    7.7700   -0.0817
    7.7800   -0.0818
    7.7900   -0.0819
    7.8000   -0.0819
    7.8100   -0.0819
    7.8200   -0.0819
    7.8300   -0.0818
    7.8400   -0.0816
    7.8500   -0.0816
    7.8600   -0.0816
    7.8700   -0.0815
    7.8800   -0.0815
    7.8900   -0.0814
    7.9000   -0.0812
    7.9100   -0.0810
    7.9200   -0.0809
    7.9300   -0.0807
    7.9400   -0.0806
    7.9500   -0.0804
    7.9600   -0.0803
    7.9700   -0.0800
    7.9800   -0.0798
    7.9900   -0.0795
    8.0000   -0.0791
    8.0100   -0.0789
    8.0200   -0.0786
    8.0300   -0.0784
    8.0400   -0.0782
    8.0500   -0.0779
    8.0600   -0.0776
    8.0700   -0.0773
    8.0800   -0.0770
    8.0900   -0.0766
    8.1000   -0.0763
    8.1100   -0.0761
    8.1200   -0.0757
    8.1300   -0.0754
    8.1400   -0.0750
    8.1500   -0.0746
    8.1600   -0.0743
    8.1700   -0.0740
    8.1800   -0.0736
    8.1900   -0.0732
    8.2000   -0.0728
    8.2100   -0.0724
    8.2200   -0.0721
    8.2300   -0.0718
    8.2400   -0.0715
    8.2500   -0.0710
    8.2600   -0.0706
    8.2700   -0.0701
    8.2800   -0.0696
    8.2900   -0.0692
    8.3000   -0.0687
    8.3100   -0.0683
    8.3200   -0.0677
    8.3300   -0.0673
    8.3400   -0.0668
    8.3500   -0.0662
    8.3600   -0.0657
    8.3700   -0.0652
    8.3800   -0.0646
    8.3900   -0.0641
    8.4000   -0.0636
    8.4100   -0.0631
    8.4200   -0.0625
    8.4300   -0.0618
    8.4400   -0.0612
    8.4500   -0.0607
    8.4600   -0.0601
    8.4700   -0.0595
    8.4800   -0.0589
    8.4900   -0.0584
    8.5000   -0.0578
    8.5100   -0.0571
    8.5200   -0.0565
    8.5300   -0.0557
    8.5400   -0.0551
    8.5500   -0.0545
    8.5600   -0.0539
    8.5700   -0.0532
    8.5800   -0.0525
    8.5900   -0.0518
    8.6000   -0.0512
    8.6100   -0.0506
    8.6200   -0.0499
    8.6300   -0.0491
    8.6400   -0.0484
    8.6500   -0.0476
    8.6600   -0.0469
    8.6700   -0.0463
    8.6800   -0.0456
    8.6900   -0.0450
    8.7000   -0.0443
    8.7100   -0.0436
    8.7200   -0.0431
    8.7300   -0.0424
    8.7400   -0.0418
    8.7500   -0.0413
    8.7600   -0.0406
    8.7700   -0.0400
    8.7800   -0.0394
    8.7900   -0.0387
    8.8000   -0.0380
    8.8100   -0.0373
    8.8200   -0.0366
    8.8300   -0.0359
    8.8400   -0.0353
    8.8500   -0.0346
    8.8600   -0.0340
    8.8700   -0.0332
    8.8800   -0.0324
    8.8900   -0.0317
    8.9000   -0.0309
    8.9100   -0.0300
    8.9200   -0.0292
    8.9300   -0.0284
    8.9400   -0.0277
    8.9500   -0.0270
    8.9600   -0.0262
    8.9700   -0.0254
    8.9800   -0.0245
    8.9900   -0.0237
    9.0000   -0.0230
    9.0100   -0.0222
    9.0200   -0.0214
    9.0300   -0.0207
    9.0400   -0.0199
    9.0500   -0.0192
    9.0600   -0.0183
    9.0700   -0.0175
    9.0800   -0.0166
    9.0900   -0.0158
    9.1000   -0.0151
    9.1100   -0.0143
    9.1200   -0.0136
    9.1300   -0.0128
    9.1400   -0.0119
    9.1500   -0.0111
    9.1600   -0.0102
    9.1700   -0.0095
    9.1800   -0.0087
    9.1900   -0.0080
    9.2000   -0.0073
    9.2100   -0.0066
    9.2200   -0.0058
    9.2300   -0.0050
    9.2400   -0.0041
    9.2500   -0.0033
    9.2600   -0.0026
    9.2700   -0.0017
    9.2800   -0.0008
    9.2900   -0.0000
    9.3000    0.0008
    9.3100    0.0015
    9.3200    0.0023
    9.3300    0.0031
    9.3400    0.0039
    9.3500    0.0047
    9.3600    0.0054
    9.3700    0.0062
    9.3800    0.0069
    9.3900    0.0077
    9.4000    0.0085
    9.4100    0.0093
    9.4200    0.0101
    9.4300    0.0110
    9.4400    0.0118
    9.4500    0.0124
    9.4600    0.0131
    9.4700    0.0138
    9.4800    0.0145
    9.4900    0.0153
    9.5000    0.0161
    9.5100    0.0168
    9.5200    0.0176
    9.5300    0.0184
    9.5400    0.0192
    9.5500    0.0199
    9.5600    0.0207
    9.5700    0.0214
    9.5800    0.0221
    9.5900    0.0229
    9.6000    0.0237
    9.6100    0.0245
    9.6200    0.0253
    9.6300    0.0262
    9.6400    0.0270
    9.6500    0.0278
    9.6600    0.0285
    9.6700    0.0292
    9.6800    0.0300
    9.6900    0.0307
    9.7000    0.0314
    9.7100    0.0322
    9.7200    0.0330
    9.7300    0.0338
    9.7400    0.0345
    9.7500    0.0352
    9.7600    0.0358
    9.7700    0.0365
    9.7800    0.0372
    9.7900    0.0379
    9.8000    0.0386
    9.8100    0.0392
    9.8200    0.0400
    9.8300    0.0408
    9.8400    0.0415
    9.8500    0.0422
    9.8600    0.0429
    9.8700    0.0435
    9.8800    0.0441
    9.8900    0.0447
    9.9000    0.0455
    9.9100    0.0460
    9.9200    0.0467
    9.9300    0.0474
    9.9400    0.0480
    9.9500    0.0485
    9.9600    0.0491
    9.9700    0.0497
    9.9800    0.0503
    9.9900    0.0510
   10.0000    0.0516
    };

==> Data/Oscillator/sigma01/kf_tr_pos.tex <==
    \addplot[
    thick,
    dashed,
    magenta
    ]
    table {
         0    1.0000
    0.0100    0.9972
    0.0200    0.9928
    0.0300    0.9838
    0.0400    0.9791
    0.0500    0.9755
    0.0600    0.9712
    0.0700    0.9672
    0.0800    0.9636
    0.0900    0.9548
    0.1000    0.9458
    0.1100    0.9473
    0.1200    0.9486
    0.1300    0.9481
    0.1400    0.9450
    0.1500    0.9405
    0.1600    0.9371
    0.1700    0.9336
    0.1800    0.9280
    0.1900    0.9216
    0.2000    0.9167
    0.2100    0.9112
    0.2200    0.9068
    0.2300    0.9088
    0.2400    0.9060
    0.2500    0.8993
    0.2600    0.8928
    0.2700    0.8873
    0.2800    0.8881
    0.2900    0.8820
    0.3000    0.8778
    0.3100    0.8749
    0.3200    0.8678
    0.3300    0.8654
    0.3400    0.8619
    0.3500    0.8598
    0.3600    0.8623
    0.3700    0.8613
    0.3800    0.8529
    0.3900    0.8444
    0.4000    0.8378
    0.4100    0.8302
    0.4200    0.8224
    0.4300    0.8150
    0.4400    0.8130
    0.4500    0.8094
    0.4600    0.8017
    0.4700    0.7973
    0.4800    0.7948
    0.4900    0.7909
    0.5000    0.7866
    0.5100    0.7833
    0.5200    0.7776
    0.5300    0.7715
    0.5400    0.7658
    0.5500    0.7578
    0.5600    0.7512
    0.5700    0.7460
    0.5800    0.7393
    0.5900    0.7329
    0.6000    0.7280
    0.6100    0.7232
    0.6200    0.7171
    0.6300    0.7110
    0.6400    0.7049
    0.6500    0.6971
    0.6600    0.6899
    0.6700    0.6863
    0.6800    0.6799
    0.6900    0.6745
    0.7000    0.6699
    0.7100    0.6619
    0.7200    0.6536
    0.7300    0.6444
    0.7400    0.6352
    0.7500    0.6270
    0.7600    0.6222
    0.7700    0.6174
    0.7800    0.6110
    0.7900    0.6068
    0.8000    0.5977
    0.8100    0.5865
    0.8200    0.5795
    0.8300    0.5733
    0.8400    0.5650
    0.8500    0.5541
    0.8600    0.5464
    0.8700    0.5395
    0.8800    0.5321
    0.8900    0.5242
    0.9000    0.5128
    0.9100    0.5038
    0.9200    0.4982
    0.9300    0.4939
    0.9400    0.4860
    0.9500    0.4743
    0.9600    0.4630
    0.9700    0.4533
    0.9800    0.4443
    0.9900    0.4372
    1.0000    0.4293
    1.0100    0.4167
    1.0200    0.4067
    1.0300    0.4006
    1.0400    0.3930
    1.0500    0.3818
    1.0600    0.3722
    1.0700    0.3618
    1.0800    0.3513
    1.0900    0.3443
    1.1000    0.3376
    1.1100    0.3269
    1.1200    0.3155
    1.1300    0.3062
    1.1400    0.2996
    1.1500    0.2949
    1.1600    0.2869
    1.1700    0.2802
    1.1800    0.2722
    1.1900    0.2615
    1.2000    0.2544
    1.2100    0.2497
    1.2200    0.2437
    1.2300    0.2367
    1.2400    0.2278
    1.2500    0.2196
    1.2600    0.2110
    1.2700    0.2020
    1.2800    0.1945
    1.2900    0.1878
    1.3000    0.1801
    1.3100    0.1714
    1.3200    0.1651
    1.3300    0.1563
    1.3400    0.1463
    1.3500    0.1403
    1.3600    0.1340
    1.3700    0.1248
    1.3800    0.1166
    1.3900    0.1082
    1.4000    0.0999
    1.4100    0.0918
    1.4200    0.0830
    1.4300    0.0749
    1.4400    0.0688
    1.4500    0.0622
    1.4600    0.0566
    1.4700    0.0477
    1.4800    0.0355
    1.4900    0.0274
    1.5000    0.0184
    1.5100    0.0070
    1.5200   -0.0022
    1.5300   -0.0087
    1.5400   -0.0162
    1.5500   -0.0235
    1.5600   -0.0324
    1.5700   -0.0426
    1.5800   -0.0514
    1.5900   -0.0606
    1.6000   -0.0698
    1.6100   -0.0741
    1.6200   -0.0801
    1.6300   -0.0882
    1.6400   -0.0970
    1.6500   -0.1047
    1.6600   -0.1121
    1.6700   -0.1214
    1.6800   -0.1298
    1.6900   -0.1381
    1.7000   -0.1450
    1.7100   -0.1538
    1.7200   -0.1578
    1.7300   -0.1624
    1.7400   -0.1724
    1.7500   -0.1762
    1.7600   -0.1823
    1.7700   -0.1911
    1.7800   -0.1994
    1.7900   -0.2074
    1.8000   -0.2132
    1.8100   -0.2199
    1.8200   -0.2269
    1.8300   -0.2351
    1.8400   -0.2400
    1.8500   -0.2483
    1.8600   -0.2613
    1.8700   -0.2697
    1.8800   -0.2772
    1.8900   -0.2857
    1.9000   -0.2950
    1.9100   -0.3053
    1.9200   -0.3138
    1.9300   -0.3221
    1.9400   -0.3312
    1.9500   -0.3395
    1.9600   -0.3484
    1.9700   -0.3545
    1.9800   -0.3611
    1.9900   -0.3671
    2.0000   -0.3715
    2.0100   -0.3809
    2.0200   -0.3901
    2.0300   -0.3963
    2.0400   -0.4003
    2.0500   -0.4054
    2.0600   -0.4117
    2.0700   -0.4166
    2.0800   -0.4241
    2.0900   -0.4328
    2.1000   -0.4416
    2.1100   -0.4508
    2.1200   -0.4559
    2.1300   -0.4603
    2.1400   -0.4629
    2.1500   -0.4654
    2.1600   -0.4744
    2.1700   -0.4811
    2.1800   -0.4827
    2.1900   -0.4880
    2.2000   -0.4944
    2.2100   -0.4987
    2.2200   -0.5030
    2.2300   -0.5074
    2.2400   -0.5121
    2.2500   -0.5179
    2.2600   -0.5230
    2.2700   -0.5294
    2.2800   -0.5338
    2.2900   -0.5372
    2.3000   -0.5417
    2.3100   -0.5467
    2.3200   -0.5542
    2.3300   -0.5602
    2.3400   -0.5655
    2.3500   -0.5693
    2.3600   -0.5719
    2.3700   -0.5752
    2.3800   -0.5808
    2.3900   -0.5884
    2.4000   -0.5933
    2.4100   -0.5980
    2.4200   -0.6015
    2.4300   -0.6024
    2.4400   -0.6061
    2.4500   -0.6103
    2.4600   -0.6116
    2.4700   -0.6140
    2.4800   -0.6161
    2.4900   -0.6169
    2.5000   -0.6197
    2.5100   -0.6224
    2.5200   -0.6248
    2.5300   -0.6289
    2.5400   -0.6327
    2.5500   -0.6355
    2.5600   -0.6398
    2.5700   -0.6414
    2.5800   -0.6429
    2.5900   -0.6431
    2.6000   -0.6435
    2.6100   -0.6470
    2.6200   -0.6479
    2.6300   -0.6463
    2.6400   -0.6459
    2.6500   -0.6500
    2.6600   -0.6526
    2.6700   -0.6558
    2.6800   -0.6605
    2.6900   -0.6631
    2.7000   -0.6640
    2.7100   -0.6632
    2.7200   -0.6645
    2.7300   -0.6660
    2.7400   -0.6676
    2.7500   -0.6700
    2.7600   -0.6692
    2.7700   -0.6692
    2.7800   -0.6716
    2.7900   -0.6745
    2.8000   -0.6763
    2.8100   -0.6762
    2.8200   -0.6743
    2.8300   -0.6739
    2.8400   -0.6754
    2.8500   -0.6777
    2.8600   -0.6783
    2.8700   -0.6778
    2.8800   -0.6804
    2.8900   -0.6799
    2.9000   -0.6780
    2.9100   -0.6777
    2.9200   -0.6792
    2.9300   -0.6812
    2.9400   -0.6808
    2.9500   -0.6824
    2.9600   -0.6847
    2.9700   -0.6861
    2.9800   -0.6865
    2.9900   -0.6877
    3.0000   -0.6885
    3.0100   -0.6857
    3.0200   -0.6847
    3.0300   -0.6857
    3.0400   -0.6855
    3.0500   -0.6840
    3.0600   -0.6825
    3.0700   -0.6817
    3.0800   -0.6819
    3.0900   -0.6827
    3.1000   -0.6823
    3.1100   -0.6798
    3.1200   -0.6771
    3.1300   -0.6778
    3.1400   -0.6783
    3.1500   -0.6772
    3.1600   -0.6772
    3.1700   -0.6770
    3.1800   -0.6774
    3.1900   -0.6779
    3.2000   -0.6781
    3.2100   -0.6784
    3.2200   -0.6777
    3.2300   -0.6763
    3.2400   -0.6753
    3.2500   -0.6745
    3.2600   -0.6734
    3.2700   -0.6718
    3.2800   -0.6687
    3.2900   -0.6653
    3.3000   -0.6638
    3.3100   -0.6620
    3.3200   -0.6598
    3.3300   -0.6600
    3.3400   -0.6623
    3.3500   -0.6645
    3.3600   -0.6643
    3.3700   -0.6630
    3.3800   -0.6624
    3.3900   -0.6608
    3.4000   -0.6591
    3.4100   -0.6583
    3.4200   -0.6560
    3.4300   -0.6524
    3.4400   -0.6468
    3.4500   -0.6415
    3.4600   -0.6389
    3.4700   -0.6368
    3.4800   -0.6350
    3.4900   -0.6322
    3.5000   -0.6312
    3.5100   -0.6306
    3.5200   -0.6268
    3.5300   -0.6237
    3.5400   -0.6210
    3.5500   -0.6163
    3.5600   -0.6113
    3.5700   -0.6060
    3.5800   -0.6043
    3.5900   -0.6042
    3.6000   -0.6001
    3.6100   -0.5954
    3.6200   -0.5916
    3.6300   -0.5878
    3.6400   -0.5826
    3.6500   -0.5776
    3.6600   -0.5746
    3.6700   -0.5718
    3.6800   -0.5684
    3.6900   -0.5639
    3.7000   -0.5586
    3.7100   -0.5538
    3.7200   -0.5491
    3.7300   -0.5453
    3.7400   -0.5416
    3.7500   -0.5369
    3.7600   -0.5339
    3.7700   -0.5311
    3.7800   -0.5253
    3.7900   -0.5204
    3.8000   -0.5147
    3.8100   -0.5079
    3.8200   -0.5035
    3.8300   -0.4995
    3.8400   -0.4953
    3.8500   -0.4908
    3.8600   -0.4850
    3.8700   -0.4799
    3.8800   -0.4753
    3.8900   -0.4682
    3.9000   -0.4608
    3.9100   -0.4542
    3.9200   -0.4493
    3.9300   -0.4459
    3.9400   -0.4411
    3.9500   -0.4357
    3.9600   -0.4322
    3.9700   -0.4305
    3.9800   -0.4254
    3.9900   -0.4202
    4.0000   -0.4134
    4.0100   -0.4082
    4.0200   -0.4051
    4.0300   -0.3987
    4.0400   -0.3944
    4.0500   -0.3892
    4.0600   -0.3841
    4.0700   -0.3787
    4.0800   -0.3719
    4.0900   -0.3678
    4.1000   -0.3663
    4.1100   -0.3635
    4.1200   -0.3566
    4.1300   -0.3495
    4.1400   -0.3439
    4.1500   -0.3370
    4.1600   -0.3323
    4.1700   -0.3264
    4.1800   -0.3197
    4.1900   -0.3150
    4.2000   -0.3093
    4.2100   -0.3033
    4.2200   -0.2994
    4.2300   -0.2939
    4.2400   -0.2857
    4.2500   -0.2775
    4.2600   -0.2679
    4.2700   -0.2606
    4.2800   -0.2554
    4.2900   -0.2521
    4.3000   -0.2477
    4.3100   -0.2412
    4.3200   -0.2337
    4.3300   -0.2275
    4.3400   -0.2217
    4.3500   -0.2142
    4.3600   -0.2091
    4.3700   -0.2029
    4.3800   -0.1953
    4.3900   -0.1894
    4.4000   -0.1815
    4.4100   -0.1726
    4.4200   -0.1661
    4.4300   -0.1597
    4.4400   -0.1530
    4.4500   -0.1466
    4.4600   -0.1395
    4.4700   -0.1333
    4.4800   -0.1285
    4.4900   -0.1228
    4.5000   -0.1140
    4.5100   -0.1059
    4.5200   -0.1012
    4.5300   -0.0960
    4.5400   -0.0902
    4.5500   -0.0847
    4.5600   -0.0781
    4.5700   -0.0713
    4.5800   -0.0657
    4.5900   -0.0602
    4.6000   -0.0555
    4.6100   -0.0512
    4.6200   -0.0469
    4.6300   -0.0423
    4.6400   -0.0373
    4.6500   -0.0327
    4.6600   -0.0270
    4.6700   -0.0221
    4.6800   -0.0170
    4.6900   -0.0099
    4.7000   -0.0044
    4.7100    0.0024
    4.7200    0.0084
    4.7300    0.0128
    4.7400    0.0175
    4.7500    0.0221
    4.7600    0.0271
    4.7700    0.0316
    4.7800    0.0369
    4.7900    0.0416
    4.8000    0.0447
    4.8100    0.0494
    4.8200    0.0584
    4.8300    0.0691
    4.8400    0.0770
    4.8500    0.0825
    4.8600    0.0884
    4.8700    0.0943
    4.8800    0.1001
    4.8900    0.1033
    4.9000    0.1077
    4.9100    0.1133
    4.9200    0.1158
    4.9300    0.1228
    4.9400    0.1315
    4.9500    0.1371
    4.9600    0.1454
    4.9700    0.1509
    4.9800    0.1554
    4.9900    0.1628
    5.0000    0.1692
    5.0100    0.1756
    5.0200    0.1811
    5.0300    0.1874
    5.0400    0.1935
    5.0500    0.1975
    5.0600    0.2033
    5.0700    0.2118
    5.0800    0.2190
    5.0900    0.2236
    5.1000    0.2293
    5.1100    0.2366
    5.1200    0.2443
    5.1300    0.2513
    5.1400    0.2563
    5.1500    0.2621
    5.1600    0.2681
    5.1700    0.2751
    5.1800    0.2807
    5.1900    0.2844
    5.2000    0.2917
    5.2100    0.2979
    5.2200    0.3021
    5.2300    0.3060
    5.2400    0.3102
    5.2500    0.3151
    5.2600    0.3205
    5.2700    0.3249
    5.2800    0.3293
    5.2900    0.3341
    5.3000    0.3383
    5.3100    0.3423
    5.3200    0.3458
    5.3300    0.3539
    5.3400    0.3660
    5.3500    0.3749
    5.3600    0.3816
    5.3700    0.3858
    5.3800    0.3886
    5.3900    0.3923
    5.4000    0.3968
    5.4100    0.4025
    5.4200    0.4076
    5.4300    0.4120
    5.4400    0.4152
    5.4500    0.4186
    5.4600    0.4242
    5.4700    0.4301
    5.4800    0.4348
    5.4900    0.4397
    5.5000    0.4454
    5.5100    0.4484
    5.5200    0.4507
    5.5300    0.4549
    5.5400    0.4564
    5.5500    0.4571
    5.5600    0.4594
    5.5700    0.4640
    5.5800    0.4684
    5.5900    0.4721
    5.6000    0.4755
    5.6100    0.4759
    5.6200    0.4777
    5.6300    0.4806
    5.6400    0.4840
    5.6500    0.4907
    5.6600    0.4952
    5.6700    0.4990
    5.6800    0.5048
    5.6900    0.5074
    5.7000    0.5089
    5.7100    0.5125
    5.7200    0.5162
    5.7300    0.5204
    5.7400    0.5245
    5.7500    0.5288
    5.7600    0.5318
    5.7700    0.5349
    5.7800    0.5360
    5.7900    0.5348
    5.8000    0.5380
    5.8100    0.5412
    5.8200    0.5429
    5.8300    0.5475
    5.8400    0.5506
    5.8500    0.5509
    5.8600    0.5518
    5.8700    0.5541
    5.8800    0.5567
    5.8900    0.5577
    5.9000    0.5572
    5.9100    0.5574
    5.9200    0.5590
    5.9300    0.5601
    5.9400    0.5614
    5.9500    0.5617
    5.9600    0.5632
    5.9700    0.5634
    5.9800    0.5627
    5.9900    0.5656
    6.0000    0.5669
    6.0100    0.5672
    6.0200    0.5691
    6.0300    0.5701
    6.0400    0.5706
    6.0500    0.5725
    6.0600    0.5731
    6.0700    0.5739
    6.0800    0.5770
    6.0900    0.5793
    6.1000    0.5806
    6.1100    0.5802
    6.1200    0.5805
    6.1300    0.5805
    6.1400    0.5814
    6.1500    0.5844
    6.1600    0.5855
    6.1700    0.5862
    6.1800    0.5841
    6.1900    0.5812
    6.2000    0.5807
    6.2100    0.5839
    6.2200    0.5872
    6.2300    0.5882
    6.2400    0.5881
    6.2500    0.5875
    6.2600    0.5888
    6.2700    0.5891
    6.2800    0.5907
    6.2900    0.5914
    6.3000    0.5891
    6.3100    0.5890
    6.3200    0.5866
    6.3300    0.5848
    6.3400    0.5853
    6.3500    0.5847
    6.3600    0.5850
    6.3700    0.5861
    6.3800    0.5872
    6.3900    0.5867
    6.4000    0.5852
    6.4100    0.5849
    6.4200    0.5831
    6.4300    0.5798
    6.4400    0.5775
    6.4500    0.5759
    6.4600    0.5766
    6.4700    0.5781
    6.4800    0.5770
    6.4900    0.5744
    6.5000    0.5736
    6.5100    0.5766
    6.5200    0.5778
    6.5300    0.5758
    6.5400    0.5721
    6.5500    0.5700
    6.5600    0.5696
    6.5700    0.5692
    6.5800    0.5675
    6.5900    0.5649
    6.6000    0.5624
    6.6100    0.5610
    6.6200    0.5598
    6.6300    0.5568
    6.6400    0.5542
    6.6500    0.5525
    6.6600    0.5518
    6.6700    0.5487
    6.6800    0.5447
    6.6900    0.5406
    6.7000    0.5375
    6.7100    0.5361
    6.7200    0.5323
    6.7300    0.5260
    6.7400    0.5214
    6.7500    0.5195
    6.7600    0.5176
    6.7700    0.5135
    6.7800    0.5073
    6.7900    0.5038
    6.8000    0.5019
    6.8100    0.4979
    6.8200    0.4959
    6.8300    0.4934
    6.8400    0.4892
    6.8500    0.4866
    6.8600    0.4846
    6.8700    0.4813
    6.8800    0.4768
    6.8900    0.4769
    6.9000    0.4746
    6.9100    0.4695
    6.9200    0.4666
    6.9300    0.4618
    6.9400    0.4566
    6.9500    0.4522
    6.9600    0.4516
    6.9700    0.4492
    6.9800    0.4449
    6.9900    0.4409
    7.0000    0.4382
    7.0100    0.4370
    7.0200    0.4330
    7.0300    0.4295
    7.0400    0.4258
    7.0500    0.4227
    7.0600    0.4196
    7.0700    0.4139
    7.0800    0.4085
    7.0900    0.4064
    7.1000    0.4025
    7.1100    0.3961
    7.1200    0.3930
    7.1300    0.3875
    7.1400    0.3814
    7.1500    0.3786
    7.1600    0.3750
    7.1700    0.3697
    7.1800    0.3643
    7.1900    0.3597
    7.2000    0.3559
    7.2100    0.3529
    7.2200    0.3481
    7.2300    0.3445
    7.2400    0.3415
    7.2500    0.3355
    7.2600    0.3293
    7.2700    0.3249
    7.2800    0.3209
    7.2900    0.3170
    7.3000    0.3125
    7.3100    0.3101
    7.3200    0.3060
    7.3300    0.2983
    7.3400    0.2931
    7.3500    0.2876
    7.3600    0.2840
    7.3700    0.2805
    7.3800    0.2751
    7.3900    0.2697
    7.4000    0.2653
    7.4100    0.2599
    7.4200    0.2544
    7.4300    0.2480
    7.4400    0.2409
    7.4500    0.2348
    7.4600    0.2275
    7.4700    0.2220
    7.4800    0.2158
    7.4900    0.2082
    7.5000    0.2006
    7.5100    0.1914
    7.5200    0.1835
    7.5300    0.1793
    7.5400    0.1747
    7.5500    0.1688
    7.5600    0.1617
    7.5700    0.1567
    7.5800    0.1525
    7.5900    0.1476
    7.6000    0.1439
    7.6100    0.1379
    7.6200    0.1330
    7.6300    0.1295
    7.6400    0.1244
    7.6500    0.1195
    7.6600    0.1170
    7.6700    0.1129
    7.6800    0.1065
    7.6900    0.1010
    7.7000    0.0959
    7.7100    0.0913
    7.7200    0.0859
    7.7300    0.0803
    7.7400    0.0764
    7.7500    0.0717
    7.7600    0.0662
    7.7700    0.0594
    7.7800    0.0512
    7.7900    0.0431
    7.8000    0.0345
    7.8100    0.0278
    7.8200    0.0200
    7.8300    0.0147
    7.8400    0.0125
    7.8500    0.0051
    7.8600   -0.0041
    7.8700   -0.0106
    7.8800   -0.0180
    7.8900   -0.0262
    7.9000   -0.0310
    7.9100   -0.0358
    7.9200   -0.0418
    7.9300   -0.0485
    7.9400   -0.0556
    7.9500   -0.0631
    7.9600   -0.0697
    7.9700   -0.0753
    7.9800   -0.0809
    7.9900   -0.0845
    8.0000   -0.0879
    8.0100   -0.0925
    8.0200   -0.0987
    8.0300   -0.1060
    8.0400   -0.1128
    8.0500   -0.1170
    8.0600   -0.1219
    8.0700   -0.1282
    8.0800   -0.1333
    8.0900   -0.1371
    8.1000   -0.1432
    8.1100   -0.1501
    8.1200   -0.1548
    8.1300   -0.1604
    8.1400   -0.1650
    8.1500   -0.1697
    8.1600   -0.1765
    8.1700   -0.1824
    8.1800   -0.1867
    8.1900   -0.1920
    8.2000   -0.1965
    8.2100   -0.2024
    8.2200   -0.2099
    8.2300   -0.2192
    8.2400   -0.2268
    8.2500   -0.2318
    8.2600   -0.2386
    8.2700   -0.2426
    8.2800   -0.2465
    8.2900   -0.2520
    8.3000   -0.2581
    8.3100   -0.2643
    8.3200   -0.2685
    8.3300   -0.2742
    8.3400   -0.2810
    8.3500   -0.2845
    8.3600   -0.2901
    8.3700   -0.2958
    8.3800   -0.2988
    8.3900   -0.3036
    8.4000   -0.3108
    8.4100   -0.3165
    8.4200   -0.3196
    8.4300   -0.3230
    8.4400   -0.3259
    8.4500   -0.3310
    8.4600   -0.3361
    8.4700   -0.3402
    8.4800   -0.3456
    8.4900   -0.3521
    8.5000   -0.3568
    8.5100   -0.3596
    8.5200   -0.3630
    8.5300   -0.3644
    8.5400   -0.3684
    8.5500   -0.3731
    8.5600   -0.3764
    8.5700   -0.3798
    8.5800   -0.3818
    8.5900   -0.3837
    8.6000   -0.3878
    8.6100   -0.3926
    8.6200   -0.3966
    8.6300   -0.3970
    8.6400   -0.3966
    8.6500   -0.3972
    8.6600   -0.3981
    8.6700   -0.4016
    8.6800   -0.4043
    8.6900   -0.4080
    8.7000   -0.4109
    8.7100   -0.4130
    8.7200   -0.4184
    8.7300   -0.4221
    8.7400   -0.4257
    8.7500   -0.4329
    8.7600   -0.4374
    8.7700   -0.4409
    8.7800   -0.4461
    8.7900   -0.4501
    8.8000   -0.4537
    8.8100   -0.4576
    8.8200   -0.4603
    8.8300   -0.4640
    8.8400   -0.4691
    8.8500   -0.4751
    8.8600   -0.4805
    8.8700   -0.4825
    8.8800   -0.4853
    8.8900   -0.4882
    8.9000   -0.4897
    8.9100   -0.4909
    8.9200   -0.4914
    8.9300   -0.4935
    8.9400   -0.4977
    8.9500   -0.5005
    8.9600   -0.5035
    8.9700   -0.5052
    8.9800   -0.5044
    8.9900   -0.5052
    9.0000   -0.5079
    9.0100   -0.5097
    9.0200   -0.5118
    9.0300   -0.5146
    9.0400   -0.5170
    9.0500   -0.5195
    9.0600   -0.5200
    9.0700   -0.5200
    9.0800   -0.5198
    9.0900   -0.5214
    9.1000   -0.5237
    9.1100   -0.5260
    9.1200   -0.5282
    9.1300   -0.5289
    9.1400   -0.5288
    9.1500   -0.5279
    9.1600   -0.5275
    9.1700   -0.5287
    9.1800   -0.5307
    9.1900   -0.5344
    9.2000   -0.5377
    9.2100   -0.5406
    9.2200   -0.5424
    9.2300   -0.5412
    9.2400   -0.5411
    9.2500   -0.5423
    9.2600   -0.5434
    9.2700   -0.5425
    9.2800   -0.5401
    9.2900   -0.5401
    9.3000   -0.5409
    9.3100   -0.5424
    9.3200   -0.5437
    9.3300   -0.5429
    9.3400   -0.5414
    9.3500   -0.5426
    9.3600   -0.5439
    9.3700   -0.5441
    9.3800   -0.5458
    9.3900   -0.5453
    9.4000   -0.5442
    9.4100   -0.5442
    9.4200   -0.5439
    9.4300   -0.5414
    9.4400   -0.5401
    9.4500   -0.5420
    9.4600   -0.5441
    9.4700   -0.5456
    9.4800   -0.5469
    9.4900   -0.5461
    9.5000   -0.5471
    9.5100   -0.5484
    9.5200   -0.5482
    9.5300   -0.5471
    9.5400   -0.5460
    9.5500   -0.5462
    9.5600   -0.5460
    9.5700   -0.5468
    9.5800   -0.5466
    9.5900   -0.5459
    9.6000   -0.5457
    9.6100   -0.5440
    9.6200   -0.5413
    9.6300   -0.5376
    9.6400   -0.5350
    9.6500   -0.5328
    9.6600   -0.5324
    9.6700   -0.5328
    9.6800   -0.5298
    9.6900   -0.5285
    9.7000   -0.5267
    9.7100   -0.5235
    9.7200   -0.5200
    9.7300   -0.5170
    9.7400   -0.5143
    9.7500   -0.5124
    9.7600   -0.5124
    9.7700   -0.5117
    9.7800   -0.5098
    9.7900   -0.5065
    9.8000   -0.5041
    9.8100   -0.5039
    9.8200   -0.4988
    9.8300   -0.4944
    9.8400   -0.4914
    9.8500   -0.4858
    9.8600   -0.4834
    9.8700   -0.4817
    9.8800   -0.4794
    9.8900   -0.4770
    9.9000   -0.4722
    9.9100   -0.4702
    9.9200   -0.4675
    9.9300   -0.4615
    9.9400   -0.4590
    9.9500   -0.4569
    9.9600   -0.4539
    9.9700   -0.4505
    9.9800   -0.4463
    9.9900   -0.4410
   10.0000   -0.4372
    };

==> Data/Oscillator/sigma01/kf_tr_vel.tex <==
    \addplot[
    thick,
    dashed,
    magenta
    ]
    table {
         0         0
    0.0100   -0.0100
    0.0200   -0.0199
    0.0300   -0.0298
    0.0400   -0.0396
    0.0500   -0.0493
    0.0600   -0.0590
    0.0700   -0.0686
    0.0800   -0.0782
    0.0900   -0.0878
    0.1000   -0.0973
    0.1100   -0.1066
    0.1200   -0.1160
    0.1300   -0.1253
    0.1400   -0.1347
    0.1500   -0.1441
    0.1600   -0.1534
    0.1700   -0.1626
    0.1800   -0.1719
    0.1900   -0.1811
    0.2000   -0.1903
    0.2100   -0.1994
    0.2200   -0.2084
    0.2300   -0.2170
    0.2400   -0.2259
    0.2500   -0.2350
    0.2600   -0.2441
    0.2700   -0.2529
    0.2800   -0.2613
    0.2900   -0.2702
    0.3000   -0.2788
    0.3100   -0.2873
    0.3200   -0.2962
    0.3300   -0.3045
    0.3400   -0.3129
    0.3500   -0.3210
    0.3600   -0.3285
    0.3700   -0.3365
    0.3800   -0.3455
    0.3900   -0.3544
    0.4000   -0.3630
    0.4100   -0.3717
    0.4200   -0.3803
    0.4300   -0.3888
    0.4400   -0.3962
    0.4500   -0.4038
    0.4600   -0.4122
    0.4700   -0.4199
    0.4800   -0.4270
    0.4900   -0.4344
    0.5000   -0.4418
    0.5100   -0.4489
    0.5200   -0.4566
    0.5300   -0.4643
    0.5400   -0.4718
    0.5500   -0.4799
    0.5600   -0.4875
    0.5700   -0.4946
    0.5800   -0.5021
    0.5900   -0.5094
    0.6000   -0.5161
    0.6100   -0.5227
    0.6200   -0.5296
    0.6300   -0.5365
    0.6400   -0.5434
    0.6500   -0.5507
    0.6600   -0.5577
    0.6700   -0.5632
    0.6800   -0.5698
    0.6900   -0.5759
    0.7000   -0.5815
    0.7100   -0.5885
    0.7200   -0.5955
    0.7300   -0.6028
    0.7400   -0.6100
    0.7500   -0.6166
    0.7600   -0.6216
    0.7700   -0.6265
    0.7800   -0.6320
    0.7900   -0.6365
    0.8000   -0.6432
    0.8100   -0.6507
    0.8200   -0.6561
    0.8300   -0.6611
    0.8400   -0.6669
    0.8500   -0.6739
    0.8600   -0.6792
    0.8700   -0.6840
    0.8800   -0.6890
    0.8900   -0.6941
    0.9000   -0.7009
    0.9100   -0.7063
    0.9200   -0.7098
    0.9300   -0.7126
    0.9400   -0.7172
    0.9500   -0.7237
    0.9600   -0.7299
    0.9700   -0.7350
    0.9800   -0.7397
    0.9900   -0.7432
    1.0000   -0.7470
    1.0100   -0.7533
    1.0200   -0.7581
    1.0300   -0.7605
    1.0400   -0.7637
    1.0500   -0.7688
    1.0600   -0.7729
    1.0700   -0.7773
    1.0800   -0.7816
    1.0900   -0.7839
    1.1000   -0.7858
    1.1100   -0.7899
    1.1200   -0.7944
    1.1300   -0.7975
    1.1400   -0.7989
    1.1500   -0.7992
    1.1600   -0.8013
    1.1700   -0.8026
    1.1800   -0.8045
    1.1900   -0.8079
    1.2000   -0.8091
    1.2100   -0.8089
    1.2200   -0.8093
    1.2300   -0.8102
    1.2400   -0.8122
    1.2500   -0.8137
    1.2600   -0.8153
    1.2700   -0.8170
    1.2800   -0.8178
    1.2900   -0.8181
    1.3000   -0.8188
    1.3100   -0.8200
    1.3200   -0.8198
    1.3300   -0.8209
    1.3400   -0.8226
    1.3500   -0.8220
    1.3600   -0.8214
    1.3700   -0.8225
    1.3800   -0.8229
    1.3900   -0.8232
    1.4000   -0.8235
    1.4100   -0.8235
    1.4200   -0.8239
    1.4300   -0.8238
    1.4400   -0.8225
    1.4500   -0.8215
    1.4600   -0.8198
    1.4700   -0.8199
    1.4800   -0.8216
    1.4900   -0.8211
    1.5000   -0.8209
    1.5100   -0.8219
    1.5200   -0.8216
    1.5300   -0.8199
    1.5400   -0.8186
    1.5500   -0.8171
    1.5600   -0.8164
    1.5700   -0.8163
    1.5800   -0.8153
    1.5900   -0.8145
    1.6000   -0.8135
    1.6100   -0.8101
    1.6200   -0.8074
    1.6300   -0.8058
    1.6400   -0.8044
    1.6500   -0.8024
    1.6600   -0.8003
    1.6700   -0.7989
    1.6800   -0.7971
    1.6900   -0.7951
    1.7000   -0.7924
    1.7100   -0.7906
    1.7200   -0.7863
    1.7300   -0.7824
    1.7400   -0.7810
    1.7500   -0.7765
    1.7600   -0.7732
    1.7700   -0.7711
    1.7800   -0.7686
    1.7900   -0.7660
    1.8000   -0.7623
    1.8100   -0.7589
    1.8200   -0.7557
    1.8300   -0.7529
    1.8400   -0.7486
    1.8500   -0.7458
    1.8600   -0.7450
    1.8700   -0.7420
    1.8800   -0.7386
    1.8900   -0.7355
    1.9000   -0.7328
    1.9100   -0.7304
    1.9200   -0.7271
    1.9300   -0.7236
    1.9400   -0.7205
    1.9500   -0.7169
    1.9600   -0.7135
    1.9700   -0.7088
    1.9800   -0.7043
    1.9900   -0.6996
    2.0000   -0.6941
    2.0100   -0.6906
    2.0200   -0.6871
    2.0300   -0.6822
    2.0400   -0.6764
    2.0500   -0.6710
    2.0600   -0.6661
    2.0700   -0.6606
    2.0800   -0.6561
    2.0900   -0.6520
    2.1000   -0.6479
    2.1100   -0.6439
    2.1200   -0.6383
    2.1300   -0.6322
    2.1400   -0.6255
    2.1500   -0.6187
    2.1600   -0.6146
    2.1700   -0.6094
    2.1800   -0.6022
    2.1900   -0.5965
    2.2000   -0.5912
    2.2100   -0.5850
    2.2200   -0.5788
    2.2300   -0.5726
    2.2400   -0.5666
    2.2500   -0.5609
    2.2600   -0.5550
    2.2700   -0.5495
    2.2800   -0.5432
    2.2900   -0.5366
    2.3000   -0.5303
    2.3100   -0.5243
    2.3200   -0.5191
    2.3300   -0.5133
    2.3400   -0.5073
    2.3500   -0.5006
    2.3600   -0.4935
    2.3700   -0.4867
    2.3800   -0.4807
    2.3900   -0.4754
    2.4000   -0.4691
    2.4100   -0.4627
    2.4200   -0.4559
    2.4300   -0.4481
    2.4400   -0.4413
    2.4500   -0.4347
    2.4600   -0.4270
    2.4700   -0.4198
    2.4800   -0.4125
    2.4900   -0.4047
    2.5000   -0.3977
    2.5100   -0.3906
    2.5200   -0.3834
    2.5300   -0.3769
    2.5400   -0.3702
    2.5500   -0.3632
    2.5600   -0.3567
    2.5700   -0.3493
    2.5800   -0.3418
    2.5900   -0.3339
    2.6000   -0.3261
    2.6100   -0.3194
    2.6200   -0.3118
    2.6300   -0.3033
    2.6400   -0.2953
    2.6500   -0.2889
    2.6600   -0.2820
    2.6700   -0.2754
    2.6800   -0.2692
    2.6900   -0.2623
    2.7000   -0.2548
    2.7100   -0.2467
    2.7200   -0.2394
    2.7300   -0.2322
    2.7400   -0.2251
    2.7500   -0.2182
    2.7600   -0.2103
    2.7700   -0.2026
    2.7800   -0.1959
    2.7900   -0.1893
    2.8000   -0.1823
    2.8100   -0.1747
    2.8200   -0.1664
    2.8300   -0.1588
    2.8400   -0.1519
    2.8500   -0.1453
    2.8600   -0.1380
    2.8700   -0.1304
    2.8800   -0.1240
    2.8900   -0.1165
    2.9000   -0.1084
    2.9100   -0.1011
    2.9200   -0.0944
    2.9300   -0.0879
    2.9400   -0.0805
    2.9500   -0.0740
    2.9600   -0.0676
    2.9700   -0.0610
    2.9800   -0.0540
    2.9900   -0.0474
    3.0000   -0.0406
    3.0100   -0.0325
    3.0200   -0.0251
    3.0300   -0.0185
    3.0400   -0.0115
    3.0500   -0.0041
    3.0600    0.0033
    3.0700    0.0104
    3.0800    0.0171
    3.0900    0.0235
    3.1000    0.0303
    3.1100    0.0379
    3.1200    0.0456
    3.1300    0.0518
    3.1400    0.0582
    3.1500    0.0651
    3.1600    0.0715
    3.1700    0.0780
    3.1800    0.0842
    3.1900    0.0904
    3.2000    0.0966
    3.2100    0.1028
    3.2200    0.1094
    3.2300    0.1161
    3.2400    0.1227
    3.2500    0.1291
    3.2600    0.1356
    3.2700    0.1423
    3.2800    0.1495
    3.2900    0.1567
    3.3000    0.1632
    3.3100    0.1697
    3.3200    0.1764
    3.3300    0.1819
    3.3400    0.1867
    3.3500    0.1916
    3.3600    0.1973
    3.3700    0.2035
    3.3800    0.2094
    3.3900    0.2155
    3.4000    0.2217
    3.4100    0.2275
    3.4200    0.2339
    3.4300    0.2406
    3.4400    0.2482
    3.4500    0.2555
    3.4600    0.2616
    3.4700    0.2675
    3.4800    0.2732
    3.4900    0.2793
    3.5000    0.2846
    3.5100    0.2897
    3.5200    0.2961
    3.5300    0.3021
    3.5400    0.3078
    3.5500    0.3143
    3.5600    0.3209
    3.5700    0.3275
    3.5800    0.3326
    3.5900    0.3370
    3.6000    0.3429
    3.6100    0.3491
    3.6200    0.3548
    3.6300    0.3604
    3.6400    0.3665
    3.6500    0.3725
    3.6600    0.3776
    3.6700    0.3825
    3.6800    0.3877
    3.6900    0.3932
    3.7000    0.3989
    3.7100    0.4044
    3.7200    0.4098
    3.7300    0.4147
    3.7400    0.4196
    3.7500    0.4247
    3.7600    0.4291
    3.7700    0.4334
    3.7800    0.4388
    3.7900    0.4438
    3.8000    0.4491
    3.8100    0.4547
    3.8200    0.4592
    3.8300    0.4635
    3.8400    0.4678
    3.8500    0.4722
    3.8600    0.4770
    3.8700    0.4815
    3.8800    0.4857
    3.8900    0.4908
    3.9000    0.4960
    3.9100    0.5008
    3.9200    0.5047
    3.9300    0.5080
    3.9400    0.5118
    3.9500    0.5158
    3.9600    0.5189
    3.9700    0.5212
    3.9800    0.5249
    3.9900    0.5286
    4.0000    0.5329
    4.0100    0.5364
    4.0200    0.5390
    4.0300    0.5429
    4.0400    0.5458
    4.0500    0.5491
    4.0600    0.5522
    4.0700    0.5554
    4.0800    0.5591
    4.0900    0.5616
    4.1000    0.5630
    4.1100    0.5649
    4.1200    0.5685
    4.1300    0.5720
    4.1400    0.5749
    4.1500    0.5781
    4.1600    0.5805
    4.1700    0.5832
    4.1800    0.5862
    4.1900    0.5883
    4.2000    0.5907
    4.2100    0.5932
    4.2200    0.5948
    4.2300    0.5970
    4.2400    0.6002
    4.2500    0.6033
    4.2600    0.6069
    4.2700    0.6095
    4.2800    0.6111
    4.2900    0.6118
    4.3000    0.6130
    4.3100    0.6150
    4.3200    0.6173
    4.3300    0.6190
    4.3400    0.6205
    4.3500    0.6225
    4.3600    0.6236
    4.3700    0.6250
    4.3800    0.6269
    4.3900    0.6280
    4.4000    0.6299
    4.4100    0.6322
    4.4200    0.6333
    4.4300    0.6343
    4.4400    0.6354
    4.4500    0.6363
    4.4600    0.6374
    4.4700    0.6380
    4.4800    0.6381
    4.4900    0.6384
    4.5000    0.6399
    4.5100    0.6411
    4.5200    0.6408
    4.5300    0.6406
    4.5400    0.6407
    4.5500    0.6405
    4.5600    0.6407
    4.5700    0.6410
    4.5800    0.6407
    4.5900    0.6403
    4.6000    0.6396
    4.6100    0.6386
    4.6200    0.6376
    4.6300    0.6367
    4.6400    0.6359
    4.6500    0.6349
    4.6600    0.6343
    4.6700    0.6333
    4.6800    0.6323
    4.6900    0.6322
    4.7000    0.6313
    4.7100    0.6309
    4.7200    0.6301
    4.7300    0.6285
    4.7400    0.6271
    4.7500    0.6256
    4.7600    0.6242
    4.7700    0.6226
    4.7800    0.6213
    4.7900    0.6196
    4.8000    0.6173
    4.8100    0.6156
    4.8200    0.6156
    4.8300    0.6163
    4.8400    0.6156
    4.8500    0.6139
    4.8600    0.6124
    4.8700    0.6108
    4.8800    0.6090
    4.8900    0.6063
    4.9000    0.6039
    4.9100    0.6020
    4.9200    0.5989
    4.9300    0.5975
    4.9400    0.5967
    4.9500    0.5947
    4.9600    0.5936
    4.9700    0.5913
    4.9800    0.5887
    4.9900    0.5871
    5.0000    0.5851
    5.0100    0.5830
    5.0200    0.5805
    5.0300    0.5783
    5.0400    0.5759
    5.0500    0.5727
    5.0600    0.5701
    5.0700    0.5687
    5.0800    0.5665
    5.0900    0.5634
    5.1000    0.5606
    5.1100    0.5583
    5.1200    0.5563
    5.1300    0.5538
    5.1400    0.5505
    5.1500    0.5475
    5.1600    0.5445
    5.1700    0.5419
    5.1800    0.5386
    5.1900    0.5346
    5.2000    0.5320
    5.2100    0.5289
    5.2200    0.5249
    5.2300    0.5208
    5.2400    0.5168
    5.2500    0.5131
    5.2600    0.5095
    5.2700    0.5055
    5.2800    0.5015
    5.2900    0.4976
    5.3000    0.4934
    5.3100    0.4892
    5.3200    0.4847
    5.3300    0.4820
    5.3400    0.4809
    5.3500    0.4784
    5.3600    0.4749
    5.3700    0.4704
    5.3800    0.4653
    5.3900    0.4605
    5.4000    0.4561
    5.4100    0.4521
    5.4200    0.4478
    5.4300    0.4433
    5.4400    0.4382
    5.4500    0.4332
    5.4600    0.4291
    5.4700    0.4251
    5.4800    0.4205
    5.4900    0.4160
    5.5000    0.4118
    5.5100    0.4065
    5.5200    0.4009
    5.5300    0.3960
    5.5400    0.3901
    5.5500    0.3838
    5.5600    0.3783
    5.5700    0.3736
    5.5800    0.3688
    5.5900    0.3638
    5.6000    0.3586
    5.6100    0.3522
    5.6200    0.3464
    5.6300    0.3411
    5.6400    0.3359
    5.6500    0.3321
    5.6600    0.3273
    5.6700    0.3222
    5.6800    0.3179
    5.6900    0.3123
    5.7000    0.3063
    5.7100    0.3011
    5.7200    0.2960
    5.7300    0.2910
    5.7400    0.2860
    5.7500    0.2810
    5.7600    0.2756
    5.7700    0.2701
    5.7800    0.2638
    5.7900    0.2567
    5.8000    0.2513
    5.8100    0.2460
    5.8200    0.2400
    5.8300    0.2352
    5.8400    0.2298
    5.8500    0.2233
    5.8600    0.2170
    5.8700    0.2113
    5.8800    0.2058
    5.8900    0.1996
    5.9000    0.1928
    5.9100    0.1864
    5.9200    0.1805
    5.9300    0.1745
    5.9400    0.1685
    5.9500    0.1622
    5.9600    0.1564
    5.9700    0.1500
    5.9800    0.1434
    5.9900    0.1382
    6.0000    0.1324
    6.0100    0.1262
    6.0200    0.1207
    6.0300    0.1148
    6.0400    0.1087
    6.0500    0.1032
    6.0600    0.0972
    6.0700    0.0913
    6.0800    0.0864
    6.0900    0.0811
    6.1000    0.0755
    6.1100    0.0691
    6.1200    0.0631
    6.1300    0.0570
    6.1400    0.0513
    6.1500    0.0464
    6.1600    0.0408
    6.1700    0.0350
    6.1800    0.0282
    6.1900    0.0210
    6.2000    0.0149
    6.2100    0.0103
    6.2200    0.0058
    6.2300    0.0003
    6.2400   -0.0056
    6.2500   -0.0117
    6.2600   -0.0170
    6.2700   -0.0226
    6.2800   -0.0277
    6.2900   -0.0332
    6.3000   -0.0399
    6.3100   -0.0456
    6.3200   -0.0522
    6.3300   -0.0585
    6.3400   -0.0638
    6.3500   -0.0696
    6.3600   -0.0750
    6.3700   -0.0800
    6.3800   -0.0850
    6.3900   -0.0906
    6.4000   -0.0966
    6.4100   -0.1021
    6.4200   -0.1081
    6.4300   -0.1147
    6.4400   -0.1208
    6.4500   -0.1266
    6.4600   -0.1314
    6.4700   -0.1359
    6.4800   -0.1414
    6.4900   -0.1475
    6.5000   -0.1528
    6.5100   -0.1566
    6.5200   -0.1610
    6.5300   -0.1668
    6.5400   -0.1732
    6.5500   -0.1788
    6.5600   -0.1838
    6.5700   -0.1887
    6.5800   -0.1941
    6.5900   -0.1998
    6.6000   -0.2054
    6.6100   -0.2106
    6.6200   -0.2156
    6.6300   -0.2213
    6.6400   -0.2268
    6.6500   -0.2319
    6.6600   -0.2365
    6.6700   -0.2420
    6.6800   -0.2479
    6.6900   -0.2537
    6.7000   -0.2591
    6.7100   -0.2637
    6.7200   -0.2692
    6.7300   -0.2757
    6.7400   -0.2814
    6.7500   -0.2859
    6.7600   -0.2904
    6.7700   -0.2957
    6.7800   -0.3019
    6.7900   -0.3068
    6.8000   -0.3110
    6.8100   -0.3161
    6.8200   -0.3202
    6.8300   -0.3246
    6.8400   -0.3295
    6.8500   -0.3338
    6.8600   -0.3378
    6.8700   -0.3422
    6.8800   -0.3471
    6.8900   -0.3500
    6.9000   -0.3540
    6.9100   -0.3589
    6.9200   -0.3630
    6.9300   -0.3677
    6.9400   -0.3726
    6.9500   -0.3770
    6.9600   -0.3798
    6.9700   -0.3834
    6.9800   -0.3876
    6.9900   -0.3917
    7.0000   -0.3952
    7.0100   -0.3980
    7.0200   -0.4020
    7.0300   -0.4057
    7.0400   -0.4094
    7.0500   -0.4128
    7.0600   -0.4162
    7.0700   -0.4206
    7.0800   -0.4247
    7.0900   -0.4275
    7.1000   -0.4310
    7.1100   -0.4354
    7.1200   -0.4383
    7.1300   -0.4423
    7.1400   -0.4463
    7.1500   -0.4490
    7.1600   -0.4520
    7.1700   -0.4555
    7.1800   -0.4591
    7.1900   -0.4622
    7.2000   -0.4650
    7.2100   -0.4674
    7.2200   -0.4705
    7.2300   -0.4730
    7.2400   -0.4753
    7.2500   -0.4787
    7.2600   -0.4821
    7.2700   -0.4847
    7.2800   -0.4871
    7.2900   -0.4894
    7.3000   -0.4919
    7.3100   -0.4935
    7.3200   -0.4957
    7.3300   -0.4994
    7.3400   -0.5019
    7.3500   -0.5045
    7.3600   -0.5063
    7.3700   -0.5079
    7.3800   -0.5103
    7.3900   -0.5127
    7.4000   -0.5145
    7.4100   -0.5167
    7.4200   -0.5189
    7.4300   -0.5214
    7.4400   -0.5241
    7.4500   -0.5263
    7.4600   -0.5289
    7.4700   -0.5307
    7.4800   -0.5327
    7.4900   -0.5352
    7.5000   -0.5376
    7.5100   -0.5406
    7.5200   -0.5430
    7.5300   -0.5437
    7.5400   -0.5446
    7.5500   -0.5460
    7.5600   -0.5477
    7.5700   -0.5486
    7.5800   -0.5490
    7.5900   -0.5498
    7.6000   -0.5499
    7.6100   -0.5510
    7.6200   -0.5516
    7.6300   -0.5515
    7.6400   -0.5520
    7.6500   -0.5524
    7.6600   -0.5518
    7.6700   -0.5519
    7.6800   -0.5527
    7.6900   -0.5532
    7.7000   -0.5535
    7.7100   -0.5535
    7.7200   -0.5537
    7.7300   -0.5540
    7.7400   -0.5536
    7.7500   -0.5535
    7.7600   -0.5536
    7.7700   -0.5542
    7.7800   -0.5553
    7.7900   -0.5562
    7.8000   -0.5573
    7.8100   -0.5575
    7.8200   -0.5581
    7.8300   -0.5576
    7.8400   -0.5558
    7.8500   -0.5561
    7.8600   -0.5570
    7.8700   -0.5568
    7.8800   -0.5568
    7.8900   -0.5571
    7.9000   -0.5559
    7.9100   -0.5547
    7.9200   -0.5540
    7.9300   -0.5535
    7.9400   -0.5530
    7.9500   -0.5527
    7.9600   -0.5519
    7.9700   -0.5507
    7.9800   -0.5494
    7.9900   -0.5472
    8.0000   -0.5450
    8.0100   -0.5432
    8.0200   -0.5420
    8.0300   -0.5412
    8.0400   -0.5401
    8.0500   -0.5380
    8.0600   -0.5361
    8.0700   -0.5346
    8.0800   -0.5327
    8.0900   -0.5302
    8.1000   -0.5286
    8.1100   -0.5273
    8.1200   -0.5250
    8.1300   -0.5231
    8.1400   -0.5207
    8.1500   -0.5183
    8.1600   -0.5167
    8.1700   -0.5146
    8.1800   -0.5120
    8.1900   -0.5096
    8.2000   -0.5069
    8.2100   -0.5048
    8.2200   -0.5032
    8.2300   -0.5023
    8.2400   -0.5006
    8.2500   -0.4979
    8.2600   -0.4957
    8.2700   -0.4925
    8.2800   -0.4891
    8.2900   -0.4864
    8.3000   -0.4839
    8.3100   -0.4813
    8.3200   -0.4779
    8.3300   -0.4752
    8.3400   -0.4727
    8.3500   -0.4689
    8.3600   -0.4660
    8.3700   -0.4630
    8.3800   -0.4589
    8.3900   -0.4555
    8.4000   -0.4531
    8.4100   -0.4500
    8.4200   -0.4458
    8.4300   -0.4417
    8.4400   -0.4374
    8.4500   -0.4340
    8.4600   -0.4305
    8.4700   -0.4267
    8.4800   -0.4233
    8.4900   -0.4203
    8.5000   -0.4166
    8.5100   -0.4120
    8.5200   -0.4077
    8.5300   -0.4026
    8.5400   -0.3985
    8.5500   -0.3947
    8.5600   -0.3903
    8.5700   -0.3859
    8.5800   -0.3810
    8.5900   -0.3761
    8.6000   -0.3719
    8.6100   -0.3681
    8.6200   -0.3640
    8.6300   -0.3583
    8.6400   -0.3524
    8.6500   -0.3469
    8.6600   -0.3415
    8.6700   -0.3372
    8.6800   -0.3326
    8.6900   -0.3284
    8.7000   -0.3238
    8.7100   -0.3189
    8.7200   -0.3154
    8.7300   -0.3111
    8.7400   -0.3067
    8.7500   -0.3038
    8.7600   -0.2997
    8.7700   -0.2953
    8.7800   -0.2915
    8.7900   -0.2872
    8.8000   -0.2827
    8.8100   -0.2783
    8.8200   -0.2734
    8.8300   -0.2689
    8.8400   -0.2650
    8.8500   -0.2613
    8.8600   -0.2574
    8.8700   -0.2521
    8.8800   -0.2472
    8.8900   -0.2423
    8.9000   -0.2368
    8.9100   -0.2312
    8.9200   -0.2253
    8.9300   -0.2201
    8.9400   -0.2157
    8.9500   -0.2108
    8.9600   -0.2060
    8.9700   -0.2006
    8.9800   -0.1942
    8.9900   -0.1885
    9.0000   -0.1836
    9.0100   -0.1783
    9.0200   -0.1732
    9.0300   -0.1683
    9.0400   -0.1633
    9.0500   -0.1583
    9.0600   -0.1525
    9.0700   -0.1466
    9.0800   -0.1406
    9.0900   -0.1353
    9.1000   -0.1304
    9.1100   -0.1254
    9.1200   -0.1204
    9.1300   -0.1148
    9.1400   -0.1089
    9.1500   -0.1027
    9.1600   -0.0968
    9.1700   -0.0915
    9.1800   -0.0866
    9.1900   -0.0823
    9.2000   -0.0779
    9.2100   -0.0733
    9.2200   -0.0683
    9.2300   -0.0620
    9.2400   -0.0563
    9.2500   -0.0511
    9.2600   -0.0459
    9.2700   -0.0398
    9.2800   -0.0333
    9.2900   -0.0277
    9.3000   -0.0225
    9.3100   -0.0176
    9.3200   -0.0126
    9.3300   -0.0068
    9.3400   -0.0008
    9.3500    0.0042
    9.3600    0.0090
    9.3700    0.0143
    9.3800    0.0190
    9.3900    0.0246
    9.4000    0.0303
    9.4100    0.0356
    9.4200    0.0409
    9.4300    0.0472
    9.4400    0.0529
    9.4500    0.0572
    9.4600    0.0615
    9.4700    0.0660
    9.4800    0.0706
    9.4900    0.0760
    9.5000    0.0807
    9.5100    0.0852
    9.5200    0.0903
    9.5300    0.0958
    9.5400    0.1012
    9.5500    0.1060
    9.5600    0.1110
    9.5700    0.1156
    9.5800    0.1205
    9.5900    0.1257
    9.6000    0.1305
    9.6100    0.1360
    9.6200    0.1419
    9.6300    0.1480
    9.6400    0.1537
    9.6500    0.1591
    9.6600    0.1638
    9.6700    0.1681
    9.6800    0.1738
    9.6900    0.1787
    9.7000    0.1838
    9.7100    0.1894
    9.7200    0.1951
    9.7300    0.2005
    9.7400    0.2057
    9.7500    0.2106
    9.7600    0.2146
    9.7700    0.2189
    9.7800    0.2237
    9.7900    0.2289
    9.8000    0.2338
    9.8100    0.2377
    9.8200    0.2436
    9.8300    0.2491
    9.8400    0.2540
    9.8500    0.2598
    9.8600    0.2643
    9.8700    0.2685
    9.8800    0.2728
    9.8900    0.2772
    9.9000    0.2825
    9.9100    0.2866
    9.9200    0.2909
    9.9300    0.2965
    9.9400    0.3006
    9.9500    0.3045
    9.9600    0.3088
    9.9700    0.3131
    9.9800    0.3177
    9.9900    0.3226
   10.0000    0.3269
    };

==> Data/Oscillator/sigma01/kf_varn_pos.tex <==
    \addplot[
    thick,
    dotted,
    black
    ]
    table {
         0    1.0000
    0.0100    0.9972
    0.0200    0.9928
    0.0300    0.9838
    0.0400    0.9791
    0.0500    0.9755
    0.0600    0.9713
    0.0700    0.9672
    0.0800    0.9637
    0.0900    0.9550
    0.1000    0.9460
    0.1100    0.9476
    0.1200    0.9490
    0.1300    0.9486
    0.1400    0.9456
    0.1500    0.9412
    0.1600    0.9380
    0.1700    0.9347
    0.1800    0.9293
    0.1900    0.9230
    0.2000    0.9184
    0.2100    0.9132
    0.2200    0.9090
    0.2300    0.9113
    0.2400    0.9088
    0.2500    0.9025
    0.2600    0.8964
    0.2700    0.8913
    0.2800    0.8925
    0.2900    0.8869
    0.3000    0.8831
    0.3100    0.8807
    0.3200    0.8742
    0.3300    0.8724
    0.3400    0.8694
    0.3500    0.8678
    0.3600    0.8707
    0.3700    0.8703
    0.3800    0.8627
    0.3900    0.8552
    0.4000    0.8494
    0.4100    0.8428
    0.4200    0.8359
    0.4300    0.8296
    0.4400    0.8283
    0.4500    0.8255
    0.4600    0.8190
    0.4700    0.8155
    0.4800    0.8139
    0.4900    0.8109
    0.5000    0.8077
    0.5100    0.8053
    0.5200    0.8009
    0.5300    0.7960
    0.5400    0.7915
    0.5500    0.7850
    0.5600    0.7799
    0.5700    0.7760
    0.5800    0.7708
    0.5900    0.7658
    0.6000    0.7623
    0.6100    0.7588
    0.6200    0.7543
    0.6300    0.7497
    0.6400    0.7451
    0.6500    0.7392
    0.6600    0.7339
    0.6700    0.7314
    0.6800    0.7268
    0.6900    0.7230
    0.7000    0.7198
    0.7100    0.7140
    0.7200    0.7078
    0.7300    0.7011
    0.7400    0.6943
    0.7500    0.6884
    0.7600    0.6852
    0.7700    0.6819
    0.7800    0.6775
    0.7900    0.6747
    0.8000    0.6683
    0.8100    0.6603
    0.8200    0.6554
    0.8300    0.6512
    0.8400    0.6455
    0.8500    0.6379
    0.8600    0.6326
    0.8700    0.6280
    0.8800    0.6230
    0.8900    0.6176
    0.9000    0.6098
    0.9100    0.6038
    0.9200    0.6002
    0.9300    0.5973
    0.9400    0.5921
    0.9500    0.5843
    0.9600    0.5768
    0.9700    0.5704
    0.9800    0.5645
    0.9900    0.5599
    1.0000    0.5548
    1.0100    0.5467
    1.0200    0.5402
    1.0300    0.5362
    1.0400    0.5313
    1.0500    0.5242
    1.0600    0.5181
    1.0700    0.5116
    1.0800    0.5049
    1.0900    0.5004
    1.1000    0.4961
    1.1100    0.4895
    1.1200    0.4824
    1.1300    0.4766
    1.1400    0.4724
    1.1500    0.4693
    1.1600    0.4643
    1.1700    0.4600
    1.1800    0.4551
    1.1900    0.4485
    1.2000    0.4441
    1.2100    0.4409
    1.2200    0.4370
    1.2300    0.4326
    1.2400    0.4272
    1.2500    0.4221
    1.2600    0.4168
    1.2700    0.4113
    1.2800    0.4067
    1.2900    0.4024
    1.3000    0.3977
    1.3100    0.3924
    1.3200    0.3884
    1.3300    0.3830
    1.3400    0.3771
    1.3500    0.3732
    1.3600    0.3692
    1.3700    0.3637
    1.3800    0.3588
    1.3900    0.3537
    1.4000    0.3487
    1.4100    0.3438
    1.4200    0.3385
    1.4300    0.3336
    1.4400    0.3297
    1.4500    0.3255
    1.4600    0.3219
    1.4700    0.3166
    1.4800    0.3098
    1.4900    0.3049
    1.5000    0.2996
    1.5100    0.2932
    1.5200    0.2878
    1.5300    0.2837
    1.5400    0.2792
    1.5500    0.2747
    1.5600    0.2695
    1.5700    0.2637
    1.5800    0.2585
    1.5900    0.2532
    1.6000    0.2479
    1.6100    0.2448
    1.6200    0.2410
    1.6300    0.2362
    1.6400    0.2311
    1.6500    0.2265
    1.6600    0.2220
    1.6700    0.2167
    1.6800    0.2118
    1.6900    0.2069
    1.7000    0.2026
    1.7100    0.1976
    1.7200    0.1946
    1.7300    0.1914
    1.7400    0.1858
    1.7500    0.1829
    1.7600    0.1791
    1.7700    0.1740
    1.7800    0.1692
    1.7900    0.1645
    1.8000    0.1608
    1.8100    0.1567
    1.8200    0.1524
    1.8300    0.1477
    1.8400    0.1443
    1.8500    0.1396
    1.8600    0.1328
    1.8700    0.1280
    1.8800    0.1236
    1.8900    0.1188
    1.9000    0.1136
    1.9100    0.1080
    1.9200    0.1032
    1.9300    0.0984
    1.9400    0.0934
    1.9500    0.0886
    1.9600    0.0837
    1.9700    0.0798
    1.9800    0.0758
    1.9900    0.0720
    2.0000    0.0689
    2.0100    0.0637
    2.0200    0.0586
    2.0300    0.0548
    2.0400    0.0518
    2.0500    0.0484
    2.0600    0.0445
    2.0700    0.0412
    2.0800    0.0368
    2.0900    0.0320
    2.1000    0.0271
    2.1100    0.0221
    2.1200    0.0187
    2.1300    0.0156
    2.1400    0.0132
    2.1500    0.0108
    2.1600    0.0059
    2.1700    0.0019
    2.1800   -0.0001
    2.1900   -0.0036
    2.2000   -0.0075
    2.2100   -0.0105
    2.2200   -0.0136
    2.2300   -0.0166
    2.2400   -0.0199
    2.2500   -0.0235
    2.2600   -0.0268
    2.2700   -0.0307
    2.2800   -0.0338
    2.2900   -0.0365
    2.3000   -0.0396
    2.3100   -0.0429
    2.3200   -0.0472
    2.3300   -0.0509
    2.3400   -0.0543
    2.3500   -0.0572
    2.3600   -0.0595
    2.3700   -0.0622
    2.3800   -0.0657
    2.3900   -0.0700
    2.4000   -0.0733
    2.4100   -0.0765
    2.4200   -0.0792
    2.4300   -0.0809
    2.4400   -0.0837
    2.4500   -0.0866
    2.4600   -0.0885
    2.4700   -0.0908
    2.4800   -0.0929
    2.4900   -0.0945
    2.5000   -0.0970
    2.5100   -0.0993
    2.5200   -0.1016
    2.5300   -0.1045
    2.5400   -0.1073
    2.5500   -0.1098
    2.5600   -0.1128
    2.5700   -0.1147
    2.5800   -0.1166
    2.5900   -0.1180
    2.6000   -0.1195
    2.6100   -0.1222
    2.6200   -0.1238
    2.6300   -0.1245
    2.6400   -0.1257
    2.6500   -0.1286
    2.6600   -0.1309
    2.6700   -0.1335
    2.6800   -0.1366
    2.6900   -0.1389
    2.7000   -0.1406
    2.7100   -0.1416
    2.7200   -0.1434
    2.7300   -0.1453
    2.7400   -0.1472
    2.7500   -0.1495
    2.7600   -0.1505
    2.7700   -0.1517
    2.7800   -0.1540
    2.7900   -0.1564
    2.8000   -0.1584
    2.8100   -0.1597
    2.8200   -0.1602
    2.8300   -0.1614
    2.8400   -0.1633
    2.8500   -0.1655
    2.8600   -0.1670
    2.8700   -0.1681
    2.8800   -0.1705
    2.8900   -0.1715
    2.9000   -0.1721
    2.9100   -0.1733
    2.9200   -0.1752
    2.9300   -0.1772
    2.9400   -0.1784
    2.9500   -0.1803
    2.9600   -0.1825
    2.9700   -0.1844
    2.9800   -0.1858
    2.9900   -0.1876
    3.0000   -0.1892
    3.0100   -0.1894
    3.0200   -0.1904
    3.0300   -0.1920
    3.0400   -0.1933
    3.0500   -0.1940
    3.0600   -0.1947
    3.0700   -0.1957
    3.0800   -0.1970
    3.0900   -0.1987
    3.1000   -0.1998
    3.1100   -0.2001
    3.1200   -0.2004
    3.1300   -0.2019
    3.1400   -0.2034
    3.1500   -0.2043
    3.1600   -0.2056
    3.1700   -0.2068
    3.1800   -0.2083
    3.1900   -0.2097
    3.2000   -0.2111
    3.2100   -0.2126
    3.2200   -0.2136
    3.2300   -0.2143
    3.2400   -0.2152
    3.2500   -0.2162
    3.2600   -0.2171
    3.2700   -0.2178
    3.2800   -0.2179
    3.2900   -0.2178
    3.3000   -0.2185
    3.3100   -0.2191
    3.3200   -0.2195
    3.3300   -0.2209
    3.3400   -0.2231
    3.3500   -0.2253
    3.3600   -0.2265
    3.3700   -0.2273
    3.3800   -0.2284
    3.3900   -0.2290
    3.4000   -0.2297
    3.4100   -0.2307
    3.4200   -0.2310
    3.4300   -0.2309
    3.4400   -0.2300
    3.4500   -0.2293
    3.4600   -0.2295
    3.4700   -0.2300
    3.4800   -0.2305
    3.4900   -0.2307
    3.5000   -0.2316
    3.5100   -0.2327
    3.5200   -0.2324
    3.5300   -0.2325
    3.5400   -0.2327
    3.5500   -0.2322
    3.5600   -0.2315
    3.5700   -0.2306
    3.5800   -0.2312
    3.5900   -0.2324
    3.6000   -0.2321
    3.6100   -0.2315
    3.6200   -0.2313
    3.6300   -0.2310
    3.6400   -0.2302
    3.6500   -0.2295
    3.6600   -0.2296
    3.6700   -0.2297
    3.6800   -0.2296
    3.6900   -0.2291
    3.7000   -0.2282
    3.7100   -0.2276
    3.7200   -0.2269
    3.7300   -0.2267
    3.7400   -0.2264
    3.7500   -0.2258
    3.7600   -0.2258
    3.7700   -0.2259
    3.7800   -0.2248
    3.7900   -0.2241
    3.8000   -0.2230
    3.8100   -0.2216
    3.8200   -0.2210
    3.8300   -0.2206
    3.8400   -0.2201
    3.8500   -0.2195
    3.8600   -0.2184
    3.8700   -0.2176
    3.8800   -0.2169
    3.8900   -0.2153
    3.9000   -0.2135
    3.9100   -0.2121
    3.9200   -0.2113
    3.9300   -0.2111
    3.9400   -0.2103
    3.9500   -0.2093
    3.9600   -0.2090
    3.9700   -0.2094
    3.9800   -0.2085
    3.9900   -0.2075
    4.0000   -0.2060
    4.0100   -0.2050
    4.0200   -0.2049
    4.0300   -0.2034
    4.0400   -0.2028
    4.0500   -0.2018
    4.0600   -0.2008
    4.0700   -0.1998
    4.0800   -0.1981
    4.0900   -0.1975
    4.1000   -0.1980
    4.1100   -0.1978
    4.1200   -0.1962
    4.1300   -0.1944
    4.1400   -0.1932
    4.1500   -0.1915
    4.1600   -0.1906
    4.1700   -0.1893
    4.1800   -0.1877
    4.1900   -0.1867
    4.2000   -0.1855
    4.2100   -0.1841
    4.2200   -0.1835
    4.2300   -0.1822
    4.2400   -0.1800
    4.2500   -0.1777
    4.2600   -0.1749
    4.2700   -0.1729
    4.2800   -0.1717
    4.2900   -0.1713
    4.3000   -0.1704
    4.3100   -0.1688
    4.3200   -0.1667
    4.3300   -0.1651
    4.3400   -0.1637
    4.3500   -0.1616
    4.3600   -0.1604
    4.3700   -0.1587
    4.3800   -0.1566
    4.3900   -0.1551
    4.4000   -0.1528
    4.4100   -0.1501
    4.4200   -0.1483
    4.4300   -0.1466
    4.4400   -0.1447
    4.4500   -0.1429
    4.4600   -0.1409
    4.4700   -0.1392
    4.4800   -0.1380
    4.4900   -0.1364
    4.5000   -0.1337
    4.5100   -0.1312
    4.5200   -0.1300
    4.5300   -0.1287
    4.5400   -0.1270
    4.5500   -0.1255
    4.5600   -0.1236
    4.5700   -0.1215
    4.5800   -0.1200
    4.5900   -0.1184
    4.6000   -0.1171
    4.6100   -0.1160
    4.6200   -0.1149
    4.6300   -0.1137
    4.6400   -0.1122
    4.6500   -0.1110
    4.6600   -0.1093
    4.6700   -0.1079
    4.6800   -0.1064
    4.6900   -0.1041
    4.7000   -0.1025
    4.7100   -0.1003
    4.7200   -0.0984
    4.7300   -0.0972
    4.7400   -0.0958
    4.7500   -0.0944
    4.7600   -0.0929
    4.7700   -0.0916
    4.7800   -0.0899
    4.7900   -0.0884
    4.8000   -0.0876
    4.8100   -0.0861
    4.8200   -0.0830
    4.8300   -0.0793
    4.8400   -0.0766
    4.8500   -0.0747
    4.8600   -0.0728
    4.8700   -0.0708
    4.8800   -0.0688
    4.8900   -0.0679
    4.9000   -0.0664
    4.9100   -0.0645
    4.9200   -0.0638
    4.9300   -0.0613
    4.9400   -0.0582
    4.9500   -0.0562
    4.9600   -0.0532
    4.9700   -0.0513
    4.9800   -0.0497
    4.9900   -0.0471
    5.0000   -0.0447
    5.0100   -0.0424
    5.0200   -0.0404
    5.0300   -0.0381
    5.0400   -0.0359
    5.0500   -0.0344
    5.0600   -0.0323
    5.0700   -0.0291
    5.0800   -0.0264
    5.0900   -0.0246
    5.1000   -0.0225
    5.1100   -0.0197
    5.1200   -0.0168
    5.1300   -0.0141
    5.1400   -0.0121
    5.1500   -0.0099
    5.1600   -0.0076
    5.1700   -0.0048
    5.1800   -0.0026
    5.1900   -0.0011
    5.2000    0.0018
    5.2100    0.0043
    5.2200    0.0060
    5.2300    0.0076
    5.2400    0.0093
    5.2500    0.0113
    5.2600    0.0135
    5.2700    0.0154
    5.2800    0.0172
    5.2900    0.0192
    5.3000    0.0210
    5.3100    0.0228
    5.3200    0.0243
    5.3300    0.0276
    5.3400    0.0325
    5.3500    0.0362
    5.3600    0.0390
    5.3700    0.0409
    5.3800    0.0423
    5.3900    0.0439
    5.4000    0.0460
    5.4100    0.0485
    5.4200    0.0508
    5.4300    0.0528
    5.4400    0.0543
    5.4500    0.0560
    5.4600    0.0585
    5.4700    0.0612
    5.4800    0.0633
    5.4900    0.0656
    5.5000    0.0682
    5.5100    0.0698
    5.5200    0.0711
    5.5300    0.0731
    5.5400    0.0741
    5.5500    0.0748
    5.5600    0.0762
    5.5700    0.0784
    5.5800    0.0806
    5.5900    0.0825
    5.6000    0.0843
    5.6100    0.0849
    5.6200    0.0861
    5.6300    0.0878
    5.6400    0.0896
    5.6500    0.0927
    5.6600    0.0950
    5.6700    0.0970
    5.6800    0.0998
    5.6900    0.1014
    5.7000    0.1025
    5.7100    0.1045
    5.7200    0.1065
    5.7300    0.1088
    5.7400    0.1110
    5.7500    0.1133
    5.7600    0.1151
    5.7700    0.1169
    5.7800    0.1180
    5.7900    0.1182
    5.8000    0.1200
    5.8100    0.1220
    5.8200    0.1233
    5.8300    0.1258
    5.8400    0.1277
    5.8500    0.1285
    5.8600    0.1296
    5.8700    0.1312
    5.8800    0.1329
    5.8900    0.1340
    5.9000    0.1346
    5.9100    0.1354
    5.9200    0.1368
    5.9300    0.1380
    5.9400    0.1393
    5.9500    0.1402
    5.9600    0.1415
    5.9700    0.1424
    5.9800    0.1429
    5.9900    0.1448
    6.0000    0.1461
    6.0100    0.1471
    6.0200    0.1486
    6.0300    0.1499
    6.0400    0.1509
    6.0500    0.1525
    6.0600    0.1535
    6.0700    0.1547
    6.0800    0.1568
    6.0900    0.1585
    6.1000    0.1599
    6.1100    0.1606
    6.1200    0.1617
    6.1300    0.1625
    6.1400    0.1638
    6.1500    0.1659
    6.1600    0.1672
    6.1700    0.1684
    6.1800    0.1685
    6.1900    0.1683
    6.2000    0.1690
    6.2100    0.1712
    6.2200    0.1734
    6.2300    0.1747
    6.2400    0.1756
    6.2500    0.1764
    6.2600    0.1778
    6.2700    0.1789
    6.2800    0.1805
    6.2900    0.1817
    6.3000    0.1818
    6.3100    0.1828
    6.3200    0.1829
    6.3300    0.1831
    6.3400    0.1843
    6.3500    0.1851
    6.3600    0.1862
    6.3700    0.1876
    6.3800    0.1891
    6.3900    0.1899
    6.4000    0.1903
    6.4100    0.1912
    6.4200    0.1916
    6.4300    0.1913
    6.4400    0.1915
    6.4500    0.1919
    6.4600    0.1932
    6.4700    0.1948
    6.4800    0.1954
    6.4900    0.1954
    6.5000    0.1962
    6.5100    0.1984
    6.5200    0.1999
    6.5300    0.2002
    6.5400    0.1998
    6.5500    0.2001
    6.5600    0.2009
    6.5700    0.2018
    6.5800    0.2023
    6.5900    0.2023
    6.6000    0.2024
    6.6100    0.2029
    6.6200    0.2035
    6.6300    0.2034
    6.6400    0.2035
    6.6500    0.2039
    6.6600    0.2047
    6.6700    0.2046
    6.6800    0.2041
    6.6900    0.2036
    6.7000    0.2035
    6.7100    0.2040
    6.7200    0.2036
    6.7300    0.2022
    6.7400    0.2015
    6.7500    0.2018
    6.7600    0.2022
    6.7700    0.2017
    6.7800    0.2003
    6.7900    0.2000
    6.8000    0.2003
    6.8100    0.1998
    6.8200    0.2001
    6.8300    0.2002
    6.8400    0.1996
    6.8500    0.1997
    6.8600    0.1999
    6.8700    0.1997
    6.8800    0.1990
    6.8900    0.2001
    6.9000    0.2002
    6.9100    0.1993
    6.9200    0.1992
    6.9300    0.1984
    6.9400    0.1974
    6.9500    0.1968
    6.9600    0.1976
    6.9700    0.1977
    6.9800    0.1970
    6.9900    0.1965
    7.0000    0.1965
    7.0100    0.1970
    7.0200    0.1965
    7.0300    0.1961
    7.0400    0.1957
    7.0500    0.1955
    7.0600    0.1953
    7.0700    0.1941
    7.0800    0.1930
    7.0900    0.1932
    7.1000    0.1927
    7.1100    0.1912
    7.1200    0.1910
    7.1300    0.1898
    7.1400    0.1884
    7.1500    0.1883
    7.1600    0.1879
    7.1700    0.1868
    7.1800    0.1856
    7.1900    0.1848
    7.2000    0.1843
    7.2100    0.1841
    7.2200    0.1831
    7.2300    0.1827
    7.2400    0.1824
    7.2500    0.1810
    7.2600    0.1795
    7.2700    0.1787
    7.2800    0.1781
    7.2900    0.1774
    7.3000    0.1766
    7.3100    0.1766
    7.3200    0.1758
    7.3300    0.1737
    7.3400    0.1726
    7.3500    0.1713
    7.3600    0.1708
    7.3700    0.1703
    7.3800    0.1690
    7.3900    0.1678
    7.4000    0.1669
    7.4100    0.1656
    7.4200    0.1643
    7.4300    0.1626
    7.4400    0.1607
    7.4500    0.1591
    7.4600    0.1571
    7.4700    0.1557
    7.4800    0.1541
    7.4900    0.1520
    7.5000    0.1498
    7.5100    0.1470
    7.5200    0.1446
    7.5300    0.1437
    7.5400    0.1427
    7.5500    0.1411
    7.5600    0.1390
    7.5700    0.1378
    7.5800    0.1368
    7.5900    0.1356
    7.6000    0.1348
    7.6100    0.1332
    7.6200    0.1319
    7.6300    0.1313
    7.6400    0.1299
    7.6500    0.1287
    7.6600    0.1283
    7.6700    0.1273
    7.6800    0.1255
    7.6900    0.1239
    7.7000    0.1225
    7.7100    0.1213
    7.7200    0.1199
    7.7300    0.1183
    7.7400    0.1173
    7.7500    0.1160
    7.7600    0.1144
    7.7700    0.1123
    7.7800    0.1097
    7.7900    0.1071
    7.8000    0.1043
    7.8100    0.1021
    7.8200    0.0996
    7.8300    0.0980
    7.8400    0.0976
    7.8500    0.0952
    7.8600    0.0921
    7.8700    0.0900
    7.8800    0.0876
    7.8900    0.0848
    7.9000    0.0834
    7.9100    0.0819
    7.9200    0.0800
    7.9300    0.0777
    7.9400    0.0753
    7.9500    0.0728
    7.9600    0.0706
    7.9700    0.0687
    7.9800    0.0669
    7.9900    0.0658
    8.0000    0.0647
    8.0100    0.0632
    8.0200    0.0611
    8.0300    0.0586
    8.0400    0.0562
    8.0500    0.0548
    8.0600    0.0532
    8.0700    0.0510
    8.0800    0.0492
    8.0900    0.0479
    8.1000    0.0458
    8.1100    0.0433
    8.1200    0.0416
    8.1300    0.0396
    8.1400    0.0380
    8.1500    0.0363
    8.1600    0.0339
    8.1700    0.0317
    8.1800    0.0301
    8.1900    0.0282
    8.2000    0.0265
    8.2100    0.0243
    8.2200    0.0215
    8.2300    0.0180
    8.2400    0.0151
    8.2500    0.0132
    8.2600    0.0106
    8.2700    0.0090
    8.2800    0.0075
    8.2900    0.0054
    8.3000    0.0030
    8.3100    0.0006
    8.3200   -0.0011
    8.3300   -0.0033
    8.3400   -0.0060
    8.3500   -0.0075
    8.3600   -0.0097
    8.3700   -0.0120
    8.3800   -0.0132
    8.3900   -0.0152
    8.4000   -0.0181
    8.4100   -0.0204
    8.4200   -0.0218
    8.4300   -0.0233
    8.4400   -0.0246
    8.4500   -0.0267
    8.4600   -0.0289
    8.4700   -0.0307
    8.4800   -0.0330
    8.4900   -0.0357
    8.5000   -0.0377
    8.5100   -0.0390
    8.5200   -0.0406
    8.5300   -0.0414
    8.5400   -0.0432
    8.5500   -0.0453
    8.5600   -0.0469
    8.5700   -0.0485
    8.5800   -0.0495
    8.5900   -0.0506
    8.6000   -0.0525
    8.6100   -0.0547
    8.6200   -0.0566
    8.6300   -0.0571
    8.6400   -0.0573
    8.6500   -0.0579
    8.6600   -0.0586
    8.6700   -0.0604
    8.6800   -0.0618
    8.6900   -0.0636
    8.7000   -0.0651
    8.7100   -0.0663
    8.7200   -0.0689
    8.7300   -0.0707
    8.7400   -0.0726
    8.7500   -0.0758
    8.7600   -0.0780
    8.7700   -0.0798
    8.7800   -0.0823
    8.7900   -0.0844
    8.8000   -0.0862
    8.8100   -0.0882
    8.8200   -0.0898
    8.8300   -0.0918
    8.8400   -0.0943
    8.8500   -0.0972
    8.8600   -0.0998
    8.8700   -0.1011
    8.8800   -0.1028
    8.8900   -0.1045
    8.9000   -0.1057
    8.9100   -0.1068
    8.9200   -0.1076
    8.9300   -0.1090
    8.9400   -0.1112
    8.9500   -0.1130
    8.9600   -0.1148
    8.9700   -0.1161
    8.9800   -0.1164
    8.9900   -0.1174
    9.0000   -0.1191
    9.0100   -0.1205
    9.0200   -0.1220
    9.0300   -0.1238
    9.0400   -0.1254
    9.0500   -0.1270
    9.0600   -0.1279
    9.0700   -0.1287
    9.0800   -0.1293
    9.0900   -0.1307
    9.1000   -0.1323
    9.1100   -0.1339
    9.1200   -0.1355
    9.1300   -0.1366
    9.1400   -0.1373
    9.1500   -0.1377
    9.1600   -0.1383
    9.1700   -0.1396
    9.1800   -0.1412
    9.1900   -0.1434
    9.2000   -0.1455
    9.2100   -0.1474
    9.2200   -0.1489
    9.2300   -0.1493
    9.2400   -0.1501
    9.2500   -0.1513
    9.2600   -0.1526
    9.2700   -0.1531
    9.2800   -0.1530
    9.2900   -0.1539
    9.3000   -0.1551
    9.3100   -0.1565
    9.3200   -0.1578
    9.3300   -0.1584
    9.3400   -0.1587
    9.3500   -0.1601
    9.3600   -0.1615
    9.3700   -0.1624
    9.3800   -0.1640
    9.3900   -0.1647
    9.4000   -0.1652
    9.4100   -0.1661
    9.4200   -0.1669
    9.4300   -0.1668
    9.4400   -0.1673
    9.4500   -0.1689
    9.4600   -0.1706
    9.4700   -0.1721
    9.4800   -0.1736
    9.4900   -0.1742
    9.5000   -0.1756
    9.5100   -0.1770
    9.5200   -0.1779
    9.5300   -0.1784
    9.5400   -0.1790
    9.5500   -0.1800
    9.5600   -0.1809
    9.5700   -0.1821
    9.5800   -0.1831
    9.5900   -0.1838
    9.6000   -0.1847
    9.6100   -0.1850
    9.6200   -0.1849
    9.6300   -0.1845
    9.6400   -0.1845
    9.6500   -0.1846
    9.6600   -0.1854
    9.6700   -0.1866
    9.6800   -0.1864
    9.6900   -0.1869
    9.7000   -0.1872
    9.7100   -0.1870
    9.7200   -0.1866
    9.7300   -0.1864
    9.7400   -0.1864
    9.7500   -0.1866
    9.7600   -0.1876
    9.7700   -0.1884
    9.7800   -0.1886
    9.7900   -0.1884
    9.8000   -0.1884
    9.8100   -0.1894
    9.8200   -0.1884
    9.8300   -0.1877
    9.8400   -0.1875
    9.8500   -0.1864
    9.8600   -0.1864
    9.8700   -0.1868
    9.8800   -0.1869
    9.8900   -0.1869
    9.9000   -0.1861
    9.9100   -0.1863
    9.9200   -0.1862
    9.9300   -0.1849
    9.9400   -0.1849
    9.9500   -0.1851
    9.9600   -0.1849
    9.9700   -0.1846
    9.9800   -0.1840
    9.9900   -0.1829
   10.0000   -0.1824
    };

==> Data/Oscillator/sigma01/kf_varn_vel.tex <==
    \addplot[
    thick,
    dotted,
    black
    ]
    table {
         0         0
    0.0100   -0.0099
    0.0200   -0.0196
    0.0300   -0.0291
    0.0400   -0.0384
    0.0500   -0.0475
    0.0600   -0.0565
    0.0700   -0.0652
    0.0800   -0.0738
    0.0900   -0.0822
    0.1000   -0.0904
    0.1100   -0.0984
    0.1200   -0.1064
    0.1300   -0.1142
    0.1400   -0.1219
    0.1500   -0.1294
    0.1600   -0.1368
    0.1700   -0.1441
    0.1800   -0.1512
    0.1900   -0.1581
    0.2000   -0.1649
    0.2100   -0.1716
    0.2200   -0.1781
    0.2300   -0.1845
    0.2400   -0.1909
    0.2500   -0.1970
    0.2600   -0.2031
    0.2700   -0.2090
    0.2800   -0.2148
    0.2900   -0.2205
    0.3000   -0.2261
    0.3100   -0.2316
    0.3200   -0.2370
    0.3300   -0.2423
    0.3400   -0.2475
    0.3500   -0.2526
    0.3600   -0.2577
    0.3700   -0.2627
    0.3800   -0.2675
    0.3900   -0.2722
    0.4000   -0.2768
    0.4100   -0.2812
    0.4200   -0.2855
    0.4300   -0.2897
    0.4400   -0.2939
    0.4500   -0.2981
    0.4600   -0.3020
    0.4700   -0.3059
    0.4800   -0.3098
    0.4900   -0.3136
    0.5000   -0.3173
    0.5100   -0.3209
    0.5200   -0.3245
    0.5300   -0.3279
    0.5400   -0.3313
    0.5500   -0.3345
    0.5600   -0.3377
    0.5700   -0.3408
    0.5800   -0.3438
    0.5900   -0.3467
    0.6000   -0.3496
    0.6100   -0.3524
    0.6200   -0.3552
    0.6300   -0.3578
    0.6400   -0.3604
    0.6500   -0.3629
    0.6600   -0.3653
    0.6700   -0.3677
    0.6800   -0.3700
    0.6900   -0.3723
    0.7000   -0.3745
    0.7100   -0.3766
    0.7200   -0.3786
    0.7300   -0.3806
    0.7400   -0.3824
    0.7500   -0.3842
    0.7600   -0.3860
    0.7700   -0.3877
    0.7800   -0.3893
    0.7900   -0.3909
    0.8000   -0.3925
    0.8100   -0.3939
    0.8200   -0.3953
    0.8300   -0.3966
    0.8400   -0.3979
    0.8500   -0.3990
    0.8600   -0.4002
    0.8700   -0.4012
    0.8800   -0.4023
    0.8900   -0.4032
    0.9000   -0.4041
    0.9100   -0.4049
    0.9200   -0.4057
    0.9300   -0.4064
    0.9400   -0.4071
    0.9500   -0.4078
    0.9600   -0.4083
    0.9700   -0.4088
    0.9800   -0.4093
    0.9900   -0.4097
    1.0000   -0.4100
    1.0100   -0.4103
    1.0200   -0.4105
    1.0300   -0.4107
    1.0400   -0.4108
    1.0500   -0.4109
    1.0600   -0.4109
    1.0700   -0.4109
    1.0800   -0.4108
    1.0900   -0.4107
    1.1000   -0.4105
    1.1100   -0.4103
    1.1200   -0.4101
    1.1300   -0.4097
    1.1400   -0.4094
    1.1500   -0.4089
    1.1600   -0.4085
    1.1700   -0.4080
    1.1800   -0.4075
    1.1900   -0.4070
    1.2000   -0.4064
    1.2100   -0.4057
    1.2200   -0.4051
    1.2300   -0.4044
    1.2400   -0.4037
    1.2500   -0.4030
    1.2600   -0.4022
    1.2700   -0.4014
    1.2800   -0.4006
    1.2900   -0.3997
    1.3000   -0.3988
    1.3100   -0.3978
    1.3200   -0.3968
    1.3300   -0.3959
    1.3400   -0.3949
    1.3500   -0.3938
    1.3600   -0.3926
    1.3700   -0.3916
    1.3800   -0.3904
    1.3900   -0.3892
    1.4000   -0.3880
    1.4100   -0.3868
    1.4200   -0.3856
    1.4300   -0.3843
    1.4400   -0.3829
    1.4500   -0.3815
    1.4600   -0.3801
    1.4700   -0.3788
    1.4800   -0.3774
    1.4900   -0.3760
    1.5000   -0.3745
    1.5100   -0.3731
    1.5200   -0.3716
    1.5300   -0.3700
    1.5400   -0.3684
    1.5500   -0.3668
    1.5600   -0.3651
    1.5700   -0.3635
    1.5800   -0.3619
    1.5900   -0.3602
    1.6000   -0.3585
    1.6100   -0.3566
    1.6200   -0.3547
    1.6300   -0.3530
    1.6400   -0.3512
    1.6500   -0.3493
    1.6600   -0.3474
    1.6700   -0.3456
    1.6800   -0.3437
    1.6900   -0.3418
    1.7000   -0.3398
    1.7100   -0.3379
    1.7200   -0.3358
    1.7300   -0.3337
    1.7400   -0.3318
    1.7500   -0.3296
    1.7600   -0.3276
    1.7700   -0.3256
    1.7800   -0.3235
    1.7900   -0.3215
    1.8000   -0.3193
    1.8100   -0.3172
    1.8200   -0.3150
    1.8300   -0.3129
    1.8400   -0.3107
    1.8500   -0.3086
    1.8600   -0.3066
    1.8700   -0.3044
    1.8800   -0.3022
    1.8900   -0.3000
    1.9000   -0.2978
    1.9100   -0.2956
    1.9200   -0.2933
    1.9300   -0.2910
    1.9400   -0.2887
    1.9500   -0.2864
    1.9600   -0.2841
    1.9700   -0.2816
    1.9800   -0.2792
    1.9900   -0.2768
    2.0000   -0.2742
    2.0100   -0.2719
    2.0200   -0.2695
    2.0300   -0.2670
    2.0400   -0.2644
    2.0500   -0.2619
    2.0600   -0.2594
    2.0700   -0.2568
    2.0800   -0.2544
    2.0900   -0.2520
    2.1000   -0.2495
    2.1100   -0.2471
    2.1200   -0.2445
    2.1300   -0.2418
    2.1400   -0.2391
    2.1500   -0.2364
    2.1600   -0.2340
    2.1700   -0.2314
    2.1800   -0.2287
    2.1900   -0.2261
    2.2000   -0.2235
    2.2100   -0.2209
    2.2200   -0.2182
    2.2300   -0.2156
    2.2400   -0.2129
    2.2500   -0.2104
    2.2600   -0.2078
    2.2700   -0.2052
    2.2800   -0.2025
    2.2900   -0.1999
    2.3000   -0.1972
    2.3100   -0.1946
    2.3200   -0.1921
    2.3300   -0.1895
    2.3400   -0.1869
    2.3500   -0.1842
    2.3600   -0.1815
    2.3700   -0.1788
    2.3800   -0.1762
    2.3900   -0.1737
    2.4000   -0.1711
    2.4100   -0.1684
    2.4200   -0.1657
    2.4300   -0.1629
    2.4400   -0.1602
    2.4500   -0.1576
    2.4600   -0.1548
    2.4700   -0.1521
    2.4800   -0.1494
    2.4900   -0.1466
    2.5000   -0.1440
    2.5100   -0.1413
    2.5200   -0.1386
    2.5300   -0.1361
    2.5400   -0.1335
    2.5500   -0.1309
    2.5600   -0.1283
    2.5700   -0.1256
    2.5800   -0.1230
    2.5900   -0.1202
    2.6000   -0.1175
    2.6100   -0.1150
    2.6200   -0.1123
    2.6300   -0.1096
    2.6400   -0.1069
    2.6500   -0.1044
    2.6600   -0.1019
    2.6700   -0.0995
    2.6800   -0.0971
    2.6900   -0.0946
    2.7000   -0.0920
    2.7100   -0.0893
    2.7200   -0.0868
    2.7300   -0.0843
    2.7400   -0.0818
    2.7500   -0.0793
    2.7600   -0.0767
    2.7700   -0.0742
    2.7800   -0.0718
    2.7900   -0.0694
    2.8000   -0.0670
    2.8100   -0.0645
    2.8200   -0.0619
    2.8300   -0.0594
    2.8400   -0.0570
    2.8500   -0.0547
    2.8600   -0.0523
    2.8700   -0.0498
    2.8800   -0.0476
    2.8900   -0.0451
    2.9000   -0.0426
    2.9100   -0.0402
    2.9200   -0.0379
    2.9300   -0.0357
    2.9400   -0.0333
    2.9500   -0.0311
    2.9600   -0.0289
    2.9700   -0.0267
    2.9800   -0.0244
    2.9900   -0.0222
    3.0000   -0.0200
    3.0100   -0.0175
    3.0200   -0.0152
    3.0300   -0.0130
    3.0400   -0.0108
    3.0500   -0.0085
    3.0600   -0.0062
    3.0700   -0.0039
    3.0800   -0.0018
    3.0900    0.0003
    3.1000    0.0025
    3.1100    0.0048
    3.1200    0.0070
    3.1300    0.0091
    3.1400    0.0111
    3.1500    0.0132
    3.1600    0.0153
    3.1700    0.0173
    3.1800    0.0193
    3.1900    0.0213
    3.2000    0.0233
    3.2100    0.0253
    3.2200    0.0273
    3.2300    0.0294
    3.2400    0.0314
    3.2500    0.0334
    3.2600    0.0354
    3.2700    0.0374
    3.2800    0.0395
    3.2900    0.0416
    3.3000    0.0436
    3.3100    0.0455
    3.3200    0.0475
    3.3300    0.0493
    3.3400    0.0509
    3.3500    0.0525
    3.3600    0.0544
    3.3700    0.0562
    3.3800    0.0580
    3.3900    0.0599
    3.4000    0.0618
    3.4100    0.0635
    3.4200    0.0654
    3.4300    0.0674
    3.4400    0.0695
    3.4500    0.0715
    3.4600    0.0733
    3.4700    0.0750
    3.4800    0.0767
    3.4900    0.0785
    3.5000    0.0801
    3.5100    0.0817
    3.5200    0.0835
    3.5300    0.0852
    3.5400    0.0869
    3.5500    0.0887
    3.5600    0.0905
    3.5700    0.0923
    3.5800    0.0938
    3.5900    0.0951
    3.6000    0.0968
    3.6100    0.0985
    3.6200    0.1001
    3.6300    0.1017
    3.6400    0.1033
    3.6500    0.1049
    3.6600    0.1064
    3.6700    0.1078
    3.6800    0.1092
    3.6900    0.1107
    3.7000    0.1123
    3.7100    0.1138
    3.7200    0.1152
    3.7300    0.1166
    3.7400    0.1179
    3.7500    0.1193
    3.7600    0.1205
    3.7700    0.1218
    3.7800    0.1232
    3.7900    0.1245
    3.8000    0.1259
    3.8100    0.1273
    3.8200    0.1285
    3.8300    0.1297
    3.8400    0.1309
    3.8500    0.1320
    3.8600    0.1333
    3.8700    0.1344
    3.8800    0.1356
    3.8900    0.1368
    3.9000    0.1381
    3.9100    0.1393
    3.9200    0.1403
    3.9300    0.1412
    3.9400    0.1422
    3.9500    0.1432
    3.9600    0.1441
    3.9700    0.1448
    3.9800    0.1457
    3.9900    0.1467
    4.0000    0.1477
    4.0100    0.1486
    4.0200    0.1493
    4.0300    0.1503
    4.0400    0.1510
    4.0500    0.1519
    4.0600    0.1527
    4.0700    0.1535
    4.0800    0.1543
    4.0900    0.1550
    4.1000    0.1554
    4.1100    0.1560
    4.1200    0.1568
    4.1300    0.1577
    4.1400    0.1584
    4.1500    0.1592
    4.1600    0.1597
    4.1700    0.1604
    4.1800    0.1611
    4.1900    0.1616
    4.2000    0.1622
    4.2100    0.1628
    4.2200    0.1632
    4.2300    0.1637
    4.2400    0.1644
    4.2500    0.1651
    4.2600    0.1659
    4.2700    0.1664
    4.2800    0.1668
    4.2900    0.1670
    4.3000    0.1673
    4.3100    0.1677
    4.3200    0.1682
    4.3300    0.1685
    4.3400    0.1688
    4.3500    0.1692
    4.3600    0.1695
    4.3700    0.1697
    4.3800    0.1701
    4.3900    0.1703
    4.4000    0.1707
    4.4100    0.1711
    4.4200    0.1712
    4.4300    0.1714
    4.4400    0.1716
    4.4500    0.1717
    4.4600    0.1718
    4.4700    0.1719
    4.4800    0.1718
    4.4900    0.1718
    4.5000    0.1721
    4.5100    0.1722
    4.5200    0.1720
    4.5300    0.1719
    4.5400    0.1718
    4.5500    0.1717
    4.5600    0.1717
    4.5700    0.1716
    4.5800    0.1714
    4.5900    0.1712
    4.6000    0.1710
    4.6100    0.1707
    4.6200    0.1704
    4.6300    0.1701
    4.6400    0.1698
    4.6500    0.1695
    4.6600    0.1692
    4.6700    0.1689
    4.6800    0.1686
    4.6900    0.1684
    4.7000    0.1681
    4.7100    0.1679
    4.7200    0.1676
    4.7300    0.1672
    4.7400    0.1667
    4.7500    0.1663
    4.7600    0.1659
    4.7700    0.1654
    4.7800    0.1650
    4.7900    0.1645
    4.8000    0.1639
    4.8100    0.1634
    4.8200    0.1632
    4.8300    0.1632
    4.8400    0.1628
    4.8500    0.1623
    4.8600    0.1618
    4.8700    0.1613
    4.8800    0.1608
    4.8900    0.1600
    4.9000    0.1594
    4.9100    0.1588
    4.9200    0.1580
    4.9300    0.1575
    4.9400    0.1571
    4.9500    0.1565
    4.9600    0.1560
    4.9700    0.1554
    4.9800    0.1546
    4.9900    0.1541
    5.0000    0.1534
    5.0100    0.1528
    5.0200    0.1520
    5.0300    0.1513
    5.0400    0.1506
    5.0500    0.1497
    5.0600    0.1489
    5.0700    0.1484
    5.0800    0.1477
    5.0900    0.1467
    5.1000    0.1459
    5.1100    0.1452
    5.1200    0.1445
    5.1300    0.1437
    5.1400    0.1427
    5.1500    0.1418
    5.1600    0.1409
    5.1700    0.1401
    5.1800    0.1391
    5.1900    0.1380
    5.2000    0.1372
    5.2100    0.1362
    5.2200    0.1351
    5.2300    0.1339
    5.2400    0.1328
    5.2500    0.1317
    5.2600    0.1307
    5.2700    0.1296
    5.2800    0.1284
    5.2900    0.1273
    5.3000    0.1262
    5.3100    0.1250
    5.3200    0.1238
    5.3300    0.1229
    5.3400    0.1223
    5.3500    0.1214
    5.3600    0.1203
    5.3700    0.1191
    5.3800    0.1177
    5.3900    0.1164
    5.4000    0.1151
    5.4100    0.1139
    5.4200    0.1127
    5.4300    0.1114
    5.4400    0.1100
    5.4500    0.1086
    5.4600    0.1074
    5.4700    0.1062
    5.4800    0.1049
    5.4900    0.1037
    5.5000    0.1024
    5.5100    0.1010
    5.5200    0.0995
    5.5300    0.0981
    5.5400    0.0965
    5.5500    0.0949
    5.5600    0.0934
    5.5700    0.0921
    5.5800    0.0908
    5.5900    0.0894
    5.6000    0.0879
    5.6100    0.0863
    5.6200    0.0848
    5.6300    0.0833
    5.6400    0.0819
    5.6500    0.0807
    5.6600    0.0794
    5.6700    0.0780
    5.6800    0.0768
    5.6900    0.0752
    5.7000    0.0736
    5.7100    0.0722
    5.7200    0.0708
    5.7300    0.0694
    5.7400    0.0680
    5.7500    0.0666
    5.7600    0.0651
    5.7700    0.0636
    5.7800    0.0619
    5.7900    0.0601
    5.8000    0.0587
    5.8100    0.0572
    5.8200    0.0556
    5.8300    0.0543
    5.8400    0.0528
    5.8500    0.0511
    5.8600    0.0494
    5.8700    0.0479
    5.8800    0.0464
    5.8900    0.0448
    5.9000    0.0430
    5.9100    0.0414
    5.9200    0.0398
    5.9300    0.0382
    5.9400    0.0367
    5.9500    0.0350
    5.9600    0.0335
    5.9700    0.0319
    5.9800    0.0302
    5.9900    0.0288
    6.0000    0.0272
    6.0100    0.0256
    6.0200    0.0242
    6.0300    0.0226
    6.0400    0.0210
    6.0500    0.0196
    6.0600    0.0180
    6.0700    0.0165
    6.0800    0.0151
    6.0900    0.0137
    6.1000    0.0122
    6.1100    0.0106
    6.1200    0.0090
    6.1300    0.0074
    6.1400    0.0059
    6.1500    0.0046
    6.1600    0.0031
    6.1700    0.0016
    6.1800   -0.0001
    6.1900   -0.0019
    6.2000   -0.0035
    6.2100   -0.0048
    6.2200   -0.0060
    6.2300   -0.0075
    6.2400   -0.0090
    6.2500   -0.0106
    6.2600   -0.0120
    6.2700   -0.0135
    6.2800   -0.0149
    6.2900   -0.0163
    6.3000   -0.0180
    6.3100   -0.0195
    6.3200   -0.0212
    6.3300   -0.0228
    6.3400   -0.0242
    6.3500   -0.0257
    6.3600   -0.0271
    6.3700   -0.0284
    6.3800   -0.0298
    6.3900   -0.0312
    6.4000   -0.0328
    6.4100   -0.0342
    6.4200   -0.0357
    6.4300   -0.0374
    6.4400   -0.0389
    6.4500   -0.0404
    6.4600   -0.0417
    6.4700   -0.0429
    6.4800   -0.0444
    6.4900   -0.0459
    6.5000   -0.0473
    6.5100   -0.0484
    6.5200   -0.0496
    6.5300   -0.0511
    6.5400   -0.0527
    6.5500   -0.0541
    6.5600   -0.0554
    6.5700   -0.0567
    6.5800   -0.0581
    6.5900   -0.0596
    6.6000   -0.0610
    6.6100   -0.0623
    6.6200   -0.0636
    6.6300   -0.0651
    6.6400   -0.0665
    6.6500   -0.0678
    6.6600   -0.0690
    6.6700   -0.0704
    6.6800   -0.0718
    6.6900   -0.0733
    6.7000   -0.0746
    6.7100   -0.0758
    6.7200   -0.0772
    6.7300   -0.0788
    6.7400   -0.0801
    6.7500   -0.0813
    6.7600   -0.0824
    6.7700   -0.0838
    6.7800   -0.0852
    6.7900   -0.0864
    6.8000   -0.0875
    6.8100   -0.0887
    6.8200   -0.0898
    6.8300   -0.0909
    6.8400   -0.0921
    6.8500   -0.0932
    6.8600   -0.0942
    6.8700   -0.0953
    6.8800   -0.0965
    6.8900   -0.0973
    6.9000   -0.0983
    6.9100   -0.0995
    6.9200   -0.1005
    6.9300   -0.1017
    6.9400   -0.1028
    6.9500   -0.1039
    6.9600   -0.1047
    6.9700   -0.1056
    6.9800   -0.1066
    6.9900   -0.1076
    7.0000   -0.1085
    7.0100   -0.1092
    7.0200   -0.1102
    7.0300   -0.1111
    7.0400   -0.1121
    7.0500   -0.1129
    7.0600   -0.1138
    7.0700   -0.1148
    7.0800   -0.1158
    7.0900   -0.1165
    7.1000   -0.1174
    7.1100   -0.1184
    7.1200   -0.1192
    7.1300   -0.1201
    7.1400   -0.1211
    7.1500   -0.1217
    7.1600   -0.1225
    7.1700   -0.1233
    7.1800   -0.1242
    7.1900   -0.1249
    7.2000   -0.1256
    7.2100   -0.1262
    7.2200   -0.1269
    7.2300   -0.1276
    7.2400   -0.1281
    7.2500   -0.1289
    7.2600   -0.1297
    7.2700   -0.1303
    7.2800   -0.1309
    7.2900   -0.1315
    7.3000   -0.1321
    7.3100   -0.1325
    7.3200   -0.1330
    7.3300   -0.1339
    7.3400   -0.1345
    7.3500   -0.1350
    7.3600   -0.1355
    7.3700   -0.1359
    7.3800   -0.1364
    7.3900   -0.1370
    7.4000   -0.1374
    7.4100   -0.1379
    7.4200   -0.1384
    7.4300   -0.1390
    7.4400   -0.1396
    7.4500   -0.1400
    7.4600   -0.1406
    7.4700   -0.1410
    7.4800   -0.1414
    7.4900   -0.1419
    7.5000   -0.1424
    7.5100   -0.1430
    7.5200   -0.1434
    7.5300   -0.1436
    7.5400   -0.1437
    7.5500   -0.1440
    7.5600   -0.1443
    7.5700   -0.1445
    7.5800   -0.1445
    7.5900   -0.1446
    7.6000   -0.1447
    7.6100   -0.1448
    7.6200   -0.1449
    7.6300   -0.1449
    7.6400   -0.1449
    7.6500   -0.1450
    7.6600   -0.1448
    7.6700   -0.1448
    7.6800   -0.1449
    7.6900   -0.1450
    7.7000   -0.1450
    7.7100   -0.1450
    7.7200   -0.1450
    7.7300   -0.1450
    7.7400   -0.1448
    7.7500   -0.1447
    7.7600   -0.1447
    7.7700   -0.1448
    7.7800   -0.1449
    7.7900   -0.1450
    7.8000   -0.1451
    7.8100   -0.1451
    7.8200   -0.1451
    7.8300   -0.1449
    7.8400   -0.1444
    7.8500   -0.1444
    7.8600   -0.1444
    7.8700   -0.1442
    7.8800   -0.1441
    7.8900   -0.1440
    7.9000   -0.1437
    7.9100   -0.1433
    7.9200   -0.1430
    7.9300   -0.1427
    7.9400   -0.1425
    7.9500   -0.1423
    7.9600   -0.1419
    7.9700   -0.1415
    7.9800   -0.1411
    7.9900   -0.1405
    8.0000   -0.1399
    8.0100   -0.1394
    8.0200   -0.1389
    8.0300   -0.1386
    8.0400   -0.1382
    8.0500   -0.1376
    8.0600   -0.1370
    8.0700   -0.1365
    8.0800   -0.1360
    8.0900   -0.1353
    8.1000   -0.1348
    8.1100   -0.1343
    8.1200   -0.1336
    8.1300   -0.1330
    8.1400   -0.1324
    8.1500   -0.1317
    8.1600   -0.1311
    8.1700   -0.1305
    8.1800   -0.1298
    8.1900   -0.1291
    8.2000   -0.1283
    8.2100   -0.1277
    8.2200   -0.1271
    8.2300   -0.1267
    8.2400   -0.1261
    8.2500   -0.1253
    8.2600   -0.1246
    8.2700   -0.1237
    8.2800   -0.1228
    8.2900   -0.1220
    8.3000   -0.1212
    8.3100   -0.1205
    8.3200   -0.1195
    8.3300   -0.1187
    8.3400   -0.1179
    8.3500   -0.1169
    8.3600   -0.1160
    8.3700   -0.1152
    8.3800   -0.1141
    8.3900   -0.1131
    8.4000   -0.1123
    8.4100   -0.1114
    8.4200   -0.1103
    8.4300   -0.1092
    8.4400   -0.1081
    8.4500   -0.1071
    8.4600   -0.1061
    8.4700   -0.1050
    8.4800   -0.1041
    8.4900   -0.1032
    8.5000   -0.1021
    8.5100   -0.1009
    8.5200   -0.0998
    8.5300   -0.0984
    8.5400   -0.0973
    8.5500   -0.0963
    8.5600   -0.0951
    8.5700   -0.0939
    8.5800   -0.0926
    8.5900   -0.0913
    8.6000   -0.0902
    8.6100   -0.0892
    8.6200   -0.0880
    8.6300   -0.0866
    8.6400   -0.0851
    8.6500   -0.0838
    8.6600   -0.0824
    8.6700   -0.0813
    8.6800   -0.0801
    8.6900   -0.0790
    8.7000   -0.0778
    8.7100   -0.0765
    8.7200   -0.0755
    8.7300   -0.0744
    8.7400   -0.0732
    8.7500   -0.0723
    8.7600   -0.0712
    8.7700   -0.0700
    8.7800   -0.0690
    8.7900   -0.0678
    8.8000   -0.0666
    8.8100   -0.0654
    8.8200   -0.0641
    8.8300   -0.0629
    8.8400   -0.0618
    8.8500   -0.0607
    8.8600   -0.0596
    8.8700   -0.0582
    8.8800   -0.0569
    8.8900   -0.0556
    8.9000   -0.0541
    8.9100   -0.0527
    8.9200   -0.0512
    8.9300   -0.0498
    8.9400   -0.0486
    8.9500   -0.0473
    8.9600   -0.0460
    8.9700   -0.0446
    8.9800   -0.0430
    8.9900   -0.0415
    9.0000   -0.0402
    9.0100   -0.0388
    9.0200   -0.0375
    9.0300   -0.0362
    9.0400   -0.0348
    9.0500   -0.0335
    9.0600   -0.0320
    9.0700   -0.0305
    9.0800   -0.0290
    9.0900   -0.0276
    9.1000   -0.0263
    9.1100   -0.0250
    9.1200   -0.0237
    9.1300   -0.0222
    9.1400   -0.0207
    9.1500   -0.0192
    9.1600   -0.0177
    9.1700   -0.0163
    9.1800   -0.0150
    9.1900   -0.0138
    9.2000   -0.0126
    9.2100   -0.0114
    9.2200   -0.0100
    9.2300   -0.0085
    9.2400   -0.0070
    9.2500   -0.0056
    9.2600   -0.0043
    9.2700   -0.0028
    9.2800   -0.0011
    9.2900    0.0003
    9.3000    0.0016
    9.3100    0.0029
    9.3200    0.0042
    9.3300    0.0057
    9.3400    0.0072
    9.3500    0.0085
    9.3600    0.0098
    9.3700    0.0111
    9.3800    0.0124
    9.3900    0.0138
    9.4000    0.0153
    9.4100    0.0166
    9.4200    0.0180
    9.4300    0.0195
    9.4400    0.0210
    9.4500    0.0221
    9.4600    0.0233
    9.4700    0.0245
    9.4800    0.0257
    9.4900    0.0271
    9.5000    0.0283
    9.5100    0.0295
    9.5200    0.0309
    9.5300    0.0323
    9.5400    0.0337
    9.5500    0.0349
    9.5600    0.0362
    9.5700    0.0375
    9.5800    0.0387
    9.5900    0.0401
    9.6000    0.0414
    9.6100    0.0428
    9.6200    0.0442
    9.6300    0.0457
    9.6400    0.0471
    9.6500    0.0485
    9.6600    0.0497
    9.6700    0.0509
    9.6800    0.0523
    9.6900    0.0535
    9.7000    0.0548
    9.7100    0.0562
    9.7200    0.0576
    9.7300    0.0590
    9.7400    0.0603
    9.7500    0.0615
    9.7600    0.0626
    9.7700    0.0637
    9.7800    0.0649
    9.7900    0.0662
    9.8000    0.0674
    9.8100    0.0684
    9.8200    0.0698
    9.8300    0.0712
    9.8400    0.0724
    9.8500    0.0738
    9.8600    0.0749
    9.8700    0.0759
    9.8800    0.0770
    9.8900    0.0781
    9.9000    0.0794
    9.9100    0.0804
    9.9200    0.0815
    9.9300    0.0828
    9.9400    0.0838
    9.9500    0.0848
    9.9600    0.0858
    9.9700    0.0869
    9.9800    0.0880
    9.9900    0.0891
   10.0000    0.0902
    };

==> Data/Oscillator/sigma01/x_tr_pos.tex <==
    \addplot[
    thick,
    red
    ]
    table {
         0    0.7884
    0.0100    0.7871
    0.0200    0.7858
    0.0300    0.7843
    0.0400    0.7828
    0.0500    0.7812
    0.0600    0.7795
    0.0700    0.7777
    0.0800    0.7759
    0.0900    0.7740
    0.1000    0.7722
    0.1100    0.7702
    0.1200    0.7682
    0.1300    0.7662
    0.1400    0.7641
    0.1500    0.7619
    0.1600    0.7597
    0.1700    0.7574
    0.1800    0.7550
    0.1900    0.7526
    0.2000    0.7502
    0.2100    0.7477
    0.2200    0.7451
    0.2300    0.7424
    0.2400    0.7397
    0.2500    0.7370
    0.2600    0.7342
    0.2700    0.7313
    0.2800    0.7284
    0.2900    0.7254
    0.3000    0.7223
    0.3100    0.7192
    0.3200    0.7160
    0.3300    0.7126
    0.3400    0.7092
    0.3500    0.7057
    0.3600    0.7021
    0.3700    0.6985
    0.3800    0.6948
    0.3900    0.6910
    0.4000    0.6872
    0.4100    0.6833
    0.4200    0.6793
    0.4300    0.6752
    0.4400    0.6711
    0.4500    0.6670
    0.4600    0.6627
    0.4700    0.6584
    0.4800    0.6540
    0.4900    0.6496
    0.5000    0.6452
    0.5100    0.6407
    0.5200    0.6361
    0.5300    0.6315
    0.5400    0.6267
    0.5500    0.6219
    0.5600    0.6171
    0.5700    0.6122
    0.5800    0.6073
    0.5900    0.6023
    0.6000    0.5972
    0.6100    0.5921
    0.6200    0.5870
    0.6300    0.5818
    0.6400    0.5765
    0.6500    0.5713
    0.6600    0.5660
    0.6700    0.5606
    0.6800    0.5551
    0.6900    0.5496
    0.7000    0.5441
    0.7100    0.5385
    0.7200    0.5329
    0.7300    0.5272
    0.7400    0.5215
    0.7500    0.5157
    0.7600    0.5099
    0.7700    0.5040
    0.7800    0.4980
    0.7900    0.4920
    0.8000    0.4860
    0.8100    0.4799
    0.8200    0.4738
    0.8300    0.4677
    0.8400    0.4616
    0.8500    0.4554
    0.8600    0.4492
    0.8700    0.4429
    0.8800    0.4367
    0.8900    0.4303
    0.9000    0.4240
    0.9100    0.4175
    0.9200    0.4111
    0.9300    0.4046
    0.9400    0.3981
    0.9500    0.3916
    0.9600    0.3851
    0.9700    0.3785
    0.9800    0.3718
    0.9900    0.3652
    1.0000    0.3584
    1.0100    0.3516
    1.0200    0.3448
    1.0300    0.3380
    1.0400    0.3311
    1.0500    0.3242
    1.0600    0.3173
    1.0700    0.3103
    1.0800    0.3033
    1.0900    0.2964
    1.1000    0.2894
    1.1100    0.2824
    1.1200    0.2753
    1.1300    0.2682
    1.1400    0.2611
    1.1500    0.2540
    1.1600    0.2469
    1.1700    0.2397
    1.1800    0.2326
    1.1900    0.2254
    1.2000    0.2181
    1.2100    0.2110
    1.2200    0.2038
    1.2300    0.1966
    1.2400    0.1894
    1.2500    0.1822
    1.2600    0.1749
    1.2700    0.1677
    1.2800    0.1605
    1.2900    0.1532
    1.3000    0.1459
    1.3100    0.1386
    1.3200    0.1313
    1.3300    0.1239
    1.3400    0.1166
    1.3500    0.1092
    1.3600    0.1018
    1.3700    0.0944
    1.3800    0.0871
    1.3900    0.0797
    1.4000    0.0723
    1.4100    0.0650
    1.4200    0.0576
    1.4300    0.0502
    1.4400    0.0427
    1.4500    0.0353
    1.4600    0.0278
    1.4700    0.0204
    1.4800    0.0129
    1.4900    0.0054
    1.5000   -0.0021
    1.5100   -0.0096
    1.5200   -0.0171
    1.5300   -0.0245
    1.5400   -0.0320
    1.5500   -0.0394
    1.5600   -0.0468
    1.5700   -0.0543
    1.5800   -0.0617
    1.5900   -0.0690
    1.6000   -0.0764
    1.6100   -0.0838
    1.6200   -0.0911
    1.6300   -0.0985
    1.6400   -0.1058
    1.6500   -0.1131
    1.6600   -0.1203
    1.6700   -0.1275
    1.6800   -0.1348
    1.6900   -0.1420
    1.7000   -0.1492
    1.7100   -0.1563
    1.7200   -0.1636
    1.7300   -0.1708
    1.7400   -0.1780
    1.7500   -0.1851
    1.7600   -0.1922
    1.7700   -0.1993
    1.7800   -0.2064
    1.7900   -0.2134
    1.8000   -0.2205
    1.8100   -0.2274
    1.8200   -0.2344
    1.8300   -0.2414
    1.8400   -0.2483
    1.8500   -0.2552
    1.8600   -0.2620
    1.8700   -0.2688
    1.8800   -0.2756
    1.8900   -0.2823
    1.9000   -0.2890
    1.9100   -0.2956
    1.9200   -0.3022
    1.9300   -0.3088
    1.9400   -0.3154
    1.9500   -0.3219
    1.9600   -0.3283
    1.9700   -0.3347
    1.9800   -0.3410
    1.9900   -0.3473
    2.0000   -0.3535
    2.0100   -0.3597
    2.0200   -0.3659
    2.0300   -0.3720
    2.0400   -0.3781
    2.0500   -0.3841
    2.0600   -0.3900
    2.0700   -0.3959
    2.0800   -0.4018
    2.0900   -0.4076
    2.1000   -0.4134
    2.1100   -0.4192
    2.1200   -0.4249
    2.1300   -0.4305
    2.1400   -0.4361
    2.1500   -0.4417
    2.1600   -0.4472
    2.1700   -0.4527
    2.1800   -0.4582
    2.1900   -0.4636
    2.2000   -0.4689
    2.2100   -0.4742
    2.2200   -0.4794
    2.2300   -0.4845
    2.2400   -0.4896
    2.2500   -0.4947
    2.2600   -0.4997
    2.2700   -0.5046
    2.2800   -0.5095
    2.2900   -0.5144
    2.3000   -0.5192
    2.3100   -0.5239
    2.3200   -0.5286
    2.3300   -0.5332
    2.3400   -0.5379
    2.3500   -0.5424
    2.3600   -0.5469
    2.3700   -0.5514
    2.3800   -0.5559
    2.3900   -0.5603
    2.4000   -0.5646
    2.4100   -0.5689
    2.4200   -0.5731
    2.4300   -0.5772
    2.4400   -0.5813
    2.4500   -0.5853
    2.4600   -0.5893
    2.4700   -0.5932
    2.4800   -0.5970
    2.4900   -0.6008
    2.5000   -0.6045
    2.5100   -0.6081
    2.5200   -0.6117
    2.5300   -0.6152
    2.5400   -0.6187
    2.5500   -0.6220
    2.5600   -0.6253
    2.5700   -0.6286
    2.5800   -0.6317
    2.5900   -0.6348
    2.6000   -0.6378
    2.6100   -0.6408
    2.6200   -0.6436
    2.6300   -0.6465
    2.6400   -0.6492
    2.6500   -0.6519
    2.6600   -0.6546
    2.6700   -0.6572
    2.6800   -0.6597
    2.6900   -0.6622
    2.7000   -0.6646
    2.7100   -0.6669
    2.7200   -0.6691
    2.7300   -0.6712
    2.7400   -0.6733
    2.7500   -0.6753
    2.7600   -0.6772
    2.7700   -0.6791
    2.7800   -0.6810
    2.7900   -0.6827
    2.8000   -0.6844
    2.8100   -0.6860
    2.8200   -0.6875
    2.8300   -0.6889
    2.8400   -0.6902
    2.8500   -0.6915
    2.8600   -0.6926
    2.8700   -0.6937
    2.8800   -0.6948
    2.8900   -0.6958
    2.9000   -0.6967
    2.9100   -0.6975
    2.9200   -0.6983
    2.9300   -0.6991
    2.9400   -0.6997
    2.9500   -0.7003
    2.9600   -0.7008
    2.9700   -0.7013
    2.9800   -0.7017
    2.9900   -0.7021
    3.0000   -0.7024
    3.0100   -0.7027
    3.0200   -0.7029
    3.0300   -0.7031
    3.0400   -0.7032
    3.0500   -0.7032
    3.0600   -0.7031
    3.0700   -0.7029
    3.0800   -0.7027
    3.0900   -0.7024
    3.1000   -0.7020
    3.1100   -0.7015
    3.1200   -0.7010
    3.1300   -0.7004
    3.1400   -0.6997
    3.1500   -0.6989
    3.1600   -0.6981
    3.1700   -0.6973
    3.1800   -0.6964
    3.1900   -0.6954
    3.2000   -0.6944
    3.2100   -0.6933
    3.2200   -0.6921
    3.2300   -0.6909
    3.2400   -0.6896
    3.2500   -0.6882
    3.2600   -0.6868
    3.2700   -0.6853
    3.2800   -0.6837
    3.2900   -0.6822
    3.3000   -0.6805
    3.3100   -0.6788
    3.3200   -0.6770
    3.3300   -0.6752
    3.3400   -0.6734
    3.3500   -0.6714
    3.3600   -0.6695
    3.3700   -0.6674
    3.3800   -0.6652
    3.3900   -0.6630
    3.4000   -0.6608
    3.4100   -0.6585
    3.4200   -0.6561
    3.4300   -0.6537
    3.4400   -0.6512
    3.4500   -0.6487
    3.4600   -0.6460
    3.4700   -0.6433
    3.4800   -0.6406
    3.4900   -0.6377
    3.5000   -0.6348
    3.5100   -0.6319
    3.5200   -0.6288
    3.5300   -0.6257
    3.5400   -0.6226
    3.5500   -0.6194
    3.5600   -0.6161
    3.5700   -0.6128
    3.5800   -0.6094
    3.5900   -0.6060
    3.6000   -0.6025
    3.6100   -0.5989
    3.6200   -0.5953
    3.6300   -0.5917
    3.6400   -0.5880
    3.6500   -0.5842
    3.6600   -0.5803
    3.6700   -0.5764
    3.6800   -0.5725
    3.6900   -0.5685
    3.7000   -0.5645
    3.7100   -0.5605
    3.7200   -0.5564
    3.7300   -0.5522
    3.7400   -0.5480
    3.7500   -0.5438
    3.7600   -0.5395
    3.7700   -0.5352
    3.7800   -0.5309
    3.7900   -0.5265
    3.8000   -0.5220
    3.8100   -0.5175
    3.8200   -0.5129
    3.8300   -0.5082
    3.8400   -0.5035
    3.8500   -0.4987
    3.8600   -0.4939
    3.8700   -0.4890
    3.8800   -0.4841
    3.8900   -0.4791
    3.9000   -0.4741
    3.9100   -0.4690
    3.9200   -0.4639
    3.9300   -0.4588
    3.9400   -0.4537
    3.9500   -0.4485
    3.9600   -0.4433
    3.9700   -0.4381
    3.9800   -0.4329
    3.9900   -0.4276
    4.0000   -0.4223
    4.0100   -0.4169
    4.0200   -0.4115
    4.0300   -0.4061
    4.0400   -0.4006
    4.0500   -0.3952
    4.0600   -0.3896
    4.0700   -0.3841
    4.0800   -0.3785
    4.0900   -0.3729
    4.1000   -0.3672
    4.1100   -0.3614
    4.1200   -0.3557
    4.1300   -0.3499
    4.1400   -0.3441
    4.1500   -0.3382
    4.1600   -0.3324
    4.1700   -0.3265
    4.1800   -0.3206
    4.1900   -0.3147
    4.2000   -0.3087
    4.2100   -0.3028
    4.2200   -0.2969
    4.2300   -0.2909
    4.2400   -0.2849
    4.2500   -0.2788
    4.2600   -0.2728
    4.2700   -0.2666
    4.2800   -0.2605
    4.2900   -0.2543
    4.3000   -0.2481
    4.3100   -0.2418
    4.3200   -0.2355
    4.3300   -0.2293
    4.3400   -0.2229
    4.3500   -0.2167
    4.3600   -0.2104
    4.3700   -0.2041
    4.3800   -0.1978
    4.3900   -0.1915
    4.4000   -0.1852
    4.4100   -0.1788
    4.4200   -0.1725
    4.4300   -0.1661
    4.4400   -0.1597
    4.4500   -0.1533
    4.4600   -0.1469
    4.4700   -0.1404
    4.4800   -0.1340
    4.4900   -0.1275
    4.5000   -0.1210
    4.5100   -0.1145
    4.5200   -0.1080
    4.5300   -0.1016
    4.5400   -0.0951
    4.5500   -0.0887
    4.5600   -0.0822
    4.5700   -0.0758
    4.5800   -0.0694
    4.5900   -0.0630
    4.6000   -0.0565
    4.6100   -0.0501
    4.6200   -0.0437
    4.6300   -0.0372
    4.6400   -0.0308
    4.6500   -0.0244
    4.6600   -0.0180
    4.6700   -0.0117
    4.6800   -0.0053
    4.6900    0.0011
    4.7000    0.0074
    4.7100    0.0138
    4.7200    0.0202
    4.7300    0.0265
    4.7400    0.0329
    4.7500    0.0393
    4.7600    0.0457
    4.7700    0.0520
    4.7800    0.0583
    4.7900    0.0647
    4.8000    0.0710
    4.8100    0.0772
    4.8200    0.0835
    4.8300    0.0898
    4.8400    0.0960
    4.8500    0.1023
    4.8600    0.1085
    4.8700    0.1147
    4.8800    0.1209
    4.8900    0.1271
    4.9000    0.1333
    4.9100    0.1394
    4.9200    0.1455
    4.9300    0.1517
    4.9400    0.1578
    4.9500    0.1639
    4.9600    0.1700
    4.9700    0.1760
    4.9800    0.1820
    4.9900    0.1880
    5.0000    0.1939
    5.0100    0.1999
    5.0200    0.2058
    5.0300    0.2118
    5.0400    0.2176
    5.0500    0.2235
    5.0600    0.2294
    5.0700    0.2352
    5.0800    0.2410
    5.0900    0.2468
    5.1000    0.2526
    5.1100    0.2583
    5.1200    0.2639
    5.1300    0.2695
    5.1400    0.2750
    5.1500    0.2805
    5.1600    0.2860
    5.1700    0.2914
    5.1800    0.2969
    5.1900    0.3023
    5.2000    0.3077
    5.2100    0.3131
    5.2200    0.3184
    5.2300    0.3237
    5.2400    0.3289
    5.2500    0.3340
    5.2600    0.3391
    5.2700    0.3442
    5.2800    0.3493
    5.2900    0.3543
    5.3000    0.3593
    5.3100    0.3643
    5.3200    0.3692
    5.3300    0.3741
    5.3400    0.3789
    5.3500    0.3836
    5.3600    0.3883
    5.3700    0.3929
    5.3800    0.3975
    5.3900    0.4021
    5.4000    0.4066
    5.4100    0.4111
    5.4200    0.4155
    5.4300    0.4199
    5.4400    0.4243
    5.4500    0.4286
    5.4600    0.4329
    5.4700    0.4371
    5.4800    0.4413
    5.4900    0.4454
    5.5000    0.4494
    5.5100    0.4534
    5.5200    0.4573
    5.5300    0.4612
    5.5400    0.4651
    5.5500    0.4689
    5.5600    0.4727
    5.5700    0.4764
    5.5800    0.4801
    5.5900    0.4837
    5.6000    0.4873
    5.6100    0.4908
    5.6200    0.4943
    5.6300    0.4977
    5.6400    0.5011
    5.6500    0.5045
    5.6600    0.5078
    5.6700    0.5111
    5.6800    0.5143
    5.6900    0.5175
    5.7000    0.5206
    5.7100    0.5237
    5.7200    0.5267
    5.7300    0.5297
    5.7400    0.5327
    5.7500    0.5356
    5.7600    0.5384
    5.7700    0.5412
    5.7800    0.5439
    5.7900    0.5465
    5.8000    0.5491
    5.8100    0.5516
    5.8200    0.5541
    5.8300    0.5565
    5.8400    0.5588
    5.8500    0.5610
    5.8600    0.5632
    5.8700    0.5653
    5.8800    0.5674
    5.8900    0.5693
    5.9000    0.5712
    5.9100    0.5731
    5.9200    0.5749
    5.9300    0.5766
    5.9400    0.5782
    5.9500    0.5799
    5.9600    0.5814
    5.9700    0.5830
    5.9800    0.5844
    5.9900    0.5859
    6.0000    0.5873
    6.0100    0.5886
    6.0200    0.5899
    6.0300    0.5912
    6.0400    0.5924
    6.0500    0.5935
    6.0600    0.5946
    6.0700    0.5957
    6.0800    0.5967
    6.0900    0.5976
    6.1000    0.5986
    6.1100    0.5994
    6.1200    0.6002
    6.1300    0.6010
    6.1400    0.6017
    6.1500    0.6023
    6.1600    0.6028
    6.1700    0.6034
    6.1800    0.6038
    6.1900    0.6042
    6.2000    0.6046
    6.2100    0.6050
    6.2200    0.6053
    6.2300    0.6055
    6.2400    0.6057
    6.2500    0.6058
    6.2600    0.6059
    6.2700    0.6059
    6.2800    0.6058
    6.2900    0.6057
    6.3000    0.6055
    6.3100    0.6053
    6.3200    0.6050
    6.3300    0.6046
    6.3400    0.6042
    6.3500    0.6037
    6.3600    0.6031
    6.3700    0.6025
    6.3800    0.6017
    6.3900    0.6009
    6.4000    0.5999
    6.4100    0.5989
    6.4200    0.5978
    6.4300    0.5966
    6.4400    0.5954
    6.4500    0.5941
    6.4600    0.5927
    6.4700    0.5912
    6.4800    0.5897
    6.4900    0.5882
    6.5000    0.5865
    6.5100    0.5848
    6.5200    0.5831
    6.5300    0.5813
    6.5400    0.5795
    6.5500    0.5776
    6.5600    0.5756
    6.5700    0.5736
    6.5800    0.5715
    6.5900    0.5694
    6.6000    0.5672
    6.6100    0.5649
    6.6200    0.5626
    6.6300    0.5602
    6.6400    0.5577
    6.6500    0.5552
    6.6600    0.5526
    6.6700    0.5499
    6.6800    0.5472
    6.6900    0.5445
    6.7000    0.5417
    6.7100    0.5389
    6.7200    0.5360
    6.7300    0.5331
    6.7400    0.5302
    6.7500    0.5272
    6.7600    0.5243
    6.7700    0.5213
    6.7800    0.5182
    6.7900    0.5151
    6.8000    0.5120
    6.8100    0.5087
    6.8200    0.5054
    6.8300    0.5021
    6.8400    0.4987
    6.8500    0.4953
    6.8600    0.4918
    6.8700    0.4882
    6.8800    0.4846
    6.8900    0.4809
    6.9000    0.4772
    6.9100    0.4735
    6.9200    0.4697
    6.9300    0.4659
    6.9400    0.4621
    6.9500    0.4582
    6.9600    0.4542
    6.9700    0.4502
    6.9800    0.4461
    6.9900    0.4420
    7.0000    0.4378
    7.0100    0.4337
    7.0200    0.4295
    7.0300    0.4253
    7.0400    0.4210
    7.0500    0.4167
    7.0600    0.4124
    7.0700    0.4081
    7.0800    0.4037
    7.0900    0.3992
    7.1000    0.3947
    7.1100    0.3901
    7.1200    0.3854
    7.1300    0.3808
    7.1400    0.3760
    7.1500    0.3713
    7.1600    0.3665
    7.1700    0.3617
    7.1800    0.3568
    7.1900    0.3519
    7.2000    0.3470
    7.2100    0.3421
    7.2200    0.3372
    7.2300    0.3322
    7.2400    0.3272
    7.2500    0.3221
    7.2600    0.3171
    7.2700    0.3119
    7.2800    0.3068
    7.2900    0.3016
    7.3000    0.2964
    7.3100    0.2911
    7.3200    0.2858
    7.3300    0.2805
    7.3400    0.2751
    7.3500    0.2696
    7.3600    0.2641
    7.3700    0.2585
    7.3800    0.2529
    7.3900    0.2473
    7.4000    0.2417
    7.4100    0.2361
    7.4200    0.2304
    7.4300    0.2247
    7.4400    0.2190
    7.4500    0.2132
    7.4600    0.2075
    7.4700    0.2017
    7.4800    0.1959
    7.4900    0.1900
    7.5000    0.1842
    7.5100    0.1783
    7.5200    0.1725
    7.5300    0.1667
    7.5400    0.1608
    7.5500    0.1550
    7.5600    0.1491
    7.5700    0.1432
    7.5800    0.1374
    7.5900    0.1314
    7.6000    0.1255
    7.6100    0.1195
    7.6200    0.1136
    7.6300    0.1076
    7.6400    0.1017
    7.6500    0.0957
    7.6600    0.0898
    7.6700    0.0839
    7.6800    0.0780
    7.6900    0.0721
    7.7000    0.0661
    7.7100    0.0602
    7.7200    0.0542
    7.7300    0.0483
    7.7400    0.0423
    7.7500    0.0364
    7.7600    0.0304
    7.7700    0.0244
    7.7800    0.0184
    7.7900    0.0125
    7.8000    0.0065
    7.8100    0.0006
    7.8200   -0.0053
    7.8300   -0.0112
    7.8400   -0.0171
    7.8500   -0.0231
    7.8600   -0.0289
    7.8700   -0.0348
    7.8800   -0.0406
    7.8900   -0.0464
    7.9000   -0.0523
    7.9100   -0.0581
    7.9200   -0.0639
    7.9300   -0.0697
    7.9400   -0.0755
    7.9500   -0.0813
    7.9600   -0.0870
    7.9700   -0.0928
    7.9800   -0.0985
    7.9900   -0.1042
    8.0000   -0.1098
    8.0100   -0.1154
    8.0200   -0.1210
    8.0300   -0.1266
    8.0400   -0.1322
    8.0500   -0.1378
    8.0600   -0.1433
    8.0700   -0.1489
    8.0800   -0.1544
    8.0900   -0.1598
    8.1000   -0.1653
    8.1100   -0.1708
    8.1200   -0.1762
    8.1300   -0.1817
    8.1400   -0.1871
    8.1500   -0.1925
    8.1600   -0.1979
    8.1700   -0.2032
    8.1800   -0.2086
    8.1900   -0.2139
    8.2000   -0.2192
    8.2100   -0.2244
    8.2200   -0.2297
    8.2300   -0.2349
    8.2400   -0.2402
    8.2500   -0.2454
    8.2600   -0.2506
    8.2700   -0.2558
    8.2800   -0.2610
    8.2900   -0.2661
    8.3000   -0.2712
    8.3100   -0.2762
    8.3200   -0.2812
    8.3300   -0.2862
    8.3400   -0.2911
    8.3500   -0.2960
    8.3600   -0.3009
    8.3700   -0.3057
    8.3800   -0.3105
    8.3900   -0.3152
    8.4000   -0.3200
    8.4100   -0.3247
    8.4200   -0.3294
    8.4300   -0.3340
    8.4400   -0.3386
    8.4500   -0.3432
    8.4600   -0.3477
    8.4700   -0.3523
    8.4800   -0.3568
    8.4900   -0.3613
    8.5000   -0.3657
    8.5100   -0.3701
    8.5200   -0.3745
    8.5300   -0.3789
    8.5400   -0.3831
    8.5500   -0.3874
    8.5600   -0.3916
    8.5700   -0.3959
    8.5800   -0.4001
    8.5900   -0.4042
    8.6000   -0.4083
    8.6100   -0.4123
    8.6200   -0.4163
    8.6300   -0.4203
    8.6400   -0.4242
    8.6500   -0.4282
    8.6600   -0.4321
    8.6700   -0.4359
    8.6800   -0.4398
    8.6900   -0.4436
    8.7000   -0.4473
    8.7100   -0.4511
    8.7200   -0.4547
    8.7300   -0.4583
    8.7400   -0.4619
    8.7500   -0.4654
    8.7600   -0.4688
    8.7700   -0.4723
    8.7800   -0.4757
    8.7900   -0.4791
    8.8000   -0.4824
    8.8100   -0.4856
    8.8200   -0.4888
    8.8300   -0.4919
    8.8400   -0.4950
    8.8500   -0.4980
    8.8600   -0.5010
    8.8700   -0.5040
    8.8800   -0.5069
    8.8900   -0.5097
    8.9000   -0.5126
    8.9100   -0.5153
    8.9200   -0.5180
    8.9300   -0.5206
    8.9400   -0.5232
    8.9500   -0.5257
    8.9600   -0.5282
    8.9700   -0.5307
    8.9800   -0.5331
    8.9900   -0.5354
    9.0000   -0.5376
    9.0100   -0.5399
    9.0200   -0.5420
    9.0300   -0.5441
    9.0400   -0.5461
    9.0500   -0.5481
    9.0600   -0.5500
    9.0700   -0.5519
    9.0800   -0.5537
    9.0900   -0.5555
    9.1000   -0.5573
    9.1100   -0.5589
    9.1200   -0.5605
    9.1300   -0.5621
    9.1400   -0.5636
    9.1500   -0.5651
    9.1600   -0.5665
    9.1700   -0.5679
    9.1800   -0.5693
    9.1900   -0.5706
    9.2000   -0.5718
    9.2100   -0.5729
    9.2200   -0.5739
    9.2300   -0.5749
    9.2400   -0.5759
    9.2500   -0.5767
    9.2600   -0.5775
    9.2700   -0.5782
    9.2800   -0.5789
    9.2900   -0.5795
    9.3000   -0.5800
    9.3100   -0.5805
    9.3200   -0.5810
    9.3300   -0.5814
    9.3400   -0.5817
    9.3500   -0.5820
    9.3600   -0.5822
    9.3700   -0.5824
    9.3800   -0.5824
    9.3900   -0.5825
    9.4000   -0.5824
    9.4100   -0.5823
    9.4200   -0.5821
    9.4300   -0.5819
    9.4400   -0.5816
    9.4500   -0.5812
    9.4600   -0.5808
    9.4700   -0.5803
    9.4800   -0.5798
    9.4900   -0.5793
    9.5000   -0.5786
    9.5100   -0.5780
    9.5200   -0.5772
    9.5300   -0.5765
    9.5400   -0.5756
    9.5500   -0.5747
    9.5600   -0.5738
    9.5700   -0.5727
    9.5800   -0.5716
    9.5900   -0.5704
    9.6000   -0.5691
    9.6100   -0.5678
    9.6200   -0.5665
    9.6300   -0.5650
    9.6400   -0.5635
    9.6500   -0.5620
    9.6600   -0.5604
    9.6700   -0.5588
    9.6800   -0.5570
    9.6900   -0.5552
    9.7000   -0.5534
    9.7100   -0.5515
    9.7200   -0.5496
    9.7300   -0.5476
    9.7400   -0.5455
    9.7500   -0.5433
    9.7600   -0.5411
    9.7700   -0.5389
    9.7800   -0.5366
    9.7900   -0.5341
    9.8000   -0.5316
    9.8100   -0.5291
    9.8200   -0.5265
    9.8300   -0.5239
    9.8400   -0.5211
    9.8500   -0.5183
    9.8600   -0.5155
    9.8700   -0.5126
    9.8800   -0.5096
    9.8900   -0.5066
    9.9000   -0.5036
    9.9100   -0.5006
    9.9200   -0.4975
    9.9300   -0.4944
    9.9400   -0.4913
    9.9500   -0.4880
    9.9600   -0.4847
    9.9700   -0.4814
    9.9800   -0.4780
    9.9900   -0.4745
   10.0000   -0.4710
    };

==> Data/Oscillator/sigma01/x_tr_vel.tex <==
    \addplot[
    thick,
    red
    ]
    table {
         0   -0.1266
    0.0100   -0.1317
    0.0200   -0.1399
    0.0300   -0.1491
    0.0400   -0.1555
    0.0500   -0.1643
    0.0600   -0.1739
    0.0700   -0.1816
    0.0800   -0.1848
    0.0900   -0.1852
    0.1000   -0.1912
    0.1100   -0.1968
    0.1200   -0.2001
    0.1300   -0.2068
    0.1400   -0.2136
    0.1500   -0.2204
    0.1600   -0.2282
    0.1700   -0.2340
    0.1800   -0.2381
    0.1900   -0.2422
    0.2000   -0.2471
    0.2100   -0.2550
    0.2200   -0.2627
    0.2300   -0.2673
    0.2400   -0.2721
    0.2500   -0.2774
    0.2600   -0.2826
    0.2700   -0.2891
    0.2800   -0.2961
    0.2900   -0.3037
    0.3000   -0.3105
    0.3100   -0.3177
    0.3200   -0.3270
    0.3300   -0.3359
    0.3400   -0.3469
    0.3500   -0.3553
    0.3600   -0.3600
    0.3700   -0.3671
    0.3800   -0.3730
    0.3900   -0.3800
    0.4000   -0.3885
    0.4100   -0.3953
    0.4200   -0.4017
    0.4300   -0.4073
    0.4400   -0.4143
    0.4500   -0.4215
    0.4600   -0.4280
    0.4700   -0.4336
    0.4800   -0.4378
    0.4900   -0.4414
    0.5000   -0.4472
    0.5100   -0.4540
    0.5200   -0.4612
    0.5300   -0.4697
    0.5400   -0.4768
    0.5500   -0.4808
    0.5600   -0.4857
    0.5700   -0.4918
    0.5800   -0.4972
    0.5900   -0.5018
    0.6000   -0.5073
    0.6100   -0.5139
    0.6200   -0.5186
    0.6300   -0.5221
    0.6400   -0.5244
    0.6500   -0.5278
    0.6600   -0.5345
    0.6700   -0.5421
    0.6800   -0.5491
    0.6900   -0.5527
    0.7000   -0.5557
    0.7100   -0.5604
    0.7200   -0.5645
    0.7300   -0.5685
    0.7400   -0.5730
    0.7500   -0.5801
    0.7600   -0.5878
    0.7700   -0.5933
    0.7800   -0.5974
    0.7900   -0.6021
    0.8000   -0.6050
    0.8100   -0.6073
    0.8200   -0.6110
    0.8300   -0.6131
    0.8400   -0.6162
    0.8500   -0.6203
    0.8600   -0.6225
    0.8700   -0.6257
    0.8800   -0.6295
    0.8900   -0.6342
    0.9000   -0.6405
    0.9100   -0.6452
    0.9200   -0.6478
    0.9300   -0.6475
    0.9400   -0.6487
    0.9500   -0.6525
    0.9600   -0.6557
    0.9700   -0.6611
    0.9800   -0.6668
    0.9900   -0.6723
    1.0000   -0.6763
    1.0100   -0.6793
    1.0200   -0.6829
    1.0300   -0.6862
    1.0400   -0.6891
    1.0500   -0.6920
    1.0600   -0.6947
    1.0700   -0.6957
    1.0800   -0.6954
    1.0900   -0.6960
    1.1000   -0.7008
    1.1100   -0.7063
    1.1200   -0.7078
    1.1300   -0.7095
    1.1400   -0.7115
    1.1500   -0.7122
    1.1600   -0.7122
    1.1700   -0.7145
    1.1800   -0.7186
    1.1900   -0.7217
    1.2000   -0.7213
    1.2100   -0.7186
    1.2200   -0.7174
    1.2300   -0.7184
    1.2400   -0.7213
    1.2500   -0.7233
    1.2600   -0.7234
    1.2700   -0.7235
    1.2800   -0.7239
    1.2900   -0.7263
    1.3000   -0.7297
    1.3100   -0.7317
    1.3200   -0.7350
    1.3300   -0.7368
    1.3400   -0.7364
    1.3500   -0.7364
    1.3600   -0.7382
    1.3700   -0.7386
    1.3800   -0.7372
    1.3900   -0.7372
    1.4000   -0.7375
    1.4100   -0.7378
    1.4200   -0.7399
    1.4300   -0.7419
    1.4400   -0.7429
    1.4500   -0.7446
    1.4600   -0.7465
    1.4700   -0.7479
    1.4800   -0.7502
    1.4900   -0.7507
    1.5000   -0.7483
    1.5100   -0.7469
    1.5200   -0.7461
    1.5300   -0.7461
    1.5400   -0.7448
    1.5500   -0.7427
    1.5600   -0.7425
    1.5700   -0.7406
    1.5800   -0.7380
    1.5900   -0.7375
    1.6000   -0.7370
    1.6100   -0.7368
    1.6200   -0.7373
    1.6300   -0.7341
    1.6400   -0.7277
    1.6500   -0.7236
    1.6600   -0.7228
    1.6700   -0.7232
    1.6800   -0.7224
    1.6900   -0.7196
    1.7000   -0.7180
    1.7100   -0.7198
    1.7200   -0.7217
    1.7300   -0.7206
    1.7400   -0.7173
    1.7500   -0.7139
    1.7600   -0.7109
    1.7700   -0.7082
    1.7800   -0.7058
    1.7900   -0.7025
    1.8000   -0.7002
    1.8100   -0.6983
    1.8200   -0.6957
    1.8300   -0.6940
    1.8400   -0.6906
    1.8500   -0.6856
    1.8600   -0.6824
    1.8700   -0.6789
    1.8800   -0.6734
    1.8900   -0.6692
    1.9000   -0.6660
    1.9100   -0.6629
    1.9200   -0.6598
    1.9300   -0.6564
    1.9400   -0.6526
    1.9500   -0.6477
    1.9600   -0.6412
    1.9700   -0.6350
    1.9800   -0.6307
    1.9900   -0.6262
    2.0000   -0.6212
    2.0100   -0.6179
    2.0200   -0.6138
    2.0300   -0.6081
    2.0400   -0.6032
    2.0500   -0.5981
    2.0600   -0.5928
    2.0700   -0.5890
    2.0800   -0.5857
    2.0900   -0.5814
    2.1000   -0.5775
    2.1100   -0.5714
    2.1200   -0.5657
    2.1300   -0.5624
    2.1400   -0.5589
    2.1500   -0.5560
    2.1600   -0.5526
    2.1700   -0.5480
    2.1800   -0.5415
    2.1900   -0.5349
    2.2000   -0.5312
    2.2100   -0.5254
    2.2200   -0.5169
    2.2300   -0.5105
    2.2400   -0.5070
    2.2500   -0.5038
    2.2600   -0.4990
    2.2700   -0.4933
    2.2800   -0.4877
    2.2900   -0.4819
    2.3000   -0.4753
    2.3100   -0.4706
    2.3200   -0.4673
    2.3300   -0.4635
    2.3400   -0.4590
    2.3500   -0.4541
    2.3600   -0.4486
    2.3700   -0.4460
    2.3800   -0.4439
    2.3900   -0.4370
    2.4000   -0.4308
    2.4100   -0.4248
    2.4200   -0.4172
    2.4300   -0.4107
    2.4400   -0.4043
    2.4500   -0.3996
    2.4600   -0.3952
    2.4700   -0.3872
    2.4800   -0.3790
    2.4900   -0.3725
    2.5000   -0.3668
    2.5100   -0.3613
    2.5200   -0.3546
    2.5300   -0.3474
    2.5400   -0.3408
    2.5500   -0.3349
    2.5600   -0.3264
    2.5700   -0.3200
    2.5800   -0.3134
    2.5900   -0.3039
    2.6000   -0.2958
    2.6100   -0.2898
    2.6200   -0.2856
    2.6300   -0.2799
    2.6400   -0.2729
    2.6500   -0.2676
    2.6600   -0.2621
    2.6700   -0.2561
    2.6800   -0.2506
    2.6900   -0.2429
    2.7000   -0.2349
    2.7100   -0.2265
    2.7200   -0.2172
    2.7300   -0.2099
    2.7400   -0.2034
    2.7500   -0.1973
    2.7600   -0.1928
    2.7700   -0.1863
    2.7800   -0.1783
    2.7900   -0.1714
    2.8000   -0.1634
    2.8100   -0.1547
    2.8200   -0.1466
    2.8300   -0.1378
    2.8400   -0.1284
    2.8500   -0.1200
    2.8600   -0.1135
    2.8700   -0.1079
    2.8800   -0.1003
    2.8900   -0.0937
    2.9000   -0.0885
    2.9100   -0.0837
    2.9200   -0.0776
    2.9300   -0.0685
    2.9400   -0.0604
    2.9500   -0.0535
    2.9600   -0.0493
    2.9700   -0.0443
    2.9800   -0.0391
    2.9900   -0.0371
    3.0000   -0.0325
    3.0100   -0.0264
    3.0200   -0.0200
    3.0300   -0.0117
    3.0400   -0.0030
    3.0500    0.0042
    3.0600    0.0110
    3.0700    0.0186
    3.0800    0.0267
    3.0900    0.0352
    3.1000    0.0438
    3.1100    0.0516
    3.1200    0.0583
    3.1300    0.0662
    3.1400    0.0718
    3.1500    0.0758
    3.1600    0.0807
    3.1700    0.0858
    3.1800    0.0930
    3.1900    0.1015
    3.2000    0.1081
    3.2100    0.1133
    3.2200    0.1197
    3.2300    0.1263
    3.2400    0.1331
    3.2500    0.1407
    3.2600    0.1468
    3.2700    0.1523
    3.2800    0.1564
    3.2900    0.1620
    3.3000    0.1692
    3.3100    0.1738
    3.3200    0.1787
    3.3300    0.1834
    3.3400    0.1884
    3.3500    0.1943
    3.3600    0.2026
    3.3700    0.2127
    3.3800    0.2177
    3.3900    0.2218
    3.4000    0.2271
    3.4100    0.2317
    3.4200    0.2379
    3.4300    0.2452
    3.4400    0.2520
    3.4500    0.2597
    3.4600    0.2671
    3.4700    0.2731
    3.4800    0.2804
    3.4900    0.2873
    3.5000    0.2945
    3.5100    0.3019
    3.5200    0.3074
    3.5300    0.3104
    3.5400    0.3164
    3.5500    0.3237
    3.5600    0.3290
    3.5700    0.3356
    3.5800    0.3421
    3.5900    0.3469
    3.6000    0.3511
    3.6100    0.3561
    3.6200    0.3632
    3.6300    0.3695
    3.6400    0.3749
    3.6500    0.3816
    3.6600    0.3871
    3.6700    0.3911
    3.6800    0.3949
    3.6900    0.3998
    3.7000    0.4034
    3.7100    0.4072
    3.7200    0.4116
    3.7300    0.4157
    3.7400    0.4211
    3.7500    0.4255
    3.7600    0.4291
    3.7700    0.4341
    3.7800    0.4374
    3.7900    0.4413
    3.8000    0.4500
    3.8100    0.4585
    3.8200    0.4639
    3.8300    0.4687
    3.8400    0.4726
    3.8500    0.4781
    3.8600    0.4857
    3.8700    0.4921
    3.8800    0.4964
    3.8900    0.5001
    3.9000    0.5041
    3.9100    0.5073
    3.9200    0.5104
    3.9300    0.5128
    3.9400    0.5147
    3.9500    0.5174
    3.9600    0.5192
    3.9700    0.5219
    3.9800    0.5263
    3.9900    0.5307
    4.0000    0.5355
    4.0100    0.5400
    4.0200    0.5425
    4.0300    0.5432
    4.0400    0.5451
    4.0500    0.5481
    4.0600    0.5529
    4.0700    0.5572
    4.0800    0.5615
    4.0900    0.5666
    4.1000    0.5716
    4.1100    0.5761
    4.1200    0.5786
    4.1300    0.5791
    4.1400    0.5805
    4.1500    0.5844
    4.1600    0.5878
    4.1700    0.5895
    4.1800    0.5912
    4.1900    0.5923
    4.2000    0.5930
    4.2100    0.5947
    4.2200    0.5970
    4.2300    0.5993
    4.2400    0.6022
    4.2500    0.6052
    4.2600    0.6095
    4.2700    0.6139
    4.2800    0.6183
    4.2900    0.6215
    4.3000    0.6232
    4.3100    0.6253
    4.3200    0.6274
    4.3300    0.6305
    4.3400    0.6303
    4.3500    0.6280
    4.3600    0.6264
    4.3700    0.6267
    4.3800    0.6301
    4.3900    0.6327
    4.4000    0.6345
    4.4100    0.6372
    4.4200    0.6378
    4.4300    0.6381
    4.4400    0.6387
    4.4500    0.6405
    4.4600    0.6430
    4.4700    0.6456
    4.4800    0.6476
    4.4900    0.6485
    4.5000    0.6497
    4.5100    0.6479
    4.5200    0.6450
    4.5300    0.6450
    4.5400    0.6459
    4.5500    0.6449
    4.5600    0.6431
    4.5700    0.6429
    4.5800    0.6421
    4.5900    0.6421
    4.6000    0.6424
    4.6100    0.6436
    4.6200    0.6443
    4.6300    0.6431
    4.6400    0.6413
    4.6500    0.6384
    4.6600    0.6365
    4.6700    0.6358
    4.6800    0.6367
    4.6900    0.6375
    4.7000    0.6368
    4.7100    0.6365
    4.7200    0.6375
    4.7300    0.6377
    4.7400    0.6375
    4.7500    0.6376
    4.7600    0.6359
    4.7700    0.6345
    4.7800    0.6335
    4.7900    0.6308
    4.8000    0.6290
    4.8100    0.6275
    4.8200    0.6256
    4.8300    0.6246
    4.8400    0.6249
    4.8500    0.6242
    4.8600    0.6227
    4.8700    0.6210
    4.8800    0.6192
    4.8900    0.6181
    4.9000    0.6160
    4.9100    0.6137
    4.9200    0.6126
    4.9300    0.6113
    4.9400    0.6111
    4.9500    0.6102
    4.9600    0.6064
    4.9700    0.6013
    4.9800    0.5979
    4.9900    0.5975
    5.0000    0.5959
    5.0100    0.5942
    5.0200    0.5928
    5.0300    0.5906
    5.0400    0.5884
    5.0500    0.5862
    5.0600    0.5839
    5.0700    0.5843
    5.0800    0.5831
    5.0900    0.5767
    5.1000    0.5703
    5.1100    0.5647
    5.1200    0.5598
    5.1300    0.5559
    5.1400    0.5522
    5.1500    0.5492
    5.1600    0.5469
    5.1700    0.5447
    5.1800    0.5441
    5.1900    0.5439
    5.2000    0.5402
    5.2100    0.5325
    5.2200    0.5273
    5.2300    0.5225
    5.2400    0.5167
    5.2500    0.5130
    5.2600    0.5117
    5.2700    0.5101
    5.2800    0.5055
    5.2900    0.5012
    5.3000    0.4977
    5.3100    0.4939
    5.3200    0.4891
    5.3300    0.4829
    5.3400    0.4776
    5.3500    0.4722
    5.3600    0.4652
    5.3700    0.4612
    5.3800    0.4578
    5.3900    0.4527
    5.4000    0.4491
    5.4100    0.4452
    5.4200    0.4414
    5.4300    0.4376
    5.4400    0.4337
    5.4500    0.4308
    5.4600    0.4266
    5.4700    0.4206
    5.4800    0.4136
    5.4900    0.4073
    5.5000    0.4016
    5.5100    0.3958
    5.5200    0.3915
    5.5300    0.3873
    5.5400    0.3832
    5.5500    0.3788
    5.5600    0.3743
    5.5700    0.3696
    5.5800    0.3641
    5.5900    0.3602
    5.6000    0.3556
    5.6100    0.3494
    5.6200    0.3459
    5.6300    0.3439
    5.6400    0.3391
    5.6500    0.3340
    5.6600    0.3290
    5.6700    0.3239
    5.6800    0.3208
    5.6900    0.3152
    5.7000    0.3090
    5.7100    0.3063
    5.7200    0.3024
    5.7300    0.2988
    5.7400    0.2953
    5.7500    0.2885
    5.7600    0.2790
    5.7700    0.2705
    5.7800    0.2652
    5.7900    0.2607
    5.8000    0.2558
    5.8100    0.2498
    5.8200    0.2436
    5.8300    0.2361
    5.8400    0.2276
    5.8500    0.2200
    5.8600    0.2138
    5.8700    0.2086
    5.8800    0.2014
    5.8900    0.1942
    5.9000    0.1875
    5.9100    0.1801
    5.9200    0.1744
    5.9300    0.1696
    5.9400    0.1642
    5.9500    0.1597
    5.9600    0.1549
    5.9700    0.1498
    5.9800    0.1452
    5.9900    0.1412
    6.0000    0.1371
    6.0100    0.1332
    6.0200    0.1287
    6.0300    0.1227
    6.0400    0.1185
    6.0500    0.1138
    6.0600    0.1072
    6.0700    0.1021
    6.0800    0.0973
    6.0900    0.0929
    6.1000    0.0896
    6.1100    0.0850
    6.1200    0.0784
    6.1300    0.0720
    6.1400    0.0650
    6.1500    0.0577
    6.1600    0.0528
    6.1700    0.0478
    6.1800    0.0430
    6.1900    0.0402
    6.2000    0.0374
    6.2100    0.0326
    6.2200    0.0276
    6.2300    0.0227
    6.2400    0.0156
    6.2500    0.0076
    6.2600    0.0025
    6.2700   -0.0023
    6.2800   -0.0077
    6.2900   -0.0143
    6.3000   -0.0213
    6.3100   -0.0266
    6.3200   -0.0335
    6.3300   -0.0407
    6.3400   -0.0465
    6.3500   -0.0537
    6.3600   -0.0608
    6.3700   -0.0689
    6.3800   -0.0793
    6.3900   -0.0890
    6.4000   -0.0973
    6.4100   -0.1056
    6.4200   -0.1147
    6.4300   -0.1222
    6.4400   -0.1295
    6.4500   -0.1370
    6.4600   -0.1418
    6.4700   -0.1467
    6.4800   -0.1523
    6.4900   -0.1584
    6.5000   -0.1662
    6.5100   -0.1736
    6.5200   -0.1782
    6.5300   -0.1808
    6.5400   -0.1850
    6.5500   -0.1929
    6.5600   -0.2001
    6.5700   -0.2050
    6.5800   -0.2104
    6.5900   -0.2174
    6.6000   -0.2219
    6.6100   -0.2277
    6.6200   -0.2363
    6.6300   -0.2438
    6.6400   -0.2513
    6.6500   -0.2569
    6.6600   -0.2617
    6.6700   -0.2676
    6.6800   -0.2727
    6.6900   -0.2764
    6.7000   -0.2801
    6.7100   -0.2850
    6.7200   -0.2894
    6.7300   -0.2925
    6.7400   -0.2940
    6.7500   -0.2950
    6.7600   -0.2975
    6.7700   -0.3011
    6.7800   -0.3073
    6.7900   -0.3140
    6.8000   -0.3201
    6.8100   -0.3264
    6.8200   -0.3311
    6.8300   -0.3358
    6.8400   -0.3421
    6.8500   -0.3482
    6.8600   -0.3534
    6.8700   -0.3577
    6.8800   -0.3628
    6.8900   -0.3680
    6.9000   -0.3719
    6.9100   -0.3748
    6.9200   -0.3779
    6.9300   -0.3826
    6.9400   -0.3883
    6.9500   -0.3953
    6.9600   -0.4007
    6.9700   -0.4047
    6.9800   -0.4085
    6.9900   -0.4130
    7.0000   -0.4158
    7.0100   -0.4175
    7.0200   -0.4201
    7.0300   -0.4230
    7.0400   -0.4273
    7.0500   -0.4304
    7.0600   -0.4328
    7.0700   -0.4371
    7.0800   -0.4437
    7.0900   -0.4502
    7.1000   -0.4565
    7.1100   -0.4615
    7.1200   -0.4653
    7.1300   -0.4695
    7.1400   -0.4748
    7.1500   -0.4787
    7.1600   -0.4805
    7.1700   -0.4833
    7.1800   -0.4854
    7.1900   -0.4882
    7.2000   -0.4918
    7.2100   -0.4939
    7.2200   -0.4960
    7.2300   -0.4993
    7.2400   -0.5025
    7.2500   -0.5054
    7.2600   -0.5097
    7.2700   -0.5147
    7.2800   -0.5175
    7.2900   -0.5198
    7.3000   -0.5234
    7.3100   -0.5273
    7.3200   -0.5314
    7.3300   -0.5376
    7.3400   -0.5447
    7.3500   -0.5497
    7.3600   -0.5545
    7.3700   -0.5579
    7.3800   -0.5605
    7.3900   -0.5607
    7.4000   -0.5610
    7.4100   -0.5637
    7.4200   -0.5675
    7.4300   -0.5715
    7.4400   -0.5752
    7.4500   -0.5783
    7.4600   -0.5788
    7.4700   -0.5789
    7.4800   -0.5806
    7.4900   -0.5846
    7.5000   -0.5860
    7.5100   -0.5833
    7.5200   -0.5821
    7.5300   -0.5842
    7.5400   -0.5850
    7.5500   -0.5853
    7.5600   -0.5874
    7.5700   -0.5878
    7.5800   -0.5892
    7.5900   -0.5937
    7.6000   -0.5961
    7.6100   -0.5958
    7.6200   -0.5958
    7.6300   -0.5957
    7.6400   -0.5944
    7.6500   -0.5925
    7.6600   -0.5923
    7.6700   -0.5923
    7.6800   -0.5915
    7.6900   -0.5920
    7.7000   -0.5940
    7.7100   -0.5946
    7.7200   -0.5943
    7.7300   -0.5945
    7.7400   -0.5952
    7.7500   -0.5976
    7.7600   -0.5989
    7.7700   -0.5985
    7.7800   -0.5968
    7.7900   -0.5941
    7.8000   -0.5916
    7.8100   -0.5907
    7.8200   -0.5919
    7.8300   -0.5937
    7.8400   -0.5939
    7.8500   -0.5894
    7.8600   -0.5846
    7.8700   -0.5838
    7.8800   -0.5827
    7.8900   -0.5820
    7.9000   -0.5838
    7.9100   -0.5835
    7.9200   -0.5824
    7.9300   -0.5816
    7.9400   -0.5784
    7.9500   -0.5750
    7.9600   -0.5721
    7.9700   -0.5714
    7.9800   -0.5709
    7.9900   -0.5662
    8.0000   -0.5616
    8.0100   -0.5610
    8.0200   -0.5612
    8.0300   -0.5602
    8.0400   -0.5585
    8.0500   -0.5557
    8.0600   -0.5528
    8.0700   -0.5507
    8.0800   -0.5497
    8.0900   -0.5489
    8.1000   -0.5465
    8.1100   -0.5454
    8.1200   -0.5454
    8.1300   -0.5430
    8.1400   -0.5410
    8.1500   -0.5388
    8.1600   -0.5358
    8.1700   -0.5344
    8.1800   -0.5327
    8.1900   -0.5302
    8.2000   -0.5282
    8.2100   -0.5267
    8.2200   -0.5247
    8.2300   -0.5238
    8.2400   -0.5234
    8.2500   -0.5215
    8.2600   -0.5202
    8.2700   -0.5174
    8.2800   -0.5144
    8.2900   -0.5115
    8.3000   -0.5066
    8.3100   -0.5024
    8.3200   -0.4990
    8.3300   -0.4946
    8.3400   -0.4906
    8.3500   -0.4867
    8.3600   -0.4840
    8.3700   -0.4807
    8.3800   -0.4770
    8.3900   -0.4765
    8.4000   -0.4734
    8.4100   -0.4682
    8.4200   -0.4641
    8.4300   -0.4602
    8.4400   -0.4579
    8.4500   -0.4586
    8.4600   -0.4574
    8.4700   -0.4531
    8.4800   -0.4496
    8.4900   -0.4454
    8.5000   -0.4424
    8.5100   -0.4407
    8.5200   -0.4361
    8.5300   -0.4299
    8.5400   -0.4265
    8.5500   -0.4261
    8.5600   -0.4249
    8.5700   -0.4209
    8.5800   -0.4152
    8.5900   -0.4096
    8.6000   -0.4063
    8.6100   -0.4027
    8.6200   -0.3991
    8.6300   -0.3969
    8.6400   -0.3941
    8.6500   -0.3916
    8.6600   -0.3885
    8.6700   -0.3851
    8.6800   -0.3817
    8.6900   -0.3777
    8.7000   -0.3739
    8.7100   -0.3700
    8.7200   -0.3643
    8.7300   -0.3573
    8.7400   -0.3516
    8.7500   -0.3482
    8.7600   -0.3466
    8.7700   -0.3456
    8.7800   -0.3398
    8.7900   -0.3307
    8.8000   -0.3242
    8.8100   -0.3198
    8.8200   -0.3170
    8.8300   -0.3125
    8.8400   -0.3049
    8.8500   -0.2997
    8.8600   -0.2968
    8.8700   -0.2921
    8.8800   -0.2891
    8.8900   -0.2850
    8.9000   -0.2791
    8.9100   -0.2720
    8.9200   -0.2649
    8.9300   -0.2594
    8.9400   -0.2548
    8.9500   -0.2512
    8.9600   -0.2477
    8.9700   -0.2431
    8.9800   -0.2356
    8.9900   -0.2292
    9.0000   -0.2238
    9.0100   -0.2183
    9.0200   -0.2131
    9.0300   -0.2060
    9.0400   -0.1989
    9.0500   -0.1943
    9.0600   -0.1907
    9.0700   -0.1861
    9.0800   -0.1808
    9.0900   -0.1763
    9.1000   -0.1713
    9.1100   -0.1639
    9.1200   -0.1571
    9.1300   -0.1518
    9.1400   -0.1487
    9.1500   -0.1462
    9.1600   -0.1429
    9.1700   -0.1390
    9.1800   -0.1331
    9.1900   -0.1249
    9.2000   -0.1154
    9.2100   -0.1077
    9.2200   -0.1023
    9.2300   -0.0959
    9.2400   -0.0886
    9.2500   -0.0814
    9.2600   -0.0738
    9.2700   -0.0687
    9.2800   -0.0639
    9.2900   -0.0576
    9.3000   -0.0527
    9.3100   -0.0485
    9.3200   -0.0419
    9.3300   -0.0356
    9.3400   -0.0320
    9.3500   -0.0273
    9.3600   -0.0189
    9.3700   -0.0108
    9.3800   -0.0046
    9.3900    0.0005
    9.4000    0.0071
    9.4100    0.0150
    9.4200    0.0215
    9.4300    0.0268
    9.4400    0.0325
    9.4500    0.0397
    9.4600    0.0446
    9.4700    0.0491
    9.4800    0.0544
    9.4900    0.0597
    9.5000    0.0653
    9.5100    0.0705
    9.5200    0.0749
    9.5300    0.0790
    9.5400    0.0852
    9.5500    0.0937
    9.5600    0.1000
    9.5700    0.1070
    9.5800    0.1170
    9.5900    0.1244
    9.6000    0.1299
    9.6100    0.1343
    9.6200    0.1400
    9.6300    0.1456
    9.6400    0.1498
    9.6500    0.1558
    9.6600    0.1627
    9.6700    0.1696
    9.6800    0.1766
    9.6900    0.1821
    9.7000    0.1864
    9.7100    0.1921
    9.7200    0.1975
    9.7300    0.2034
    9.7400    0.2109
    9.7500    0.2173
    9.7600    0.2228
    9.7700    0.2284
    9.7800    0.2379
    9.7900    0.2468
    9.8000    0.2501
    9.8100    0.2555
    9.8200    0.2634
    9.8300    0.2683
    9.8400    0.2755
    9.8500    0.2839
    9.8600    0.2897
    9.8700    0.2940
    9.8800    0.2968
    9.8900    0.2984
    9.9000    0.3007
    9.9100    0.3038
    9.9200    0.3080
    9.9300    0.3130
    9.9400    0.3193
    9.9500    0.3275
    9.9600    0.3339
    9.9700    0.3383
    9.9800    0.3437
    9.9900    0.3481
   10.0000    0.3520
    };

==> Data/Oscillator/sigma3/E_mah_dist_en.tex <==
    \addplot[
    thick,
    dashed,
    cyan
    ]
    table {
         0         0
    0.0100    0.0000
    0.0200    0.0000
    0.0300    0.0000
    0.0400    0.0000
    0.0500    0.0000
    0.0600    0.0000
    0.0700    0.0000
    0.0800    0.0001
    0.0900    0.0001
    0.1000    0.0002
    0.1100    0.0003
    0.1200    0.0004
    0.1300    0.0005
    0.1400    0.0007
    0.1500    0.0009
    0.1600    0.0012
    0.1700    0.0015
    0.1800    0.0020
    0.1900    0.0024
    0.2000    0.0030
    0.2100    0.0037
    0.2200    0.0044
    0.2300    0.0051
    0.2400    0.0060
    0.2500    0.0071
    0.2600    0.0084
    0.2700    0.0097
    0.2800    0.0110
    0.2900    0.0127
    0.3000    0.0144
    0.3100    0.0163
    0.3200    0.0185
    0.3300    0.0206
    0.3400    0.0230
    0.3500    0.0254
    0.3600    0.0276
    0.3700    0.0302
    0.3800    0.0338
    0.3900    0.0377
    0.4000    0.0416
    0.4100    0.0459
    0.4200    0.0505
    0.4300    0.0552
    0.4400    0.0593
    0.4500    0.0638
    0.4600    0.0694
    0.4700    0.0745
    0.4800    0.0794
    0.4900    0.0848
    0.5000    0.0905
    0.5100    0.0962
    0.5200    0.1027
    0.5300    0.1096
    0.5400    0.1166
    0.5500    0.1247
    0.5600    0.1324
    0.5700    0.1399
    0.5800    0.1482
    0.5900    0.1565
    0.6000    0.1644
    0.6100    0.1725
    0.6200    0.1813
    0.6300    0.1903
    0.6400    0.1996
    0.6500    0.2099
    0.6600    0.2200
    0.6700    0.2283
    0.6800    0.2383
    0.6900    0.2479
    0.7000    0.2571
    0.7100    0.2686
    0.7200    0.2807
    0.7300    0.2934
    0.7400    0.3065
    0.7500    0.3188
    0.7600    0.3286
    0.7700    0.3386
    0.7800    0.3498
    0.7900    0.3593
    0.8000    0.3732
    0.8100    0.3889
    0.8200    0.4011
    0.8300    0.4125
    0.8400    0.4259
    0.8500    0.4421
    0.8600    0.4551
    0.8700    0.4674
    0.8800    0.4801
    0.8900    0.4936
    0.9000    0.5108
    0.9100    0.5253
    0.9200    0.5361
    0.9300    0.5455
    0.9400    0.5589
    0.9500    0.5769
    0.9600    0.5944
    0.9700    0.6100
    0.9800    0.6247
    0.9900    0.6370
    1.0000    0.6502
    1.0100    0.6695
    1.0200    0.6855
    1.0300    0.6962
    1.0400    0.7088
    1.0500    0.7263
    1.0600    0.7415
    1.0700    0.7578
    1.0800    0.7743
    1.0900    0.7856
    1.1000    0.7964
    1.1100    0.8128
    1.1200    0.8304
    1.1300    0.8448
    1.1400    0.8549
    1.1500    0.8619
    1.1600    0.8739
    1.1700    0.8839
    1.1800    0.8957
    1.1900    0.9118
    1.2000    0.9219
    1.2100    0.9282
    1.2200    0.9364
    1.2300    0.9460
    1.2400    0.9588
    1.2500    0.9703
    1.2600    0.9823
    1.2700    0.9949
    1.2800    1.0047
    1.2900    1.0132
    1.3000    1.0232
    1.3100    1.0348
    1.3200    1.0422
    1.3300    1.0538
    1.3400    1.0672
    1.3500    1.0737
    1.3600    1.0804
    1.3700    1.0922
    1.3800    1.1022
    1.3900    1.1122
    1.4000    1.1222
    1.4100    1.1314
    1.4200    1.1419
    1.4300    1.1511
    1.4400    1.1562
    1.4500    1.1623
    1.4600    1.1664
    1.4700    1.1766
    1.4800    1.1928
    1.4900    1.2012
    1.5000    1.2112
    1.5100    1.2256
    1.5200    1.2356
    1.5300    1.2404
    1.5400    1.2468
    1.5500    1.2530
    1.5600    1.2620
    1.5700    1.2736
    1.5800    1.2821
    1.5900    1.2914
    1.6000    1.3006
    1.6100    1.2998
    1.6200    1.3023
    1.6300    1.3091
    1.6400    1.3171
    1.6500    1.3228
    1.6600    1.3278
    1.6700    1.3366
    1.6800    1.3434
    1.6900    1.3500
    1.7000    1.3536
    1.7100    1.3610
    1.7200    1.3580
    1.7300    1.3566
    1.7400    1.3664
    1.7500    1.3630
    1.7600    1.3643
    1.7700    1.3715
    1.7800    1.3775
    1.7900    1.3829
    1.8000    1.3833
    1.8100    1.3854
    1.8200    1.3886
    1.8300    1.3940
    1.8400    1.3922
    1.8500    1.3979
    1.8600    1.4140
    1.8700    1.4197
    1.8800    1.4234
    1.8900    1.4292
    1.9000    1.4369
    1.9100    1.4469
    1.9200    1.4526
    1.9300    1.4580
    1.9400    1.4650
    1.9500    1.4703
    1.9600    1.4770
    1.9700    1.4768
    1.9800    1.4780
    1.9900    1.4778
    2.0000    1.4737
    2.0100    1.4815
    2.0200    1.4890
    2.0300    1.4891
    2.0400    1.4839
    2.0500    1.4815
    2.0600    1.4819
    2.0700    1.4792
    2.0800    1.4825
    2.0900    1.4889
    2.1000    1.4958
    2.1100    1.5035
    2.1200    1.5012
    2.1300    1.4969
    2.1400    1.4882
    2.1500    1.4794
    2.1600    1.4872
    2.1700    1.4888
    2.1800    1.4777
    2.1900    1.4762
    2.2000    1.4775
    2.2100    1.4735
    2.2200    1.4697
    2.2300    1.4658
    2.2400    1.4632
    2.2500    1.4634
    2.2600    1.4616
    2.2700    1.4635
    2.2800    1.4603
    2.2900    1.4545
    2.3000    1.4516
    2.3100    1.4501
    2.3200    1.4552
    2.3300    1.4566
    2.3400    1.4562
    2.3500    1.4517
    2.3600    1.4444
    2.3700    1.4390
    2.3800    1.4396
    2.3900    1.4458
    2.4000    1.4451
    2.4100    1.4435
    2.4200    1.4392
    2.4300    1.4278
    2.4400    1.4240
    2.4500    1.4219
    2.4600    1.4118
    2.4700    1.4051
    2.4800    1.3975
    2.4900    1.3865
    2.5000    1.3812
    2.5100    1.3756
    2.5200    1.3695
    2.5300    1.3682
    2.5400    1.3658
    2.5500    1.3613
    2.5600    1.3606
    2.5700    1.3531
    2.5800    1.3451
    2.5900    1.3337
    2.6000    1.3233
    2.6100    1.3213
    2.6200    1.3124
    2.6300    1.2968
    2.6400    1.2848
    2.6500    1.2850
    2.6600    1.2813
    2.6700    1.2795
    2.6800    1.2818
    2.6900    1.2784
    2.7000    1.2705
    2.7100    1.2583
    2.7200    1.2519
    2.7300    1.2463
    2.7400    1.2411
    2.7500    1.2381
    2.7600    1.2267
    2.7700    1.2174
    2.7800    1.2150
    2.7900    1.2141
    2.8000    1.2102
    2.8100    1.2012
    2.8200    1.1877
    2.8300    1.1784
    2.8400    1.1746
    2.8500    1.1729
    2.8600    1.1666
    2.8700    1.1576
    2.8800    1.1573
    2.8900    1.1485
    2.9000    1.1363
    2.9100    1.1287
    2.9200    1.1259
    2.9300    1.1245
    2.9400    1.1169
    2.9500    1.1149
    2.9600    1.1147
    2.9700    1.1124
    2.9800    1.1075
    2.9900    1.1048
    3.0000    1.1016
    3.0100    1.0884
    3.0200    1.0806
    3.0300    1.0780
    3.0400    1.0726
    3.0500    1.0637
    3.0600    1.0549
    3.0700    1.0484
    3.0800    1.0443
    3.0900    1.0423
    3.1000    1.0372
    3.1100    1.0267
    3.1200    1.0158
    3.1300    1.0140
    3.1400    1.0118
    3.1500    1.0058
    3.1600    1.0025
    3.1700    0.9988
    3.1800    0.9971
    3.1900    0.9954
    3.2000    0.9933
    3.2100    0.9917
    3.2200    0.9874
    3.2300    0.9817
    3.2400    0.9769
    3.2500    0.9731
    3.2600    0.9685
    3.2700    0.9627
    3.2800    0.9534
    3.2900    0.9433
    3.3000    0.9382
    3.3100    0.9326
    3.3200    0.9261
    3.3300    0.9260
    3.3400    0.9311
    3.3500    0.9361
    3.3600    0.9352
    3.3700    0.9314
    3.3800    0.9298
    3.3900    0.9258
    3.4000    0.9216
    3.4100    0.9199
    3.4200    0.9143
    3.4300    0.9059
    3.4400    0.8925
    3.4500    0.8803
    3.4600    0.8747
    3.4700    0.8704
    3.4800    0.8672
    3.4900    0.8616
    3.5000    0.8606
    3.5100    0.8606
    3.5200    0.8529
    3.5300    0.8471
    3.5400    0.8424
    3.5500    0.8331
    3.5600    0.8232
    3.5700    0.8126
    3.5800    0.8109
    3.5900    0.8128
    3.6000    0.8057
    3.6100    0.7970
    3.6200    0.7909
    3.6300    0.7847
    3.6400    0.7755
    3.6500    0.7668
    3.6600    0.7631
    3.6700    0.7597
    3.6800    0.7551
    3.6900    0.7481
    3.7000    0.7396
    3.7100    0.7323
    3.7200    0.7252
    3.7300    0.7204
    3.7400    0.7158
    3.7500    0.7091
    3.7600    0.7064
    3.7700    0.7041
    3.7800    0.6955
    3.7900    0.6889
    3.8000    0.6808
    3.8100    0.6704
    3.8200    0.6653
    3.8300    0.6611
    3.8400    0.6566
    3.8500    0.6516
    3.8600    0.6439
    3.8700    0.6377
    3.8800    0.6328
    3.8900    0.6230
    3.9000    0.6126
    3.9100    0.6041
    3.9200    0.5989
    3.9300    0.5968
    3.9400    0.5920
    3.9500    0.5862
    3.9600    0.5841
    3.9700    0.5856
    3.9800    0.5805
    3.9900    0.5753
    4.0000    0.5673
    4.0100    0.5623
    4.0200    0.5614
    4.0300    0.5544
    4.0400    0.5513
    4.0500    0.5466
    4.0600    0.5423
    4.0700    0.5375
    4.0800    0.5302
    4.0900    0.5278
    4.1000    0.5303
    4.1100    0.5303
    4.1200    0.5231
    4.1300    0.5157
    4.1400    0.5110
    4.1500    0.5042
    4.1600    0.5011
    4.1700    0.4961
    4.1800    0.4899
    4.1900    0.4870
    4.2000    0.4826
    4.2100    0.4777
    4.2200    0.4763
    4.2300    0.4725
    4.2400    0.4640
    4.2500    0.4559
    4.2600    0.4455
    4.2700    0.4390
    4.2800    0.4358
    4.2900    0.4356
    4.3000    0.4337
    4.3100    0.4287
    4.3200    0.4221
    4.3300    0.4176
    4.3400    0.4138
    4.3500    0.4076
    4.3600    0.4047
    4.3700    0.4004
    4.3800    0.3942
    4.3900    0.3905
    4.4000    0.3840
    4.4100    0.3759
    4.4200    0.3716
    4.4300    0.3672
    4.4400    0.3626
    4.4500    0.3584
    4.4600    0.3534
    4.4700    0.3495
    4.4800    0.3476
    4.4900    0.3445
    4.5000    0.3374
    4.5100    0.3313
    4.5200    0.3296
    4.5300    0.3272
    4.5400    0.3242
    4.5500    0.3216
    4.5600    0.3176
    4.5700    0.3133
    4.5800    0.3106
    4.5900    0.3080
    4.6000    0.3065
    4.6100    0.3054
    4.6200    0.3044
    4.6300    0.3030
    4.6400    0.3011
    4.6500    0.2998
    4.6600    0.2971
    4.6700    0.2954
    4.6800    0.2935
    4.6900    0.2892
    4.7000    0.2868
    4.7100    0.2830
    4.7200    0.2799
    4.7300    0.2790
    4.7400    0.2775
    4.7500    0.2762
    4.7600    0.2745
    4.7700    0.2734
    4.7800    0.2713
    4.7900    0.2699
    4.8000    0.2705
    4.8100    0.2691
    4.8200    0.2629
    4.8300    0.2549
    4.8400    0.2501
    4.8500    0.2479
    4.8600    0.2452
    4.8700    0.2426
    4.8800    0.2401
    4.8900    0.2402
    4.9000    0.2391
    4.9100    0.2368
    4.9200    0.2377
    4.9300    0.2340
    4.9400    0.2285
    4.9500    0.2262
    4.9600    0.2213
    4.9700    0.2191
    4.9800    0.2178
    4.9900    0.2138
    5.0000    0.2107
    5.0100    0.2077
    5.0200    0.2055
    5.0300    0.2026
    5.0400    0.1999
    5.0500    0.1990
    5.0600    0.1966
    5.0700    0.1917
    5.0800    0.1880
    5.0900    0.1865
    5.1000    0.1842
    5.1100    0.1805
    5.1200    0.1764
    5.1300    0.1730
    5.1400    0.1712
    5.1500    0.1688
    5.1600    0.1662
    5.1700    0.1628
    5.1800    0.1606
    5.1900    0.1597
    5.2000    0.1562
    5.2100    0.1534
    5.2200    0.1522
    5.2300    0.1511
    5.2400    0.1499
    5.2500    0.1481
    5.2600    0.1460
    5.2700    0.1446
    5.2800    0.1431
    5.2900    0.1414
    5.3000    0.1401
    5.3100    0.1388
    5.3200    0.1380
    5.3300    0.1340
    5.3400    0.1275
    5.3500    0.1232
    5.3600    0.1204
    5.3700    0.1189
    5.3800    0.1183
    5.3900    0.1173
    5.4000    0.1157
    5.4100    0.1133
    5.4200    0.1114
    5.4300    0.1099
    5.4400    0.1090
    5.4500    0.1080
    5.4600    0.1058
    5.4700    0.1034
    5.4800    0.1017
    5.4900    0.0998
    5.5000    0.0976
    5.5100    0.0967
    5.5200    0.0962
    5.5300    0.0947
    5.5400    0.0945
    5.5500    0.0948
    5.5600    0.0942
    5.5700    0.0925
    5.5800    0.0909
    5.5900    0.0896
    5.6000    0.0884
    5.6100    0.0887
    5.6200    0.0883
    5.6300    0.0874
    5.6400    0.0862
    5.6500    0.0834
    5.6600    0.0818
    5.6700    0.0804
    5.6800    0.0781
    5.6900    0.0773
    5.7000    0.0768
    5.7100    0.0756
    5.7200    0.0742
    5.7300    0.0726
    5.7400    0.0711
    5.7500    0.0695
    5.7600    0.0685
    5.7700    0.0674
    5.7800    0.0670
    5.7900    0.0674
    5.8000    0.0663
    5.8100    0.0651
    5.8200    0.0644
    5.8300    0.0627
    5.8400    0.0616
    5.8500    0.0614
    5.8600    0.0610
    5.8700    0.0601
    5.8800    0.0591
    5.8900    0.0586
    5.9000    0.0587
    5.9100    0.0585
    5.9200    0.0578
    5.9300    0.0573
    5.9400    0.0567
    5.9500    0.0564
    5.9600    0.0557
    5.9700    0.0554
    5.9800    0.0555
    5.9900    0.0543
    6.0000    0.0536
    6.0100    0.0533
    6.0200    0.0524
    6.0300    0.0518
    6.0400    0.0514
    6.0500    0.0505
    6.0600    0.0500
    6.0700    0.0495
    6.0800    0.0481
    6.0900    0.0471
    6.1000    0.0463
    6.1100    0.0461
    6.1200    0.0456
    6.1300    0.0452
    6.1400    0.0446
    6.1500    0.0433
    6.1600    0.0426
    6.1700    0.0420
    6.1800    0.0421
    6.1900    0.0425
    6.2000    0.0422
    6.2100    0.0409
    6.2200    0.0395
    6.2300    0.0388
    6.2400    0.0383
    6.2500    0.0380
    6.2600    0.0372
    6.2700    0.0366
    6.2800    0.0357
    6.2900    0.0351
    6.3000    0.0351
    6.3100    0.0345
    6.3200    0.0346
    6.3300    0.0345
    6.3400    0.0338
    6.3500    0.0334
    6.3600    0.0328
    6.3700    0.0320
    6.3800    0.0312
    6.3900    0.0308
    6.4000    0.0305
    6.4100    0.0300
    6.4200    0.0298
    6.4300    0.0299
    6.4400    0.0298
    6.4500    0.0295
    6.4600    0.0288
    6.4700    0.0280
    6.4800    0.0276
    6.4900    0.0275
    6.5000    0.0270
    6.5100    0.0260
    6.5200    0.0253
    6.5300    0.0250
    6.5400    0.0250
    6.5500    0.0248
    6.5600    0.0243
    6.5700    0.0238
    6.5800    0.0235
    6.5900    0.0234
    6.6000    0.0232
    6.6100    0.0228
    6.6200    0.0224
    6.6300    0.0223
    6.6400    0.0221
    6.6500    0.0218
    6.6600    0.0214
    6.6700    0.0212
    6.6800    0.0212
    6.6900    0.0212
    6.7000    0.0211
    6.7100    0.0207
    6.7200    0.0206
    6.7300    0.0209
    6.7400    0.0210
    6.7500    0.0207
    6.7600    0.0203
    6.7700    0.0203
    6.7800    0.0207
    6.7900    0.0205
    6.8000    0.0202
    6.8100    0.0202
    6.8200    0.0198
    6.8300    0.0195
    6.8400    0.0195
    6.8500    0.0192
    6.8600    0.0188
    6.8700    0.0187
    6.8800    0.0187
    6.8900    0.0180
    6.9000    0.0177
    6.9100    0.0177
    6.9200    0.0175
    6.9300    0.0175
    6.9400    0.0176
    6.9500    0.0175
    6.9600    0.0170
    6.9700    0.0166
    6.9800    0.0166
    6.9900    0.0164
    7.0000    0.0162
    7.0100    0.0157
    7.0200    0.0156
    7.0300    0.0154
    7.0400    0.0152
    7.0500    0.0150
    7.0600    0.0148
    7.0700    0.0148
    7.0800    0.0148
    7.0900    0.0145
    7.1000    0.0144
    7.1100    0.0145
    7.1200    0.0142
    7.1300    0.0142
    7.1400    0.0143
    7.1500    0.0140
    7.1600    0.0139
    7.1700    0.0138
    7.1800    0.0138
    7.1900    0.0137
    7.2000    0.0136
    7.2100    0.0133
    7.2200    0.0132
    7.2300    0.0130
    7.2400    0.0128
    7.2500    0.0128
    7.2600    0.0129
    7.2700    0.0127
    7.2800    0.0126
    7.2900    0.0124
    7.3000    0.0123
    7.3100    0.0120
    7.3200    0.0119
    7.3300    0.0120
    7.3400    0.0120
    7.3500    0.0119
    7.3600    0.0117
    7.3700    0.0115
    7.3800    0.0115
    7.3900    0.0114
    7.4000    0.0113
    7.4100    0.0113
    7.4200    0.0112
    7.4300    0.0113
    7.4400    0.0114
    7.4500    0.0114
    7.4600    0.0115
    7.4700    0.0115
    7.4800    0.0115
    7.4900    0.0117
    7.5000    0.0119
    7.5100    0.0124
    7.5200    0.0127
    7.5300    0.0125
    7.5400    0.0123
    7.5500    0.0123
    7.5600    0.0125
    7.5700    0.0123
    7.5800    0.0121
    7.5900    0.0119
    7.6000    0.0116
    7.6100    0.0116
    7.6200    0.0115
    7.6300    0.0111
    7.6400    0.0110
    7.6500    0.0109
    7.6600    0.0104
    7.6700    0.0102
    7.6800    0.0102
    7.6900    0.0102
    7.7000    0.0101
    7.7100    0.0099
    7.7200    0.0098
    7.7300    0.0098
    7.7400    0.0096
    7.7500    0.0094
    7.7600    0.0094
    7.7700    0.0095
    7.7800    0.0097
    7.7900    0.0100
    7.8000    0.0103
    7.8100    0.0104
    7.8200    0.0107
    7.8300    0.0106
    7.8400    0.0100
    7.8500    0.0103
    7.8600    0.0108
    7.8700    0.0109
    7.8800    0.0111
    7.8900    0.0115
    7.9000    0.0113
    7.9100    0.0111
    7.9200    0.0111
    7.9300    0.0113
    7.9400    0.0115
    7.9500    0.0119
    7.9600    0.0120
    7.9700    0.0120
    7.9800    0.0119
    7.9900    0.0115
    8.0000    0.0110
    8.0100    0.0108
    8.0200    0.0108
    8.0300    0.0111
    8.0400    0.0114
    8.0500    0.0111
    8.0600    0.0109
    8.0700    0.0110
    8.0800    0.0109
    8.0900    0.0105
    8.1000    0.0106
    8.1100    0.0109
    8.1200    0.0107
    8.1300    0.0107
    8.1400    0.0105
    8.1500    0.0103
    8.1600    0.0105
    8.1700    0.0106
    8.1800    0.0104
    8.1900    0.0103
    8.2000    0.0101
    8.2100    0.0103
    8.2200    0.0107
    8.2300    0.0116
    8.2400    0.0122
    8.2500    0.0121
    8.2600    0.0125
    8.2700    0.0122
    8.2800    0.0118
    8.2900    0.0119
    8.3000    0.0122
    8.3100    0.0124
    8.3200    0.0122
    8.3300    0.0124
    8.3400    0.0128
    8.3500    0.0124
    8.3600    0.0126
    8.3700    0.0128
    8.3800    0.0123
    8.3900    0.0122
    8.4000    0.0129
    8.4100    0.0131
    8.4200    0.0127
    8.4300    0.0123
    8.4400    0.0118
    8.4500    0.0119
    8.4600    0.0120
    8.4700    0.0119
    8.4800    0.0121
    8.4900    0.0127
    8.5000    0.0128
    8.5100    0.0123
    8.5200    0.0120
    8.5300    0.0112
    8.5400    0.0111
    8.5500    0.0112
    8.5600    0.0109
    8.5700    0.0107
    8.5800    0.0101
    8.5900    0.0096
    8.6000    0.0096
    8.6100    0.0098
    8.6200    0.0098
    8.6300    0.0089
    8.6400    0.0079
    8.6500    0.0072
    8.6600    0.0066
    8.6700    0.0065
    8.6800    0.0063
    8.6900    0.0063
    8.7000    0.0062
    8.7100    0.0059
    8.7200    0.0062
    8.7300    0.0063
    8.7400    0.0063
    8.7500    0.0070
    8.7600    0.0072
    8.7700    0.0073
    8.7800    0.0077
    8.7900    0.0079
    8.8000    0.0079
    8.8100    0.0081
    8.8200    0.0080
    8.8300    0.0082
    8.8400    0.0087
    8.8500    0.0094
    8.8600    0.0100
    8.8700    0.0098
    8.8800    0.0098
    8.8900    0.0098
    8.9000    0.0095
    8.9100    0.0091
    8.9200    0.0086
    8.9300    0.0084
    8.9400    0.0088
    8.9500    0.0089
    8.9600    0.0091
    8.9700    0.0089
    8.9800    0.0081
    8.9900    0.0078
    9.0000    0.0079
    9.0100    0.0078
    9.0200    0.0078
    9.0300    0.0079
    9.0400    0.0080
    9.0500    0.0081
    9.0600    0.0078
    9.0700    0.0074
    9.0800    0.0069
    9.0900    0.0068
    9.1000    0.0070
    9.1100    0.0071
    9.1200    0.0072
    9.1300    0.0070
    9.1400    0.0067
    9.1500    0.0062
    9.1600    0.0058
    9.1700    0.0058
    9.1800    0.0059
    9.1900    0.0064
    9.2000    0.0069
    9.2100    0.0072
    9.2200    0.0074
    9.2300    0.0069
    9.2400    0.0067
    9.2500    0.0067
    9.2600    0.0068
    9.2700    0.0064
    9.2800    0.0057
    9.2900    0.0056
    9.3000    0.0056
    9.3100    0.0057
    9.3200    0.0059
    9.3300    0.0056
    9.3400    0.0052
    9.3500    0.0054
    9.3600    0.0056
    9.3700    0.0055
    9.3800    0.0058
    9.3900    0.0057
    9.4000    0.0054
    9.4100    0.0054
    9.4200    0.0054
    9.4300    0.0049
    9.4400    0.0047
    9.4500    0.0050
    9.4600    0.0054
    9.4700    0.0058
    9.4800    0.0061
    9.4900    0.0060
    9.5000    0.0063
    9.5100    0.0067
    9.5200    0.0067
    9.5300    0.0066
    9.5400    0.0065
    9.5500    0.0067
    9.5600    0.0068
    9.5700    0.0071
    9.5800    0.0073
    9.5900    0.0073
    9.6000    0.0075
    9.6100    0.0073
    9.6200    0.0069
    9.6300    0.0064
    9.6400    0.0060
    9.6500    0.0058
    9.6600    0.0060
    9.6700    0.0063
    9.6800    0.0060
    9.6900    0.0060
    9.7000    0.0059
    9.7100    0.0056
    9.7200    0.0052
    9.7300    0.0049
    9.7400    0.0047
    9.7500    0.0047
    9.7600    0.0050
    9.7700    0.0052
    9.7800    0.0052
    9.7900    0.0049
    9.8000    0.0048
    9.8100    0.0051
    9.8200    0.0046
    9.8300    0.0042
    9.8400    0.0040
    9.8500    0.0035
    9.8600    0.0035
    9.8700    0.0035
    9.8800    0.0035
    9.8900    0.0035
    9.9000    0.0032
    9.9100    0.0032
    9.9200    0.0032
    9.9300    0.0028
    9.9400    0.0028
    9.9500    0.0028
    9.9600    0.0028
    9.9700    0.0027
    9.9800    0.0025
    9.9900    0.0022
   10.0000    0.0021
    };

==> Data/Oscillator/sigma3/E_mah_dist_exp.tex <==
    \addplot[
    thick,
    green
    ]
    table {
         0         0
    0.0100    0.0000
    0.0200    0.0000
    0.0300    0.0000
    0.0400    0.0000
    0.0500    0.0000
    0.0600    0.0000
    0.0700    0.0000
    0.0800    0.0001
    0.0900    0.0001
    0.1000    0.0002
    0.1100    0.0003
    0.1200    0.0004
    0.1300    0.0005
    0.1400    0.0007
    0.1500    0.0010
    0.1600    0.0013
    0.1700    0.0016
    0.1800    0.0021
    0.1900    0.0026
    0.2000    0.0032
    0.2100    0.0039
    0.2200    0.0047
    0.2300    0.0056
    0.2400    0.0066
    0.2500    0.0078
    0.2600    0.0093
    0.2700    0.0108
    0.2800    0.0123
    0.2900    0.0143
    0.3000    0.0163
    0.3100    0.0185
    0.3200    0.0212
    0.3300    0.0238
    0.3400    0.0267
    0.3500    0.0297
    0.3600    0.0324
    0.3700    0.0358
    0.3800    0.0402
    0.3900    0.0450
    0.4000    0.0499
    0.4100    0.0553
    0.4200    0.0610
    0.4300    0.0671
    0.4400    0.0724
    0.4500    0.0783
    0.4600    0.0855
    0.4700    0.0922
    0.4800    0.0987
    0.4900    0.1058
    0.5000    0.1133
    0.5100    0.1209
    0.5200    0.1295
    0.5300    0.1385
    0.5400    0.1478
    0.5500    0.1582
    0.5600    0.1684
    0.5700    0.1783
    0.5800    0.1891
    0.5900    0.2001
    0.6000    0.2106
    0.6100    0.2213
    0.6200    0.2329
    0.6300    0.2447
    0.6400    0.2568
    0.6500    0.2701
    0.6600    0.2832
    0.6700    0.2943
    0.6800    0.3073
    0.6900    0.3197
    0.7000    0.3319
    0.7100    0.3464
    0.7200    0.3615
    0.7300    0.3774
    0.7400    0.3935
    0.7500    0.4089
    0.7600    0.4215
    0.7700    0.4343
    0.7800    0.4483
    0.7900    0.4607
    0.8000    0.4774
    0.8100    0.4961
    0.8200    0.5110
    0.8300    0.5251
    0.8400    0.5411
    0.8500    0.5600
    0.8600    0.5755
    0.8700    0.5902
    0.8800    0.6054
    0.8900    0.6212
    0.9000    0.6408
    0.9100    0.6575
    0.9200    0.6704
    0.9300    0.6819
    0.9400    0.6974
    0.9500    0.7173
    0.9600    0.7367
    0.9700    0.7540
    0.9800    0.7704
    0.9900    0.7844
    1.0000    0.7992
    1.0100    0.8199
    1.0200    0.8373
    1.0300    0.8494
    1.0400    0.8633
    1.0500    0.8819
    1.0600    0.8982
    1.0700    0.9155
    1.0800    0.9329
    1.0900    0.9452
    1.1000    0.9569
    1.1100    0.9740
    1.1200    0.9922
    1.1300    1.0072
    1.1400    1.0179
    1.1500    1.0257
    1.1600    1.0382
    1.1700    1.0487
    1.1800    1.0609
    1.1900    1.0773
    1.2000    1.0877
    1.2100    1.0945
    1.2200    1.1030
    1.2300    1.1130
    1.2400    1.1259
    1.2500    1.1374
    1.2600    1.1495
    1.2700    1.1620
    1.2800    1.1718
    1.2900    1.1803
    1.3000    1.1903
    1.3100    1.2017
    1.3200    1.2091
    1.3300    1.2204
    1.3400    1.2335
    1.3500    1.2399
    1.3600    1.2465
    1.3700    1.2579
    1.3800    1.2675
    1.3900    1.2771
    1.4000    1.2867
    1.4100    1.2954
    1.4200    1.3055
    1.4300    1.3142
    1.4400    1.3190
    1.4500    1.3247
    1.4600    1.3285
    1.4700    1.3381
    1.4800    1.3533
    1.4900    1.3612
    1.5000    1.3704
    1.5100    1.3839
    1.5200    1.3932
    1.5300    1.3974
    1.5400    1.4033
    1.5500    1.4088
    1.5600    1.4171
    1.5700    1.4277
    1.5800    1.4355
    1.5900    1.4440
    1.6000    1.4523
    1.6100    1.4512
    1.6200    1.4532
    1.6300    1.4592
    1.6400    1.4664
    1.6500    1.4713
    1.6600    1.4757
    1.6700    1.4835
    1.6800    1.4896
    1.6900    1.4954
    1.7000    1.4983
    1.7100    1.5048
    1.7200    1.5016
    1.7300    1.4998
    1.7400    1.5086
    1.7500    1.5049
    1.7600    1.5057
    1.7700    1.5121
    1.7800    1.5173
    1.7900    1.5219
    1.8000    1.5218
    1.8100    1.5234
    1.8200    1.5259
    1.8300    1.5306
    1.8400    1.5284
    1.8500    1.5334
    1.8600    1.5482
    1.8700    1.5531
    1.8800    1.5561
    1.8900    1.5612
    1.9000    1.5680
    1.9100    1.5770
    1.9200    1.5820
    1.9300    1.5866
    1.9400    1.5929
    1.9500    1.5974
    1.9600    1.6033
    1.9700    1.6027
    1.9800    1.6033
    1.9900    1.6027
    2.0000    1.5984
    2.0100    1.6054
    2.0200    1.6121
    2.0300    1.6118
    2.0400    1.6064
    2.0500    1.6038
    2.0600    1.6037
    2.0700    1.6007
    2.0800    1.6035
    2.0900    1.6093
    2.1000    1.6154
    2.1100    1.6225
    2.1200    1.6199
    2.1300    1.6154
    2.1400    1.6068
    2.1500    1.5980
    2.1600    1.6052
    2.1700    1.6064
    2.1800    1.5956
    2.1900    1.5938
    2.2000    1.5948
    2.2100    1.5907
    2.2200    1.5868
    2.2300    1.5829
    2.2400    1.5802
    2.2500    1.5801
    2.2600    1.5781
    2.2700    1.5797
    2.2800    1.5765
    2.2900    1.5707
    2.3000    1.5678
    2.3100    1.5661
    2.3200    1.5709
    2.3300    1.5721
    2.3400    1.5715
    2.3500    1.5670
    2.3600    1.5599
    2.3700    1.5546
    2.3800    1.5551
    2.3900    1.5609
    2.4000    1.5601
    2.4100    1.5585
    2.4200    1.5542
    2.4300    1.5433
    2.4400    1.5395
    2.4500    1.5374
    2.4600    1.5276
    2.4700    1.5211
    2.4800    1.5138
    2.4900    1.5032
    2.5000    1.4980
    2.5100    1.4927
    2.5200    1.4868
    2.5300    1.4855
    2.5400    1.4832
    2.5500    1.4788
    2.5600    1.4782
    2.5700    1.4708
    2.5800    1.4631
    2.5900    1.4522
    2.6000    1.4422
    2.6100    1.4403
    2.6200    1.4317
    2.6300    1.4167
    2.6400    1.4051
    2.6500    1.4054
    2.6600    1.4018
    2.6700    1.4001
    2.6800    1.4023
    2.6900    1.3990
    2.7000    1.3914
    2.7100    1.3797
    2.7200    1.3736
    2.7300    1.3682
    2.7400    1.3632
    2.7500    1.3603
    2.7600    1.3494
    2.7700    1.3405
    2.7800    1.3381
    2.7900    1.3373
    2.8000    1.3335
    2.8100    1.3249
    2.8200    1.3119
    2.8300    1.3029
    2.8400    1.2993
    2.8500    1.2977
    2.8600    1.2916
    2.8700    1.2830
    2.8800    1.2827
    2.8900    1.2742
    2.9000    1.2624
    2.9100    1.2550
    2.9200    1.2524
    2.9300    1.2510
    2.9400    1.2436
    2.9500    1.2418
    2.9600    1.2416
    2.9700    1.2394
    2.9800    1.2346
    2.9900    1.2320
    3.0000    1.2287
    3.0100    1.2160
    3.0200    1.2084
    3.0300    1.2058
    3.0400    1.2005
    3.0500    1.1919
    3.0600    1.1833
    3.0700    1.1769
    3.0800    1.1730
    3.0900    1.1710
    3.1000    1.1660
    3.1100    1.1557
    3.1200    1.1450
    3.1300    1.1433
    3.1400    1.1411
    3.1500    1.1351
    3.1600    1.1319
    3.1700    1.1282
    3.1800    1.1265
    3.1900    1.1248
    3.2000    1.1226
    3.2100    1.1210
    3.2200    1.1167
    3.2300    1.1110
    3.2400    1.1063
    3.2500    1.1026
    3.2600    1.0980
    3.2700    1.0922
    3.2800    1.0830
    3.2900    1.0730
    3.3000    1.0679
    3.3100    1.0623
    3.3200    1.0558
    3.3300    1.0557
    3.3400    1.0606
    3.3500    1.0654
    3.3600    1.0644
    3.3700    1.0606
    3.3800    1.0589
    3.3900    1.0548
    3.4000    1.0505
    3.4100    1.0488
    3.4200    1.0431
    3.4300    1.0347
    3.4400    1.0213
    3.4500    1.0092
    3.4600    1.0035
    3.4700    0.9992
    3.4800    0.9959
    3.4900    0.9902
    3.5000    0.9890
    3.5100    0.9889
    3.5200    0.9811
    3.5300    0.9753
    3.5400    0.9704
    3.5500    0.9611
    3.5600    0.9511
    3.5700    0.9406
    3.5800    0.9387
    3.5900    0.9405
    3.6000    0.9332
    3.6100    0.9244
    3.6200    0.9182
    3.6300    0.9119
    3.6400    0.9026
    3.6500    0.8938
    3.6600    0.8900
    3.6700    0.8864
    3.6800    0.8817
    3.6900    0.8745
    3.7000    0.8659
    3.7100    0.8584
    3.7200    0.8511
    3.7300    0.8461
    3.7400    0.8414
    3.7500    0.8346
    3.7600    0.8317
    3.7700    0.8292
    3.7800    0.8205
    3.7900    0.8137
    3.8000    0.8054
    3.8100    0.7948
    3.8200    0.7895
    3.8300    0.7852
    3.8400    0.7804
    3.8500    0.7752
    3.8600    0.7674
    3.8700    0.7610
    3.8800    0.7559
    3.8900    0.7458
    3.9000    0.7353
    3.9100    0.7266
    3.9200    0.7212
    3.9300    0.7188
    3.9400    0.7138
    3.9500    0.7078
    3.9600    0.7055
    3.9700    0.7068
    3.9800    0.7015
    3.9900    0.6961
    4.0000    0.6878
    4.0100    0.6825
    4.0200    0.6815
    4.0300    0.6742
    4.0400    0.6709
    4.0500    0.6659
    4.0600    0.6614
    4.0700    0.6563
    4.0800    0.6488
    4.0900    0.6462
    4.1000    0.6484
    4.1100    0.6481
    4.1200    0.6407
    4.1300    0.6330
    4.1400    0.6280
    4.1500    0.6209
    4.1600    0.6175
    4.1700    0.6123
    4.1800    0.6059
    4.1900    0.6027
    4.2000    0.5980
    4.2100    0.5928
    4.2200    0.5912
    4.2300    0.5871
    4.2400    0.5784
    4.2500    0.5700
    4.2600    0.5593
    4.2700    0.5524
    4.2800    0.5489
    4.2900    0.5485
    4.3000    0.5463
    4.3100    0.5411
    4.3200    0.5341
    4.3300    0.5294
    4.3400    0.5253
    4.3500    0.5187
    4.3600    0.5155
    4.3700    0.5109
    4.3800    0.5044
    4.3900    0.5004
    4.4000    0.4935
    4.4100    0.4851
    4.4200    0.4804
    4.4300    0.4758
    4.4400    0.4708
    4.4500    0.4662
    4.4600    0.4609
    4.4700    0.4567
    4.4800    0.4545
    4.4900    0.4511
    4.5000    0.4436
    4.5100    0.4371
    4.5200    0.4351
    4.5300    0.4325
    4.5400    0.4290
    4.5500    0.4261
    4.5600    0.4218
    4.5700    0.4171
    4.5800    0.4142
    4.5900    0.4113
    4.6000    0.4094
    4.6100    0.4080
    4.6200    0.4067
    4.6300    0.4050
    4.6400    0.4027
    4.6500    0.4011
    4.6600    0.3981
    4.6700    0.3961
    4.6800    0.3939
    4.6900    0.3891
    4.7000    0.3865
    4.7100    0.3823
    4.7200    0.3789
    4.7300    0.3776
    4.7400    0.3759
    4.7500    0.3743
    4.7600    0.3723
    4.7700    0.3708
    4.7800    0.3684
    4.7900    0.3667
    4.8000    0.3670
    4.8100    0.3652
    4.8200    0.3586
    4.8300    0.3502
    4.8400    0.3450
    4.8500    0.3424
    4.8600    0.3394
    4.8700    0.3364
    4.8800    0.3335
    4.8900    0.3334
    4.9000    0.3320
    4.9100    0.3293
    4.9200    0.3299
    4.9300    0.3258
    4.9400    0.3199
    4.9500    0.3172
    4.9600    0.3118
    4.9700    0.3093
    4.9800    0.3077
    4.9900    0.3033
    5.0000    0.2997
    5.0100    0.2963
    5.0200    0.2938
    5.0300    0.2905
    5.0400    0.2874
    5.0500    0.2862
    5.0600    0.2834
    5.0700    0.2780
    5.0800    0.2740
    5.0900    0.2722
    5.1000    0.2694
    5.1100    0.2653
    5.1200    0.2608
    5.1300    0.2570
    5.1400    0.2547
    5.1500    0.2520
    5.1600    0.2490
    5.1700    0.2452
    5.1800    0.2425
    5.1900    0.2413
    5.2000    0.2373
    5.2100    0.2342
    5.2200    0.2326
    5.2300    0.2312
    5.2400    0.2296
    5.2500    0.2275
    5.2600    0.2250
    5.2700    0.2231
    5.2800    0.2213
    5.2900    0.2192
    5.3000    0.2175
    5.3100    0.2159
    5.3200    0.2147
    5.3300    0.2103
    5.3400    0.2032
    5.3500    0.1984
    5.3600    0.1951
    5.3700    0.1933
    5.3800    0.1924
    5.3900    0.1910
    5.4000    0.1890
    5.4100    0.1863
    5.4200    0.1839
    5.4300    0.1820
    5.4400    0.1808
    5.4500    0.1794
    5.4600    0.1767
    5.4700    0.1739
    5.4800    0.1718
    5.4900    0.1696
    5.5000    0.1669
    5.5100    0.1657
    5.5200    0.1648
    5.5300    0.1629
    5.5400    0.1624
    5.5500    0.1624
    5.5600    0.1615
    5.5700    0.1594
    5.5800    0.1574
    5.5900    0.1557
    5.6000    0.1541
    5.6100    0.1541
    5.6200    0.1534
    5.6300    0.1521
    5.6400    0.1506
    5.6500    0.1474
    5.6600    0.1453
    5.6700    0.1435
    5.6800    0.1408
    5.6900    0.1396
    5.7000    0.1389
    5.7100    0.1372
    5.7200    0.1354
    5.7300    0.1335
    5.7400    0.1316
    5.7500    0.1296
    5.7600    0.1281
    5.7700    0.1266
    5.7800    0.1259
    5.7900    0.1261
    5.8000    0.1246
    5.8100    0.1230
    5.8200    0.1220
    5.8300    0.1199
    5.8400    0.1183
    5.8500    0.1179
    5.8600    0.1171
    5.8700    0.1159
    5.8800    0.1145
    5.8900    0.1137
    5.9000    0.1134
    5.9100    0.1129
    5.9200    0.1118
    5.9300    0.1110
    5.9400    0.1100
    5.9500    0.1094
    5.9600    0.1084
    5.9700    0.1078
    5.9800    0.1075
    5.9900    0.1059
    6.0000    0.1050
    6.0100    0.1043
    6.0200    0.1030
    6.0300    0.1021
    6.0400    0.1013
    6.0500    0.1000
    6.0600    0.0993
    6.0700    0.0984
    6.0800    0.0967
    6.0900    0.0952
    6.1000    0.0941
    6.1100    0.0936
    6.1200    0.0927
    6.1300    0.0920
    6.1400    0.0911
    6.1500    0.0894
    6.1600    0.0883
    6.1700    0.0874
    6.1800    0.0872
    6.1900    0.0874
    6.2000    0.0868
    6.2100    0.0850
    6.2200    0.0832
    6.2300    0.0822
    6.2400    0.0814
    6.2500    0.0808
    6.2600    0.0796
    6.2700    0.0787
    6.2800    0.0775
    6.2900    0.0765
    6.3000    0.0762
    6.3100    0.0753
    6.3200    0.0751
    6.3300    0.0747
    6.3400    0.0737
    6.3500    0.0730
    6.3600    0.0720
    6.3700    0.0709
    6.3800    0.0697
    6.3900    0.0690
    6.4000    0.0684
    6.4100    0.0676
    6.4200    0.0671
    6.4300    0.0670
    6.4400    0.0666
    6.4500    0.0660
    6.4600    0.0650
    6.4700    0.0637
    6.4800    0.0630
    6.4900    0.0627
    6.5000    0.0619
    6.5100    0.0605
    6.5200    0.0594
    6.5300    0.0589
    6.5400    0.0586
    6.5500    0.0581
    6.5600    0.0573
    6.5700    0.0565
    6.5800    0.0559
    6.5900    0.0555
    6.6000    0.0550
    6.6100    0.0544
    6.6200    0.0537
    6.6300    0.0533
    6.6400    0.0528
    6.6500    0.0522
    6.6600    0.0515
    6.6700    0.0511
    6.6800    0.0508
    6.6900    0.0506
    6.7000    0.0502
    6.7100    0.0495
    6.7200    0.0492
    6.7300    0.0493
    6.7400    0.0492
    6.7500    0.0485
    6.7600    0.0479
    6.7700    0.0477
    6.7800    0.0478
    6.7900    0.0474
    6.8000    0.0468
    6.8100    0.0465
    6.8200    0.0459
    6.8300    0.0454
    6.8400    0.0451
    6.8500    0.0446
    6.8600    0.0440
    6.8700    0.0435
    6.8800    0.0433
    6.8900    0.0423
    6.9000    0.0418
    6.9100    0.0416
    6.9200    0.0411
    6.9300    0.0409
    6.9400    0.0408
    6.9500    0.0405
    6.9600    0.0397
    6.9700    0.0391
    6.9800    0.0388
    6.9900    0.0385
    7.0000    0.0380
    7.0100    0.0372
    7.0200    0.0369
    7.0300    0.0365
    7.0400    0.0361
    7.0500    0.0357
    7.0600    0.0352
    7.0700    0.0351
    7.0800    0.0349
    7.0900    0.0343
    7.1000    0.0340
    7.1100    0.0339
    7.1200    0.0334
    7.1300    0.0332
    7.1400    0.0332
    7.1500    0.0327
    7.1600    0.0323
    7.1700    0.0321
    7.1800    0.0319
    7.1900    0.0316
    7.2000    0.0312
    7.2100    0.0307
    7.2200    0.0304
    7.2300    0.0300
    7.2400    0.0296
    7.2500    0.0294
    7.2600    0.0293
    7.2700    0.0290
    7.2800    0.0286
    7.2900    0.0283
    7.3000    0.0280
    7.3100    0.0275
    7.3200    0.0272
    7.3300    0.0272
    7.3400    0.0269
    7.3500    0.0267
    7.3600    0.0264
    7.3700    0.0260
    7.3800    0.0258
    7.3900    0.0256
    7.4000    0.0253
    7.4100    0.0251
    7.4200    0.0249
    7.4300    0.0248
    7.4400    0.0247
    7.4500    0.0246
    7.4600    0.0246
    7.4700    0.0244
    7.4800    0.0243
    7.4900    0.0244
    7.5000    0.0245
    7.5100    0.0249
    7.5200    0.0251
    7.5300    0.0246
    7.5400    0.0243
    7.5500    0.0242
    7.5600    0.0242
    7.5700    0.0239
    7.5800    0.0235
    7.5900    0.0232
    7.6000    0.0228
    7.6100    0.0226
    7.6200    0.0223
    7.6300    0.0218
    7.6400    0.0216
    7.6500    0.0213
    7.6600    0.0207
    7.6700    0.0203
    7.6800    0.0203
    7.6900    0.0201
    7.7000    0.0198
    7.7100    0.0195
    7.7200    0.0193
    7.7300    0.0192
    7.7400    0.0188
    7.7500    0.0185
    7.7600    0.0183
    7.7700    0.0183
    7.7800    0.0185
    7.7900    0.0187
    7.8000    0.0189
    7.8100    0.0189
    7.8200    0.0191
    7.8300    0.0189
    7.8400    0.0182
    7.8500    0.0183
    7.8600    0.0188
    7.8700    0.0188
    7.8800    0.0189
    7.8900    0.0193
    7.9000    0.0190
    7.9100    0.0187
    7.9200    0.0186
    7.9300    0.0187
    7.9400    0.0188
    7.9500    0.0191
    7.9600    0.0192
    7.9700    0.0190
    7.9800    0.0189
    7.9900    0.0183
    8.0000    0.0177
    8.0100    0.0174
    8.0200    0.0174
    8.0300    0.0176
    8.0400    0.0178
    8.0500    0.0173
    8.0600    0.0171
    8.0700    0.0171
    8.0800    0.0169
    8.0900    0.0164
    8.1000    0.0165
    8.1100    0.0167
    8.1200    0.0164
    8.1300    0.0163
    8.1400    0.0160
    8.1500    0.0158
    8.1600    0.0160
    8.1700    0.0160
    8.1800    0.0156
    8.1900    0.0155
    8.2000    0.0153
    8.2100    0.0153
    8.2200    0.0157
    8.2300    0.0166
    8.2400    0.0171
    8.2500    0.0170
    8.2600    0.0173
    8.2700    0.0169
    8.2800    0.0165
    8.2900    0.0165
    8.3000    0.0167
    8.3100    0.0169
    8.3200    0.0166
    8.3300    0.0167
    8.3400    0.0171
    8.3500    0.0166
    8.3600    0.0168
    8.3700    0.0169
    8.3800    0.0163
    8.3900    0.0162
    8.4000    0.0168
    8.4100    0.0170
    8.4200    0.0165
    8.4300    0.0160
    8.4400    0.0155
    8.4500    0.0156
    8.4600    0.0156
    8.4700    0.0154
    8.4800    0.0156
    8.4900    0.0162
    8.5000    0.0162
    8.5100    0.0156
    8.5200    0.0153
    8.5300    0.0144
    8.5400    0.0143
    8.5500    0.0143
    8.5600    0.0140
    8.5700    0.0137
    8.5800    0.0131
    8.5900    0.0125
    8.6000    0.0125
    8.6100    0.0126
    8.6200    0.0126
    8.6300    0.0116
    8.6400    0.0106
    8.6500    0.0098
    8.6600    0.0092
    8.6700    0.0091
    8.6800    0.0088
    8.6900    0.0088
    8.7000    0.0086
    8.7100    0.0082
    8.7200    0.0086
    8.7300    0.0086
    8.7400    0.0085
    8.7500    0.0093
    8.7600    0.0095
    8.7700    0.0095
    8.7800    0.0098
    8.7900    0.0100
    8.8000    0.0100
    8.8100    0.0102
    8.8200    0.0100
    8.8300    0.0102
    8.8400    0.0106
    8.8500    0.0114
    8.8600    0.0120
    8.8700    0.0117
    8.8800    0.0117
    8.8900    0.0117
    8.9000    0.0113
    8.9100    0.0109
    8.9200    0.0103
    8.9300    0.0102
    8.9400    0.0106
    8.9500    0.0106
    8.9600    0.0108
    8.9700    0.0105
    8.9800    0.0097
    8.9900    0.0093
    9.0000    0.0094
    9.0100    0.0093
    9.0200    0.0093
    9.0300    0.0094
    9.0400    0.0095
    9.0500    0.0096
    9.0600    0.0092
    9.0700    0.0088
    9.0800    0.0083
    9.0900    0.0082
    9.1000    0.0083
    9.1100    0.0084
    9.1200    0.0085
    9.1300    0.0083
    9.1400    0.0079
    9.1500    0.0074
    9.1600    0.0070
    9.1700    0.0069
    9.1800    0.0070
    9.1900    0.0075
    9.2000    0.0080
    9.2100    0.0084
    9.2200    0.0085
    9.2300    0.0080
    9.2400    0.0077
    9.2500    0.0078
    9.2600    0.0078
    9.2700    0.0074
    9.2800    0.0067
    9.2900    0.0065
    9.3000    0.0065
    9.3100    0.0067
    9.3200    0.0068
    9.3300    0.0066
    9.3400    0.0062
    9.3500    0.0063
    9.3600    0.0065
    9.3700    0.0064
    9.3800    0.0067
    9.3900    0.0066
    9.4000    0.0063
    9.4100    0.0063
    9.4200    0.0062
    9.4300    0.0057
    9.4400    0.0055
    9.4500    0.0058
    9.4600    0.0062
    9.4700    0.0066
    9.4800    0.0069
    9.4900    0.0068
    9.5000    0.0071
    9.5100    0.0074
    9.5200    0.0075
    9.5300    0.0074
    9.5400    0.0072
    9.5500    0.0074
    9.5600    0.0075
    9.5700    0.0079
    9.5800    0.0080
    9.5900    0.0080
    9.6000    0.0082
    9.6100    0.0080
    9.6200    0.0076
    9.6300    0.0070
    9.6400    0.0067
    9.6500    0.0065
    9.6600    0.0066
    9.6700    0.0070
    9.6800    0.0066
    9.6900    0.0066
    9.7000    0.0065
    9.7100    0.0062
    9.7200    0.0058
    9.7300    0.0055
    9.7400    0.0053
    9.7500    0.0052
    9.7600    0.0055
    9.7700    0.0057
    9.7800    0.0057
    9.7900    0.0054
    9.8000    0.0053
    9.8100    0.0057
    9.8200    0.0051
    9.8300    0.0047
    9.8400    0.0046
    9.8500    0.0040
    9.8600    0.0040
    9.8700    0.0040
    9.8800    0.0040
    9.8900    0.0040
    9.9000    0.0037
    9.9100    0.0037
    9.9200    0.0037
    9.9300    0.0032
    9.9400    0.0032
    9.9500    0.0033
    9.9600    0.0032
    9.9700    0.0031
    9.9800    0.0030
    9.9900    0.0027
   10.0000    0.0026
    };

==> Data/Oscillator/sigma3/E_mah_dist_varn.tex <==
    \addplot[
    thick,
    dotted,
    black
    ]
    table {
         0         0
    0.0100    0.0000
    0.0200    0.0000
    0.0300    0.0000
    0.0400    0.0000
    0.0500    0.0000
    0.0600    0.0000
    0.0700    0.0000
    0.0800    0.0001
    0.0900    0.0001
    0.1000    0.0002
    0.1100    0.0003
    0.1200    0.0004
    0.1300    0.0005
    0.1400    0.0007
    0.1500    0.0010
    0.1600    0.0013
    0.1700    0.0017
    0.1800    0.0021
    0.1900    0.0027
    0.2000    0.0033
    0.2100    0.0041
    0.2200    0.0049
    0.2300    0.0058
    0.2400    0.0069
    0.2500    0.0082
    0.2600    0.0098
    0.2700    0.0114
    0.2800    0.0130
    0.2900    0.0152
    0.3000    0.0174
    0.3100    0.0199
    0.3200    0.0228
    0.3300    0.0257
    0.3400    0.0289
    0.3500    0.0323
    0.3600    0.0353
    0.3700    0.0391
    0.3800    0.0442
    0.3900    0.0497
    0.4000    0.0553
    0.4100    0.0616
    0.4200    0.0684
    0.4300    0.0755
    0.4400    0.0817
    0.4500    0.0887
    0.4600    0.0972
    0.4700    0.1052
    0.4800    0.1129
    0.4900    0.1215
    0.5000    0.1306
    0.5100    0.1397
    0.5200    0.1502
    0.5300    0.1614
    0.5400    0.1727
    0.5500    0.1858
    0.5600    0.1986
    0.5700    0.2109
    0.5800    0.2246
    0.5900    0.2386
    0.6000    0.2518
    0.6100    0.2653
    0.6200    0.2802
    0.6300    0.2954
    0.6400    0.3110
    0.6500    0.3284
    0.6600    0.3455
    0.6700    0.3597
    0.6800    0.3767
    0.6900    0.3930
    0.7000    0.4087
    0.7100    0.4282
    0.7200    0.4486
    0.7300    0.4702
    0.7400    0.4923
    0.7500    0.5134
    0.7600    0.5300
    0.7700    0.5468
    0.7800    0.5658
    0.7900    0.5819
    0.8000    0.6053
    0.8100    0.6319
    0.8200    0.6523
    0.8300    0.6715
    0.8400    0.6940
    0.8500    0.7212
    0.8600    0.7429
    0.8700    0.7633
    0.8800    0.7845
    0.8900    0.8068
    0.9000    0.8355
    0.9100    0.8596
    0.9200    0.8770
    0.9300    0.8920
    0.9400    0.9140
    0.9500    0.9437
    0.9600    0.9726
    0.9700    0.9980
    0.9800    1.0219
    0.9900    1.0414
    1.0000    1.0626
    1.0100    1.0942
    1.0200    1.1200
    1.0300    1.1364
    1.0400    1.1561
    1.0500    1.1843
    1.0600    1.2084
    1.0700    1.2343
    1.0800    1.2604
    1.0900    1.2775
    1.1000    1.2935
    1.1100    1.3194
    1.1200    1.3470
    1.1300    1.3692
    1.1400    1.3837
    1.1500    1.3930
    1.1600    1.4108
    1.1700    1.4249
    1.1800    1.4422
    1.1900    1.4668
    1.2000    1.4811
    1.2100    1.4887
    1.2200    1.4995
    1.2300    1.5129
    1.2400    1.5315
    1.2500    1.5477
    1.2600    1.5649
    1.2700    1.5831
    1.2800    1.5963
    1.2900    1.6073
    1.3000    1.6208
    1.3100    1.6370
    1.3200    1.6461
    1.3300    1.6622
    1.3400    1.6814
    1.3500    1.6887
    1.3600    1.6965
    1.3700    1.7129
    1.3800    1.7260
    1.3900    1.7392
    1.4000    1.7523
    1.4100    1.7641
    1.4200    1.7781
    1.4300    1.7897
    1.4400    1.7947
    1.4500    1.8012
    1.4600    1.8044
    1.4700    1.8177
    1.4800    1.8408
    1.4900    1.8511
    1.5000    1.8639
    1.5100    1.8838
    1.5200    1.8967
    1.5300    1.9009
    1.5400    1.9079
    1.5500    1.9143
    1.5600    1.9255
    1.5700    1.9407
    1.5800    1.9510
    1.5900    1.9624
    1.6000    1.9737
    1.6100    1.9690
    1.6200    1.9696
    1.6300    1.9770
    1.6400    1.9863
    1.6500    1.9920
    1.6600    1.9966
    1.6700    2.0071
    1.6800    2.0146
    1.6900    2.0216
    1.7000    2.0240
    1.7100    2.0322
    1.7200    2.0244
    1.7300    2.0190
    1.7400    2.0310
    1.7500    2.0225
    1.7600    2.0214
    1.7700    2.0295
    1.7800    2.0356
    1.7900    2.0407
    1.8000    2.0382
    1.8100    2.0385
    1.8200    2.0403
    1.8300    2.0456
    1.8400    2.0398
    1.8500    2.0455
    1.8600    2.0670
    1.8700    2.0726
    1.8800    2.0752
    1.8900    2.0810
    1.9000    2.0896
    1.9100    2.1016
    1.9200    2.1073
    1.9300    2.1123
    1.9400    2.1199
    1.9500    2.1247
    1.9600    2.1317
    1.9700    2.1286
    1.9800    2.1273
    1.9900    2.1242
    2.0000    2.1153
    2.0100    2.1239
    2.0200    2.1321
    2.0300    2.1293
    2.0400    2.1188
    2.0500    2.1126
    2.0600    2.1103
    2.0700    2.1036
    2.0800    2.1058
    2.0900    2.1124
    2.1000    2.1196
    2.1100    2.1280
    2.1200    2.1219
    2.1300    2.1130
    2.1400    2.0978
    2.1500    2.0825
    2.1600    2.0910
    2.1700    2.0908
    2.1800    2.0724
    2.1900    2.0676
    2.2000    2.0670
    2.2100    2.0587
    2.2200    2.0508
    2.2300    2.0429
    2.2400    2.0367
    2.2500    2.0345
    2.2600    2.0296
    2.2700    2.0299
    2.2800    2.0229
    2.2900    2.0125
    2.3000    2.0061
    2.3100    2.0016
    2.3200    2.0066
    2.3300    2.0062
    2.3400    2.0033
    2.3500    1.9948
    2.3600    1.9823
    2.3700    1.9726
    2.3800    1.9713
    2.3900    1.9777
    2.4000    1.9746
    2.4100    1.9702
    2.4200    1.9620
    2.4300    1.9442
    2.4400    1.9368
    2.4500    1.9318
    2.4600    1.9158
    2.4700    1.9045
    2.4800    1.8921
    2.4900    1.8750
    2.5000    1.8658
    2.5100    1.8563
    2.5200    1.8460
    2.5300    1.8424
    2.5400    1.8373
    2.5500    1.8293
    2.5600    1.8266
    2.5700    1.8145
    2.5800    1.8019
    2.5900    1.7846
    2.6000    1.7687
    2.6100    1.7644
    2.6200    1.7507
    2.6300    1.7279
    2.6400    1.7099
    2.6500    1.7088
    2.6600    1.7022
    2.6700    1.6982
    2.6800    1.6999
    2.6900    1.6938
    2.7000    1.6817
    2.7100    1.6638
    2.7200    1.6538
    2.7300    1.6448
    2.7400    1.6364
    2.7500    1.6310
    2.7600    1.6144
    2.7700    1.6006
    2.7800    1.5961
    2.7900    1.5936
    2.8000    1.5872
    2.8100    1.5740
    2.8200    1.5546
    2.8300    1.5410
    2.8400    1.5348
    2.8500    1.5314
    2.8600    1.5219
    2.8700    1.5088
    2.8800    1.5073
    2.8900    1.4945
    2.9000    1.4771
    2.9100    1.4659
    2.9200    1.4613
    2.9300    1.4584
    2.9400    1.4473
    2.9500    1.4439
    2.9600    1.4427
    2.9700    1.4387
    2.9800    1.4313
    2.9900    1.4268
    3.0000    1.4216
    3.0100    1.4033
    3.0200    1.3920
    3.0300    1.3878
    3.0400    1.3797
    3.0500    1.3672
    3.0600    1.3548
    3.0700    1.3454
    3.0800    1.3393
    3.0900    1.3359
    3.1000    1.3284
    3.1100    1.3139
    3.1200    1.2987
    3.1300    1.2957
    3.1400    1.2921
    3.1500    1.2835
    3.1600    1.2786
    3.1700    1.2731
    3.1800    1.2703
    3.1900    1.2675
    3.2000    1.2641
    3.2100    1.2615
    3.2200    1.2552
    3.2300    1.2470
    3.2400    1.2403
    3.2500    1.2347
    3.2600    1.2282
    3.2700    1.2199
    3.2800    1.2072
    3.2900    1.1934
    3.3000    1.1862
    3.3100    1.1784
    3.3200    1.1694
    3.3300    1.1689
    3.3400    1.1752
    3.3500    1.1813
    3.3600    1.1797
    3.3700    1.1743
    3.3800    1.1717
    3.3900    1.1661
    3.4000    1.1601
    3.4100    1.1575
    3.4200    1.1497
    3.4300    1.1383
    3.4400    1.1203
    3.4500    1.1039
    3.4600    1.0963
    3.4700    1.0903
    3.4800    1.0858
    3.4900    1.0781
    3.5000    1.0765
    3.5100    1.0762
    3.5200    1.0659
    3.5300    1.0580
    3.5400    1.0515
    3.5500    1.0391
    3.5600    1.0258
    3.5700    1.0118
    3.5800    1.0093
    3.5900    1.0116
    3.6000    1.0021
    3.6100    0.9905
    3.6200    0.9823
    3.6300    0.9741
    3.6400    0.9619
    3.6500    0.9504
    3.6600    0.9454
    3.6700    0.9407
    3.6800    0.9346
    3.6900    0.9253
    3.7000    0.9141
    3.7100    0.9045
    3.7200    0.8951
    3.7300    0.8887
    3.7400    0.8827
    3.7500    0.8739
    3.7600    0.8702
    3.7700    0.8672
    3.7800    0.8559
    3.7900    0.8473
    3.8000    0.8366
    3.8100    0.8231
    3.8200    0.8164
    3.8300    0.8109
    3.8400    0.8050
    3.8500    0.7984
    3.8600    0.7885
    3.8700    0.7805
    3.8800    0.7741
    3.8900    0.7613
    3.9000    0.7479
    3.9100    0.7369
    3.9200    0.7302
    3.9300    0.7275
    3.9400    0.7213
    3.9500    0.7138
    3.9600    0.7111
    3.9700    0.7131
    3.9800    0.7066
    3.9900    0.6999
    4.0000    0.6895
    4.0100    0.6831
    4.0200    0.6821
    4.0300    0.6730
    4.0400    0.6692
    4.0500    0.6631
    4.0600    0.6577
    4.0700    0.6514
    4.0800    0.6421
    4.0900    0.6391
    4.1000    0.6424
    4.1100    0.6424
    4.1200    0.6333
    4.1300    0.6238
    4.1400    0.6178
    4.1500    0.6091
    4.1600    0.6052
    4.1700    0.5988
    4.1800    0.5910
    4.1900    0.5873
    4.2000    0.5818
    4.2100    0.5755
    4.2200    0.5739
    4.2300    0.5690
    4.2400    0.5583
    4.2500    0.5479
    4.2600    0.5347
    4.2700    0.5264
    4.2800    0.5224
    4.2900    0.5223
    4.3000    0.5200
    4.3100    0.5138
    4.3200    0.5053
    4.3300    0.4998
    4.3400    0.4950
    4.3500    0.4871
    4.3600    0.4836
    4.3700    0.4783
    4.3800    0.4704
    4.3900    0.4658
    4.4000    0.4575
    4.4100    0.4474
    4.4200    0.4420
    4.4300    0.4366
    4.4400    0.4308
    4.4500    0.4256
    4.4600    0.4194
    4.4700    0.4146
    4.4800    0.4123
    4.4900    0.4085
    4.5000    0.3995
    4.5100    0.3919
    4.5200    0.3899
    4.5300    0.3871
    4.5400    0.3833
    4.5500    0.3802
    4.5600    0.3752
    4.5700    0.3699
    4.5800    0.3666
    4.5900    0.3635
    4.6000    0.3617
    4.6100    0.3604
    4.6200    0.3593
    4.6300    0.3577
    4.6400    0.3555
    4.6500    0.3539
    4.6600    0.3507
    4.6700    0.3486
    4.6800    0.3464
    4.6900    0.3410
    4.7000    0.3382
    4.7100    0.3334
    4.7200    0.3297
    4.7300    0.3286
    4.7400    0.3269
    4.7500    0.3254
    4.7600    0.3234
    4.7700    0.3221
    4.7800    0.3196
    4.7900    0.3179
    4.8000    0.3188
    4.8100    0.3171
    4.8200    0.3094
    4.8300    0.2993
    4.8400    0.2934
    4.8500    0.2907
    4.8600    0.2875
    4.8700    0.2842
    4.8800    0.2812
    4.8900    0.2815
    4.9000    0.2803
    4.9100    0.2775
    4.9200    0.2788
    4.9300    0.2742
    4.9400    0.2674
    4.9500    0.2645
    4.9600    0.2584
    4.9700    0.2557
    4.9800    0.2543
    4.9900    0.2493
    5.0000    0.2455
    5.0100    0.2418
    5.0200    0.2392
    5.0300    0.2356
    5.0400    0.2323
    5.0500    0.2313
    5.0600    0.2284
    5.0700    0.2223
    5.0800    0.2178
    5.0900    0.2161
    5.1000    0.2132
    5.1100    0.2087
    5.1200    0.2037
    5.1300    0.1996
    5.1400    0.1974
    5.1500    0.1945
    5.1600    0.1914
    5.1700    0.1873
    5.1800    0.1845
    5.1900    0.1836
    5.2000    0.1792
    5.2100    0.1759
    5.2200    0.1745
    5.2300    0.1733
    5.2400    0.1718
    5.2500    0.1697
    5.2600    0.1672
    5.2700    0.1655
    5.2800    0.1638
    5.2900    0.1617
    5.3000    0.1602
    5.3100    0.1587
    5.3200    0.1578
    5.3300    0.1529
    5.3400    0.1449
    5.3500    0.1396
    5.3600    0.1362
    5.3700    0.1345
    5.3800    0.1338
    5.3900    0.1326
    5.4000    0.1307
    5.4100    0.1279
    5.4200    0.1256
    5.4300    0.1238
    5.4400    0.1228
    5.4500    0.1216
    5.4600    0.1190
    5.4700    0.1161
    5.4800    0.1140
    5.4900    0.1118
    5.5000    0.1092
    5.5100    0.1082
    5.5200    0.1076
    5.5300    0.1059
    5.5400    0.1057
    5.5500    0.1061
    5.5600    0.1055
    5.5700    0.1035
    5.5800    0.1015
    5.5900    0.1000
    5.6000    0.0986
    5.6100    0.0991
    5.6200    0.0987
    5.6300    0.0976
    5.6400    0.0963
    5.6500    0.0929
    5.6600    0.0909
    5.6700    0.0893
    5.6800    0.0865
    5.6900    0.0856
    5.7000    0.0851
    5.7100    0.0836
    5.7200    0.0820
    5.7300    0.0801
    5.7400    0.0783
    5.7500    0.0764
    5.7600    0.0752
    5.7700    0.0739
    5.7800    0.0735
    5.7900    0.0741
    5.8000    0.0727
    5.8100    0.0713
    5.8200    0.0706
    5.8300    0.0686
    5.8400    0.0672
    5.8500    0.0671
    5.8600    0.0666
    5.8700    0.0656
    5.8800    0.0644
    5.8900    0.0639
    5.9000    0.0640
    5.9100    0.0639
    5.9200    0.0631
    5.9300    0.0625
    5.9400    0.0618
    5.9500    0.0616
    5.9600    0.0608
    5.9700    0.0605
    5.9800    0.0607
    5.9900    0.0592
    6.0000    0.0585
    6.0100    0.0581
    6.0200    0.0571
    6.0300    0.0564
    6.0400    0.0559
    6.0500    0.0549
    6.0600    0.0544
    6.0700    0.0537
    6.0800    0.0521
    6.0900    0.0509
    6.1000    0.0500
    6.1100    0.0498
    6.1200    0.0493
    6.1300    0.0489
    6.1400    0.0481
    6.1500    0.0466
    6.1600    0.0457
    6.1700    0.0450
    6.1800    0.0453
    6.1900    0.0458
    6.2000    0.0455
    6.2100    0.0439
    6.2200    0.0422
    6.2300    0.0414
    6.2400    0.0409
    6.2500    0.0405
    6.2600    0.0395
    6.2700    0.0389
    6.2800    0.0379
    6.2900    0.0371
    6.3000    0.0372
    6.3100    0.0366
    6.3200    0.0367
    6.3300    0.0366
    6.3400    0.0358
    6.3500    0.0354
    6.3600    0.0346
    6.3700    0.0337
    6.3800    0.0328
    6.3900    0.0323
    6.4000    0.0320
    6.4100    0.0315
    6.4200    0.0313
    6.4300    0.0314
    6.4400    0.0314
    6.4500    0.0311
    6.4600    0.0302
    6.4700    0.0292
    6.4800    0.0288
    6.4900    0.0287
    6.5000    0.0282
    6.5100    0.0269
    6.5200    0.0261
    6.5300    0.0258
    6.5400    0.0259
    6.5500    0.0256
    6.5600    0.0251
    6.5700    0.0245
    6.5800    0.0242
    6.5900    0.0240
    6.6000    0.0238
    6.6100    0.0234
    6.6200    0.0230
    6.6300    0.0229
    6.6400    0.0227
    6.6500    0.0224
    6.6600    0.0219
    6.6700    0.0217
    6.6800    0.0218
    6.6900    0.0218
    6.7000    0.0217
    6.7100    0.0213
    6.7200    0.0212
    6.7300    0.0217
    6.7400    0.0219
    6.7500    0.0215
    6.7600    0.0211
    6.7700    0.0211
    6.7800    0.0216
    6.7900    0.0215
    6.8000    0.0211
    6.8100    0.0211
    6.8200    0.0207
    6.8300    0.0204
    6.8400    0.0204
    6.8500    0.0201
    6.8600    0.0197
    6.8700    0.0195
    6.8800    0.0196
    6.8900    0.0187
    6.9000    0.0183
    6.9100    0.0185
    6.9200    0.0182
    6.9300    0.0183
    6.9400    0.0184
    6.9500    0.0184
    6.9600    0.0177
    6.9700    0.0173
    6.9800    0.0173
    6.9900    0.0171
    7.0000    0.0168
    7.0100    0.0162
    7.0200    0.0161
    7.0300    0.0159
    7.0400    0.0158
    7.0500    0.0155
    7.0600    0.0153
    7.0700    0.0154
    7.0800    0.0154
    7.0900    0.0150
    7.1000    0.0149
    7.1100    0.0151
    7.1200    0.0148
    7.1300    0.0149
    7.1400    0.0150
    7.1500    0.0147
    7.1600    0.0145
    7.1700    0.0145
    7.1800    0.0145
    7.1900    0.0144
    7.2000    0.0142
    7.2100    0.0139
    7.2200    0.0139
    7.2300    0.0136
    7.2400    0.0133
    7.2500    0.0134
    7.2600    0.0135
    7.2700    0.0134
    7.2800    0.0132
    7.2900    0.0130
    7.3000    0.0129
    7.3100    0.0125
    7.3200    0.0124
    7.3300    0.0126
    7.3400    0.0126
    7.3500    0.0126
    7.3600    0.0124
    7.3700    0.0121
    7.3800    0.0121
    7.3900    0.0121
    7.4000    0.0120
    7.4100    0.0119
    7.4200    0.0119
    7.4300    0.0120
    7.4400    0.0122
    7.4500    0.0123
    7.4600    0.0125
    7.4700    0.0125
    7.4800    0.0126
    7.4900    0.0129
    7.5000    0.0133
    7.5100    0.0140
    7.5200    0.0145
    7.5300    0.0141
    7.5400    0.0139
    7.5500    0.0140
    7.5600    0.0143
    7.5700    0.0141
    7.5800    0.0138
    7.5900    0.0136
    7.6000    0.0132
    7.6100    0.0132
    7.6200    0.0130
    7.6300    0.0126
    7.6400    0.0124
    7.6500    0.0123
    7.6600    0.0117
    7.6700    0.0114
    7.6800    0.0115
    7.6900    0.0115
    7.7000    0.0113
    7.7100    0.0111
    7.7200    0.0111
    7.7300    0.0110
    7.7400    0.0107
    7.7500    0.0106
    7.7600    0.0105
    7.7700    0.0107
    7.7800    0.0110
    7.7900    0.0115
    7.8000    0.0120
    7.8100    0.0122
    7.8200    0.0126
    7.8300    0.0125
    7.8400    0.0117
    7.8500    0.0120
    7.8600    0.0128
    7.8700    0.0130
    7.8800    0.0133
    7.8900    0.0140
    7.9000    0.0137
    7.9100    0.0134
    7.9200    0.0135
    7.9300    0.0137
    7.9400    0.0141
    7.9500    0.0146
    7.9600    0.0148
    7.9700    0.0148
    7.9800    0.0147
    7.9900    0.0141
    8.0000    0.0134
    8.0100    0.0132
    8.0200    0.0133
    8.0300    0.0137
    8.0400    0.0141
    8.0500    0.0136
    8.0600    0.0134
    8.0700    0.0136
    8.0800    0.0135
    8.0900    0.0129
    8.1000    0.0131
    8.1100    0.0135
    8.1200    0.0132
    8.1300    0.0133
    8.1400    0.0130
    8.1500    0.0128
    8.1600    0.0131
    8.1700    0.0133
    8.1800    0.0130
    8.1900    0.0129
    8.2000    0.0127
    8.2100    0.0128
    8.2200    0.0135
    8.2300    0.0148
    8.2400    0.0155
    8.2500    0.0155
    8.2600    0.0160
    8.2700    0.0156
    8.2800    0.0151
    8.2900    0.0152
    8.3000    0.0156
    8.3100    0.0160
    8.3200    0.0156
    8.3300    0.0159
    8.3400    0.0165
    8.3500    0.0160
    8.3600    0.0162
    8.3700    0.0165
    8.3800    0.0158
    8.3900    0.0158
    8.4000    0.0167
    8.4100    0.0170
    8.4200    0.0163
    8.4300    0.0158
    8.4400    0.0152
    8.4500    0.0153
    8.4600    0.0155
    8.4700    0.0153
    8.4800    0.0156
    8.4900    0.0164
    8.5000    0.0165
    8.5100    0.0158
    8.5200    0.0155
    8.5300    0.0143
    8.5400    0.0142
    8.5500    0.0144
    8.5600    0.0140
    8.5700    0.0137
    8.5800    0.0130
    8.5900    0.0122
    8.6000    0.0122
    8.6100    0.0125
    8.6200    0.0125
    8.6300    0.0113
    8.6400    0.0100
    8.6500    0.0090
    8.6600    0.0082
    8.6700    0.0082
    8.6800    0.0079
    8.6900    0.0079
    8.7000    0.0077
    8.7100    0.0073
    8.7200    0.0078
    8.7300    0.0078
    8.7400    0.0079
    8.7500    0.0089
    8.7600    0.0092
    8.7700    0.0092
    8.7800    0.0098
    8.7900    0.0100
    8.8000    0.0101
    8.8100    0.0103
    8.8200    0.0102
    8.8300    0.0104
    8.8400    0.0111
    8.8500    0.0121
    8.8600    0.0130
    8.8700    0.0126
    8.8800    0.0126
    8.8900    0.0127
    8.9000    0.0122
    8.9100    0.0117
    8.9200    0.0110
    8.9300    0.0108
    8.9400    0.0113
    8.9500    0.0115
    8.9600    0.0117
    8.9700    0.0114
    8.9800    0.0104
    8.9900    0.0099
    9.0000    0.0100
    9.0100    0.0099
    9.0200    0.0099
    9.0300    0.0101
    9.0400    0.0102
    9.0500    0.0104
    9.0600    0.0099
    9.0700    0.0093
    9.0800    0.0087
    9.0900    0.0086
    9.1000    0.0088
    9.1100    0.0090
    9.1200    0.0092
    9.1300    0.0089
    9.1400    0.0084
    9.1500    0.0077
    9.1600    0.0073
    9.1700    0.0072
    9.1800    0.0074
    9.1900    0.0081
    9.2000    0.0087
    9.2100    0.0092
    9.2200    0.0094
    9.2300    0.0087
    9.2400    0.0084
    9.2500    0.0084
    9.2600    0.0085
    9.2700    0.0080
    9.2800    0.0071
    9.2900    0.0069
    9.3000    0.0070
    9.3100    0.0072
    9.3200    0.0074
    9.3300    0.0070
    9.3400    0.0065
    9.3500    0.0067
    9.3600    0.0070
    9.3700    0.0069
    9.3800    0.0073
    9.3900    0.0071
    9.4000    0.0068
    9.4100    0.0068
    9.4200    0.0067
    9.4300    0.0060
    9.4400    0.0058
    9.4500    0.0062
    9.4600    0.0068
    9.4700    0.0072
    9.4800    0.0077
    9.4900    0.0075
    9.5000    0.0079
    9.5100    0.0084
    9.5200    0.0085
    9.5300    0.0083
    9.5400    0.0082
    9.5500    0.0084
    9.5600    0.0085
    9.5700    0.0090
    9.5800    0.0092
    9.5900    0.0092
    9.6000    0.0094
    9.6100    0.0092
    9.6200    0.0087
    9.6300    0.0079
    9.6400    0.0075
    9.6500    0.0072
    9.6600    0.0075
    9.6700    0.0079
    9.6800    0.0074
    9.6900    0.0075
    9.7000    0.0073
    9.7100    0.0069
    9.7200    0.0064
    9.7300    0.0060
    9.7400    0.0058
    9.7500    0.0057
    9.7600    0.0061
    9.7700    0.0064
    9.7800    0.0063
    9.7900    0.0060
    9.8000    0.0059
    9.8100    0.0063
    9.8200    0.0056
    9.8300    0.0051
    9.8400    0.0049
    9.8500    0.0042
    9.8600    0.0042
    9.8700    0.0043
    9.8800    0.0043
    9.8900    0.0042
    9.9000    0.0038
    9.9100    0.0039
    9.9200    0.0038
    9.9300    0.0033
    9.9400    0.0033
    9.9500    0.0033
    9.9600    0.0033
    9.9700    0.0032
    9.9800    0.0029
    9.9900    0.0026
   10.0000    0.0025
    };

==> Data/Oscillator/sigma3/kf_en_pos.tex <==
    \addplot[
    thick,
    dashed,
    cyan
    ]
    table {
         0    1.0000
    0.0100    0.9972
    0.0200    0.9928
    0.0300    0.9839
    0.0400    0.9791
    0.0500    0.9755
    0.0600    0.9713
    0.0700    0.9673
    0.0800    0.9638
    0.0900    0.9551
    0.1000    0.9462
    0.1100    0.9478
    0.1200    0.9492
    0.1300    0.9489
    0.1400    0.9460
    0.1500    0.9417
    0.1600    0.9386
    0.1700    0.9354
    0.1800    0.9301
    0.1900    0.9240
    0.2000    0.9196
    0.2100    0.9145
    0.2200    0.9106
    0.2300    0.9131
    0.2400    0.9109
    0.2500    0.9048
    0.2600    0.8990
    0.2700    0.8942
    0.2800    0.8957
    0.2900    0.8905
    0.3000    0.8871
    0.3100    0.8850
    0.3200    0.8790
    0.3300    0.8776
    0.3400    0.8751
    0.3500    0.8740
    0.3600    0.8773
    0.3700    0.8774
    0.3800    0.8705
    0.3900    0.8635
    0.4000    0.8584
    0.4100    0.8524
    0.4200    0.8462
    0.4300    0.8406
    0.4400    0.8400
    0.4500    0.8380
    0.4600    0.8322
    0.4700    0.8295
    0.4800    0.8286
    0.4900    0.8265
    0.5000    0.8241
    0.5100    0.8226
    0.5200    0.8190
    0.5300    0.8150
    0.5400    0.8116
    0.5500    0.8060
    0.5600    0.8019
    0.5700    0.7990
    0.5800    0.7948
    0.5900    0.7909
    0.6000    0.7884
    0.6100    0.7860
    0.6200    0.7825
    0.6300    0.7791
    0.6400    0.7757
    0.6500    0.7709
    0.6600    0.7668
    0.6700    0.7655
    0.6800    0.7620
    0.6900    0.7594
    0.7000    0.7574
    0.7100    0.7528
    0.7200    0.7480
    0.7300    0.7426
    0.7400    0.7372
    0.7500    0.7326
    0.7600    0.7307
    0.7700    0.7287
    0.7800    0.7256
    0.7900    0.7241
    0.8000    0.7191
    0.8100    0.7126
    0.8200    0.7092
    0.8300    0.7063
    0.8400    0.7021
    0.8500    0.6960
    0.8600    0.6923
    0.8700    0.6890
    0.8800    0.6855
    0.8900    0.6816
    0.9000    0.6755
    0.9100    0.6710
    0.9200    0.6688
    0.9300    0.6674
    0.9400    0.6637
    0.9500    0.6576
    0.9600    0.6518
    0.9700    0.6470
    0.9800    0.6428
    0.9900    0.6397
    1.0000    0.6361
    1.0100    0.6298
    1.0200    0.6250
    1.0300    0.6226
    1.0400    0.6193
    1.0500    0.6139
    1.0600    0.6095
    1.0700    0.6047
    1.0800    0.5998
    1.0900    0.5969
    1.1000    0.5942
    1.1100    0.5894
    1.1200    0.5841
    1.1300    0.5800
    1.1400    0.5774
    1.1500    0.5758
    1.1600    0.5725
    1.1700    0.5698
    1.1800    0.5665
    1.1900    0.5618
    1.2000    0.5590
    1.2100    0.5573
    1.2200    0.5551
    1.2300    0.5523
    1.2400    0.5486
    1.2500    0.5453
    1.2600    0.5418
    1.2700    0.5380
    1.2800    0.5351
    1.2900    0.5325
    1.3000    0.5295
    1.3100    0.5259
    1.3200    0.5235
    1.3300    0.5200
    1.3400    0.5159
    1.3500    0.5137
    1.3600    0.5113
    1.3700    0.5076
    1.3800    0.5044
    1.3900    0.5011
    1.4000    0.4979
    1.4100    0.4947
    1.4200    0.4913
    1.4300    0.4881
    1.4400    0.4859
    1.4500    0.4834
    1.4600    0.4813
    1.4700    0.4779
    1.4800    0.4731
    1.4900    0.4700
    1.5000    0.4665
    1.5100    0.4621
    1.5200    0.4586
    1.5300    0.4561
    1.5400    0.4533
    1.5500    0.4506
    1.5600    0.4472
    1.5700    0.4433
    1.5800    0.4400
    1.5900    0.4366
    1.6000    0.4331
    1.6100    0.4315
    1.6200    0.4293
    1.6300    0.4263
    1.6400    0.4231
    1.6500    0.4202
    1.6600    0.4175
    1.6700    0.4140
    1.6800    0.4109
    1.6900    0.4079
    1.7000    0.4053
    1.7100    0.4021
    1.7200    0.4007
    1.7300    0.3990
    1.7400    0.3953
    1.7500    0.3939
    1.7600    0.3917
    1.7700    0.3885
    1.7800    0.3855
    1.7900    0.3826
    1.8000    0.3805
    1.8100    0.3781
    1.8200    0.3755
    1.8300    0.3726
    1.8400    0.3708
    1.8500    0.3678
    1.8600    0.3632
    1.8700    0.3602
    1.8800    0.3575
    1.8900    0.3544
    1.9000    0.3511
    1.9100    0.3474
    1.9200    0.3444
    1.9300    0.3414
    1.9400    0.3382
    1.9500    0.3352
    1.9600    0.3321
    1.9700    0.3298
    1.9800    0.3275
    1.9900    0.3253
    2.0000    0.3236
    2.0100    0.3203
    2.0200    0.3170
    2.0300    0.3148
    2.0400    0.3132
    2.0500    0.3113
    2.0600    0.3091
    2.0700    0.3072
    2.0800    0.3045
    2.0900    0.3014
    2.1000    0.2983
    2.1100    0.2951
    2.1200    0.2931
    2.1300    0.2915
    2.1400    0.2904
    2.1500    0.2893
    2.1600    0.2861
    2.1700    0.2837
    2.1800    0.2829
    2.1900    0.2809
    2.2000    0.2785
    2.2100    0.2769
    2.2200    0.2752
    2.2300    0.2735
    2.2400    0.2716
    2.2500    0.2695
    2.2600    0.2675
    2.2700    0.2652
    2.2800    0.2634
    2.2900    0.2620
    2.3000    0.2602
    2.3100    0.2583
    2.3200    0.2556
    2.3300    0.2533
    2.3400    0.2512
    2.3500    0.2497
    2.3600    0.2485
    2.3700    0.2470
    2.3800    0.2449
    2.3900    0.2421
    2.4000    0.2401
    2.4100    0.2382
    2.4200    0.2367
    2.4300    0.2360
    2.4400    0.2344
    2.4500    0.2326
    2.4600    0.2317
    2.4700    0.2305
    2.4800    0.2294
    2.4900    0.2287
    2.5000    0.2273
    2.5100    0.2260
    2.5200    0.2248
    2.5300    0.2230
    2.5400    0.2213
    2.5500    0.2199
    2.5600    0.2180
    2.5700    0.2170
    2.5800    0.2160
    2.5900    0.2154
    2.6000    0.2147
    2.6100    0.2130
    2.6200    0.2122
    2.6300    0.2121
    2.6400    0.2117
    2.6500    0.2098
    2.6600    0.2084
    2.6700    0.2068
    2.6800    0.2047
    2.6900    0.2033
    2.7000    0.2023
    2.7100    0.2019
    2.7200    0.2009
    2.7300    0.1997
    2.7400    0.1986
    2.7500    0.1971
    2.7600    0.1967
    2.7700    0.1960
    2.7800    0.1945
    2.7900    0.1929
    2.8000    0.1916
    2.8100    0.1909
    2.8200    0.1907
    2.8300    0.1901
    2.8400    0.1888
    2.8500    0.1873
    2.8600    0.1863
    2.8700    0.1857
    2.8800    0.1841
    2.8900    0.1834
    2.9000    0.1831
    2.9100    0.1824
    2.9200    0.1810
    2.9300    0.1796
    2.9400    0.1788
    2.9500    0.1774
    2.9600    0.1758
    2.9700    0.1744
    2.9800    0.1734
    2.9900    0.1720
    3.0000    0.1708
    3.0100    0.1707
    3.0200    0.1700
    3.0300    0.1687
    3.0400    0.1678
    3.0500    0.1672
    3.0600    0.1667
    3.0700    0.1659
    3.0800    0.1648
    3.0900    0.1634
    3.1000    0.1625
    3.1100    0.1622
    3.1200    0.1619
    3.1300    0.1606
    3.1400    0.1593
    3.1500    0.1585
    3.1600    0.1573
    3.1700    0.1562
    3.1800    0.1549
    3.1900    0.1536
    3.2000    0.1523
    3.2100    0.1510
    3.2200    0.1500
    3.2300    0.1492
    3.2400    0.1482
    3.2500    0.1472
    3.2600    0.1462
    3.2700    0.1455
    3.2800    0.1451
    3.2900    0.1448
    3.3000    0.1440
    3.3100    0.1432
    3.3200    0.1425
    3.3300    0.1410
    3.3400    0.1389
    3.3500    0.1369
    3.3600    0.1355
    3.3700    0.1345
    3.3800    0.1332
    3.3900    0.1323
    3.4000    0.1313
    3.4100    0.1301
    3.4200    0.1293
    3.4300    0.1289
    3.4400    0.1291
    3.4500    0.1292
    3.4600    0.1285
    3.4700    0.1276
    3.4800    0.1266
    3.4900    0.1258
    3.5000    0.1246
    3.5100    0.1232
    3.5200    0.1227
    3.5300    0.1220
    3.5400    0.1212
    3.5500    0.1210
    3.5600    0.1209
    3.5700    0.1209
    3.5800    0.1197
    3.5900    0.1181
    3.6000    0.1176
    3.6100    0.1174
    3.6200    0.1168
    3.6300    0.1162
    3.6400    0.1161
    3.6500    0.1159
    3.6600    0.1150
    3.6700    0.1141
    3.6800    0.1134
    3.6900    0.1130
    3.7000    0.1128
    3.7100    0.1124
    3.7200    0.1120
    3.7300    0.1114
    3.7400    0.1107
    3.7500    0.1102
    3.7600    0.1093
    3.7700    0.1083
    3.7800    0.1082
    3.7900    0.1078
    3.8000    0.1076
    3.8100    0.1078
    3.8200    0.1072
    3.8300    0.1065
    3.8400    0.1059
    3.8500    0.1053
    3.8600    0.1051
    3.8700    0.1047
    3.8800    0.1042
    3.8900    0.1043
    3.9000    0.1046
    3.9100    0.1046
    3.9200    0.1041
    3.9300    0.1032
    3.9400    0.1026
    3.9500    0.1023
    3.9600    0.1013
    3.9700    0.0998
    3.9800    0.0993
    3.9900    0.0989
    4.0000    0.0989
    4.0100    0.0984
    4.0200    0.0973
    4.0300    0.0971
    4.0400    0.0964
    4.0500    0.0959
    4.0600    0.0953
    4.0700    0.0949
    4.0800    0.0948
    4.0900    0.0940
    4.1000    0.0923
    4.1100    0.0911
    4.1200    0.0910
    4.1300    0.0910
    4.1400    0.0906
    4.1500    0.0905
    4.1600    0.0898
    4.1700    0.0895
    4.1800    0.0893
    4.1900    0.0886
    4.2000    0.0881
    4.2100    0.0878
    4.2200    0.0868
    4.2300    0.0863
    4.2400    0.0866
    4.2500    0.0869
    4.2600    0.0876
    4.2700    0.0876
    4.2800    0.0870
    4.2900    0.0858
    4.3000    0.0850
    4.3100    0.0847
    4.3200    0.0848
    4.3300    0.0844
    4.3400    0.0840
    4.3500    0.0840
    4.3600    0.0834
    4.3700    0.0831
    4.3800    0.0831
    4.3900    0.0827
    4.4000    0.0829
    4.4100    0.0833
    4.4200    0.0831
    4.4300    0.0828
    4.4400    0.0826
    4.4500    0.0823
    4.4600    0.0822
    4.4700    0.0819
    4.4800    0.0812
    4.4900    0.0807
    4.5000    0.0811
    4.5100    0.0813
    4.5200    0.0806
    4.5300    0.0799
    4.5400    0.0795
    4.5500    0.0789
    4.5600    0.0787
    4.5700    0.0786
    4.5800    0.0780
    4.5900    0.0775
    4.6000    0.0767
    4.6100    0.0759
    4.6200    0.0750
    4.6300    0.0742
    4.6400    0.0735
    4.6500    0.0727
    4.6600    0.0722
    4.6700    0.0715
    4.6800    0.0709
    4.6900    0.0708
    4.7000    0.0703
    4.7100    0.0702
    4.7200    0.0698
    4.7300    0.0690
    4.7400    0.0682
    4.7500    0.0675
    4.7600    0.0668
    4.7700    0.0660
    4.7800    0.0655
    4.7900    0.0648
    4.8000    0.0636
    4.8100    0.0629
    4.8200    0.0634
    4.8300    0.0645
    4.8400    0.0647
    4.8500    0.0643
    4.8600    0.0640
    4.8700    0.0636
    4.8800    0.0633
    4.8900    0.0622
    4.9000    0.0615
    4.9100    0.0611
    4.9200    0.0598
    4.9300    0.0598
    4.9400    0.0603
    4.9500    0.0600
    4.9600    0.0604
    4.9700    0.0601
    4.9800    0.0594
    4.9900    0.0596
    5.0000    0.0595
    5.0100    0.0594
    5.0200    0.0591
    5.0300    0.0590
    5.0400    0.0589
    5.0500    0.0581
    5.0600    0.0579
    5.0700    0.0585
    5.0800    0.0587
    5.0900    0.0582
    5.1000    0.0580
    5.1100    0.0583
    5.1200    0.0587
    5.1300    0.0589
    5.1400    0.0586
    5.1500    0.0585
    5.1600    0.0584
    5.1700    0.0587
    5.1800    0.0585
    5.1900    0.0579
    5.2000    0.0582
    5.2100    0.0583
    5.2200    0.0578
    5.2300    0.0572
    5.2400    0.0567
    5.2500    0.0565
    5.2600    0.0563
    5.2700    0.0559
    5.2800    0.0556
    5.2900    0.0553
    5.3000    0.0549
    5.3100    0.0544
    5.3200    0.0538
    5.3300    0.0546
    5.3400    0.0566
    5.3500    0.0576
    5.3600    0.0580
    5.3700    0.0577
    5.3800    0.0570
    5.3900    0.0565
    5.4000    0.0563
    5.4100    0.0565
    5.4200    0.0565
    5.4300    0.0563
    5.4400    0.0558
    5.4500    0.0554
    5.4600    0.0556
    5.4700    0.0559
    5.4800    0.0559
    5.4900    0.0560
    5.5000    0.0563
    5.5100    0.0558
    5.5200    0.0551
    5.5300    0.0550
    5.5400    0.0542
    5.5500    0.0530
    5.5600    0.0524
    5.5700    0.0525
    5.5800    0.0525
    5.5900    0.0524
    5.6000    0.0522
    5.6100    0.0511
    5.6200    0.0504
    5.6300    0.0501
    5.6400    0.0499
    5.6500    0.0507
    5.6600    0.0509
    5.6700    0.0509
    5.6800    0.0515
    5.6900    0.0512
    5.7000    0.0506
    5.7100    0.0506
    5.7200    0.0506
    5.7300    0.0508
    5.7400    0.0511
    5.7500    0.0514
    5.7600    0.0513
    5.7700    0.0512
    5.7800    0.0506
    5.7900    0.0493
    5.8000    0.0494
    5.8100    0.0494
    5.8200    0.0491
    5.8300    0.0496
    5.8400    0.0496
    5.8500    0.0489
    5.8600    0.0484
    5.8700    0.0483
    5.8800    0.0483
    5.8900    0.0478
    5.9000    0.0469
    5.9100    0.0463
    5.9200    0.0460
    5.9300    0.0457
    5.9400    0.0454
    5.9500    0.0448
    5.9600    0.0446
    5.9700    0.0441
    5.9800    0.0432
    5.9900    0.0435
    6.0000    0.0433
    6.0100    0.0429
    6.0200    0.0429
    6.0300    0.0427
    6.0400    0.0423
    6.0500    0.0424
    6.0600    0.0421
    6.0700    0.0419
    6.0800    0.0424
    6.0900    0.0427
    6.1000    0.0427
    6.1100    0.0422
    6.1200    0.0419
    6.1300    0.0416
    6.1400    0.0415
    6.1500    0.0421
    6.1600    0.0422
    6.1700    0.0421
    6.1800    0.0412
    6.1900    0.0401
    6.2000    0.0398
    6.2100    0.0405
    6.2200    0.0413
    6.2300    0.0414
    6.2400    0.0413
    6.2500    0.0410
    6.2600    0.0413
    6.2700    0.0413
    6.2800    0.0417
    6.2900    0.0418
    6.3000    0.0411
    6.3100    0.0411
    6.3200    0.0404
    6.3300    0.0398
    6.3400    0.0400
    6.3500    0.0399
    6.3600    0.0400
    6.3700    0.0405
    6.3800    0.0409
    6.3900    0.0409
    6.4000    0.0406
    6.4100    0.0406
    6.4200    0.0403
    6.4300    0.0395
    6.4400    0.0390
    6.4500    0.0388
    6.4600    0.0392
    6.4700    0.0399
    6.4800    0.0399
    6.4900    0.0394
    6.5000    0.0395
    6.5100    0.0407
    6.5200    0.0414
    6.5300    0.0411
    6.5400    0.0404
    6.5500    0.0402
    6.5600    0.0405
    6.5700    0.0408
    6.5800    0.0408
    6.5900    0.0404
    6.6000    0.0402
    6.6100    0.0403
    6.6200    0.0404
    6.6300    0.0400
    6.6400    0.0398
    6.6500    0.0399
    6.6600    0.0402
    6.6700    0.0399
    6.6800    0.0393
    6.6900    0.0387
    6.7000    0.0384
    6.7100    0.0387
    6.7200    0.0382
    6.7300    0.0370
    6.7400    0.0363
    6.7500    0.0365
    6.7600    0.0366
    6.7700    0.0362
    6.7800    0.0351
    6.7900    0.0348
    6.8000    0.0350
    6.8100    0.0346
    6.8200    0.0348
    6.8300    0.0349
    6.8400    0.0345
    6.8500    0.0345
    6.8600    0.0348
    6.8700    0.0347
    6.8800    0.0343
    6.8900    0.0352
    6.9000    0.0354
    6.9100    0.0349
    6.9200    0.0349
    6.9300    0.0345
    6.9400    0.0339
    6.9500    0.0336
    6.9600    0.0344
    6.9700    0.0347
    6.9800    0.0344
    6.9900    0.0343
    7.0000    0.0345
    7.0100    0.0352
    7.0200    0.0351
    7.0300    0.0352
    7.0400    0.0352
    7.0500    0.0354
    7.0600    0.0356
    7.0700    0.0350
    7.0800    0.0346
    7.0900    0.0351
    7.1000    0.0351
    7.1100    0.0344
    7.1200    0.0346
    7.1300    0.0342
    7.1400    0.0336
    7.1500    0.0340
    7.1600    0.0342
    7.1700    0.0338
    7.1800    0.0335
    7.1900    0.0334
    7.2000    0.0335
    7.2100    0.0339
    7.2200    0.0338
    7.2300    0.0340
    7.2400    0.0344
    7.2500    0.0340
    7.2600    0.0334
    7.2700    0.0335
    7.2800    0.0336
    7.2900    0.0338
    7.3000    0.0338
    7.3100    0.0345
    7.3200    0.0347
    7.3300    0.0338
    7.3400    0.0336
    7.3500    0.0334
    7.3600    0.0337
    7.3700    0.0341
    7.3800    0.0339
    7.3900    0.0338
    7.4000    0.0339
    7.4100    0.0337
    7.4200    0.0336
    7.4300    0.0331
    7.4400    0.0325
    7.4500    0.0321
    7.4600    0.0315
    7.4700    0.0313
    7.4800    0.0309
    7.4900    0.0302
    7.5000    0.0294
    7.5100    0.0282
    7.5200    0.0273
    7.5300    0.0276
    7.5400    0.0277
    7.5500    0.0275
    7.5600    0.0269
    7.5700    0.0269
    7.5800    0.0272
    7.5900    0.0273
    7.6000    0.0277
    7.6100    0.0275
    7.6200    0.0275
    7.6300    0.0281
    7.6400    0.0281
    7.6500    0.0282
    7.6600    0.0290
    7.6700    0.0294
    7.6800    0.0290
    7.6900    0.0289
    7.7000    0.0290
    7.7100    0.0292
    7.7200    0.0292
    7.7300    0.0291
    7.7400    0.0295
    7.7500    0.0297
    7.7600    0.0296
    7.7700    0.0292
    7.7800    0.0284
    7.7900    0.0275
    7.8000    0.0266
    7.8100    0.0261
    7.8200    0.0254
    7.8300    0.0254
    7.8400    0.0263
    7.8500    0.0257
    7.8600    0.0246
    7.8700    0.0242
    7.8800    0.0236
    7.8900    0.0227
    7.9000    0.0228
    7.9100    0.0230
    7.9200    0.0228
    7.9300    0.0223
    7.9400    0.0218
    7.9500    0.0211
    7.9600    0.0207
    7.9700    0.0206
    7.9800    0.0204
    7.9900    0.0209
    8.0000    0.0214
    8.0100    0.0216
    8.0200    0.0213
    8.0300    0.0207
    8.0400    0.0202
    8.0500    0.0204
    8.0600    0.0205
    8.0700    0.0202
    8.0800    0.0201
    8.0900    0.0205
    8.1000    0.0202
    8.1100    0.0197
    8.1200    0.0198
    8.1300    0.0196
    8.1400    0.0197
    8.1500    0.0198
    8.1600    0.0192
    8.1700    0.0189
    8.1800    0.0191
    8.1900    0.0190
    8.2000    0.0191
    8.2100    0.0188
    8.2200    0.0180
    8.2300    0.0166
    8.2400    0.0158
    8.2500    0.0157
    8.2600    0.0151
    8.2700    0.0153
    8.2800    0.0155
    8.2900    0.0153
    8.3000    0.0148
    8.3100    0.0143
    8.3200    0.0144
    8.3300    0.0141
    8.3400    0.0134
    8.3500    0.0136
    8.3600    0.0133
    8.3700    0.0129
    8.3800    0.0133
    8.3900    0.0132
    8.4000    0.0123
    8.4100    0.0119
    8.4200    0.0122
    8.4300    0.0125
    8.4400    0.0128
    8.4500    0.0125
    8.4600    0.0123
    8.4700    0.0122
    8.4800    0.0118
    8.4900    0.0111
    8.5000    0.0109
    8.5100    0.0112
    8.5200    0.0113
    8.5300    0.0121
    8.5400    0.0120
    8.5500    0.0117
    8.5600    0.0119
    8.5700    0.0120
    8.5800    0.0125
    8.5900    0.0130
    8.6000    0.0129
    8.6100    0.0125
    8.6200    0.0123
    8.6300    0.0133
    8.6400    0.0144
    8.6500    0.0152
    8.6600    0.0160
    8.6700    0.0159
    8.6800    0.0161
    8.6900    0.0160
    8.7000    0.0161
    8.7100    0.0164
    8.7200    0.0158
    8.7300    0.0156
    8.7400    0.0154
    8.7500    0.0142
    8.7600    0.0137
    8.7700    0.0135
    8.7800    0.0129
    8.7900    0.0125
    8.8000    0.0123
    8.8100    0.0119
    8.8200    0.0119
    8.8300    0.0116
    8.8400    0.0108
    8.8500    0.0098
    8.8600    0.0090
    8.8700    0.0091
    8.8800    0.0090
    8.8900    0.0088
    8.9000    0.0090
    8.9100    0.0093
    8.9200    0.0098
    8.9300    0.0098
    8.9400    0.0092
    8.9500    0.0090
    8.9600    0.0087
    8.9700    0.0088
    8.9800    0.0096
    8.9900    0.0099
    9.0000    0.0097
    9.0100    0.0096
    9.0200    0.0095
    9.0300    0.0092
    9.0400    0.0090
    9.0500    0.0087
    9.0600    0.0090
    9.0700    0.0094
    9.0800    0.0099
    9.0900    0.0099
    9.1000    0.0096
    9.1100    0.0093
    9.1200    0.0090
    9.1300    0.0091
    9.1400    0.0095
    9.1500    0.0101
    9.1600    0.0105
    9.1700    0.0104
    9.1800    0.0101
    9.1900    0.0093
    9.2000    0.0085
    9.2100    0.0079
    9.2200    0.0076
    9.2300    0.0081
    9.2400    0.0083
    9.2500    0.0082
    9.2600    0.0080
    9.2700    0.0084
    9.2800    0.0092
    9.2900    0.0093
    9.3000    0.0092
    9.3100    0.0088
    9.3200    0.0085
    9.3300    0.0088
    9.3400    0.0092
    9.3500    0.0089
    9.3600    0.0085
    9.3700    0.0084
    9.3800    0.0079
    9.3900    0.0080
    9.4000    0.0083
    9.4100    0.0082
    9.4200    0.0082
    9.4300    0.0088
    9.4400    0.0091
    9.4500    0.0084
    9.4600    0.0076
    9.4700    0.0070
    9.4800    0.0064
    9.4900    0.0065
    9.5000    0.0059
    9.5100    0.0053
    9.5200    0.0051
    9.5300    0.0052
    9.5400    0.0052
    9.5500    0.0049
    9.5600    0.0046
    9.5700    0.0040
    9.5800    0.0038
    9.5900    0.0036
    9.6000    0.0033
    9.6100    0.0034
    9.6200    0.0038
    9.6300    0.0045
    9.6400    0.0048
    9.6500    0.0050
    9.6600    0.0047
    9.6700    0.0041
    9.6800    0.0045
    9.6900    0.0043
    9.7000    0.0044
    9.7100    0.0048
    9.7200    0.0053
    9.7300    0.0056
    9.7400    0.0058
    9.7500    0.0058
    9.7600    0.0052
    9.7700    0.0048
    9.7800    0.0047
    9.7900    0.0050
    9.8000    0.0051
    9.8100    0.0045
    9.8200    0.0053
    9.8300    0.0059
    9.8400    0.0061
    9.8500    0.0070
    9.8600    0.0070
    9.8700    0.0067
    9.8800    0.0066
    9.8900    0.0066
    9.9000    0.0072
    9.9100    0.0070
    9.9200    0.0070
    9.9300    0.0079
    9.9400    0.0078
    9.9500    0.0076
    9.9600    0.0076
    9.9700    0.0077
    9.9800    0.0081
    9.9900    0.0087
   10.0000    0.0089
    };

==> Data/Oscillator/sigma3/kf_en_vel.tex <==
    \addplot[
    thick,
    dashed,
    cyan
    ]
    table {
         0         0
    0.0100   -0.0099
    0.0200   -0.0196
    0.0300   -0.0291
    0.0400   -0.0384
    0.0500   -0.0475
    0.0600   -0.0563
    0.0700   -0.0650
    0.0800   -0.0735
    0.0900   -0.0818
    0.1000   -0.0898
    0.1100   -0.0976
    0.1200   -0.1054
    0.1300   -0.1129
    0.1400   -0.1203
    0.1500   -0.1275
    0.1600   -0.1346
    0.1700   -0.1414
    0.1800   -0.1481
    0.1900   -0.1545
    0.2000   -0.1607
    0.2100   -0.1668
    0.2200   -0.1727
    0.2300   -0.1786
    0.2400   -0.1843
    0.2500   -0.1897
    0.2600   -0.1950
    0.2700   -0.2001
    0.2800   -0.2052
    0.2900   -0.2100
    0.3000   -0.2148
    0.3100   -0.2194
    0.3200   -0.2237
    0.3300   -0.2281
    0.3400   -0.2324
    0.3500   -0.2365
    0.3600   -0.2409
    0.3700   -0.2450
    0.3800   -0.2486
    0.3900   -0.2520
    0.4000   -0.2555
    0.4100   -0.2587
    0.4200   -0.2618
    0.4300   -0.2648
    0.4400   -0.2680
    0.4500   -0.2711
    0.4600   -0.2738
    0.4700   -0.2766
    0.4800   -0.2795
    0.4900   -0.2823
    0.5000   -0.2849
    0.5100   -0.2875
    0.5200   -0.2899
    0.5300   -0.2922
    0.5400   -0.2945
    0.5500   -0.2965
    0.5600   -0.2985
    0.5700   -0.3006
    0.5800   -0.3025
    0.5900   -0.3043
    0.6000   -0.3063
    0.6100   -0.3082
    0.6200   -0.3099
    0.6300   -0.3116
    0.6400   -0.3132
    0.6500   -0.3146
    0.6600   -0.3160
    0.6700   -0.3177
    0.6800   -0.3191
    0.6900   -0.3206
    0.7000   -0.3220
    0.7100   -0.3232
    0.7200   -0.3242
    0.7300   -0.3252
    0.7400   -0.3260
    0.7500   -0.3269
    0.7600   -0.3281
    0.7700   -0.3293
    0.7800   -0.3303
    0.7900   -0.3314
    0.8000   -0.3321
    0.8100   -0.3325
    0.8200   -0.3333
    0.8300   -0.3341
    0.8400   -0.3347
    0.8500   -0.3350
    0.8600   -0.3355
    0.8700   -0.3361
    0.8800   -0.3367
    0.8900   -0.3371
    0.9000   -0.3372
    0.9100   -0.3375
    0.9200   -0.3380
    0.9300   -0.3387
    0.9400   -0.3390
    0.9500   -0.3389
    0.9600   -0.3388
    0.9700   -0.3388
    0.9800   -0.3389
    0.9900   -0.3391
    1.0000   -0.3392
    1.0100   -0.3389
    1.0200   -0.3387
    1.0300   -0.3389
    1.0400   -0.3389
    1.0500   -0.3385
    1.0600   -0.3383
    1.0700   -0.3380
    1.0800   -0.3377
    1.0900   -0.3376
    1.1000   -0.3375
    1.1100   -0.3371
    1.1200   -0.3366
    1.1300   -0.3362
    1.1400   -0.3360
    1.1500   -0.3359
    1.1600   -0.3356
    1.1700   -0.3354
    1.1800   -0.3350
    1.1900   -0.3344
    1.2000   -0.3341
    1.2100   -0.3339
    1.2200   -0.3337
    1.2300   -0.3333
    1.2400   -0.3328
    1.2500   -0.3323
    1.2600   -0.3318
    1.2700   -0.3312
    1.2800   -0.3307
    1.2900   -0.3302
    1.3000   -0.3297
    1.3100   -0.3291
    1.3200   -0.3286
    1.3300   -0.3279
    1.3400   -0.3272
    1.3500   -0.3266
    1.3600   -0.3261
    1.3700   -0.3254
    1.3800   -0.3247
    1.3900   -0.3239
    1.4000   -0.3232
    1.4100   -0.3225
    1.4200   -0.3217
    1.4300   -0.3209
    1.4400   -0.3202
    1.4500   -0.3195
    1.4600   -0.3189
    1.4700   -0.3180
    1.4800   -0.3170
    1.4900   -0.3161
    1.5000   -0.3152
    1.5100   -0.3142
    1.5200   -0.3132
    1.5300   -0.3124
    1.5400   -0.3115
    1.5500   -0.3106
    1.5600   -0.3096
    1.5700   -0.3086
    1.5800   -0.3076
    1.5900   -0.3065
    1.6000   -0.3055
    1.6100   -0.3046
    1.6200   -0.3037
    1.6300   -0.3027
    1.6400   -0.3016
    1.6500   -0.3006
    1.6600   -0.2996
    1.6700   -0.2985
    1.6800   -0.2974
    1.6900   -0.2963
    1.7000   -0.2953
    1.7100   -0.2941
    1.7200   -0.2932
    1.7300   -0.2922
    1.7400   -0.2910
    1.7500   -0.2900
    1.7600   -0.2890
    1.7700   -0.2879
    1.7800   -0.2867
    1.7900   -0.2856
    1.8000   -0.2845
    1.8100   -0.2834
    1.8200   -0.2823
    1.8300   -0.2811
    1.8400   -0.2800
    1.8500   -0.2788
    1.8600   -0.2775
    1.8700   -0.2763
    1.8800   -0.2751
    1.8900   -0.2739
    1.9000   -0.2726
    1.9100   -0.2714
    1.9200   -0.2701
    1.9300   -0.2688
    1.9400   -0.2676
    1.9500   -0.2663
    1.9600   -0.2650
    1.9700   -0.2637
    1.9800   -0.2625
    1.9900   -0.2612
    2.0000   -0.2600
    2.0100   -0.2587
    2.0200   -0.2574
    2.0300   -0.2561
    2.0400   -0.2549
    2.0500   -0.2536
    2.0600   -0.2523
    2.0700   -0.2511
    2.0800   -0.2498
    2.0900   -0.2485
    2.1000   -0.2472
    2.1100   -0.2458
    2.1200   -0.2445
    2.1300   -0.2433
    2.1400   -0.2420
    2.1500   -0.2408
    2.1600   -0.2395
    2.1700   -0.2382
    2.1800   -0.2369
    2.1900   -0.2357
    2.2000   -0.2344
    2.2100   -0.2331
    2.2200   -0.2318
    2.2300   -0.2306
    2.2400   -0.2293
    2.2500   -0.2281
    2.2600   -0.2268
    2.2700   -0.2255
    2.2800   -0.2243
    2.2900   -0.2230
    2.3000   -0.2218
    2.3100   -0.2205
    2.3200   -0.2192
    2.3300   -0.2180
    2.3400   -0.2167
    2.3500   -0.2154
    2.3600   -0.2142
    2.3700   -0.2129
    2.3800   -0.2117
    2.3900   -0.2104
    2.4000   -0.2092
    2.4100   -0.2079
    2.4200   -0.2067
    2.4300   -0.2054
    2.4400   -0.2042
    2.4500   -0.2030
    2.4600   -0.2017
    2.4700   -0.2005
    2.4800   -0.1993
    2.4900   -0.1981
    2.5000   -0.1969
    2.5100   -0.1957
    2.5200   -0.1945
    2.5300   -0.1933
    2.5400   -0.1921
    2.5500   -0.1910
    2.5600   -0.1898
    2.5700   -0.1886
    2.5800   -0.1874
    2.5900   -0.1863
    2.6000   -0.1851
    2.6100   -0.1840
    2.6200   -0.1828
    2.6300   -0.1817
    2.6400   -0.1805
    2.6500   -0.1794
    2.6600   -0.1783
    2.6700   -0.1773
    2.6800   -0.1762
    2.6900   -0.1751
    2.7000   -0.1740
    2.7100   -0.1729
    2.7200   -0.1718
    2.7300   -0.1707
    2.7400   -0.1696
    2.7500   -0.1686
    2.7600   -0.1675
    2.7700   -0.1664
    2.7800   -0.1654
    2.7900   -0.1644
    2.8000   -0.1633
    2.8100   -0.1623
    2.8200   -0.1612
    2.8300   -0.1601
    2.8400   -0.1591
    2.8500   -0.1582
    2.8600   -0.1572
    2.8700   -0.1561
    2.8800   -0.1552
    2.8900   -0.1542
    2.9000   -0.1531
    2.9100   -0.1522
    2.9200   -0.1512
    2.9300   -0.1503
    2.9400   -0.1493
    2.9500   -0.1484
    2.9600   -0.1474
    2.9700   -0.1465
    2.9800   -0.1455
    2.9900   -0.1446
    3.0000   -0.1437
    3.0100   -0.1427
    3.0200   -0.1417
    3.0300   -0.1408
    3.0400   -0.1399
    3.0500   -0.1389
    3.0600   -0.1380
    3.0700   -0.1371
    3.0800   -0.1362
    3.0900   -0.1353
    3.1000   -0.1345
    3.1100   -0.1335
    3.1200   -0.1326
    3.1300   -0.1318
    3.1400   -0.1309
    3.1500   -0.1300
    3.1600   -0.1292
    3.1700   -0.1284
    3.1800   -0.1275
    3.1900   -0.1267
    3.2000   -0.1259
    3.2100   -0.1251
    3.2200   -0.1242
    3.2300   -0.1233
    3.2400   -0.1225
    3.2500   -0.1217
    3.2600   -0.1208
    3.2700   -0.1200
    3.2800   -0.1191
    3.2900   -0.1183
    3.3000   -0.1174
    3.3100   -0.1166
    3.3200   -0.1158
    3.3300   -0.1151
    3.3400   -0.1144
    3.3500   -0.1137
    3.3600   -0.1129
    3.3700   -0.1121
    3.3800   -0.1113
    3.3900   -0.1105
    3.4000   -0.1097
    3.4100   -0.1089
    3.4200   -0.1081
    3.4300   -0.1073
    3.4400   -0.1064
    3.4500   -0.1056
    3.4600   -0.1048
    3.4700   -0.1040
    3.4800   -0.1033
    3.4900   -0.1025
    3.5000   -0.1018
    3.5100   -0.1011
    3.5200   -0.1004
    3.5300   -0.0996
    3.5400   -0.0989
    3.5500   -0.0981
    3.5600   -0.0973
    3.5700   -0.0965
    3.5800   -0.0959
    3.5900   -0.0953
    3.6000   -0.0945
    3.6100   -0.0938
    3.6200   -0.0931
    3.6300   -0.0924
    3.6400   -0.0916
    3.6500   -0.0909
    3.6600   -0.0903
    3.6700   -0.0896
    3.6800   -0.0890
    3.6900   -0.0883
    3.7000   -0.0876
    3.7100   -0.0869
    3.7200   -0.0863
    3.7300   -0.0857
    3.7400   -0.0850
    3.7500   -0.0844
    3.7600   -0.0838
    3.7700   -0.0832
    3.7800   -0.0826
    3.7900   -0.0820
    3.8000   -0.0813
    3.8100   -0.0807
    3.8200   -0.0801
    3.8300   -0.0795
    3.8400   -0.0790
    3.8500   -0.0784
    3.8600   -0.0778
    3.8700   -0.0772
    3.8800   -0.0767
    3.8900   -0.0760
    3.9000   -0.0754
    3.9100   -0.0748
    3.9200   -0.0743
    3.9300   -0.0739
    3.9400   -0.0734
    3.9500   -0.0728
    3.9600   -0.0724
    3.9700   -0.0720
    3.9800   -0.0714
    3.9900   -0.0709
    4.0000   -0.0704
    4.0100   -0.0699
    4.0200   -0.0695
    4.0300   -0.0689
    4.0400   -0.0685
    4.0500   -0.0680
    4.0600   -0.0675
    4.0700   -0.0670
    4.0800   -0.0665
    4.0900   -0.0661
    4.1000   -0.0657
    4.1100   -0.0653
    4.1200   -0.0648
    4.1300   -0.0643
    4.1400   -0.0638
    4.1500   -0.0633
    4.1600   -0.0629
    4.1700   -0.0624
    4.1800   -0.0619
    4.1900   -0.0615
    4.2000   -0.0611
    4.2100   -0.0606
    4.2200   -0.0603
    4.2300   -0.0598
    4.2400   -0.0593
    4.2500   -0.0588
    4.2600   -0.0583
    4.2700   -0.0578
    4.2800   -0.0575
    4.2900   -0.0572
    4.3000   -0.0568
    4.3100   -0.0564
    4.3200   -0.0560
    4.3300   -0.0556
    4.3400   -0.0552
    4.3500   -0.0548
    4.3600   -0.0544
    4.3700   -0.0541
    4.3800   -0.0537
    4.3900   -0.0533
    4.4000   -0.0529
    4.4100   -0.0525
    4.4200   -0.0521
    4.4300   -0.0518
    4.4400   -0.0514
    4.4500   -0.0511
    4.4600   -0.0508
    4.4700   -0.0504
    4.4800   -0.0502
    4.4900   -0.0499
    4.5000   -0.0495
    4.5100   -0.0491
    4.5200   -0.0489
    4.5300   -0.0486
    4.5400   -0.0483
    4.5500   -0.0481
    4.5600   -0.0478
    4.5700   -0.0475
    4.5800   -0.0472
    4.5900   -0.0469
    4.6000   -0.0467
    4.6100   -0.0465
    4.6200   -0.0462
    4.6300   -0.0460
    4.6400   -0.0457
    4.6500   -0.0455
    4.6600   -0.0452
    4.6700   -0.0449
    4.6800   -0.0447
    4.6900   -0.0443
    4.7000   -0.0441
    4.7100   -0.0437
    4.7200   -0.0434
    4.7300   -0.0432
    4.7400   -0.0430
    4.7500   -0.0427
    4.7600   -0.0425
    4.7700   -0.0422
    4.7800   -0.0419
    4.7900   -0.0417
    4.8000   -0.0415
    4.8100   -0.0412
    4.8200   -0.0408
    4.8300   -0.0404
    4.8400   -0.0400
    4.8500   -0.0398
    4.8600   -0.0395
    4.8700   -0.0392
    4.8800   -0.0390
    4.8900   -0.0388
    4.9000   -0.0386
    4.9100   -0.0383
    4.9200   -0.0381
    4.9300   -0.0378
    4.9400   -0.0375
    4.9500   -0.0372
    4.9600   -0.0369
    4.9700   -0.0366
    4.9800   -0.0364
    4.9900   -0.0361
    5.0000   -0.0358
    5.0100   -0.0356
    5.0200   -0.0354
    5.0300   -0.0351
    5.0400   -0.0349
    5.0500   -0.0347
    5.0600   -0.0345
    5.0700   -0.0341
    5.0800   -0.0339
    5.0900   -0.0337
    5.1000   -0.0335
    5.1100   -0.0332
    5.1200   -0.0329
    5.1300   -0.0327
    5.1400   -0.0325
    5.1500   -0.0323
    5.1600   -0.0321
    5.1700   -0.0319
    5.1800   -0.0317
    5.1900   -0.0316
    5.2000   -0.0314
    5.2100   -0.0312
    5.2200   -0.0311
    5.2300   -0.0310
    5.2400   -0.0308
    5.2500   -0.0307
    5.2600   -0.0305
    5.2700   -0.0304
    5.2800   -0.0302
    5.2900   -0.0301
    5.3000   -0.0299
    5.3100   -0.0298
    5.3200   -0.0297
    5.3300   -0.0294
    5.3400   -0.0290
    5.3500   -0.0288
    5.3600   -0.0286
    5.3700   -0.0285
    5.3800   -0.0285
    5.3900   -0.0284
    5.4000   -0.0283
    5.4100   -0.0281
    5.4200   -0.0280
    5.4300   -0.0279
    5.4400   -0.0278
    5.4500   -0.0278
    5.4600   -0.0276
    5.4700   -0.0275
    5.4800   -0.0274
    5.4900   -0.0272
    5.5000   -0.0271
    5.5100   -0.0271
    5.5200   -0.0270
    5.5300   -0.0269
    5.5400   -0.0269
    5.5500   -0.0270
    5.5600   -0.0269
    5.5700   -0.0268
    5.5800   -0.0266
    5.5900   -0.0265
    5.6000   -0.0264
    5.6100   -0.0265
    5.6200   -0.0264
    5.6300   -0.0263
    5.6400   -0.0262
    5.6500   -0.0260
    5.6600   -0.0258
    5.6700   -0.0257
    5.6800   -0.0255
    5.6900   -0.0255
    5.7000   -0.0255
    5.7100   -0.0253
    5.7200   -0.0252
    5.7300   -0.0251
    5.7400   -0.0250
    5.7500   -0.0249
    5.7600   -0.0248
    5.7700   -0.0247
    5.7800   -0.0247
    5.7900   -0.0248
    5.8000   -0.0247
    5.8100   -0.0246
    5.8200   -0.0245
    5.8300   -0.0244
    5.8400   -0.0243
    5.8500   -0.0243
    5.8600   -0.0243
    5.8700   -0.0242
    5.8800   -0.0241
    5.8900   -0.0241
    5.9000   -0.0241
    5.9100   -0.0241
    5.9200   -0.0240
    5.9300   -0.0239
    5.9400   -0.0239
    5.9500   -0.0238
    5.9600   -0.0237
    5.9700   -0.0237
    5.9800   -0.0237
    5.9900   -0.0235
    6.0000   -0.0234
    6.0100   -0.0234
    6.0200   -0.0233
    6.0300   -0.0232
    6.0400   -0.0231
    6.0500   -0.0230
    6.0600   -0.0229
    6.0700   -0.0228
    6.0800   -0.0227
    6.0900   -0.0225
    6.1000   -0.0224
    6.1100   -0.0224
    6.1200   -0.0223
    6.1300   -0.0223
    6.1400   -0.0222
    6.1500   -0.0220
    6.1600   -0.0219
    6.1700   -0.0219
    6.1800   -0.0219
    6.1900   -0.0219
    6.2000   -0.0219
    6.2100   -0.0217
    6.2200   -0.0215
    6.2300   -0.0214
    6.2400   -0.0213
    6.2500   -0.0213
    6.2600   -0.0212
    6.2700   -0.0211
    6.2800   -0.0210
    6.2900   -0.0209
    6.3000   -0.0210
    6.3100   -0.0209
    6.3200   -0.0209
    6.3300   -0.0209
    6.3400   -0.0208
    6.3500   -0.0208
    6.3600   -0.0207
    6.3700   -0.0206
    6.3800   -0.0205
    6.3900   -0.0204
    6.4000   -0.0204
    6.4100   -0.0203
    6.4200   -0.0203
    6.4300   -0.0204
    6.4400   -0.0204
    6.4500   -0.0203
    6.4600   -0.0202
    6.4700   -0.0201
    6.4800   -0.0200
    6.4900   -0.0200
    6.5000   -0.0200
    6.5100   -0.0198
    6.5200   -0.0197
    6.5300   -0.0197
    6.5400   -0.0197
    6.5500   -0.0197
    6.5600   -0.0197
    6.5700   -0.0196
    6.5800   -0.0196
    6.5900   -0.0196
    6.6000   -0.0196
    6.6100   -0.0196
    6.6200   -0.0195
    6.6300   -0.0196
    6.6400   -0.0196
    6.6500   -0.0195
    6.6600   -0.0195
    6.6700   -0.0195
    6.6800   -0.0195
    6.6900   -0.0196
    6.7000   -0.0196
    6.7100   -0.0195
    6.7200   -0.0195
    6.7300   -0.0196
    6.7400   -0.0196
    6.7500   -0.0196
    6.7600   -0.0195
    6.7700   -0.0195
    6.7800   -0.0196
    6.7900   -0.0196
    6.8000   -0.0195
    6.8100   -0.0194
    6.8200   -0.0194
    6.8300   -0.0193
    6.8400   -0.0193
    6.8500   -0.0192
    6.8600   -0.0191
    6.8700   -0.0191
    6.8800   -0.0191
    6.8900   -0.0189
    6.9000   -0.0188
    6.9100   -0.0189
    6.9200   -0.0188
    6.9300   -0.0188
    6.9400   -0.0188
    6.9500   -0.0188
    6.9600   -0.0187
    6.9700   -0.0186
    6.9800   -0.0186
    6.9900   -0.0186
    7.0000   -0.0185
    7.0100   -0.0184
    7.0200   -0.0183
    7.0300   -0.0183
    7.0400   -0.0183
    7.0500   -0.0182
    7.0600   -0.0182
    7.0700   -0.0182
    7.0800   -0.0183
    7.0900   -0.0182
    7.1000   -0.0182
    7.1100   -0.0182
    7.1200   -0.0181
    7.1300   -0.0182
    7.1400   -0.0182
    7.1500   -0.0181
    7.1600   -0.0181
    7.1700   -0.0181
    7.1800   -0.0181
    7.1900   -0.0181
    7.2000   -0.0180
    7.2100   -0.0180
    7.2200   -0.0180
    7.2300   -0.0179
    7.2400   -0.0178
    7.2500   -0.0179
    7.2600   -0.0179
    7.2700   -0.0179
    7.2800   -0.0178
    7.2900   -0.0178
    7.3000   -0.0178
    7.3100   -0.0177
    7.3200   -0.0176
    7.3300   -0.0177
    7.3400   -0.0177
    7.3500   -0.0177
    7.3600   -0.0177
    7.3700   -0.0176
    7.3800   -0.0176
    7.3900   -0.0177
    7.4000   -0.0176
    7.4100   -0.0176
    7.4200   -0.0176
    7.4300   -0.0177
    7.4400   -0.0177
    7.4500   -0.0177
    7.4600   -0.0178
    7.4700   -0.0178
    7.4800   -0.0178
    7.4900   -0.0178
    7.5000   -0.0179
    7.5100   -0.0180
    7.5200   -0.0180
    7.5300   -0.0179
    7.5400   -0.0178
    7.5500   -0.0177
    7.5600   -0.0177
    7.5700   -0.0177
    7.5800   -0.0176
    7.5900   -0.0175
    7.6000   -0.0174
    7.6100   -0.0173
    7.6200   -0.0173
    7.6300   -0.0171
    7.6400   -0.0171
    7.6500   -0.0170
    7.6600   -0.0169
    7.6700   -0.0168
    7.6800   -0.0168
    7.6900   -0.0168
    7.7000   -0.0167
    7.7100   -0.0167
    7.7200   -0.0166
    7.7300   -0.0166
    7.7400   -0.0165
    7.7500   -0.0165
    7.7600   -0.0165
    7.7700   -0.0165
    7.7800   -0.0166
    7.7900   -0.0166
    7.8000   -0.0167
    7.8100   -0.0167
    7.8200   -0.0167
    7.8300   -0.0167
    7.8400   -0.0165
    7.8500   -0.0165
    7.8600   -0.0166
    7.8700   -0.0166
    7.8800   -0.0166
    7.8900   -0.0166
    7.9000   -0.0165
    7.9100   -0.0164
    7.9200   -0.0163
    7.9300   -0.0163
    7.9400   -0.0163
    7.9500   -0.0162
    7.9600   -0.0162
    7.9700   -0.0161
    7.9800   -0.0160
    7.9900   -0.0159
    8.0000   -0.0157
    8.0100   -0.0156
    8.0200   -0.0156
    8.0300   -0.0155
    8.0400   -0.0155
    8.0500   -0.0154
    8.0600   -0.0153
    8.0700   -0.0152
    8.0800   -0.0152
    8.0900   -0.0150
    8.1000   -0.0150
    8.1100   -0.0150
    8.1200   -0.0149
    8.1300   -0.0148
    8.1400   -0.0147
    8.1500   -0.0146
    8.1600   -0.0146
    8.1700   -0.0145
    8.1800   -0.0144
    8.1900   -0.0144
    8.2000   -0.0143
    8.2100   -0.0142
    8.2200   -0.0142
    8.2300   -0.0143
    8.2400   -0.0143
    8.2500   -0.0142
    8.2600   -0.0141
    8.2700   -0.0140
    8.2800   -0.0139
    8.2900   -0.0138
    8.3000   -0.0137
    8.3100   -0.0137
    8.3200   -0.0135
    8.3300   -0.0135
    8.3400   -0.0134
    8.3500   -0.0133
    8.3600   -0.0132
    8.3700   -0.0131
    8.3800   -0.0129
    8.3900   -0.0128
    8.4000   -0.0128
    8.4100   -0.0128
    8.4200   -0.0126
    8.4300   -0.0124
    8.4400   -0.0123
    8.4500   -0.0122
    8.4600   -0.0121
    8.4700   -0.0120
    8.4800   -0.0120
    8.4900   -0.0119
    8.5000   -0.0118
    8.5100   -0.0117
    8.5200   -0.0116
    8.5300   -0.0114
    8.5400   -0.0113
    8.5500   -0.0112
    8.5600   -0.0111
    8.5700   -0.0110
    8.5800   -0.0108
    8.5900   -0.0107
    8.6000   -0.0106
    8.6100   -0.0106
    8.6200   -0.0105
    8.6300   -0.0103
    8.6400   -0.0101
    8.6500   -0.0100
    8.6600   -0.0098
    8.6700   -0.0098
    8.6800   -0.0098
    8.6900   -0.0097
    8.7000   -0.0097
    8.7100   -0.0096
    8.7200   -0.0097
    8.7300   -0.0097
    8.7400   -0.0096
    8.7500   -0.0097
    8.7600   -0.0097
    8.7700   -0.0097
    8.7800   -0.0097
    8.7900   -0.0097
    8.8000   -0.0097
    8.8100   -0.0096
    8.8200   -0.0096
    8.8300   -0.0095
    8.8400   -0.0095
    8.8500   -0.0096
    8.8600   -0.0096
    8.8700   -0.0095
    8.8800   -0.0094
    8.8900   -0.0093
    8.9000   -0.0092
    8.9100   -0.0091
    8.9200   -0.0089
    8.9300   -0.0088
    8.9400   -0.0088
    8.9500   -0.0088
    8.9600   -0.0087
    8.9700   -0.0086
    8.9800   -0.0084
    8.9900   -0.0083
    9.0000   -0.0083
    9.0100   -0.0082
    9.0200   -0.0082
    9.0300   -0.0081
    9.0400   -0.0081
    9.0500   -0.0080
    9.0600   -0.0079
    9.0700   -0.0078
    9.0800   -0.0077
    9.0900   -0.0076
    9.1000   -0.0076
    9.1100   -0.0076
    9.1200   -0.0075
    9.1300   -0.0075
    9.1400   -0.0074
    9.1500   -0.0072
    9.1600   -0.0071
    9.1700   -0.0071
    9.1800   -0.0071
    9.1900   -0.0071
    9.2000   -0.0072
    9.2100   -0.0072
    9.2200   -0.0071
    9.2300   -0.0070
    9.2400   -0.0069
    9.2500   -0.0069
    9.2600   -0.0068
    9.2700   -0.0067
    9.2800   -0.0066
    9.2900   -0.0065
    9.3000   -0.0065
    9.3100   -0.0065
    9.3200   -0.0065
    9.3300   -0.0064
    9.3400   -0.0063
    9.3500   -0.0063
    9.3600   -0.0063
    9.3700   -0.0062
    9.3800   -0.0062
    9.3900   -0.0062
    9.4000   -0.0061
    9.4100   -0.0060
    9.4200   -0.0060
    9.4300   -0.0059
    9.4400   -0.0058
    9.4500   -0.0059
    9.4600   -0.0059
    9.4700   -0.0059
    9.4800   -0.0059
    9.4900   -0.0059
    9.5000   -0.0059
    9.5100   -0.0059
    9.5200   -0.0058
    9.5300   -0.0057
    9.5400   -0.0056
    9.5500   -0.0056
    9.5600   -0.0056
    9.5700   -0.0056
    9.5800   -0.0055
    9.5900   -0.0054
    9.6000   -0.0054
    9.6100   -0.0053
    9.6200   -0.0052
    9.6300   -0.0050
    9.6400   -0.0049
    9.6500   -0.0048
    9.6600   -0.0048
    9.6700   -0.0048
    9.6800   -0.0047
    9.6900   -0.0046
    9.7000   -0.0046
    9.7100   -0.0045
    9.7200   -0.0044
    9.7300   -0.0043
    9.7400   -0.0042
    9.7500   -0.0042
    9.7600   -0.0042
    9.7700   -0.0042
    9.7800   -0.0042
    9.7900   -0.0041
    9.8000   -0.0040
    9.8100   -0.0040
    9.8200   -0.0039
    9.8300   -0.0038
    9.8400   -0.0037
    9.8500   -0.0036
    9.8600   -0.0036
    9.8700   -0.0036
    9.8800   -0.0036
    9.8900   -0.0036
    9.9000   -0.0035
    9.9100   -0.0035
    9.9200   -0.0035
    9.9300   -0.0033
    9.9400   -0.0033
    9.9500   -0.0034
    9.9600   -0.0034
    9.9700   -0.0033
    9.9800   -0.0033
    9.9900   -0.0032
   10.0000   -0.0032
    };

==> Data/Oscillator/sigma3/kf_exp_pos.tex <==
    \addplot[
    thick,
    green
    ]
    table {
         0    1.0000
    0.0100    0.9972
    0.0200    0.9928
    0.0300    0.9839
    0.0400    0.9791
    0.0500    0.9755
    0.0600    0.9713
    0.0700    0.9673
    0.0800    0.9638
    0.0900    0.9551
    0.1000    0.9461
    0.1100    0.9478
    0.1200    0.9492
    0.1300    0.9488
    0.1400    0.9459
    0.1500    0.9415
    0.1600    0.9384
    0.1700    0.9352
    0.1800    0.9299
    0.1900    0.9237
    0.2000    0.9192
    0.2100    0.9141
    0.2200    0.9101
    0.2300    0.9125
    0.2400    0.9102
    0.2500    0.9040
    0.2600    0.8981
    0.2700    0.8932
    0.2800    0.8946
    0.2900    0.8892
    0.3000    0.8856
    0.3100    0.8834
    0.3200    0.8772
    0.3300    0.8756
    0.3400    0.8729
    0.3500    0.8717
    0.3600    0.8748
    0.3700    0.8747
    0.3800    0.8675
    0.3900    0.8603
    0.4000    0.8549
    0.4100    0.8487
    0.4200    0.8422
    0.4300    0.8363
    0.4400    0.8354
    0.4500    0.8331
    0.4600    0.8271
    0.4700    0.8241
    0.4800    0.8229
    0.4900    0.8204
    0.5000    0.8177
    0.5100    0.8159
    0.5200    0.8120
    0.5300    0.8076
    0.5400    0.8038
    0.5500    0.7979
    0.5600    0.7934
    0.5700    0.7902
    0.5800    0.7856
    0.5900    0.7814
    0.6000    0.7785
    0.6100    0.7757
    0.6200    0.7719
    0.6300    0.7680
    0.6400    0.7642
    0.6500    0.7591
    0.6600    0.7546
    0.6700    0.7529
    0.6800    0.7491
    0.6900    0.7461
    0.7000    0.7437
    0.7100    0.7388
    0.7200    0.7336
    0.7300    0.7279
    0.7400    0.7221
    0.7500    0.7172
    0.7600    0.7148
    0.7700    0.7125
    0.7800    0.7091
    0.7900    0.7072
    0.8000    0.7018
    0.8100    0.6950
    0.8200    0.6912
    0.8300    0.6881
    0.8400    0.6835
    0.8500    0.6771
    0.8600    0.6730
    0.8700    0.6695
    0.8800    0.6656
    0.8900    0.6614
    0.9000    0.6550
    0.9100    0.6503
    0.9200    0.6477
    0.9300    0.6459
    0.9400    0.6419
    0.9500    0.6356
    0.9600    0.6295
    0.9700    0.6246
    0.9800    0.6200
    0.9900    0.6166
    1.0000    0.6128
    1.0100    0.6063
    1.0200    0.6013
    1.0300    0.5986
    1.0400    0.5950
    1.0500    0.5895
    1.0600    0.5848
    1.0700    0.5798
    1.0800    0.5747
    1.0900    0.5716
    1.1000    0.5686
    1.1100    0.5636
    1.1200    0.5582
    1.1300    0.5539
    1.1400    0.5511
    1.1500    0.5492
    1.1600    0.5457
    1.1700    0.5428
    1.1800    0.5394
    1.1900    0.5345
    1.2000    0.5315
    1.2100    0.5296
    1.2200    0.5271
    1.2300    0.5242
    1.2400    0.5203
    1.2500    0.5168
    1.2600    0.5131
    1.2700    0.5093
    1.2800    0.5061
    1.2900    0.5033
    1.3000    0.5001
    1.3100    0.4965
    1.3200    0.4939
    1.3300    0.4902
    1.3400    0.4861
    1.3500    0.4836
    1.3600    0.4811
    1.3700    0.4773
    1.3800    0.4739
    1.3900    0.4705
    1.4000    0.4671
    1.4100    0.4638
    1.4200    0.4603
    1.4300    0.4570
    1.4400    0.4546
    1.4500    0.4519
    1.4600    0.4497
    1.4700    0.4461
    1.4800    0.4413
    1.4900    0.4381
    1.5000    0.4346
    1.5100    0.4301
    1.5200    0.4265
    1.5300    0.4239
    1.5400    0.4210
    1.5500    0.4181
    1.5600    0.4147
    1.5700    0.4108
    1.5800    0.4074
    1.5900    0.4038
    1.6000    0.4003
    1.6100    0.3986
    1.6200    0.3962
    1.6300    0.3931
    1.6400    0.3898
    1.6500    0.3868
    1.6600    0.3840
    1.6700    0.3805
    1.6800    0.3774
    1.6900    0.3742
    1.7000    0.3716
    1.7100    0.3683
    1.7200    0.3666
    1.7300    0.3648
    1.7400    0.3611
    1.7500    0.3595
    1.7600    0.3572
    1.7700    0.3539
    1.7800    0.3509
    1.7900    0.3479
    1.8000    0.3457
    1.8100    0.3431
    1.8200    0.3405
    1.8300    0.3375
    1.8400    0.3355
    1.8500    0.3325
    1.8600    0.3280
    1.8700    0.3249
    1.8800    0.3222
    1.8900    0.3191
    1.9000    0.3158
    1.9100    0.3121
    1.9200    0.3091
    1.9300    0.3060
    1.9400    0.3028
    1.9500    0.2998
    1.9600    0.2966
    1.9700    0.2943
    1.9800    0.2919
    1.9900    0.2896
    2.0000    0.2878
    2.0100    0.2845
    2.0200    0.2812
    2.0300    0.2789
    2.0400    0.2772
    2.0500    0.2752
    2.0600    0.2728
    2.0700    0.2709
    2.0800    0.2682
    2.0900    0.2651
    2.1000    0.2620
    2.1100    0.2588
    2.1200    0.2567
    2.1300    0.2549
    2.1400    0.2537
    2.1500    0.2525
    2.1600    0.2493
    2.1700    0.2468
    2.1800    0.2459
    2.1900    0.2438
    2.2000    0.2414
    2.2100    0.2396
    2.2200    0.2378
    2.2300    0.2361
    2.2400    0.2342
    2.2500    0.2319
    2.2600    0.2299
    2.2700    0.2275
    2.2800    0.2257
    2.2900    0.2242
    2.3000    0.2224
    2.3100    0.2204
    2.3200    0.2177
    2.3300    0.2154
    2.3400    0.2133
    2.3500    0.2116
    2.3600    0.2103
    2.3700    0.2088
    2.3800    0.2066
    2.3900    0.2038
    2.4000    0.2018
    2.4100    0.1999
    2.4200    0.1983
    2.4300    0.1974
    2.4400    0.1958
    2.4500    0.1940
    2.4600    0.1930
    2.4700    0.1917
    2.4800    0.1905
    2.4900    0.1897
    2.5000    0.1882
    2.5100    0.1868
    2.5200    0.1855
    2.5300    0.1837
    2.5400    0.1820
    2.5500    0.1805
    2.5600    0.1787
    2.5700    0.1775
    2.5800    0.1765
    2.5900    0.1758
    2.6000    0.1750
    2.6100    0.1733
    2.6200    0.1724
    2.6300    0.1722
    2.6400    0.1716
    2.6500    0.1698
    2.6600    0.1683
    2.6700    0.1667
    2.6800    0.1646
    2.6900    0.1632
    2.7000    0.1622
    2.7100    0.1617
    2.7200    0.1606
    2.7300    0.1594
    2.7400    0.1582
    2.7500    0.1568
    2.7600    0.1562
    2.7700    0.1555
    2.7800    0.1540
    2.7900    0.1524
    2.8000    0.1511
    2.8100    0.1503
    2.8200    0.1501
    2.8300    0.1494
    2.8400    0.1481
    2.8500    0.1466
    2.8600    0.1456
    2.8700    0.1449
    2.8800    0.1433
    2.8900    0.1426
    2.9000    0.1423
    2.9100    0.1415
    2.9200    0.1401
    2.9300    0.1387
    2.9400    0.1379
    2.9500    0.1365
    2.9600    0.1349
    2.9700    0.1335
    2.9800    0.1324
    2.9900    0.1311
    3.0000    0.1299
    3.0100    0.1298
    3.0200    0.1291
    3.0300    0.1278
    3.0400    0.1268
    3.0500    0.1262
    3.0600    0.1257
    3.0700    0.1249
    3.0800    0.1238
    3.0900    0.1225
    3.1000    0.1215
    3.1100    0.1212
    3.1200    0.1209
    3.1300    0.1196
    3.1400    0.1183
    3.1500    0.1175
    3.1600    0.1164
    3.1700    0.1153
    3.1800    0.1140
    3.1900    0.1127
    3.2000    0.1114
    3.2100    0.1101
    3.2200    0.1092
    3.2300    0.1083
    3.2400    0.1074
    3.2500    0.1064
    3.2600    0.1054
    3.2700    0.1047
    3.2800    0.1043
    3.2900    0.1040
    3.3000    0.1032
    3.3100    0.1024
    3.3200    0.1017
    3.3300    0.1003
    3.3400    0.0983
    3.3500    0.0962
    3.3600    0.0949
    3.3700    0.0939
    3.3800    0.0927
    3.3900    0.0917
    3.4000    0.0908
    3.4100    0.0896
    3.4200    0.0889
    3.4300    0.0885
    3.4400    0.0887
    3.4500    0.0888
    3.4600    0.0881
    3.4700    0.0872
    3.4800    0.0862
    3.4900    0.0855
    3.5000    0.0843
    3.5100    0.0829
    3.5200    0.0825
    3.5300    0.0819
    3.5400    0.0811
    3.5500    0.0809
    3.5600    0.0808
    3.5700    0.0808
    3.5800    0.0797
    3.5900    0.0781
    3.6000    0.0776
    3.6100    0.0774
    3.6200    0.0769
    3.6300    0.0764
    3.6400    0.0762
    3.6500    0.0760
    3.6600    0.0752
    3.6700    0.0743
    3.6800    0.0736
    3.6900    0.0733
    3.7000    0.0731
    3.7100    0.0728
    3.7200    0.0725
    3.7300    0.0718
    3.7400    0.0712
    3.7500    0.0708
    3.7600    0.0699
    3.7700    0.0689
    3.7800    0.0688
    3.7900    0.0685
    3.8000    0.0684
    3.8100    0.0686
    3.8200    0.0680
    3.8300    0.0673
    3.8400    0.0667
    3.8500    0.0662
    3.8600    0.0661
    3.8700    0.0657
    3.8800    0.0652
    3.8900    0.0654
    3.9000    0.0657
    3.9100    0.0658
    3.9200    0.0653
    3.9300    0.0644
    3.9400    0.0639
    3.9500    0.0636
    3.9600    0.0627
    3.9700    0.0612
    3.9800    0.0608
    3.9900    0.0604
    4.0000    0.0604
    4.0100    0.0600
    4.0200    0.0589
    4.0300    0.0588
    4.0400    0.0581
    4.0500    0.0577
    4.0600    0.0572
    4.0700    0.0567
    4.0800    0.0568
    4.0900    0.0559
    4.1000    0.0543
    4.1100    0.0531
    4.1200    0.0531
    4.1300    0.0532
    4.1400    0.0528
    4.1500    0.0528
    4.1600    0.0522
    4.1700    0.0518
    4.1800    0.0517
    4.1900    0.0511
    4.2000    0.0507
    4.2100    0.0504
    4.2200    0.0494
    4.2300    0.0490
    4.2400    0.0493
    4.2500    0.0496
    4.2600    0.0504
    4.2700    0.0505
    4.2800    0.0499
    4.2900    0.0488
    4.3000    0.0480
    4.3100    0.0478
    4.3200    0.0479
    4.3300    0.0477
    4.3400    0.0473
    4.3500    0.0474
    4.3600    0.0468
    4.3700    0.0465
    4.3800    0.0466
    4.3900    0.0463
    4.4000    0.0465
    4.4100    0.0470
    4.4200    0.0468
    4.4300    0.0466
    4.4400    0.0465
    4.4500    0.0463
    4.4600    0.0462
    4.4700    0.0460
    4.4800    0.0453
    4.4900    0.0449
    4.5000    0.0454
    4.5100    0.0456
    4.5200    0.0449
    4.5300    0.0443
    4.5400    0.0440
    4.5500    0.0435
    4.5600    0.0433
    4.5700    0.0432
    4.5800    0.0428
    4.5900    0.0423
    4.6000    0.0416
    4.6100    0.0408
    4.6200    0.0399
    4.6300    0.0392
    4.6400    0.0386
    4.6500    0.0378
    4.6600    0.0374
    4.6700    0.0368
    4.6800    0.0362
    4.6900    0.0362
    4.7000    0.0358
    4.7100    0.0357
    4.7200    0.0354
    4.7300    0.0346
    4.7400    0.0340
    4.7500    0.0333
    4.7600    0.0327
    4.7700    0.0319
    4.7800    0.0315
    4.7900    0.0308
    4.8000    0.0297
    4.8100    0.0290
    4.8200    0.0296
    4.8300    0.0308
    4.8400    0.0311
    4.8500    0.0307
    4.8600    0.0305
    4.8700    0.0302
    4.8800    0.0300
    4.8900    0.0289
    4.9000    0.0282
    4.9100    0.0279
    4.9200    0.0267
    4.9300    0.0268
    4.9400    0.0274
    4.9500    0.0271
    4.9600    0.0277
    4.9700    0.0274
    4.9800    0.0268
    4.9900    0.0270
    5.0000    0.0271
    5.0100    0.0271
    5.0200    0.0268
    5.0300    0.0268
    5.0400    0.0267
    5.0500    0.0260
    5.0600    0.0259
    5.0700    0.0266
    5.0800    0.0269
    5.0900    0.0265
    5.1000    0.0263
    5.1100    0.0267
    5.1200    0.0272
    5.1300    0.0275
    5.1400    0.0272
    5.1500    0.0272
    5.1600    0.0272
    5.1700    0.0276
    5.1800    0.0275
    5.1900    0.0269
    5.2000    0.0274
    5.2100    0.0275
    5.2200    0.0271
    5.2300    0.0266
    5.2400    0.0262
    5.2500    0.0260
    5.2600    0.0259
    5.2700    0.0256
    5.2800    0.0253
    5.2900    0.0252
    5.3000    0.0248
    5.3100    0.0244
    5.3200    0.0239
    5.3300    0.0248
    5.3400    0.0269
    5.3500    0.0280
    5.3600    0.0285
    5.3700    0.0283
    5.3800    0.0276
    5.3900    0.0273
    5.4000    0.0271
    5.4100    0.0274
    5.4200    0.0275
    5.4300    0.0274
    5.4400    0.0270
    5.4500    0.0266
    5.4600    0.0269
    5.4700    0.0274
    5.4800    0.0274
    5.4900    0.0276
    5.5000    0.0280
    5.5100    0.0276
    5.5200    0.0270
    5.5300    0.0270
    5.5400    0.0262
    5.5500    0.0251
    5.5600    0.0246
    5.5700    0.0248
    5.5800    0.0249
    5.5900    0.0248
    5.6000    0.0247
    5.6100    0.0236
    5.6200    0.0230
    5.6300    0.0228
    5.6400    0.0227
    5.6500    0.0236
    5.6600    0.0239
    5.6700    0.0240
    5.6800    0.0247
    5.6900    0.0245
    5.7000    0.0240
    5.7100    0.0240
    5.7200    0.0242
    5.7300    0.0245
    5.7400    0.0248
    5.7500    0.0252
    5.7600    0.0252
    5.7700    0.0253
    5.7800    0.0247
    5.7900    0.0235
    5.8000    0.0236
    5.8100    0.0238
    5.8200    0.0235
    5.8300    0.0241
    5.8400    0.0243
    5.8500    0.0236
    5.8600    0.0232
    5.8700    0.0232
    5.8800    0.0232
    5.8900    0.0229
    5.9000    0.0221
    5.9100    0.0215
    5.9200    0.0214
    5.9300    0.0211
    5.9400    0.0209
    5.9500    0.0204
    5.9600    0.0203
    5.9700    0.0198
    5.9800    0.0191
    5.9900    0.0194
    6.0000    0.0193
    6.0100    0.0190
    6.0200    0.0191
    6.0300    0.0190
    6.0400    0.0187
    6.0500    0.0189
    6.0600    0.0187
    6.0700    0.0186
    6.0800    0.0192
    6.0900    0.0195
    6.1000    0.0196
    6.1100    0.0192
    6.1200    0.0191
    6.1300    0.0188
    6.1400    0.0188
    6.1500    0.0195
    6.1600    0.0197
    6.1700    0.0197
    6.1800    0.0189
    6.1900    0.0179
    6.2000    0.0176
    6.2100    0.0185
    6.2200    0.0194
    6.2300    0.0196
    6.2400    0.0195
    6.2500    0.0193
    6.2600    0.0197
    6.2700    0.0198
    6.2800    0.0203
    6.2900    0.0206
    6.3000    0.0199
    6.3100    0.0200
    6.3200    0.0194
    6.3300    0.0189
    6.3400    0.0192
    6.3500    0.0192
    6.3600    0.0194
    6.3700    0.0199
    6.3800    0.0205
    6.3900    0.0205
    6.4000    0.0203
    6.4100    0.0205
    6.4200    0.0202
    6.4300    0.0195
    6.4400    0.0191
    6.4500    0.0189
    6.4600    0.0195
    6.4700    0.0203
    6.4800    0.0204
    6.4900    0.0200
    6.5000    0.0201
    6.5100    0.0215
    6.5200    0.0223
    6.5300    0.0221
    6.5400    0.0215
    6.5500    0.0214
    6.5600    0.0217
    6.5700    0.0222
    6.5800    0.0222
    6.5900    0.0220
    6.6000    0.0218
    6.6100    0.0220
    6.6200    0.0222
    6.6300    0.0219
    6.6400    0.0218
    6.6500    0.0219
    6.6600    0.0224
    6.6700    0.0222
    6.6800    0.0217
    6.6900    0.0212
    6.7000    0.0210
    6.7100    0.0213
    6.7200    0.0209
    6.7300    0.0198
    6.7400    0.0192
    6.7500    0.0194
    6.7600    0.0197
    6.7700    0.0193
    6.7800    0.0183
    6.7900    0.0181
    6.8000    0.0184
    6.8100    0.0180
    6.8200    0.0184
    6.8300    0.0185
    6.8400    0.0182
    6.8500    0.0183
    6.8600    0.0187
    6.8700    0.0187
    6.8800    0.0183
    6.8900    0.0194
    6.9000    0.0197
    6.9100    0.0192
    6.9200    0.0194
    6.9300    0.0190
    6.9400    0.0185
    6.9500    0.0183
    6.9600    0.0192
    6.9700    0.0196
    6.9800    0.0194
    6.9900    0.0193
    7.0000    0.0197
    7.0100    0.0205
    7.0200    0.0204
    7.0300    0.0205
    7.0400    0.0207
    7.0500    0.0209
    7.0600    0.0212
    7.0700    0.0207
    7.0800    0.0204
    7.0900    0.0210
    7.1000    0.0211
    7.1100    0.0204
    7.1200    0.0208
    7.1300    0.0204
    7.1400    0.0199
    7.1500    0.0204
    7.1600    0.0206
    7.1700    0.0204
    7.1800    0.0201
    7.1900    0.0201
    7.2000    0.0203
    7.2100    0.0208
    7.2200    0.0207
    7.2300    0.0211
    7.2400    0.0215
    7.2500    0.0212
    7.2600    0.0207
    7.2700    0.0208
    7.2800    0.0211
    7.2900    0.0213
    7.3000    0.0215
    7.3100    0.0222
    7.3200    0.0225
    7.3300    0.0216
    7.3400    0.0215
    7.3500    0.0214
    7.3600    0.0218
    7.3700    0.0223
    7.3800    0.0222
    7.3900    0.0221
    7.4000    0.0223
    7.4100    0.0222
    7.4200    0.0221
    7.4300    0.0217
    7.4400    0.0211
    7.4500    0.0209
    7.4600    0.0202
    7.4700    0.0201
    7.4800    0.0199
    7.4900    0.0191
    7.5000    0.0184
    7.5100    0.0173
    7.5200    0.0165
    7.5300    0.0168
    7.5400    0.0170
    7.5500    0.0168
    7.5600    0.0163
    7.5700    0.0164
    7.5800    0.0168
    7.5900    0.0169
    7.6000    0.0174
    7.6100    0.0173
    7.6200    0.0174
    7.6300    0.0180
    7.6400    0.0181
    7.6500    0.0183
    7.6600    0.0192
    7.6700    0.0196
    7.6800    0.0193
    7.6900    0.0193
    7.7000    0.0195
    7.7100    0.0197
    7.7200    0.0198
    7.7300    0.0198
    7.7400    0.0203
    7.7500    0.0205
    7.7600    0.0205
    7.7700    0.0201
    7.7800    0.0193
    7.7900    0.0185
    7.8000    0.0176
    7.8100    0.0173
    7.8200    0.0166
    7.8300    0.0166
    7.8400    0.0177
    7.8500    0.0171
    7.8600    0.0160
    7.8700    0.0157
    7.8800    0.0151
    7.8900    0.0142
    7.9000    0.0145
    7.9100    0.0147
    7.9200    0.0145
    7.9300    0.0141
    7.9400    0.0136
    7.9500    0.0130
    7.9600    0.0126
    7.9700    0.0125
    7.9800    0.0125
    7.9900    0.0130
    8.0000    0.0136
    8.0100    0.0138
    8.0200    0.0136
    8.0300    0.0130
    8.0400    0.0126
    8.0500    0.0129
    8.0600    0.0130
    8.0700    0.0127
    8.0800    0.0127
    8.0900    0.0132
    8.1000    0.0129
    8.1100    0.0124
    8.1200    0.0126
    8.1300    0.0124
    8.1400    0.0126
    8.1500    0.0127
    8.1600    0.0123
    8.1700    0.0120
    8.1800    0.0122
    8.1900    0.0122
    8.2000    0.0123
    8.2100    0.0121
    8.2200    0.0113
    8.2300    0.0100
    8.2400    0.0092
    8.2500    0.0091
    8.2600    0.0085
    8.2700    0.0088
    8.2800    0.0091
    8.2900    0.0089
    8.3000    0.0084
    8.3100    0.0080
    8.3200    0.0081
    8.3300    0.0078
    8.3400    0.0072
    8.3500    0.0075
    8.3600    0.0072
    8.3700    0.0068
    8.3800    0.0073
    8.3900    0.0072
    8.4000    0.0064
    8.4100    0.0060
    8.4200    0.0064
    8.4300    0.0067
    8.4400    0.0071
    8.4500    0.0068
    8.4600    0.0066
    8.4700    0.0066
    8.4800    0.0063
    8.4900    0.0055
    8.5000    0.0053
    8.5100    0.0057
    8.5200    0.0059
    8.5300    0.0067
    8.5400    0.0067
    8.5500    0.0065
    8.5600    0.0066
    8.5700    0.0068
    8.5800    0.0073
    8.5900    0.0079
    8.6000    0.0078
    8.6100    0.0075
    8.6200    0.0074
    8.6300    0.0083
    8.6400    0.0095
    8.6500    0.0104
    8.6600    0.0112
    8.6700    0.0112
    8.6800    0.0115
    8.6900    0.0114
    8.7000    0.0115
    8.7100    0.0119
    8.7200    0.0112
    8.7300    0.0111
    8.7400    0.0109
    8.7500    0.0097
    8.7600    0.0093
    8.7700    0.0091
    8.7800    0.0085
    8.7900    0.0081
    8.8000    0.0079
    8.8100    0.0076
    8.8200    0.0076
    8.8300    0.0073
    8.8400    0.0066
    8.8500    0.0056
    8.8600    0.0048
    8.8700    0.0049
    8.8800    0.0048
    8.8900    0.0046
    8.9000    0.0049
    8.9100    0.0052
    8.9200    0.0058
    8.9300    0.0059
    8.9400    0.0053
    8.9500    0.0050
    8.9600    0.0048
    8.9700    0.0049
    8.9800    0.0057
    8.9900    0.0061
    9.0000    0.0059
    9.0100    0.0059
    9.0200    0.0058
    9.0300    0.0055
    9.0400    0.0053
    9.0500    0.0050
    9.0600    0.0053
    9.0700    0.0058
    9.0800    0.0063
    9.0900    0.0063
    9.1000    0.0060
    9.1100    0.0058
    9.1200    0.0055
    9.1300    0.0057
    9.1400    0.0060
    9.1500    0.0067
    9.1600    0.0071
    9.1700    0.0071
    9.1800    0.0068
    9.1900    0.0060
    9.2000    0.0052
    9.2100    0.0046
    9.2200    0.0043
    9.2300    0.0049
    9.2400    0.0051
    9.2500    0.0050
    9.2600    0.0048
    9.2700    0.0052
    9.2800    0.0061
    9.2900    0.0062
    9.3000    0.0061
    9.3100    0.0058
    9.3200    0.0055
    9.3300    0.0058
    9.3400    0.0062
    9.3500    0.0059
    9.3600    0.0055
    9.3700    0.0055
    9.3800    0.0049
    9.3900    0.0050
    9.4000    0.0053
    9.4100    0.0053
    9.4200    0.0053
    9.4300    0.0059
    9.4400    0.0062
    9.4500    0.0055
    9.4600    0.0048
    9.4700    0.0041
    9.4800    0.0036
    9.4900    0.0036
    9.5000    0.0031
    9.5100    0.0025
    9.5200    0.0023
    9.5300    0.0024
    9.5400    0.0024
    9.5500    0.0021
    9.5600    0.0018
    9.5700    0.0013
    9.5800    0.0010
    9.5900    0.0008
    9.6000    0.0005
    9.6100    0.0007
    9.6200    0.0011
    9.6300    0.0018
    9.6400    0.0021
    9.6500    0.0024
    9.6600    0.0020
    9.6700    0.0014
    9.6800    0.0019
    9.6900    0.0017
    9.7000    0.0018
    9.7100    0.0022
    9.7200    0.0027
    9.7300    0.0031
    9.7400    0.0033
    9.7500    0.0033
    9.7600    0.0027
    9.7700    0.0023
    9.7800    0.0022
    9.7900    0.0025
    9.8000    0.0026
    9.8100    0.0020
    9.8200    0.0028
    9.8300    0.0035
    9.8400    0.0036
    9.8500    0.0046
    9.8600    0.0046
    9.8700    0.0043
    9.8800    0.0042
    9.8900    0.0042
    9.9000    0.0049
    9.9100    0.0046
    9.9200    0.0046
    9.9300    0.0056
    9.9400    0.0055
    9.9500    0.0053
    9.9600    0.0053
    9.9700    0.0054
    9.9800    0.0058
    9.9900    0.0065
   10.0000    0.0067
    };

==> Data/Oscillator/sigma3/kf_exp_vel.tex <==
    \addplot[
    thick,
    green
    ]
    table {
         0         0
    0.0100   -0.0099
    0.0200   -0.0196
    0.0300   -0.0291
    0.0400   -0.0384
    0.0500   -0.0475
    0.0600   -0.0564
    0.0700   -0.0652
    0.0800   -0.0738
    0.0900   -0.0821
    0.1000   -0.0903
    0.1100   -0.0983
    0.1200   -0.1062
    0.1300   -0.1140
    0.1400   -0.1216
    0.1500   -0.1291
    0.1600   -0.1364
    0.1700   -0.1436
    0.1800   -0.1506
    0.1900   -0.1575
    0.2000   -0.1641
    0.2100   -0.1707
    0.2200   -0.1771
    0.2300   -0.1834
    0.2400   -0.1897
    0.2500   -0.1957
    0.2600   -0.2015
    0.2700   -0.2072
    0.2800   -0.2130
    0.2900   -0.2185
    0.3000   -0.2239
    0.3100   -0.2293
    0.3200   -0.2343
    0.3300   -0.2395
    0.3400   -0.2444
    0.3500   -0.2494
    0.3600   -0.2544
    0.3700   -0.2593
    0.3800   -0.2638
    0.3900   -0.2681
    0.4000   -0.2724
    0.4100   -0.2765
    0.4200   -0.2804
    0.4300   -0.2843
    0.4400   -0.2883
    0.4500   -0.2922
    0.4600   -0.2958
    0.4700   -0.2994
    0.4800   -0.3031
    0.4900   -0.3066
    0.5000   -0.3100
    0.5100   -0.3135
    0.5200   -0.3167
    0.5300   -0.3197
    0.5400   -0.3228
    0.5500   -0.3256
    0.5600   -0.3284
    0.5700   -0.3312
    0.5800   -0.3338
    0.5900   -0.3364
    0.6000   -0.3390
    0.6100   -0.3415
    0.6200   -0.3439
    0.6300   -0.3462
    0.6400   -0.3485
    0.6500   -0.3505
    0.6600   -0.3526
    0.6700   -0.3548
    0.6800   -0.3568
    0.6900   -0.3587
    0.7000   -0.3607
    0.7100   -0.3624
    0.7200   -0.3640
    0.7300   -0.3654
    0.7400   -0.3668
    0.7500   -0.3681
    0.7600   -0.3697
    0.7700   -0.3713
    0.7800   -0.3726
    0.7900   -0.3742
    0.8000   -0.3752
    0.8100   -0.3760
    0.8200   -0.3771
    0.8300   -0.3782
    0.8400   -0.3791
    0.8500   -0.3797
    0.8600   -0.3805
    0.8700   -0.3814
    0.8800   -0.3821
    0.8900   -0.3828
    0.9000   -0.3831
    0.9100   -0.3835
    0.9200   -0.3843
    0.9300   -0.3850
    0.9400   -0.3855
    0.9500   -0.3856
    0.9600   -0.3856
    0.9700   -0.3857
    0.9800   -0.3859
    0.9900   -0.3862
    1.0000   -0.3863
    1.0100   -0.3861
    1.0200   -0.3859
    1.0300   -0.3861
    1.0400   -0.3862
    1.0500   -0.3858
    1.0600   -0.3856
    1.0700   -0.3853
    1.0800   -0.3849
    1.0900   -0.3848
    1.1000   -0.3847
    1.1100   -0.3842
    1.1200   -0.3836
    1.1300   -0.3832
    1.1400   -0.3829
    1.1500   -0.3828
    1.1600   -0.3824
    1.1700   -0.3820
    1.1800   -0.3816
    1.1900   -0.3809
    1.2000   -0.3804
    1.2100   -0.3801
    1.2200   -0.3797
    1.2300   -0.3792
    1.2400   -0.3786
    1.2500   -0.3779
    1.2600   -0.3772
    1.2700   -0.3765
    1.2800   -0.3758
    1.2900   -0.3752
    1.3000   -0.3745
    1.3100   -0.3737
    1.3200   -0.3730
    1.3300   -0.3722
    1.3400   -0.3712
    1.3500   -0.3705
    1.3600   -0.3698
    1.3700   -0.3688
    1.3800   -0.3679
    1.3900   -0.3670
    1.4000   -0.3660
    1.4100   -0.3651
    1.4200   -0.3640
    1.4300   -0.3630
    1.4400   -0.3621
    1.4500   -0.3612
    1.4600   -0.3603
    1.4700   -0.3592
    1.4800   -0.3579
    1.4900   -0.3568
    1.5000   -0.3557
    1.5100   -0.3544
    1.5200   -0.3532
    1.5300   -0.3521
    1.5400   -0.3509
    1.5500   -0.3498
    1.5600   -0.3485
    1.5700   -0.3472
    1.5800   -0.3460
    1.5900   -0.3446
    1.6000   -0.3433
    1.6100   -0.3422
    1.6200   -0.3410
    1.6300   -0.3397
    1.6400   -0.3384
    1.6500   -0.3371
    1.6600   -0.3358
    1.6700   -0.3344
    1.6800   -0.3330
    1.6900   -0.3317
    1.7000   -0.3303
    1.7100   -0.3289
    1.7200   -0.3277
    1.7300   -0.3264
    1.7400   -0.3249
    1.7500   -0.3237
    1.7600   -0.3223
    1.7700   -0.3209
    1.7800   -0.3195
    1.7900   -0.3181
    1.8000   -0.3167
    1.8100   -0.3153
    1.8200   -0.3139
    1.8300   -0.3124
    1.8400   -0.3110
    1.8500   -0.3096
    1.8600   -0.3080
    1.8700   -0.3065
    1.8800   -0.3050
    1.8900   -0.3035
    1.9000   -0.3020
    1.9100   -0.3004
    1.9200   -0.2988
    1.9300   -0.2973
    1.9400   -0.2957
    1.9500   -0.2942
    1.9600   -0.2926
    1.9700   -0.2911
    1.9800   -0.2895
    1.9900   -0.2880
    2.0000   -0.2865
    2.0100   -0.2849
    2.0200   -0.2833
    2.0300   -0.2817
    2.0400   -0.2802
    2.0500   -0.2787
    2.0600   -0.2771
    2.0700   -0.2756
    2.0800   -0.2740
    2.0900   -0.2724
    2.1000   -0.2708
    2.1100   -0.2692
    2.1200   -0.2677
    2.1300   -0.2661
    2.1400   -0.2646
    2.1500   -0.2630
    2.1600   -0.2615
    2.1700   -0.2599
    2.1800   -0.2584
    2.1900   -0.2569
    2.2000   -0.2553
    2.2100   -0.2538
    2.2200   -0.2522
    2.2300   -0.2507
    2.2400   -0.2492
    2.2500   -0.2477
    2.2600   -0.2462
    2.2700   -0.2446
    2.2800   -0.2431
    2.2900   -0.2416
    2.3000   -0.2401
    2.3100   -0.2386
    2.3200   -0.2371
    2.3300   -0.2356
    2.3400   -0.2341
    2.3500   -0.2326
    2.3600   -0.2311
    2.3700   -0.2296
    2.3800   -0.2281
    2.3900   -0.2267
    2.4000   -0.2252
    2.4100   -0.2237
    2.4200   -0.2222
    2.4300   -0.2207
    2.4400   -0.2193
    2.4500   -0.2178
    2.4600   -0.2163
    2.4700   -0.2149
    2.4800   -0.2135
    2.4900   -0.2120
    2.5000   -0.2106
    2.5100   -0.2092
    2.5200   -0.2078
    2.5300   -0.2064
    2.5400   -0.2050
    2.5500   -0.2036
    2.5600   -0.2023
    2.5700   -0.2009
    2.5800   -0.1995
    2.5900   -0.1981
    2.6000   -0.1967
    2.6100   -0.1954
    2.6200   -0.1941
    2.6300   -0.1927
    2.6400   -0.1914
    2.6500   -0.1901
    2.6600   -0.1888
    2.6700   -0.1876
    2.6800   -0.1863
    2.6900   -0.1851
    2.7000   -0.1838
    2.7100   -0.1825
    2.7200   -0.1812
    2.7300   -0.1800
    2.7400   -0.1787
    2.7500   -0.1775
    2.7600   -0.1763
    2.7700   -0.1750
    2.7800   -0.1738
    2.7900   -0.1727
    2.8000   -0.1715
    2.8100   -0.1703
    2.8200   -0.1690
    2.8300   -0.1678
    2.8400   -0.1667
    2.8500   -0.1656
    2.8600   -0.1644
    2.8700   -0.1633
    2.8800   -0.1622
    2.8900   -0.1610
    2.9000   -0.1598
    2.9100   -0.1587
    2.9200   -0.1577
    2.9300   -0.1566
    2.9400   -0.1555
    2.9500   -0.1545
    2.9600   -0.1534
    2.9700   -0.1524
    2.9800   -0.1513
    2.9900   -0.1503
    3.0000   -0.1492
    3.0100   -0.1481
    3.0200   -0.1470
    3.0300   -0.1460
    3.0400   -0.1450
    3.0500   -0.1439
    3.0600   -0.1429
    3.0700   -0.1419
    3.0800   -0.1409
    3.0900   -0.1399
    3.1000   -0.1390
    3.1100   -0.1379
    3.1200   -0.1369
    3.1300   -0.1360
    3.1400   -0.1350
    3.1500   -0.1341
    3.1600   -0.1332
    3.1700   -0.1322
    3.1800   -0.1313
    3.1900   -0.1304
    3.2000   -0.1295
    3.2100   -0.1286
    3.2200   -0.1277
    3.2300   -0.1268
    3.2400   -0.1259
    3.2500   -0.1250
    3.2600   -0.1241
    3.2700   -0.1232
    3.2800   -0.1222
    3.2900   -0.1212
    3.3000   -0.1204
    3.3100   -0.1195
    3.3200   -0.1186
    3.3300   -0.1178
    3.3400   -0.1171
    3.3500   -0.1163
    3.3600   -0.1155
    3.3700   -0.1147
    3.3800   -0.1138
    3.3900   -0.1130
    3.4000   -0.1121
    3.4100   -0.1113
    3.4200   -0.1104
    3.4300   -0.1095
    3.4400   -0.1086
    3.4500   -0.1077
    3.4600   -0.1068
    3.4700   -0.1060
    3.4800   -0.1053
    3.4900   -0.1045
    3.5000   -0.1037
    3.5100   -0.1030
    3.5200   -0.1022
    3.5300   -0.1014
    3.5400   -0.1006
    3.5500   -0.0997
    3.5600   -0.0989
    3.5700   -0.0981
    3.5800   -0.0974
    3.5900   -0.0967
    3.6000   -0.0960
    3.6100   -0.0952
    3.6200   -0.0944
    3.6300   -0.0937
    3.6400   -0.0929
    3.6500   -0.0921
    3.6600   -0.0915
    3.6700   -0.0908
    3.6800   -0.0901
    3.6900   -0.0894
    3.7000   -0.0886
    3.7100   -0.0879
    3.7200   -0.0872
    3.7300   -0.0866
    3.7400   -0.0859
    3.7500   -0.0853
    3.7600   -0.0847
    3.7700   -0.0841
    3.7800   -0.0834
    3.7900   -0.0827
    3.8000   -0.0820
    3.8100   -0.0813
    3.8200   -0.0807
    3.8300   -0.0801
    3.8400   -0.0795
    3.8500   -0.0789
    3.8600   -0.0783
    3.8700   -0.0777
    3.8800   -0.0771
    3.8900   -0.0765
    3.9000   -0.0758
    3.9100   -0.0752
    3.9200   -0.0747
    3.9300   -0.0742
    3.9400   -0.0736
    3.9500   -0.0731
    3.9600   -0.0726
    3.9700   -0.0722
    3.9800   -0.0717
    3.9900   -0.0711
    4.0000   -0.0705
    4.0100   -0.0700
    4.0200   -0.0696
    4.0300   -0.0690
    4.0400   -0.0685
    4.0500   -0.0680
    4.0600   -0.0675
    4.0700   -0.0670
    4.0800   -0.0665
    4.0900   -0.0660
    4.1000   -0.0657
    4.1100   -0.0653
    4.1200   -0.0647
    4.1300   -0.0642
    4.1400   -0.0637
    4.1500   -0.0631
    4.1600   -0.0627
    4.1700   -0.0622
    4.1800   -0.0617
    4.1900   -0.0613
    4.2000   -0.0608
    4.2100   -0.0603
    4.2200   -0.0599
    4.2300   -0.0595
    4.2400   -0.0589
    4.2500   -0.0584
    4.2600   -0.0579
    4.2700   -0.0574
    4.2800   -0.0570
    4.2900   -0.0567
    4.3000   -0.0563
    4.3100   -0.0559
    4.3200   -0.0554
    4.3300   -0.0550
    4.3400   -0.0546
    4.3500   -0.0542
    4.3600   -0.0538
    4.3700   -0.0534
    4.3800   -0.0530
    4.3900   -0.0526
    4.4000   -0.0522
    4.4100   -0.0517
    4.4200   -0.0513
    4.4300   -0.0510
    4.4400   -0.0506
    4.4500   -0.0502
    4.4600   -0.0499
    4.4700   -0.0495
    4.4800   -0.0492
    4.4900   -0.0489
    4.5000   -0.0485
    4.5100   -0.0481
    4.5200   -0.0478
    4.5300   -0.0476
    4.5400   -0.0473
    4.5500   -0.0470
    4.5600   -0.0466
    4.5700   -0.0463
    4.5800   -0.0460
    4.5900   -0.0457
    4.6000   -0.0455
    4.6100   -0.0452
    4.6200   -0.0450
    4.6300   -0.0447
    4.6400   -0.0444
    4.6500   -0.0442
    4.6600   -0.0439
    4.6700   -0.0436
    4.6800   -0.0433
    4.6900   -0.0429
    4.7000   -0.0426
    4.7100   -0.0423
    4.7200   -0.0420
    4.7300   -0.0417
    4.7400   -0.0414
    4.7500   -0.0412
    4.7600   -0.0409
    4.7700   -0.0406
    4.7800   -0.0403
    4.7900   -0.0400
    4.8000   -0.0398
    4.8100   -0.0395
    4.8200   -0.0391
    4.8300   -0.0386
    4.8400   -0.0382
    4.8500   -0.0379
    4.8600   -0.0376
    4.8700   -0.0374
    4.8800   -0.0371
    4.8900   -0.0369
    4.9000   -0.0366
    4.9100   -0.0363
    4.9200   -0.0362
    4.9300   -0.0358
    4.9400   -0.0354
    4.9500   -0.0351
    4.9600   -0.0347
    4.9700   -0.0345
    4.9800   -0.0342
    4.9900   -0.0339
    5.0000   -0.0336
    5.0100   -0.0333
    5.0200   -0.0331
    5.0300   -0.0328
    5.0400   -0.0325
    5.0500   -0.0323
    5.0600   -0.0321
    5.0700   -0.0317
    5.0800   -0.0314
    5.0900   -0.0312
    5.1000   -0.0310
    5.1100   -0.0307
    5.1200   -0.0304
    5.1300   -0.0301
    5.1400   -0.0299
    5.1500   -0.0297
    5.1600   -0.0295
    5.1700   -0.0292
    5.1800   -0.0290
    5.1900   -0.0289
    5.2000   -0.0286
    5.2100   -0.0284
    5.2200   -0.0282
    5.2300   -0.0281
    5.2400   -0.0279
    5.2500   -0.0277
    5.2600   -0.0275
    5.2700   -0.0274
    5.2800   -0.0272
    5.2900   -0.0270
    5.3000   -0.0269
    5.3100   -0.0267
    5.3200   -0.0266
    5.3300   -0.0263
    5.3400   -0.0258
    5.3500   -0.0255
    5.3600   -0.0253
    5.3700   -0.0252
    5.3800   -0.0252
    5.3900   -0.0251
    5.4000   -0.0249
    5.4100   -0.0248
    5.4200   -0.0246
    5.4300   -0.0245
    5.4400   -0.0244
    5.4500   -0.0243
    5.4600   -0.0241
    5.4700   -0.0239
    5.4800   -0.0238
    5.4900   -0.0237
    5.5000   -0.0235
    5.5100   -0.0234
    5.5200   -0.0234
    5.5300   -0.0233
    5.5400   -0.0232
    5.5500   -0.0232
    5.5600   -0.0232
    5.5700   -0.0230
    5.5800   -0.0229
    5.5900   -0.0227
    5.6000   -0.0226
    5.6100   -0.0226
    5.6200   -0.0225
    5.6300   -0.0224
    5.6400   -0.0223
    5.6500   -0.0220
    5.6600   -0.0219
    5.6700   -0.0217
    5.6800   -0.0215
    5.6900   -0.0214
    5.7000   -0.0214
    5.7100   -0.0213
    5.7200   -0.0211
    5.7300   -0.0210
    5.7400   -0.0208
    5.7500   -0.0207
    5.7600   -0.0206
    5.7700   -0.0205
    5.7800   -0.0205
    5.7900   -0.0205
    5.8000   -0.0204
    5.8100   -0.0203
    5.8200   -0.0202
    5.8300   -0.0200
    5.8400   -0.0199
    5.8500   -0.0199
    5.8600   -0.0199
    5.8700   -0.0198
    5.8800   -0.0197
    5.8900   -0.0196
    5.9000   -0.0196
    5.9100   -0.0196
    5.9200   -0.0195
    5.9300   -0.0194
    5.9400   -0.0193
    5.9500   -0.0193
    5.9600   -0.0191
    5.9700   -0.0191
    5.9800   -0.0191
    5.9900   -0.0189
    6.0000   -0.0188
    6.0100   -0.0187
    6.0200   -0.0186
    6.0300   -0.0185
    6.0400   -0.0184
    6.0500   -0.0182
    6.0600   -0.0181
    6.0700   -0.0180
    6.0800   -0.0178
    6.0900   -0.0177
    6.1000   -0.0176
    6.1100   -0.0175
    6.1200   -0.0175
    6.1300   -0.0174
    6.1400   -0.0173
    6.1500   -0.0171
    6.1600   -0.0170
    6.1700   -0.0169
    6.1800   -0.0169
    6.1900   -0.0169
    6.2000   -0.0169
    6.2100   -0.0167
    6.2200   -0.0165
    6.2300   -0.0164
    6.2400   -0.0163
    6.2500   -0.0162
    6.2600   -0.0161
    6.2700   -0.0160
    6.2800   -0.0159
    6.2900   -0.0158
    6.3000   -0.0158
    6.3100   -0.0157
    6.3200   -0.0158
    6.3300   -0.0157
    6.3400   -0.0156
    6.3500   -0.0156
    6.3600   -0.0155
    6.3700   -0.0153
    6.3800   -0.0152
    6.3900   -0.0152
    6.4000   -0.0151
    6.4100   -0.0151
    6.4200   -0.0151
    6.4300   -0.0151
    6.4400   -0.0151
    6.4500   -0.0150
    6.4600   -0.0149
    6.4700   -0.0148
    6.4800   -0.0147
    6.4900   -0.0147
    6.5000   -0.0147
    6.5100   -0.0145
    6.5200   -0.0143
    6.5300   -0.0143
    6.5400   -0.0144
    6.5500   -0.0144
    6.5600   -0.0143
    6.5700   -0.0142
    6.5800   -0.0142
    6.5900   -0.0142
    6.6000   -0.0142
    6.6100   -0.0142
    6.6200   -0.0141
    6.6300   -0.0142
    6.6400   -0.0142
    6.6500   -0.0141
    6.6600   -0.0141
    6.6700   -0.0141
    6.6800   -0.0141
    6.6900   -0.0142
    6.7000   -0.0142
    6.7100   -0.0141
    6.7200   -0.0141
    6.7300   -0.0142
    6.7400   -0.0142
    6.7500   -0.0142
    6.7600   -0.0141
    6.7700   -0.0141
    6.7800   -0.0142
    6.7900   -0.0142
    6.8000   -0.0141
    6.8100   -0.0140
    6.8200   -0.0140
    6.8300   -0.0139
    6.8400   -0.0139
    6.8500   -0.0138
    6.8600   -0.0137
    6.8700   -0.0137
    6.8800   -0.0137
    6.8900   -0.0135
    6.9000   -0.0134
    6.9100   -0.0135
    6.9200   -0.0134
    6.9300   -0.0134
    6.9400   -0.0135
    6.9500   -0.0134
    6.9600   -0.0133
    6.9700   -0.0132
    6.9800   -0.0132
    6.9900   -0.0132
    7.0000   -0.0131
    7.0100   -0.0130
    7.0200   -0.0130
    7.0300   -0.0130
    7.0400   -0.0130
    7.0500   -0.0129
    7.0600   -0.0129
    7.0700   -0.0129
    7.0800   -0.0130
    7.0900   -0.0129
    7.1000   -0.0129
    7.1100   -0.0129
    7.1200   -0.0129
    7.1300   -0.0129
    7.1400   -0.0130
    7.1500   -0.0129
    7.1600   -0.0128
    7.1700   -0.0129
    7.1800   -0.0129
    7.1900   -0.0129
    7.2000   -0.0128
    7.2100   -0.0128
    7.2200   -0.0128
    7.2300   -0.0127
    7.2400   -0.0127
    7.2500   -0.0127
    7.2600   -0.0128
    7.2700   -0.0127
    7.2800   -0.0127
    7.2900   -0.0127
    7.3000   -0.0127
    7.3100   -0.0126
    7.3200   -0.0126
    7.3300   -0.0127
    7.3400   -0.0127
    7.3500   -0.0127
    7.3600   -0.0127
    7.3700   -0.0126
    7.3800   -0.0126
    7.3900   -0.0127
    7.4000   -0.0126
    7.4100   -0.0127
    7.4200   -0.0127
    7.4300   -0.0127
    7.4400   -0.0128
    7.4500   -0.0128
    7.4600   -0.0129
    7.4700   -0.0129
    7.4800   -0.0129
    7.4900   -0.0130
    7.5000   -0.0130
    7.5100   -0.0131
    7.5200   -0.0132
    7.5300   -0.0131
    7.5400   -0.0130
    7.5500   -0.0130
    7.5600   -0.0130
    7.5700   -0.0129
    7.5800   -0.0128
    7.5900   -0.0128
    7.6000   -0.0127
    7.6100   -0.0127
    7.6200   -0.0126
    7.6300   -0.0125
    7.6400   -0.0125
    7.6500   -0.0124
    7.6600   -0.0123
    7.6700   -0.0122
    7.6800   -0.0122
    7.6900   -0.0122
    7.7000   -0.0122
    7.7100   -0.0122
    7.7200   -0.0121
    7.7300   -0.0121
    7.7400   -0.0121
    7.7500   -0.0121
    7.7600   -0.0121
    7.7700   -0.0121
    7.7800   -0.0122
    7.7900   -0.0123
    7.8000   -0.0124
    7.8100   -0.0124
    7.8200   -0.0124
    7.8300   -0.0124
    7.8400   -0.0122
    7.8500   -0.0123
    7.8600   -0.0124
    7.8700   -0.0123
    7.8800   -0.0124
    7.8900   -0.0124
    7.9000   -0.0123
    7.9100   -0.0122
    7.9200   -0.0122
    7.9300   -0.0122
    7.9400   -0.0122
    7.9500   -0.0122
    7.9600   -0.0122
    7.9700   -0.0121
    7.9800   -0.0120
    7.9900   -0.0119
    8.0000   -0.0117
    8.0100   -0.0117
    8.0200   -0.0116
    8.0300   -0.0116
    8.0400   -0.0116
    8.0500   -0.0115
    8.0600   -0.0114
    8.0700   -0.0114
    8.0800   -0.0113
    8.0900   -0.0112
    8.1000   -0.0112
    8.1100   -0.0112
    8.1200   -0.0111
    8.1300   -0.0111
    8.1400   -0.0110
    8.1500   -0.0109
    8.1600   -0.0109
    8.1700   -0.0109
    8.1800   -0.0108
    8.1900   -0.0108
    8.2000   -0.0107
    8.2100   -0.0107
    8.2200   -0.0107
    8.2300   -0.0108
    8.2400   -0.0108
    8.2500   -0.0107
    8.2600   -0.0107
    8.2700   -0.0106
    8.2800   -0.0105
    8.2900   -0.0104
    8.3000   -0.0104
    8.3100   -0.0103
    8.3200   -0.0102
    8.3300   -0.0102
    8.3400   -0.0101
    8.3500   -0.0100
    8.3600   -0.0100
    8.3700   -0.0099
    8.3800   -0.0098
    8.3900   -0.0097
    8.4000   -0.0097
    8.4100   -0.0096
    8.4200   -0.0095
    8.4300   -0.0094
    8.4400   -0.0092
    8.4500   -0.0092
    8.4600   -0.0091
    8.4700   -0.0090
    8.4800   -0.0090
    8.4900   -0.0090
    8.5000   -0.0089
    8.5100   -0.0088
    8.5200   -0.0087
    8.5300   -0.0085
    8.5400   -0.0084
    8.5500   -0.0084
    8.5600   -0.0083
    8.5700   -0.0082
    8.5800   -0.0080
    8.5900   -0.0079
    8.6000   -0.0079
    8.6100   -0.0079
    8.6200   -0.0078
    8.6300   -0.0076
    8.6400   -0.0075
    8.6500   -0.0073
    8.6600   -0.0072
    8.6700   -0.0072
    8.6800   -0.0072
    8.6900   -0.0072
    8.7000   -0.0072
    8.7100   -0.0071
    8.7200   -0.0072
    8.7300   -0.0072
    8.7400   -0.0072
    8.7500   -0.0073
    8.7600   -0.0074
    8.7700   -0.0073
    8.7800   -0.0074
    8.7900   -0.0074
    8.8000   -0.0074
    8.8100   -0.0074
    8.8200   -0.0073
    8.8300   -0.0073
    8.8400   -0.0073
    8.8500   -0.0074
    8.8600   -0.0074
    8.8700   -0.0073
    8.8800   -0.0073
    8.8900   -0.0072
    8.9000   -0.0071
    8.9100   -0.0070
    8.9200   -0.0069
    8.9300   -0.0068
    8.9400   -0.0068
    8.9500   -0.0068
    8.9600   -0.0068
    8.9700   -0.0067
    8.9800   -0.0065
    8.9900   -0.0064
    9.0000   -0.0064
    9.0100   -0.0064
    9.0200   -0.0063
    9.0300   -0.0063
    9.0400   -0.0063
    9.0500   -0.0063
    9.0600   -0.0062
    9.0700   -0.0061
    9.0800   -0.0060
    9.0900   -0.0059
    9.1000   -0.0059
    9.1100   -0.0059
    9.1200   -0.0059
    9.1300   -0.0058
    9.1400   -0.0058
    9.1500   -0.0057
    9.1600   -0.0056
    9.1700   -0.0056
    9.1800   -0.0056
    9.1900   -0.0056
    9.2000   -0.0057
    9.2100   -0.0057
    9.2200   -0.0057
    9.2300   -0.0056
    9.2400   -0.0055
    9.2500   -0.0055
    9.2600   -0.0055
    9.2700   -0.0054
    9.2800   -0.0052
    9.2900   -0.0052
    9.3000   -0.0052
    9.3100   -0.0052
    9.3200   -0.0052
    9.3300   -0.0051
    9.3400   -0.0051
    9.3500   -0.0051
    9.3600   -0.0051
    9.3700   -0.0051
    9.3800   -0.0051
    9.3900   -0.0051
    9.4000   -0.0050
    9.4100   -0.0050
    9.4200   -0.0049
    9.4300   -0.0048
    9.4400   -0.0048
    9.4500   -0.0048
    9.4600   -0.0049
    9.4700   -0.0049
    9.4800   -0.0050
    9.4900   -0.0049
    9.5000   -0.0049
    9.5100   -0.0049
    9.5200   -0.0049
    9.5300   -0.0048
    9.5400   -0.0048
    9.5500   -0.0048
    9.5600   -0.0047
    9.5700   -0.0047
    9.5800   -0.0047
    9.5900   -0.0047
    9.6000   -0.0046
    9.6100   -0.0045
    9.6200   -0.0044
    9.6300   -0.0043
    9.6400   -0.0042
    9.6500   -0.0041
    9.6600   -0.0041
    9.6700   -0.0041
    9.6800   -0.0040
    9.6900   -0.0040
    9.7000   -0.0039
    9.7100   -0.0038
    9.7200   -0.0037
    9.7300   -0.0037
    9.7400   -0.0036
    9.7500   -0.0036
    9.7600   -0.0036
    9.7700   -0.0036
    9.7800   -0.0036
    9.7900   -0.0035
    9.8000   -0.0035
    9.8100   -0.0035
    9.8200   -0.0034
    9.8300   -0.0033
    9.8400   -0.0032
    9.8500   -0.0031
    9.8600   -0.0031
    9.8700   -0.0031
    9.8800   -0.0031
    9.8900   -0.0031
    9.9000   -0.0030
    9.9100   -0.0031
    9.9200   -0.0031
    9.9300   -0.0029
    9.9400   -0.0030
    9.9500   -0.0030
    9.9600   -0.0030
    9.9700   -0.0030
    9.9800   -0.0029
    9.9900   -0.0029
   10.0000   -0.0029
    };

==> Data/Oscillator/sigma3/kf_tr_pos.tex <==
    \addplot[
    thick,
    dashed,
    magenta
    ]
    table {
     0    1.0000
    0.0100    0.9972
    0.0200    0.9928
    0.0300    0.9839
    0.0400    0.9791
    0.0500    0.9755
    0.0600    0.9714
    0.0700    0.9674
    0.0800    0.9639
    0.0900    0.9552
    0.1000    0.9464
    0.1100    0.9481
    0.1200    0.9495
    0.1300    0.9492
    0.1400    0.9465
    0.1500    0.9422
    0.1600    0.9392
    0.1700    0.9361
    0.1800    0.9310
    0.1900    0.9250
    0.2000    0.9207
    0.2100    0.9158
    0.2200    0.9120
    0.2300    0.9147
    0.2400    0.9126
    0.2500    0.9067
    0.2600    0.9011
    0.2700    0.8966
    0.2800    0.8982
    0.2900    0.8932
    0.3000    0.8900
    0.3100    0.8881
    0.3200    0.8823
    0.3300    0.8811
    0.3400    0.8789
    0.3500    0.8780
    0.3600    0.8815
    0.3700    0.8818
    0.3800    0.8751
    0.3900    0.8685
    0.4000    0.8637
    0.4100    0.8581
    0.4200    0.8523
    0.4300    0.8470
    0.4400    0.8467
    0.4500    0.8449
    0.4600    0.8396
    0.4700    0.8372
    0.4800    0.8366
    0.4900    0.8348
    0.5000    0.8327
    0.5100    0.8315
    0.5200    0.8283
    0.5300    0.8248
    0.5400    0.8217
    0.5500    0.8167
    0.5600    0.8130
    0.5700    0.8105
    0.5800    0.8068
    0.5900    0.8033
    0.6000    0.8013
    0.6100    0.7992
    0.6200    0.7963
    0.6300    0.7933
    0.6400    0.7904
    0.6500    0.7862
    0.6600    0.7827
    0.6700    0.7818
    0.6800    0.7789
    0.6900    0.7767
    0.7000    0.7752
    0.7100    0.7713
    0.7200    0.7672
    0.7300    0.7625
    0.7400    0.7578
    0.7500    0.7540
    0.7600    0.7525
    0.7700    0.7511
    0.7800    0.7486
    0.7900    0.7476
    0.8000    0.7434
    0.8100    0.7379
    0.8200    0.7351
    0.8300    0.7329
    0.8400    0.7295
    0.8500    0.7244
    0.8600    0.7213
    0.8700    0.7188
    0.8800    0.7161
    0.8900    0.7130
    0.9000    0.7079
    0.9100    0.7043
    0.9200    0.7027
    0.9300    0.7019
    0.9400    0.6990
    0.9500    0.6940
    0.9600    0.6893
    0.9700    0.6855
    0.9800    0.6822
    0.9900    0.6799
    1.0000    0.6772
    1.0100    0.6721
    1.0200    0.6683
    1.0300    0.6666
    1.0400    0.6642
    1.0500    0.6599
    1.0600    0.6565
    1.0700    0.6528
    1.0800    0.6490
    1.0900    0.6469
    1.1000    0.6450
    1.1100    0.6413
    1.1200    0.6372
    1.1300    0.6341
    1.1400    0.6323
    1.1500    0.6314
    1.1600    0.6290
    1.1700    0.6272
    1.1800    0.6248
    1.1900    0.6212
    1.2000    0.6193
    1.2100    0.6183
    1.2200    0.6169
    1.2300    0.6150
    1.2400    0.6123
    1.2500    0.6099
    1.2600    0.6073
    1.2700    0.6046
    1.2800    0.6026
    1.2900    0.6008
    1.3000    0.5987
    1.3100    0.5961
    1.3200    0.5945
    1.3300    0.5920
    1.3400    0.5890
    1.3500    0.5876
    1.3600    0.5860
    1.3700    0.5833
    1.3800    0.5810
    1.3900    0.5787
    1.4000    0.5764
    1.4100    0.5742
    1.4200    0.5717
    1.4300    0.5695
    1.4400    0.5680
    1.4500    0.5663
    1.4600    0.5650
    1.4700    0.5626
    1.4800    0.5590
    1.4900    0.5568
    1.5000    0.5543
    1.5100    0.5511
    1.5200    0.5485
    1.5300    0.5469
    1.5400    0.5449
    1.5500    0.5430
    1.5600    0.5406
    1.5700    0.5378
    1.5800    0.5354
    1.5900    0.5329
    1.6000    0.5304
    1.6100    0.5294
    1.6200    0.5279
    1.6300    0.5258
    1.6400    0.5235
    1.6500    0.5214
    1.6600    0.5195
    1.6700    0.5170
    1.6800    0.5148
    1.6900    0.5126
    1.7000    0.5108
    1.7100    0.5085
    1.7200    0.5075
    1.7300    0.5064
    1.7400    0.5037
    1.7500    0.5028
    1.7600    0.5012
    1.7700    0.4989
    1.7800    0.4967
    1.7900    0.4946
    1.8000    0.4931
    1.8100    0.4913
    1.8200    0.4895
    1.8300    0.4873
    1.8400    0.4860
    1.8500    0.4838
    1.8600    0.4804
    1.8700    0.4782
    1.8800    0.4762
    1.8900    0.4740
    1.9000    0.4715
    1.9100    0.4688
    1.9200    0.4665
    1.9300    0.4643
    1.9400    0.4619
    1.9500    0.4597
    1.9600    0.4573
    1.9700    0.4557
    1.9800    0.4539
    1.9900    0.4522
    2.0000    0.4510
    2.0100    0.4485
    2.0200    0.4460
    2.0300    0.4443
    2.0400    0.4432
    2.0500    0.4417
    2.0600    0.4400
    2.0700    0.4385
    2.0800    0.4365
    2.0900    0.4341
    2.1000    0.4317
    2.1100    0.4293
    2.1200    0.4277
    2.1300    0.4264
    2.1400    0.4255
    2.1500    0.4246
    2.1600    0.4221
    2.1700    0.4202
    2.1800    0.4195
    2.1900    0.4179
    2.2000    0.4161
    2.2100    0.4147
    2.2200    0.4133
    2.2300    0.4119
    2.2400    0.4104
    2.2500    0.4087
    2.2600    0.4071
    2.2700    0.4052
    2.2800    0.4037
    2.2900    0.4025
    2.3000    0.4010
    2.3100    0.3994
    2.3200    0.3973
    2.3300    0.3954
    2.3400    0.3937
    2.3500    0.3923
    2.3600    0.3912
    2.3700    0.3900
    2.3800    0.3882
    2.3900    0.3859
    2.4000    0.3843
    2.4100    0.3827
    2.4200    0.3813
    2.4300    0.3805
    2.4400    0.3791
    2.4500    0.3775
    2.4600    0.3766
    2.4700    0.3755
    2.4800    0.3744
    2.4900    0.3735
    2.5000    0.3723
    2.5100    0.3710
    2.5200    0.3698
    2.5300    0.3682
    2.5400    0.3667
    2.5500    0.3654
    2.5600    0.3638
    2.5700    0.3627
    2.5800    0.3616
    2.5900    0.3608
    2.6000    0.3600
    2.6100    0.3585
    2.6200    0.3575
    2.6300    0.3570
    2.6400    0.3563
    2.6500    0.3547
    2.6600    0.3533
    2.6700    0.3518
    2.6800    0.3499
    2.6900    0.3486
    2.7000    0.3475
    2.7100    0.3468
    2.7200    0.3457
    2.7300    0.3445
    2.7400    0.3432
    2.7500    0.3418
    2.7600    0.3411
    2.7700    0.3402
    2.7800    0.3387
    2.7900    0.3372
    2.8000    0.3359
    2.8100    0.3349
    2.8200    0.3344
    2.8300    0.3335
    2.8400    0.3321
    2.8500    0.3307
    2.8600    0.3295
    2.8700    0.3286
    2.8800    0.3271
    2.8900    0.3261
    2.9000    0.3255
    2.9100    0.3245
    2.9200    0.3231
    2.9300    0.3216
    2.9400    0.3206
    2.9500    0.3192
    2.9600    0.3176
    2.9700    0.3162
    2.9800    0.3150
    2.9900    0.3137
    3.0000    0.3123
    3.0100    0.3118
    3.0200    0.3108
    3.0300    0.3094
    3.0400    0.3083
    3.0500    0.3074
    3.0600    0.3065
    3.0700    0.3054
    3.0800    0.3042
    3.0900    0.3028
    3.1000    0.3016
    3.1100    0.3009
    3.1200    0.3002
    3.1300    0.2988
    3.1400    0.2974
    3.1500    0.2963
    3.1600    0.2951
    3.1700    0.2938
    3.1800    0.2924
    3.1900    0.2910
    3.2000    0.2896
    3.2100    0.2883
    3.2200    0.2871
    3.2300    0.2860
    3.2400    0.2848
    3.2500    0.2836
    3.2600    0.2824
    3.2700    0.2814
    3.2800    0.2806
    3.2900    0.2798
    3.3000    0.2787
    3.3100    0.2776
    3.3200    0.2766
    3.3300    0.2751
    3.3400    0.2733
    3.3500    0.2714
    3.3600    0.2700
    3.3700    0.2687
    3.3800    0.2674
    3.3900    0.2662
    3.4000    0.2650
    3.4100    0.2637
    3.4200    0.2626
    3.4300    0.2618
    3.4400    0.2613
    3.4500    0.2608
    3.4600    0.2597
    3.4700    0.2586
    3.4800    0.2574
    3.4900    0.2564
    3.5000    0.2550
    3.5100    0.2535
    3.5200    0.2527
    3.5300    0.2517
    3.5400    0.2506
    3.5500    0.2498
    3.5600    0.2492
    3.5700    0.2486
    3.5800    0.2473
    3.5900    0.2457
    3.6000    0.2448
    3.6100    0.2441
    3.6200    0.2431
    3.6300    0.2422
    3.6400    0.2415
    3.6500    0.2408
    3.6600    0.2397
    3.6700    0.2385
    3.6800    0.2375
    3.6900    0.2366
    3.7000    0.2359
    3.7100    0.2351
    3.7200    0.2343
    3.7300    0.2333
    3.7400    0.2323
    3.7500    0.2314
    3.7600    0.2303
    3.7700    0.2291
    3.7800    0.2284
    3.7900    0.2276
    3.8000    0.2269
    3.8100    0.2264
    3.8200    0.2255
    3.8300    0.2245
    3.8400    0.2235
    3.8500    0.2226
    3.8600    0.2219
    3.8700    0.2210
    3.8800    0.2201
    3.8900    0.2196
    3.9000    0.2192
    3.9100    0.2186
    3.9200    0.2178
    3.9300    0.2166
    3.9400    0.2157
    3.9500    0.2149
    3.9600    0.2137
    3.9700    0.2123
    3.9800    0.2114
    3.9900    0.2105
    4.0000    0.2099
    4.0100    0.2091
    4.0200    0.2078
    4.0300    0.2072
    4.0400    0.2062
    4.0500    0.2053
    4.0600    0.2044
    4.0700    0.2035
    4.0800    0.2029
    4.0900    0.2019
    4.1000    0.2003
    4.1100    0.1990
    4.1200    0.1984
    4.1300    0.1978
    4.1400    0.1970
    4.1500    0.1964
    4.1600    0.1954
    4.1700    0.1947
    4.1800    0.1940
    4.1900    0.1930
    4.2000    0.1922
    4.2100    0.1914
    4.2200    0.1903
    4.2300    0.1894
    4.2400    0.1891
    4.2500    0.1887
    4.2600    0.1885
    4.2700    0.1880
    4.2800    0.1871
    4.2900    0.1858
    4.3000    0.1848
    4.3100    0.1841
    4.3200    0.1836
    4.3300    0.1828
    4.3400    0.1820
    4.3500    0.1815
    4.3600    0.1806
    4.3700    0.1798
    4.3800    0.1793
    4.3900    0.1786
    4.4000    0.1781
    4.4100    0.1779
    4.4200    0.1772
    4.4300    0.1765
    4.4400    0.1758
    4.4500    0.1751
    4.4600    0.1746
    4.4700    0.1738
    4.4800    0.1729
    4.4900    0.1721
    4.5000    0.1718
    4.5100    0.1714
    4.5200    0.1704
    4.5300    0.1695
    4.5400    0.1688
    4.5500    0.1679
    4.5600    0.1673
    4.5700    0.1667
    4.5800    0.1659
    4.5900    0.1650
    4.6000    0.1641
    4.6100    0.1631
    4.6200    0.1620
    4.6300    0.1611
    4.6400    0.1602
    4.6500    0.1592
    4.6600    0.1584
    4.6700    0.1576
    4.6800    0.1567
    4.6900    0.1562
    4.7000    0.1554
    4.7100    0.1548
    4.7200    0.1541
    4.7300    0.1531
    4.7400    0.1522
    4.7500    0.1513
    4.7600    0.1504
    4.7700    0.1495
    4.7800    0.1487
    4.7900    0.1478
    4.8000    0.1466
    4.8100    0.1457
    4.8200    0.1456
    4.8300    0.1457
    4.8400    0.1454
    4.8500    0.1447
    4.8600    0.1440
    4.8700    0.1433
    4.8800    0.1427
    4.8900    0.1416
    4.9000    0.1407
    4.9100    0.1400
    4.9200    0.1388
    4.9300    0.1383
    4.9400    0.1382
    4.9500    0.1376
    4.9600    0.1373
    4.9700    0.1367
    4.9800    0.1359
    4.9900    0.1355
    5.0000    0.1350
    5.0100    0.1345
    5.0200    0.1339
    5.0300    0.1334
    5.0400    0.1329
    5.0500    0.1320
    5.0600    0.1314
    5.0700    0.1314
    5.0800    0.1311
    5.0900    0.1303
    5.1000    0.1298
    5.1100    0.1295
    5.1200    0.1293
    5.1300    0.1290
    5.1400    0.1284
    5.1500    0.1279
    5.1600    0.1274
    5.1700    0.1272
    5.1800    0.1267
    5.1900    0.1259
    5.2000    0.1257
    5.2100    0.1253
    5.2200    0.1246
    5.2300    0.1238
    5.2400    0.1231
    5.2500    0.1226
    5.2600    0.1221
    5.2700    0.1215
    5.2800    0.1209
    5.2900    0.1203
    5.3000    0.1197
    5.3100    0.1190
    5.3200    0.1183
    5.3300    0.1183
    5.3400    0.1190
    5.3500    0.1192
    5.3600    0.1191
    5.3700    0.1185
    5.3800    0.1177
    5.3900    0.1171
    5.4000    0.1166
    5.4100    0.1163
    5.4200    0.1159
    5.4300    0.1154
    5.4400    0.1148
    5.4500    0.1141
    5.4600    0.1139
    5.4700    0.1137
    5.4800    0.1133
    5.4900    0.1130
    5.5000    0.1128
    5.5100    0.1122
    5.5200    0.1114
    5.5300    0.1110
    5.5400    0.1102
    5.5500    0.1092
    5.5600    0.1085
    5.5700    0.1081
    5.5800    0.1078
    5.5900    0.1074
    5.6000    0.1069
    5.6100    0.1059
    5.6200    0.1052
    5.6300    0.1047
    5.6400    0.1042
    5.6500    0.1043
    5.6600    0.1041
    5.6700    0.1038
    5.6800    0.1038
    5.6900    0.1032
    5.7000    0.1026
    5.7100    0.1022
    5.7200    0.1019
    5.7300    0.1017
    5.7400    0.1015
    5.7500    0.1013
    5.7600    0.1010
    5.7700    0.1006
    5.7800    0.1000
    5.7900    0.0989
    5.8000    0.0986
    5.8100    0.0983
    5.8200    0.0978
    5.8300    0.0978
    5.8400    0.0975
    5.8500    0.0968
    5.8600    0.0962
    5.8700    0.0958
    5.8800    0.0955
    5.8900    0.0949
    5.9000    0.0941
    5.9100    0.0934
    5.9200    0.0930
    5.9300    0.0925
    5.9400    0.0920
    5.9500    0.0914
    5.9600    0.0910
    5.9700    0.0904
    5.9800    0.0896
    5.9900    0.0895
    6.0000    0.0891
    6.0100    0.0886
    6.0200    0.0883
    6.0300    0.0879
    6.0400    0.0874
    6.0500    0.0872
    6.0600    0.0867
    6.0700    0.0863
    6.0800    0.0863
    6.0900    0.0862
    6.1000    0.0859
    6.1100    0.0854
    6.1200    0.0850
    6.1300    0.0845
    6.1400    0.0842
    6.1500    0.0843
    6.1600    0.0840
    6.1700    0.0837
    6.1800    0.0830
    6.1900    0.0821
    6.2000    0.0816
    6.2100    0.0818
    6.2200    0.0820
    6.2300    0.0818
    6.2400    0.0814
    6.2500    0.0810
    6.2600    0.0809
    6.2700    0.0807
    6.2800    0.0806
    6.2900    0.0805
    6.3000    0.0798
    6.3100    0.0795
    6.3200    0.0789
    6.3300    0.0784
    6.3400    0.0782
    6.3500    0.0779
    6.3600    0.0777
    6.3700    0.0777
    6.3800    0.0777
    6.3900    0.0775
    6.4000    0.0771
    6.4100    0.0769
    6.4200    0.0765
    6.4300    0.0758
    6.4400    0.0753
    6.4500    0.0749
    6.4600    0.0749
    6.4700    0.0751
    6.4800    0.0748
    6.4900    0.0743
    6.5000    0.0742
    6.5100    0.0746
    6.5200    0.0748
    6.5300    0.0744
    6.5400    0.0738
    6.5500    0.0735
    6.5600    0.0734
    6.5700    0.0734
    6.5800    0.0731
    6.5900    0.0727
    6.6000    0.0724
    6.6100    0.0722
    6.6200    0.0721
    6.6300    0.0717
    6.6400    0.0713
    6.6500    0.0712
    6.6600    0.0712
    6.6700    0.0708
    6.6800    0.0702
    6.6900    0.0697
    6.7000    0.0693
    6.7100    0.0692
    6.7200    0.0688
    6.7300    0.0679
    6.7400    0.0673
    6.7500    0.0672
    6.7600    0.0671
    6.7700    0.0667
    6.7800    0.0658
    6.7900    0.0655
    6.8000    0.0654
    6.8100    0.0650
    6.8200    0.0649
    6.8300    0.0648
    6.8400    0.0644
    6.8500    0.0642
    6.8600    0.0642
    6.8700    0.0639
    6.8800    0.0635
    6.8900    0.0638
    6.9000    0.0638
    6.9100    0.0633
    6.9200    0.0632
    6.9300    0.0627
    6.9400    0.0622
    6.9500    0.0619
    6.9600    0.0621
    6.9700    0.0621
    6.9800    0.0618
    6.9900    0.0616
    7.0000    0.0615
    7.0100    0.0617
    7.0200    0.0615
    7.0300    0.0614
    7.0400    0.0612
    7.0500    0.0611
    7.0600    0.0611
    7.0700    0.0606
    7.0800    0.0602
    7.0900    0.0603
    7.1000    0.0602
    7.1100    0.0596
    7.1200    0.0596
    7.1300    0.0592
    7.1400    0.0587
    7.1500    0.0588
    7.1600    0.0587
    7.1700    0.0584
    7.1800    0.0580
    7.1900    0.0578
    7.2000    0.0577
    7.2100    0.0578
    7.2200    0.0576
    7.2300    0.0575
    7.2400    0.0576
    7.2500    0.0572
    7.2600    0.0568
    7.2700    0.0566
    7.2800    0.0566
    7.2900    0.0566
    7.3000    0.0564
    7.3100    0.0567
    7.3200    0.0566
    7.3300    0.0560
    7.3400    0.0557
    7.3500    0.0555
    7.3600    0.0555
    7.3700    0.0556
    7.3800    0.0553
    7.3900    0.0551
    7.4000    0.0551
    7.4100    0.0548
    7.4200    0.0546
    7.4300    0.0542
    7.4400    0.0537
    7.4500    0.0534
    7.4600    0.0529
    7.4700    0.0526
    7.4800    0.0523
    7.4900    0.0518
    7.5000    0.0512
    7.5100    0.0504
    7.5200    0.0498
    7.5300    0.0498
    7.5400    0.0497
    7.5500    0.0495
    7.5600    0.0490
    7.5700    0.0489
    7.5800    0.0489
    7.5900    0.0489
    7.6000    0.0490
    7.6100    0.0487
    7.6200    0.0486
    7.6300    0.0488
    7.6400    0.0487
    7.6500    0.0486
    7.6600    0.0490
    7.6700    0.0490
    7.6800    0.0487
    7.6900    0.0486
    7.7000    0.0485
    7.7100    0.0485
    7.7200    0.0484
    7.7300    0.0482
    7.7400    0.0483
    7.7500    0.0483
    7.7600    0.0482
    7.7700    0.0478
    7.7800    0.0472
    7.7900    0.0467
    7.8000    0.0460
    7.8100    0.0457
    7.8200    0.0451
    7.8300    0.0450
    7.8400    0.0454
    7.8500    0.0450
    7.8600    0.0442
    7.8700    0.0439
    7.8800    0.0435
    7.8900    0.0429
    7.9000    0.0428
    7.9100    0.0428
    7.9200    0.0426
    7.9300    0.0422
    7.9400    0.0418
    7.9500    0.0413
    7.9600    0.0410
    7.9700    0.0408
    7.9800    0.0407
    7.9900    0.0408
    8.0000    0.0410
    8.0100    0.0410
    8.0200    0.0407
    8.0300    0.0403
    8.0400    0.0399
    8.0500    0.0399
    8.0600    0.0399
    8.0700    0.0396
    8.0800    0.0395
    8.0900    0.0396
    8.1000    0.0393
    8.1100    0.0389
    8.1200    0.0389
    8.1300    0.0387
    8.1400    0.0386
    8.1500    0.0386
    8.1600    0.0382
    8.1700    0.0379
    8.1800    0.0379
    8.1900    0.0378
    8.2000    0.0377
    8.2100    0.0375
    8.2200    0.0369
    8.2300    0.0361
    8.2400    0.0355
    8.2500    0.0354
    8.2600    0.0349
    8.2700    0.0349
    8.2800    0.0350
    8.2900    0.0347
    8.3000    0.0344
    8.3100    0.0340
    8.3200    0.0340
    8.3300    0.0337
    8.3400    0.0332
    8.3500    0.0333
    8.3600    0.0330
    8.3700    0.0327
    8.3800    0.0328
    8.3900    0.0327
    8.4000    0.0321
    8.4100    0.0318
    8.4200    0.0318
    8.4300    0.0319
    8.4400    0.0320
    8.4500    0.0317
    8.4600    0.0315
    8.4700    0.0314
    8.4800    0.0311
    8.4900    0.0306
    8.5000    0.0304
    8.5100    0.0305
    8.5200    0.0304
    8.5300    0.0308
    8.5400    0.0307
    8.5500    0.0304
    8.5600    0.0304
    8.5700    0.0304
    8.5800    0.0306
    8.5900    0.0308
    8.6000    0.0306
    8.6100    0.0303
    8.6200    0.0301
    8.6300    0.0306
    8.6400    0.0311
    8.6500    0.0315
    8.6600    0.0318
    8.6700    0.0317
    8.6800    0.0318
    8.6900    0.0316
    8.7000    0.0316
    8.7100    0.0317
    8.7200    0.0312
    8.7300    0.0311
    8.7400    0.0309
    8.7500    0.0301
    8.7600    0.0298
    8.7700    0.0296
    8.7800    0.0291
    8.7900    0.0288
    8.8000    0.0286
    8.8100    0.0284
    8.8200    0.0283
    8.8300    0.0280
    8.8400    0.0275
    8.8500    0.0269
    8.8600    0.0263
    8.8700    0.0263
    8.8800    0.0261
    8.8900    0.0260
    8.9000    0.0260
    8.9100    0.0261
    8.9200    0.0263
    8.9300    0.0262
    8.9400    0.0258
    8.9500    0.0256
    8.9600    0.0254
    8.9700    0.0253
    8.9800    0.0257
    8.9900    0.0258
    9.0000    0.0256
    9.0100    0.0255
    9.0200    0.0254
    9.0300    0.0251
    9.0400    0.0249
    9.0500    0.0247
    9.0600    0.0247
    9.0700    0.0249
    9.0800    0.0251
    9.0900    0.0250
    9.1000    0.0247
    9.1100    0.0245
    9.1200    0.0243
    9.1300    0.0243
    9.1400    0.0244
    9.1500    0.0247
    9.1600    0.0248
    9.1700    0.0247
    9.1800    0.0245
    9.1900    0.0239
    9.2000    0.0234
    9.2100    0.0230
    9.2200    0.0228
    9.2300    0.0230
    9.2400    0.0230
    9.2500    0.0229
    9.2600    0.0227
    9.2700    0.0228
    9.2800    0.0232
    9.2900    0.0232
    9.3000    0.0230
    9.3100    0.0228
    9.3200    0.0225
    9.3300    0.0226
    9.3400    0.0228
    9.3500    0.0225
    9.3600    0.0222
    9.3700    0.0221
    9.3800    0.0218
    9.3900    0.0217
    9.4000    0.0218
    9.4100    0.0217
    9.4200    0.0216
    9.4300    0.0219
    9.4400    0.0220
    9.4500    0.0215
    9.4600    0.0210
    9.4700    0.0206
    9.4800    0.0202
    9.4900    0.0202
    9.5000    0.0198
    9.5100    0.0194
    9.5200    0.0192
    9.5300    0.0192
    9.5400    0.0192
    9.5500    0.0189
    9.5600    0.0187
    9.5700    0.0183
    9.5800    0.0181
    9.5900    0.0179
    9.6000    0.0177
    9.6100    0.0177
    9.6200    0.0178
    9.6300    0.0181
    9.6400    0.0183
    9.6500    0.0183
    9.6600    0.0180
    9.6700    0.0176
    9.6800    0.0178
    9.6900    0.0177
    9.7000    0.0176
    9.7100    0.0178
    9.7200    0.0180
    9.7300    0.0181
    9.7400    0.0182
    9.7500    0.0181
    9.7600    0.0177
    9.7700    0.0174
    9.7800    0.0173
    9.7900    0.0174
    9.8000    0.0173
    9.8100    0.0169
    9.8200    0.0173
    9.8300    0.0176
    9.8400    0.0176
    9.8500    0.0181
    9.8600    0.0180
    9.8700    0.0178
    9.8800    0.0177
    9.8900    0.0176
    9.9000    0.0179
    9.9100    0.0177
    9.9200    0.0176
    9.9300    0.0181
    9.9400    0.0180
    9.9500    0.0178
    9.9600    0.0177
    9.9700    0.0177
    9.9800    0.0179
    9.9900    0.0182
   10.0000    0.0182
    };

==> Data/Oscillator/sigma3/kf_tr_vel.tex <==
    \addplot[
    thick,
    dashed,
    magenta
    ]
    table {
         0         0
    0.0100   -0.0098
    0.0200   -0.0193
    0.0300   -0.0285
    0.0400   -0.0373
    0.0500   -0.0458
    0.0600   -0.0541
    0.0700   -0.0620
    0.0800   -0.0696
    0.0900   -0.0770
    0.1000   -0.0839
    0.1100   -0.0908
    0.1200   -0.0975
    0.1300   -0.1040
    0.1400   -0.1102
    0.1500   -0.1162
    0.1600   -0.1220
    0.1700   -0.1276
    0.1800   -0.1328
    0.1900   -0.1379
    0.2000   -0.1428
    0.2100   -0.1474
    0.2200   -0.1520
    0.2300   -0.1567
    0.2400   -0.1610
    0.2500   -0.1650
    0.2600   -0.1688
    0.2700   -0.1724
    0.2800   -0.1764
    0.2900   -0.1798
    0.3000   -0.1831
    0.3100   -0.1865
    0.3200   -0.1894
    0.3300   -0.1925
    0.3400   -0.1955
    0.3500   -0.1984
    0.3600   -0.2018
    0.3700   -0.2048
    0.3800   -0.2069
    0.3900   -0.2088
    0.4000   -0.2109
    0.4100   -0.2127
    0.4200   -0.2144
    0.4300   -0.2161
    0.4400   -0.2183
    0.4500   -0.2202
    0.4600   -0.2216
    0.4700   -0.2233
    0.4800   -0.2251
    0.4900   -0.2268
    0.5000   -0.2283
    0.5100   -0.2299
    0.5200   -0.2312
    0.5300   -0.2323
    0.5400   -0.2334
    0.5500   -0.2342
    0.5600   -0.2350
    0.5700   -0.2361
    0.5800   -0.2368
    0.5900   -0.2376
    0.6000   -0.2385
    0.6100   -0.2394
    0.6200   -0.2401
    0.6300   -0.2407
    0.6400   -0.2413
    0.6500   -0.2417
    0.6600   -0.2420
    0.6700   -0.2429
    0.6800   -0.2433
    0.6900   -0.2438
    0.7000   -0.2444
    0.7100   -0.2445
    0.7200   -0.2446
    0.7300   -0.2444
    0.7400   -0.2442
    0.7500   -0.2442
    0.7600   -0.2446
    0.7700   -0.2450
    0.7800   -0.2451
    0.7900   -0.2456
    0.8000   -0.2453
    0.8100   -0.2447
    0.8200   -0.2446
    0.8300   -0.2447
    0.8400   -0.2445
    0.8500   -0.2438
    0.8600   -0.2436
    0.8700   -0.2435
    0.8800   -0.2433
    0.8900   -0.2430
    0.9000   -0.2422
    0.9100   -0.2418
    0.9200   -0.2418
    0.9300   -0.2419
    0.9400   -0.2415
    0.9500   -0.2407
    0.9600   -0.2399
    0.9700   -0.2392
    0.9800   -0.2387
    0.9900   -0.2384
    1.0000   -0.2379
    1.0100   -0.2369
    1.0200   -0.2362
    1.0300   -0.2360
    1.0400   -0.2355
    1.0500   -0.2347
    1.0600   -0.2340
    1.0700   -0.2332
    1.0800   -0.2324
    1.0900   -0.2320
    1.1000   -0.2316
    1.1100   -0.2308
    1.1200   -0.2298
    1.1300   -0.2291
    1.1400   -0.2287
    1.1500   -0.2285
    1.1600   -0.2279
    1.1700   -0.2275
    1.1800   -0.2269
    1.1900   -0.2260
    1.2000   -0.2255
    1.2100   -0.2252
    1.2200   -0.2248
    1.2300   -0.2243
    1.2400   -0.2237
    1.2500   -0.2230
    1.2600   -0.2224
    1.2700   -0.2217
    1.2800   -0.2211
    1.2900   -0.2206
    1.3000   -0.2200
    1.3100   -0.2193
    1.3200   -0.2188
    1.3300   -0.2181
    1.3400   -0.2173
    1.3500   -0.2168
    1.3600   -0.2163
    1.3700   -0.2156
    1.3800   -0.2149
    1.3900   -0.2142
    1.4000   -0.2136
    1.4100   -0.2129
    1.4200   -0.2122
    1.4300   -0.2115
    1.4400   -0.2110
    1.4500   -0.2104
    1.4600   -0.2099
    1.4700   -0.2092
    1.4800   -0.2083
    1.4900   -0.2076
    1.5000   -0.2068
    1.5100   -0.2059
    1.5200   -0.2052
    1.5300   -0.2046
    1.5400   -0.2039
    1.5500   -0.2033
    1.5600   -0.2025
    1.5700   -0.2017
    1.5800   -0.2010
    1.5900   -0.2002
    1.6000   -0.1994
    1.6100   -0.1989
    1.6200   -0.1984
    1.6300   -0.1976
    1.6400   -0.1969
    1.6500   -0.1962
    1.6600   -0.1956
    1.6700   -0.1948
    1.6800   -0.1941
    1.6900   -0.1933
    1.7000   -0.1927
    1.7100   -0.1919
    1.7200   -0.1914
    1.7300   -0.1909
    1.7400   -0.1901
    1.7500   -0.1896
    1.7600   -0.1890
    1.7700   -0.1883
    1.7800   -0.1876
    1.7900   -0.1869
    1.8000   -0.1863
    1.8100   -0.1856
    1.8200   -0.1850
    1.8300   -0.1843
    1.8400   -0.1837
    1.8500   -0.1830
    1.8600   -0.1821
    1.8700   -0.1814
    1.8800   -0.1807
    1.8900   -0.1799
    1.9000   -0.1792
    1.9100   -0.1784
    1.9200   -0.1776
    1.9300   -0.1769
    1.9400   -0.1761
    1.9500   -0.1754
    1.9600   -0.1746
    1.9700   -0.1740
    1.9800   -0.1733
    1.9900   -0.1727
    2.0000   -0.1721
    2.0100   -0.1713
    2.0200   -0.1705
    2.0300   -0.1699
    2.0400   -0.1693
    2.0500   -0.1687
    2.0600   -0.1680
    2.0700   -0.1674
    2.0800   -0.1668
    2.0900   -0.1660
    2.1000   -0.1653
    2.1100   -0.1645
    2.1200   -0.1639
    2.1300   -0.1633
    2.1400   -0.1628
    2.1500   -0.1622
    2.1600   -0.1615
    2.1700   -0.1608
    2.1800   -0.1603
    2.1900   -0.1597
    2.2000   -0.1591
    2.2100   -0.1585
    2.2200   -0.1579
    2.2300   -0.1573
    2.2400   -0.1567
    2.2500   -0.1561
    2.2600   -0.1555
    2.2700   -0.1549
    2.2800   -0.1543
    2.2900   -0.1538
    2.3000   -0.1532
    2.3100   -0.1526
    2.3200   -0.1519
    2.3300   -0.1513
    2.3400   -0.1507
    2.3500   -0.1501
    2.3600   -0.1496
    2.3700   -0.1490
    2.3800   -0.1484
    2.3900   -0.1478
    2.4000   -0.1472
    2.4100   -0.1466
    2.4200   -0.1461
    2.4300   -0.1455
    2.4400   -0.1450
    2.4500   -0.1444
    2.4600   -0.1439
    2.4700   -0.1434
    2.4800   -0.1429
    2.4900   -0.1424
    2.5000   -0.1419
    2.5100   -0.1414
    2.5200   -0.1408
    2.5300   -0.1403
    2.5400   -0.1398
    2.5500   -0.1392
    2.5600   -0.1387
    2.5700   -0.1382
    2.5800   -0.1377
    2.5900   -0.1372
    2.6000   -0.1368
    2.6100   -0.1363
    2.6200   -0.1358
    2.6300   -0.1354
    2.6400   -0.1349
    2.6500   -0.1344
    2.6600   -0.1339
    2.6700   -0.1334
    2.6800   -0.1329
    2.6900   -0.1324
    2.7000   -0.1320
    2.7100   -0.1315
    2.7200   -0.1310
    2.7300   -0.1306
    2.7400   -0.1301
    2.7500   -0.1296
    2.7600   -0.1292
    2.7700   -0.1288
    2.7800   -0.1283
    2.7900   -0.1278
    2.8000   -0.1273
    2.8100   -0.1269
    2.8200   -0.1265
    2.8300   -0.1261
    2.8400   -0.1256
    2.8500   -0.1251
    2.8600   -0.1247
    2.8700   -0.1243
    2.8800   -0.1238
    2.8900   -0.1234
    2.9000   -0.1230
    2.9100   -0.1226
    2.9200   -0.1221
    2.9300   -0.1217
    2.9400   -0.1213
    2.9500   -0.1208
    2.9600   -0.1204
    2.9700   -0.1199
    2.9800   -0.1195
    2.9900   -0.1190
    3.0000   -0.1186
    3.0100   -0.1182
    3.0200   -0.1178
    3.0300   -0.1173
    3.0400   -0.1169
    3.0500   -0.1165
    3.0600   -0.1161
    3.0700   -0.1157
    3.0800   -0.1153
    3.0900   -0.1148
    3.1000   -0.1144
    3.1100   -0.1140
    3.1200   -0.1136
    3.1300   -0.1132
    3.1400   -0.1128
    3.1500   -0.1124
    3.1600   -0.1120
    3.1700   -0.1116
    3.1800   -0.1111
    3.1900   -0.1107
    3.2000   -0.1103
    3.2100   -0.1099
    3.2200   -0.1095
    3.2300   -0.1091
    3.2400   -0.1086
    3.2500   -0.1082
    3.2600   -0.1078
    3.2700   -0.1074
    3.2800   -0.1070
    3.2900   -0.1066
    3.3000   -0.1062
    3.3100   -0.1058
    3.3200   -0.1054
    3.3300   -0.1050
    3.3400   -0.1046
    3.3500   -0.1042
    3.3600   -0.1038
    3.3700   -0.1034
    3.3800   -0.1029
    3.3900   -0.1025
    3.4000   -0.1021
    3.4100   -0.1017
    3.4200   -0.1013
    3.4300   -0.1009
    3.4400   -0.1005
    3.4500   -0.1001
    3.4600   -0.0997
    3.4700   -0.0993
    3.4800   -0.0989
    3.4900   -0.0985
    3.5000   -0.0981
    3.5100   -0.0977
    3.5200   -0.0973
    3.5300   -0.0969
    3.5400   -0.0965
    3.5500   -0.0962
    3.5600   -0.0958
    3.5700   -0.0954
    3.5800   -0.0950
    3.5900   -0.0946
    3.6000   -0.0943
    3.6100   -0.0939
    3.6200   -0.0935
    3.6300   -0.0931
    3.6400   -0.0928
    3.6500   -0.0924
    3.6600   -0.0920
    3.6700   -0.0917
    3.6800   -0.0913
    3.6900   -0.0909
    3.7000   -0.0906
    3.7100   -0.0902
    3.7200   -0.0899
    3.7300   -0.0895
    3.7400   -0.0892
    3.7500   -0.0888
    3.7600   -0.0885
    3.7700   -0.0881
    3.7800   -0.0878
    3.7900   -0.0874
    3.8000   -0.0871
    3.8100   -0.0867
    3.8200   -0.0864
    3.8300   -0.0860
    3.8400   -0.0857
    3.8500   -0.0854
    3.8600   -0.0850
    3.8700   -0.0847
    3.8800   -0.0844
    3.8900   -0.0840
    3.9000   -0.0837
    3.9100   -0.0834
    3.9200   -0.0831
    3.9300   -0.0828
    3.9400   -0.0825
    3.9500   -0.0821
    3.9600   -0.0818
    3.9700   -0.0815
    3.9800   -0.0812
    3.9900   -0.0809
    4.0000   -0.0806
    4.0100   -0.0802
    4.0200   -0.0799
    4.0300   -0.0796
    4.0400   -0.0793
    4.0500   -0.0790
    4.0600   -0.0787
    4.0700   -0.0784
    4.0800   -0.0780
    4.0900   -0.0777
    4.1000   -0.0774
    4.1100   -0.0771
    4.1200   -0.0768
    4.1300   -0.0765
    4.1400   -0.0762
    4.1500   -0.0759
    4.1600   -0.0756
    4.1700   -0.0752
    4.1800   -0.0749
    4.1900   -0.0746
    4.2000   -0.0743
    4.2100   -0.0740
    4.2200   -0.0737
    4.2300   -0.0734
    4.2400   -0.0731
    4.2500   -0.0728
    4.2600   -0.0725
    4.2700   -0.0722
    4.2800   -0.0719
    4.2900   -0.0716
    4.3000   -0.0714
    4.3100   -0.0711
    4.3200   -0.0708
    4.3300   -0.0705
    4.3400   -0.0702
    4.3500   -0.0699
    4.3600   -0.0696
    4.3700   -0.0694
    4.3800   -0.0691
    4.3900   -0.0688
    4.4000   -0.0685
    4.4100   -0.0682
    4.4200   -0.0679
    4.4300   -0.0677
    4.4400   -0.0674
    4.4500   -0.0672
    4.4600   -0.0669
    4.4700   -0.0666
    4.4800   -0.0664
    4.4900   -0.0661
    4.5000   -0.0658
    4.5100   -0.0656
    4.5200   -0.0653
    4.5300   -0.0651
    4.5400   -0.0648
    4.5500   -0.0646
    4.5600   -0.0643
    4.5700   -0.0641
    4.5800   -0.0638
    4.5900   -0.0636
    4.6000   -0.0633
    4.6100   -0.0631
    4.6200   -0.0628
    4.6300   -0.0626
    4.6400   -0.0623
    4.6500   -0.0621
    4.6600   -0.0618
    4.6700   -0.0616
    4.6800   -0.0613
    4.6900   -0.0610
    4.7000   -0.0608
    4.7100   -0.0605
    4.7200   -0.0602
    4.7300   -0.0600
    4.7400   -0.0597
    4.7500   -0.0595
    4.7600   -0.0592
    4.7700   -0.0590
    4.7800   -0.0587
    4.7900   -0.0584
    4.8000   -0.0582
    4.8100   -0.0579
    4.8200   -0.0576
    4.8300   -0.0573
    4.8400   -0.0571
    4.8500   -0.0568
    4.8600   -0.0566
    4.8700   -0.0563
    4.8800   -0.0561
    4.8900   -0.0558
    4.9000   -0.0556
    4.9100   -0.0553
    4.9200   -0.0551
    4.9300   -0.0548
    4.9400   -0.0546
    4.9500   -0.0543
    4.9600   -0.0540
    4.9700   -0.0538
    4.9800   -0.0536
    4.9900   -0.0533
    5.0000   -0.0531
    5.0100   -0.0528
    5.0200   -0.0526
    5.0300   -0.0523
    5.0400   -0.0521
    5.0500   -0.0519
    5.0600   -0.0517
    5.0700   -0.0514
    5.0800   -0.0512
    5.0900   -0.0510
    5.1000   -0.0507
    5.1100   -0.0505
    5.1200   -0.0503
    5.1300   -0.0500
    5.1400   -0.0498
    5.1500   -0.0496
    5.1600   -0.0494
    5.1700   -0.0492
    5.1800   -0.0490
    5.1900   -0.0488
    5.2000   -0.0486
    5.2100   -0.0484
    5.2200   -0.0482
    5.2300   -0.0480
    5.2400   -0.0478
    5.2500   -0.0476
    5.2600   -0.0474
    5.2700   -0.0472
    5.2800   -0.0470
    5.2900   -0.0468
    5.3000   -0.0466
    5.3100   -0.0464
    5.3200   -0.0463
    5.3300   -0.0460
    5.3400   -0.0458
    5.3500   -0.0456
    5.3600   -0.0454
    5.3700   -0.0452
    5.3800   -0.0450
    5.3900   -0.0449
    5.4000   -0.0447
    5.4100   -0.0445
    5.4200   -0.0444
    5.4300   -0.0442
    5.4400   -0.0440
    5.4500   -0.0439
    5.4600   -0.0437
    5.4700   -0.0435
    5.4800   -0.0433
    5.4900   -0.0432
    5.5000   -0.0430
    5.5100   -0.0428
    5.5200   -0.0427
    5.5300   -0.0425
    5.5400   -0.0424
    5.5500   -0.0422
    5.5600   -0.0421
    5.5700   -0.0419
    5.5800   -0.0417
    5.5900   -0.0415
    5.6000   -0.0414
    5.6100   -0.0412
    5.6200   -0.0411
    5.6300   -0.0409
    5.6400   -0.0407
    5.6500   -0.0405
    5.6600   -0.0403
    5.6700   -0.0402
    5.6800   -0.0400
    5.6900   -0.0398
    5.7000   -0.0397
    5.7100   -0.0395
    5.7200   -0.0393
    5.7300   -0.0392
    5.7400   -0.0390
    5.7500   -0.0388
    5.7600   -0.0387
    5.7700   -0.0385
    5.7800   -0.0384
    5.7900   -0.0383
    5.8000   -0.0381
    5.8100   -0.0380
    5.8200   -0.0378
    5.8300   -0.0376
    5.8400   -0.0375
    5.8500   -0.0373
    5.8600   -0.0372
    5.8700   -0.0371
    5.8800   -0.0369
    5.8900   -0.0368
    5.9000   -0.0366
    5.9100   -0.0365
    5.9200   -0.0363
    5.9300   -0.0362
    5.9400   -0.0360
    5.9500   -0.0359
    5.9600   -0.0357
    5.9700   -0.0356
    5.9800   -0.0354
    5.9900   -0.0353
    6.0000   -0.0351
    6.0100   -0.0349
    6.0200   -0.0348
    6.0300   -0.0346
    6.0400   -0.0345
    6.0500   -0.0343
    6.0600   -0.0342
    6.0700   -0.0340
    6.0800   -0.0338
    6.0900   -0.0337
    6.1000   -0.0335
    6.1100   -0.0334
    6.1200   -0.0332
    6.1300   -0.0331
    6.1400   -0.0330
    6.1500   -0.0328
    6.1600   -0.0326
    6.1700   -0.0325
    6.1800   -0.0324
    6.1900   -0.0323
    6.2000   -0.0321
    6.2100   -0.0320
    6.2200   -0.0318
    6.2300   -0.0316
    6.2400   -0.0315
    6.2500   -0.0314
    6.2600   -0.0313
    6.2700   -0.0311
    6.2800   -0.0310
    6.2900   -0.0308
    6.3000   -0.0307
    6.3100   -0.0306
    6.3200   -0.0305
    6.3300   -0.0304
    6.3400   -0.0303
    6.3500   -0.0301
    6.3600   -0.0300
    6.3700   -0.0299
    6.3800   -0.0297
    6.3900   -0.0296
    6.4000   -0.0295
    6.4100   -0.0294
    6.4200   -0.0293
    6.4300   -0.0292
    6.4400   -0.0291
    6.4500   -0.0290
    6.4600   -0.0288
    6.4700   -0.0287
    6.4800   -0.0286
    6.4900   -0.0285
    6.5000   -0.0284
    6.5100   -0.0282
    6.5200   -0.0281
    6.5300   -0.0280
    6.5400   -0.0279
    6.5500   -0.0278
    6.5600   -0.0277
    6.5700   -0.0276
    6.5800   -0.0275
    6.5900   -0.0274
    6.6000   -0.0273
    6.6100   -0.0272
    6.6200   -0.0271
    6.6300   -0.0270
    6.6400   -0.0269
    6.6500   -0.0268
    6.6600   -0.0267
    6.6700   -0.0267
    6.6800   -0.0266
    6.6900   -0.0265
    6.7000   -0.0264
    6.7100   -0.0263
    6.7200   -0.0262
    6.7300   -0.0262
    6.7400   -0.0261
    6.7500   -0.0259
    6.7600   -0.0258
    6.7700   -0.0257
    6.7800   -0.0257
    6.7900   -0.0256
    6.8000   -0.0254
    6.8100   -0.0253
    6.8200   -0.0252
    6.8300   -0.0251
    6.8400   -0.0250
    6.8500   -0.0249
    6.8600   -0.0248
    6.8700   -0.0247
    6.8800   -0.0246
    6.8900   -0.0245
    6.9000   -0.0243
    6.9100   -0.0243
    6.9200   -0.0242
    6.9300   -0.0241
    6.9400   -0.0240
    6.9500   -0.0239
    6.9600   -0.0238
    6.9700   -0.0237
    6.9800   -0.0236
    6.9900   -0.0235
    7.0000   -0.0234
    7.0100   -0.0233
    7.0200   -0.0232
    7.0300   -0.0231
    7.0400   -0.0230
    7.0500   -0.0230
    7.0600   -0.0229
    7.0700   -0.0228
    7.0800   -0.0227
    7.0900   -0.0226
    7.1000   -0.0226
    7.1100   -0.0225
    7.1200   -0.0224
    7.1300   -0.0223
    7.1400   -0.0223
    7.1500   -0.0222
    7.1600   -0.0221
    7.1700   -0.0220
    7.1800   -0.0220
    7.1900   -0.0219
    7.2000   -0.0218
    7.2100   -0.0217
    7.2200   -0.0216
    7.2300   -0.0215
    7.2400   -0.0215
    7.2500   -0.0214
    7.2600   -0.0213
    7.2700   -0.0213
    7.2800   -0.0212
    7.2900   -0.0211
    7.3000   -0.0210
    7.3100   -0.0209
    7.3200   -0.0209
    7.3300   -0.0208
    7.3400   -0.0208
    7.3500   -0.0207
    7.3600   -0.0206
    7.3700   -0.0205
    7.3800   -0.0205
    7.3900   -0.0204
    7.4000   -0.0204
    7.4100   -0.0203
    7.4200   -0.0202
    7.4300   -0.0202
    7.4400   -0.0201
    7.4500   -0.0201
    7.4600   -0.0200
    7.4700   -0.0200
    7.4800   -0.0199
    7.4900   -0.0198
    7.5000   -0.0198
    7.5100   -0.0197
    7.5200   -0.0197
    7.5300   -0.0196
    7.5400   -0.0195
    7.5500   -0.0194
    7.5600   -0.0193
    7.5700   -0.0192
    7.5800   -0.0191
    7.5900   -0.0190
    7.6000   -0.0189
    7.6100   -0.0189
    7.6200   -0.0188
    7.6300   -0.0187
    7.6400   -0.0186
    7.6500   -0.0185
    7.6600   -0.0184
    7.6700   -0.0183
    7.6800   -0.0183
    7.6900   -0.0182
    7.7000   -0.0182
    7.7100   -0.0181
    7.7200   -0.0180
    7.7300   -0.0180
    7.7400   -0.0179
    7.7500   -0.0178
    7.7600   -0.0178
    7.7700   -0.0177
    7.7800   -0.0177
    7.7900   -0.0177
    7.8000   -0.0176
    7.8100   -0.0176
    7.8200   -0.0175
    7.8300   -0.0175
    7.8400   -0.0173
    7.8500   -0.0173
    7.8600   -0.0173
    7.8700   -0.0172
    7.8800   -0.0171
    7.8900   -0.0171
    7.9000   -0.0170
    7.9100   -0.0169
    7.9200   -0.0168
    7.9300   -0.0168
    7.9400   -0.0167
    7.9500   -0.0166
    7.9600   -0.0166
    7.9700   -0.0165
    7.9800   -0.0164
    7.9900   -0.0163
    8.0000   -0.0162
    8.0100   -0.0161
    8.0200   -0.0160
    8.0300   -0.0160
    8.0400   -0.0159
    8.0500   -0.0158
    8.0600   -0.0157
    8.0700   -0.0157
    8.0800   -0.0156
    8.0900   -0.0155
    8.1000   -0.0154
    8.1100   -0.0154
    8.1200   -0.0153
    8.1300   -0.0152
    8.1400   -0.0152
    8.1500   -0.0151
    8.1600   -0.0150
    8.1700   -0.0150
    8.1800   -0.0149
    8.1900   -0.0148
    8.2000   -0.0148
    8.2100   -0.0147
    8.2200   -0.0147
    8.2300   -0.0146
    8.2400   -0.0146
    8.2500   -0.0145
    8.2600   -0.0144
    8.2700   -0.0143
    8.2800   -0.0143
    8.2900   -0.0142
    8.3000   -0.0141
    8.3100   -0.0140
    8.3200   -0.0140
    8.3300   -0.0139
    8.3400   -0.0138
    8.3500   -0.0137
    8.3600   -0.0137
    8.3700   -0.0136
    8.3800   -0.0135
    8.3900   -0.0134
    8.4000   -0.0134
    8.4100   -0.0133
    8.4200   -0.0132
    8.4300   -0.0131
    8.4400   -0.0130
    8.4500   -0.0130
    8.4600   -0.0129
    8.4700   -0.0128
    8.4800   -0.0128
    8.4900   -0.0127
    8.5000   -0.0127
    8.5100   -0.0126
    8.5200   -0.0125
    8.5300   -0.0124
    8.5400   -0.0123
    8.5500   -0.0123
    8.5600   -0.0122
    8.5700   -0.0121
    8.5800   -0.0121
    8.5900   -0.0120
    8.6000   -0.0119
    8.6100   -0.0119
    8.6200   -0.0118
    8.6300   -0.0118
    8.6400   -0.0117
    8.6500   -0.0116
    8.6600   -0.0115
    8.6700   -0.0115
    8.6800   -0.0115
    8.6900   -0.0114
    8.7000   -0.0114
    8.7100   -0.0114
    8.7200   -0.0114
    8.7300   -0.0113
    8.7400   -0.0113
    8.7500   -0.0113
    8.7600   -0.0113
    8.7700   -0.0113
    8.7800   -0.0112
    8.7900   -0.0112
    8.8000   -0.0112
    8.8100   -0.0111
    8.8200   -0.0111
    8.8300   -0.0110
    8.8400   -0.0110
    8.8500   -0.0110
    8.8600   -0.0110
    8.8700   -0.0109
    8.8800   -0.0108
    8.8900   -0.0108
    8.9000   -0.0107
    8.9100   -0.0106
    8.9200   -0.0105
    8.9300   -0.0105
    8.9400   -0.0105
    8.9500   -0.0104
    8.9600   -0.0104
    8.9700   -0.0103
    8.9800   -0.0102
    8.9900   -0.0102
    9.0000   -0.0101
    9.0100   -0.0101
    9.0200   -0.0100
    9.0300   -0.0100
    9.0400   -0.0099
    9.0500   -0.0099
    9.0600   -0.0098
    9.0700   -0.0098
    9.0800   -0.0097
    9.0900   -0.0097
    9.1000   -0.0096
    9.1100   -0.0096
    9.1200   -0.0096
    9.1300   -0.0095
    9.1400   -0.0095
    9.1500   -0.0094
    9.1600   -0.0094
    9.1700   -0.0093
    9.1800   -0.0093
    9.1900   -0.0093
    9.2000   -0.0093
    9.2100   -0.0093
    9.2200   -0.0092
    9.2300   -0.0091
    9.2400   -0.0091
    9.2500   -0.0091
    9.2600   -0.0090
    9.2700   -0.0090
    9.2800   -0.0089
    9.2900   -0.0089
    9.3000   -0.0088
    9.3100   -0.0088
    9.3200   -0.0088
    9.3300   -0.0087
    9.3400   -0.0087
    9.3500   -0.0087
    9.3600   -0.0086
    9.3700   -0.0086
    9.3800   -0.0086
    9.3900   -0.0085
    9.4000   -0.0085
    9.4100   -0.0085
    9.4200   -0.0084
    9.4300   -0.0084
    9.4400   -0.0083
    9.4500   -0.0083
    9.4600   -0.0083
    9.4700   -0.0083
    9.4800   -0.0083
    9.4900   -0.0082
    9.5000   -0.0082
    9.5100   -0.0082
    9.5200   -0.0081
    9.5300   -0.0081
    9.5400   -0.0080
    9.5500   -0.0080
    9.5600   -0.0079
    9.5700   -0.0079
    9.5800   -0.0079
    9.5900   -0.0078
    9.6000   -0.0078
    9.6100   -0.0077
    9.6200   -0.0076
    9.6300   -0.0076
    9.6400   -0.0075
    9.6500   -0.0074
    9.6600   -0.0074
    9.6700   -0.0074
    9.6800   -0.0073
    9.6900   -0.0073
    9.7000   -0.0073
    9.7100   -0.0072
    9.7200   -0.0071
    9.7300   -0.0071
    9.7400   -0.0071
    9.7500   -0.0070
    9.7600   -0.0070
    9.7700   -0.0070
    9.7800   -0.0070
    9.7900   -0.0069
    9.8000   -0.0069
    9.8100   -0.0069
    9.8200   -0.0068
    9.8300   -0.0068
    9.8400   -0.0067
    9.8500   -0.0067
    9.8600   -0.0066
    9.8700   -0.0066
    9.8800   -0.0066
    9.8900   -0.0066
    9.9000   -0.0066
    9.9100   -0.0065
    9.9200   -0.0065
    9.9300   -0.0065
    9.9400   -0.0065
    9.9500   -0.0065
    9.9600   -0.0064
    9.9700   -0.0064
    9.9800   -0.0064
    9.9900   -0.0064
   10.0000   -0.0063
    };

==> Data/Oscillator/sigma3/kf_varn_pos.tex <==
    \addplot[
    thick,
    dotted,
    black
    ]
    table {
         0    1.0000
    0.0100    0.9972
    0.0200    0.9928
    0.0300    0.9839
    0.0400    0.9791
    0.0500    0.9755
    0.0600    0.9713
    0.0700    0.9673
    0.0800    0.9638
    0.0900    0.9551
    0.1000    0.9461
    0.1100    0.9478
    0.1200    0.9492
    0.1300    0.9488
    0.1400    0.9459
    0.1500    0.9415
    0.1600    0.9384
    0.1700    0.9352
    0.1800    0.9299
    0.1900    0.9237
    0.2000    0.9192
    0.2100    0.9141
    0.2200    0.9100
    0.2300    0.9124
    0.2400    0.9101
    0.2500    0.9039
    0.2600    0.8980
    0.2700    0.8931
    0.2800    0.8944
    0.2900    0.8890
    0.3000    0.8854
    0.3100    0.8832
    0.3200    0.8770
    0.3300    0.8754
    0.3400    0.8726
    0.3500    0.8714
    0.3600    0.8745
    0.3700    0.8743
    0.3800    0.8671
    0.3900    0.8598
    0.4000    0.8544
    0.4100    0.8481
    0.4200    0.8416
    0.4300    0.8356
    0.4400    0.8346
    0.4500    0.8323
    0.4600    0.8262
    0.4700    0.8231
    0.4800    0.8219
    0.4900    0.8194
    0.5000    0.8166
    0.5100    0.8147
    0.5200    0.8107
    0.5300    0.8063
    0.5400    0.8024
    0.5500    0.7964
    0.5600    0.7917
    0.5700    0.7884
    0.5800    0.7837
    0.5900    0.7794
    0.6000    0.7764
    0.6100    0.7735
    0.6200    0.7696
    0.6300    0.7657
    0.6400    0.7617
    0.6500    0.7565
    0.6600    0.7518
    0.6700    0.7501
    0.6800    0.7461
    0.6900    0.7430
    0.7000    0.7405
    0.7100    0.7354
    0.7200    0.7301
    0.7300    0.7241
    0.7400    0.7181
    0.7500    0.7129
    0.7600    0.7105
    0.7700    0.7081
    0.7800    0.7046
    0.7900    0.7026
    0.8000    0.6970
    0.8100    0.6899
    0.8200    0.6859
    0.8300    0.6826
    0.8400    0.6778
    0.8500    0.6711
    0.8600    0.6668
    0.8700    0.6631
    0.8800    0.6591
    0.8900    0.6547
    0.9000    0.6479
    0.9100    0.6429
    0.9200    0.6402
    0.9300    0.6384
    0.9400    0.6342
    0.9500    0.6275
    0.9600    0.6210
    0.9700    0.6158
    0.9800    0.6110
    0.9900    0.6074
    1.0000    0.6034
    1.0100    0.5964
    1.0200    0.5910
    1.0300    0.5882
    1.0400    0.5845
    1.0500    0.5786
    1.0600    0.5736
    1.0700    0.5683
    1.0800    0.5628
    1.0900    0.5595
    1.1000    0.5565
    1.1100    0.5511
    1.1200    0.5453
    1.1300    0.5407
    1.1400    0.5377
    1.1500    0.5359
    1.1600    0.5322
    1.1700    0.5292
    1.1800    0.5255
    1.1900    0.5203
    1.2000    0.5172
    1.2100    0.5153
    1.2200    0.5128
    1.2300    0.5098
    1.2400    0.5056
    1.2500    0.5019
    1.2600    0.4980
    1.2700    0.4939
    1.2800    0.4907
    1.2900    0.4878
    1.3000    0.4845
    1.3100    0.4806
    1.3200    0.4780
    1.3300    0.4741
    1.3400    0.4696
    1.3500    0.4671
    1.3600    0.4646
    1.3700    0.4605
    1.3800    0.4570
    1.3900    0.4534
    1.4000    0.4498
    1.4100    0.4464
    1.4200    0.4426
    1.4300    0.4392
    1.4400    0.4368
    1.4500    0.4341
    1.4600    0.4320
    1.4700    0.4282
    1.4800    0.4229
    1.4900    0.4195
    1.5000    0.4157
    1.5100    0.4109
    1.5200    0.4070
    1.5300    0.4044
    1.5400    0.4014
    1.5500    0.3985
    1.5600    0.3948
    1.5700    0.3906
    1.5800    0.3870
    1.5900    0.3832
    1.6000    0.3795
    1.6100    0.3779
    1.6200    0.3756
    1.6300    0.3724
    1.6400    0.3688
    1.6500    0.3658
    1.6600    0.3629
    1.6700    0.3592
    1.6800    0.3558
    1.6900    0.3525
    1.7000    0.3498
    1.7100    0.3464
    1.7200    0.3450
    1.7300    0.3433
    1.7400    0.3393
    1.7500    0.3380
    1.7600    0.3357
    1.7700    0.3322
    1.7800    0.3290
    1.7900    0.3259
    1.8000    0.3237
    1.8100    0.3212
    1.8200    0.3185
    1.8300    0.3153
    1.8400    0.3135
    1.8500    0.3103
    1.8600    0.3052
    1.8700    0.3019
    1.8800    0.2991
    1.8900    0.2958
    1.9000    0.2922
    1.9100    0.2882
    1.9200    0.2849
    1.9300    0.2817
    1.9400    0.2782
    1.9500    0.2750
    1.9600    0.2715
    1.9700    0.2692
    1.9800    0.2667
    1.9900    0.2645
    2.0000    0.2628
    2.0100    0.2592
    2.0200    0.2557
    2.0300    0.2533
    2.0400    0.2519
    2.0500    0.2499
    2.0600    0.2476
    2.0700    0.2457
    2.0800    0.2429
    2.0900    0.2395
    2.1000    0.2361
    2.1100    0.2325
    2.1200    0.2306
    2.1300    0.2289
    2.1400    0.2280
    2.1500    0.2271
    2.1600    0.2236
    2.1700    0.2210
    2.1800    0.2205
    2.1900    0.2184
    2.2000    0.2159
    2.2100    0.2143
    2.2200    0.2126
    2.2300    0.2110
    2.2400    0.2091
    2.2500    0.2068
    2.2600    0.2049
    2.2700    0.2024
    2.2800    0.2006
    2.2900    0.1993
    2.3000    0.1975
    2.3100    0.1955
    2.3200    0.1925
    2.3300    0.1901
    2.3400    0.1880
    2.3500    0.1865
    2.3600    0.1854
    2.3700    0.1840
    2.3800    0.1818
    2.3900    0.1787
    2.4000    0.1766
    2.4100    0.1747
    2.4200    0.1732
    2.4300    0.1727
    2.4400    0.1712
    2.4500    0.1694
    2.4600    0.1687
    2.4700    0.1676
    2.4800    0.1666
    2.4900    0.1662
    2.5000    0.1649
    2.5100    0.1636
    2.5200    0.1625
    2.5300    0.1606
    2.5400    0.1589
    2.5500    0.1576
    2.5600    0.1557
    2.5700    0.1548
    2.5800    0.1539
    2.5900    0.1536
    2.6000    0.1531
    2.6100    0.1514
    2.6200    0.1508
    2.6300    0.1511
    2.6400    0.1509
    2.6500    0.1490
    2.6600    0.1476
    2.6700    0.1460
    2.6800    0.1438
    2.6900    0.1424
    2.7000    0.1416
    2.7100    0.1415
    2.7200    0.1406
    2.7300    0.1395
    2.7400    0.1385
    2.7500    0.1371
    2.7600    0.1369
    2.7700    0.1364
    2.7800    0.1350
    2.7900    0.1333
    2.8000    0.1321
    2.8100    0.1316
    2.8200    0.1317
    2.8300    0.1313
    2.8400    0.1301
    2.8500    0.1286
    2.8600    0.1278
    2.8700    0.1274
    2.8800    0.1257
    2.8900    0.1252
    2.9000    0.1253
    2.9100    0.1247
    2.9200    0.1234
    2.9300    0.1219
    2.9400    0.1214
    2.9500    0.1200
    2.9600    0.1183
    2.9700    0.1170
    2.9800    0.1161
    2.9900    0.1148
    3.0000    0.1136
    3.0100    0.1139
    3.0200    0.1134
    3.0300    0.1121
    3.0400    0.1113
    3.0500    0.1110
    3.0600    0.1107
    3.0700    0.1101
    3.0800    0.1091
    3.0900    0.1078
    3.1000    0.1069
    3.1100    0.1069
    3.1200    0.1070
    3.1300    0.1057
    3.1400    0.1044
    3.1500    0.1038
    3.1600    0.1027
    3.1700    0.1017
    3.1800    0.1004
    3.1900    0.0991
    3.2000    0.0979
    3.2100    0.0966
    3.2200    0.0957
    3.2300    0.0950
    3.2400    0.0942
    3.2500    0.0933
    3.2600    0.0925
    3.2700    0.0919
    3.2800    0.0918
    3.2900    0.0918
    3.3000    0.0911
    3.3100    0.0905
    3.3200    0.0900
    3.3300    0.0885
    3.3400    0.0863
    3.3500    0.0840
    3.3600    0.0827
    3.3700    0.0818
    3.3800    0.0805
    3.3900    0.0797
    3.4000    0.0789
    3.4100    0.0777
    3.4200    0.0771
    3.4300    0.0769
    3.4400    0.0776
    3.4500    0.0781
    3.4600    0.0776
    3.4700    0.0768
    3.4800    0.0759
    3.4900    0.0754
    3.5000    0.0741
    3.5100    0.0727
    3.5200    0.0725
    3.5300    0.0721
    3.5400    0.0714
    3.5500    0.0715
    3.5600    0.0718
    3.5700    0.0721
    3.5800    0.0710
    3.5900    0.0693
    3.6000    0.0691
    3.6100    0.0692
    3.6200    0.0688
    3.6300    0.0685
    3.6400    0.0687
    3.6500    0.0688
    3.6600    0.0681
    3.6700    0.0673
    3.6800    0.0667
    3.6900    0.0666
    3.7000    0.0667
    3.7100    0.0666
    3.7200    0.0665
    3.7300    0.0661
    3.7400    0.0655
    3.7500    0.0654
    3.7600    0.0645
    3.7700    0.0636
    3.7800    0.0639
    3.7900    0.0637
    3.8000    0.0639
    3.8100    0.0645
    3.8200    0.0641
    3.8300    0.0636
    3.8400    0.0631
    3.8500    0.0628
    3.8600    0.0629
    3.8700    0.0628
    3.8800    0.0624
    3.8900    0.0630
    3.9000    0.0638
    3.9100    0.0641
    3.9200    0.0639
    3.9300    0.0630
    3.9400    0.0627
    3.9500    0.0625
    3.9600    0.0617
    3.9700    0.0601
    3.9800    0.0598
    3.9900    0.0596
    4.0000    0.0600
    4.0100    0.0598
    4.0200    0.0587
    4.0300    0.0589
    4.0400    0.0582
    4.0500    0.0579
    4.0600    0.0576
    4.0700    0.0574
    4.0800    0.0577
    4.0900    0.0569
    4.1000    0.0551
    4.1100    0.0539
    4.1200    0.0542
    4.1300    0.0545
    4.1400    0.0543
    4.1500    0.0546
    4.1600    0.0540
    4.1700    0.0539
    4.1800    0.0540
    4.1900    0.0535
    4.2000    0.0532
    4.2100    0.0531
    4.2200    0.0522
    4.2300    0.0519
    4.2400    0.0526
    4.2500    0.0533
    4.2600    0.0546
    4.2700    0.0549
    4.2800    0.0545
    4.2900    0.0533
    4.3000    0.0525
    4.3100    0.0525
    4.3200    0.0530
    4.3300    0.0529
    4.3400    0.0526
    4.3500    0.0530
    4.3600    0.0525
    4.3700    0.0524
    4.3800    0.0528
    4.3900    0.0526
    4.4000    0.0531
    4.4100    0.0540
    4.4200    0.0540
    4.4300    0.0540
    4.4400    0.0540
    4.4500    0.0540
    4.4600    0.0542
    4.4700    0.0541
    4.4800    0.0534
    4.4900    0.0531
    4.5000    0.0540
    4.5100    0.0546
    4.5200    0.0539
    4.5300    0.0534
    4.5400    0.0531
    4.5500    0.0526
    4.5600    0.0527
    4.5700    0.0528
    4.5800    0.0524
    4.5900    0.0520
    4.6000    0.0513
    4.6100    0.0505
    4.6200    0.0496
    4.6300    0.0488
    4.6400    0.0483
    4.6500    0.0475
    4.6600    0.0472
    4.6700    0.0466
    4.6800    0.0460
    4.6900    0.0463
    4.7000    0.0459
    4.7100    0.0460
    4.7200    0.0458
    4.7300    0.0450
    4.7400    0.0443
    4.7500    0.0436
    4.7600    0.0431
    4.7700    0.0423
    4.7800    0.0419
    4.7900    0.0412
    4.8000    0.0399
    4.8100    0.0393
    4.8200    0.0403
    4.8300    0.0420
    4.8400    0.0425
    4.8500    0.0422
    4.8600    0.0421
    4.8700    0.0419
    4.8800    0.0417
    4.8900    0.0406
    4.9000    0.0399
    4.9100    0.0396
    4.9200    0.0382
    4.9300    0.0385
    4.9400    0.0395
    4.9500    0.0393
    4.9600    0.0401
    4.9700    0.0398
    4.9800    0.0393
    4.9900    0.0398
    5.0000    0.0399
    5.0100    0.0401
    5.0200    0.0399
    5.0300    0.0400
    5.0400    0.0400
    5.0500    0.0393
    5.0600    0.0393
    5.0700    0.0403
    5.0800    0.0408
    5.0900    0.0404
    5.1000    0.0404
    5.1100    0.0409
    5.1200    0.0417
    5.1300    0.0422
    5.1400    0.0420
    5.1500    0.0420
    5.1600    0.0422
    5.1700    0.0428
    5.1800    0.0428
    5.1900    0.0422
    5.2000    0.0429
    5.2100    0.0432
    5.2200    0.0427
    5.2300    0.0422
    5.2400    0.0418
    5.2500    0.0416
    5.2600    0.0416
    5.2700    0.0414
    5.2800    0.0411
    5.2900    0.0409
    5.3000    0.0406
    5.3100    0.0402
    5.3200    0.0396
    5.3300    0.0408
    5.3400    0.0436
    5.3500    0.0451
    5.3600    0.0458
    5.3700    0.0456
    5.3800    0.0449
    5.3900    0.0445
    5.4000    0.0444
    5.4100    0.0448
    5.4200    0.0450
    5.4300    0.0450
    5.4400    0.0445
    5.4500    0.0441
    5.4600    0.0445
    5.4700    0.0451
    5.4800    0.0453
    5.4900    0.0455
    5.5000    0.0461
    5.5100    0.0456
    5.5200    0.0450
    5.5300    0.0450
    5.5400    0.0440
    5.5500    0.0427
    5.5600    0.0421
    5.5700    0.0424
    5.5800    0.0426
    5.5900    0.0425
    5.6000    0.0424
    5.6100    0.0412
    5.6200    0.0404
    5.6300    0.0402
    5.6400    0.0401
    5.6500    0.0413
    5.6600    0.0417
    5.6700    0.0419
    5.6800    0.0428
    5.6900    0.0425
    5.7000    0.0419
    5.7100    0.0420
    5.7200    0.0423
    5.7300    0.0427
    5.7400    0.0431
    5.7500    0.0436
    5.7600    0.0436
    5.7700    0.0437
    5.7800    0.0431
    5.7900    0.0415
    5.8000    0.0417
    5.8100    0.0419
    5.8200    0.0416
    5.8300    0.0424
    5.8400    0.0426
    5.8500    0.0418
    5.8600    0.0412
    5.8700    0.0412
    5.8800    0.0413
    5.8900    0.0408
    5.9000    0.0398
    5.9100    0.0391
    5.9200    0.0389
    5.9300    0.0386
    5.9400    0.0383
    5.9500    0.0377
    5.9600    0.0376
    5.9700    0.0369
    5.9800    0.0360
    5.9900    0.0365
    6.0000    0.0363
    6.0100    0.0359
    6.0200    0.0360
    6.0300    0.0358
    6.0400    0.0355
    6.0500    0.0357
    6.0600    0.0354
    6.0700    0.0353
    6.0800    0.0360
    6.0900    0.0365
    6.1000    0.0366
    6.1100    0.0360
    6.1200    0.0358
    6.1300    0.0355
    6.1400    0.0355
    6.1500    0.0364
    6.1600    0.0365
    6.1700    0.0365
    6.1800    0.0355
    6.1900    0.0342
    6.2000    0.0338
    6.2100    0.0349
    6.2200    0.0360
    6.2300    0.0363
    6.2400    0.0361
    6.2500    0.0358
    6.2600    0.0363
    6.2700    0.0364
    6.2800    0.0370
    6.2900    0.0373
    6.3000    0.0364
    6.3100    0.0365
    6.3200    0.0357
    6.3300    0.0350
    6.3400    0.0354
    6.3500    0.0353
    6.3600    0.0356
    6.3700    0.0362
    6.3800    0.0368
    6.3900    0.0369
    6.4000    0.0365
    6.4100    0.0367
    6.4200    0.0363
    6.4300    0.0354
    6.4400    0.0348
    6.4500    0.0346
    6.4600    0.0352
    6.4700    0.0362
    6.4800    0.0362
    6.4900    0.0357
    6.5000    0.0358
    6.5100    0.0375
    6.5200    0.0385
    6.5300    0.0382
    6.5400    0.0374
    6.5500    0.0371
    6.5600    0.0375
    6.5700    0.0380
    6.5800    0.0380
    6.5900    0.0377
    6.6000    0.0374
    6.6100    0.0376
    6.6200    0.0378
    6.6300    0.0374
    6.6400    0.0371
    6.6500    0.0373
    6.6600    0.0378
    6.6700    0.0374
    6.6800    0.0367
    6.6900    0.0360
    6.7000    0.0357
    6.7100    0.0360
    6.7200    0.0355
    6.7300    0.0340
    6.7400    0.0332
    6.7500    0.0334
    6.7600    0.0337
    6.7700    0.0331
    6.7800    0.0317
    6.7900    0.0314
    6.8000    0.0317
    6.8100    0.0313
    6.8200    0.0316
    6.8300    0.0317
    6.8400    0.0313
    6.8500    0.0314
    6.8600    0.0318
    6.8700    0.0317
    6.8800    0.0311
    6.8900    0.0324
    6.9000    0.0328
    6.9100    0.0321
    6.9200    0.0322
    6.9300    0.0317
    6.9400    0.0309
    6.9500    0.0306
    6.9600    0.0317
    6.9700    0.0321
    6.9800    0.0318
    6.9900    0.0317
    7.0000    0.0320
    7.0100    0.0330
    7.0200    0.0328
    7.0300    0.0329
    7.0400    0.0330
    7.0500    0.0333
    7.0600    0.0336
    7.0700    0.0329
    7.0800    0.0323
    7.0900    0.0330
    7.1000    0.0331
    7.1100    0.0322
    7.1200    0.0326
    7.1300    0.0321
    7.1400    0.0313
    7.1500    0.0318
    7.1600    0.0321
    7.1700    0.0317
    7.1800    0.0312
    7.1900    0.0311
    7.2000    0.0314
    7.2100    0.0319
    7.2200    0.0317
    7.2300    0.0321
    7.2400    0.0326
    7.2500    0.0321
    7.2600    0.0314
    7.2700    0.0315
    7.2800    0.0317
    7.2900    0.0320
    7.3000    0.0321
    7.3100    0.0330
    7.3200    0.0332
    7.3300    0.0320
    7.3400    0.0319
    7.3500    0.0316
    7.3600    0.0321
    7.3700    0.0326
    7.3800    0.0324
    7.3900    0.0322
    7.4000    0.0324
    7.4100    0.0322
    7.4200    0.0320
    7.4300    0.0314
    7.4400    0.0306
    7.4500    0.0302
    7.4600    0.0293
    7.4700    0.0291
    7.4800    0.0287
    7.4900    0.0277
    7.5000    0.0268
    7.5100    0.0252
    7.5200    0.0241
    7.5300    0.0245
    7.5400    0.0247
    7.5500    0.0244
    7.5600    0.0236
    7.5700    0.0237
    7.5800    0.0241
    7.5900    0.0242
    7.6000    0.0248
    7.6100    0.0245
    7.6200    0.0246
    7.6300    0.0253
    7.6400    0.0254
    7.6500    0.0255
    7.6600    0.0266
    7.6700    0.0271
    7.6800    0.0266
    7.6900    0.0266
    7.7000    0.0266
    7.7100    0.0269
    7.7200    0.0269
    7.7300    0.0268
    7.7400    0.0274
    7.7500    0.0276
    7.7600    0.0276
    7.7700    0.0270
    7.7800    0.0259
    7.7900    0.0249
    7.8000    0.0237
    7.8100    0.0231
    7.8200    0.0222
    7.8300    0.0222
    7.8400    0.0234
    7.8500    0.0226
    7.8600    0.0212
    7.8700    0.0207
    7.8800    0.0199
    7.8900    0.0188
    7.9000    0.0190
    7.9100    0.0192
    7.9200    0.0190
    7.9300    0.0184
    7.9400    0.0177
    7.9500    0.0168
    7.9600    0.0163
    7.9700    0.0162
    7.9800    0.0161
    7.9900    0.0167
    8.0000    0.0174
    8.0100    0.0176
    8.0200    0.0173
    8.0300    0.0165
    8.0400    0.0159
    8.0500    0.0162
    8.0600    0.0163
    8.0700    0.0159
    8.0800    0.0159
    8.0900    0.0164
    8.1000    0.0160
    8.1100    0.0153
    8.1200    0.0155
    8.1300    0.0153
    8.1400    0.0154
    8.1500    0.0156
    8.1600    0.0149
    8.1700    0.0145
    8.1800    0.0148
    8.1900    0.0146
    8.2000    0.0148
    8.2100    0.0144
    8.2200    0.0134
    8.2300    0.0117
    8.2400    0.0106
    8.2500    0.0105
    8.2600    0.0098
    8.2700    0.0100
    8.2800    0.0103
    8.2900    0.0100
    8.3000    0.0095
    8.3100    0.0089
    8.3200    0.0090
    8.3300    0.0086
    8.3400    0.0077
    8.3500    0.0081
    8.3600    0.0077
    8.3700    0.0072
    8.3800    0.0078
    8.3900    0.0076
    8.4000    0.0065
    8.4100    0.0060
    8.4200    0.0065
    8.4300    0.0068
    8.4400    0.0073
    8.4500    0.0070
    8.4600    0.0066
    8.4700    0.0066
    8.4800    0.0061
    8.4900    0.0052
    8.5000    0.0049
    8.5100    0.0054
    8.5200    0.0056
    8.5300    0.0066
    8.5400    0.0066
    8.5500    0.0062
    8.5600    0.0064
    8.5700    0.0066
    8.5800    0.0073
    8.5900    0.0079
    8.6000    0.0078
    8.6100    0.0073
    8.6200    0.0072
    8.6300    0.0084
    8.6400    0.0099
    8.6500    0.0110
    8.6600    0.0120
    8.6700    0.0120
    8.6800    0.0123
    8.6900    0.0121
    8.7000    0.0123
    8.7100    0.0127
    8.7200    0.0119
    8.7300    0.0117
    8.7400    0.0115
    8.7500    0.0099
    8.7600    0.0094
    8.7700    0.0091
    8.7800    0.0083
    8.7900    0.0078
    8.8000    0.0076
    8.8100    0.0072
    8.8200    0.0072
    8.8300    0.0068
    8.8400    0.0058
    8.8500    0.0045
    8.8600    0.0035
    8.8700    0.0036
    8.8800    0.0035
    8.8900    0.0033
    8.9000    0.0036
    8.9100    0.0041
    8.9200    0.0048
    8.9300    0.0048
    8.9400    0.0041
    8.9500    0.0038
    8.9600    0.0034
    8.9700    0.0036
    8.9800    0.0047
    8.9900    0.0051
    9.0000    0.0048
    9.0100    0.0048
    9.0200    0.0047
    9.0300    0.0043
    9.0400    0.0040
    9.0500    0.0037
    9.0600    0.0041
    9.0700    0.0047
    9.0800    0.0054
    9.0900    0.0054
    9.1000    0.0050
    9.1100    0.0046
    9.1200    0.0043
    9.1300    0.0045
    9.1400    0.0050
    9.1500    0.0058
    9.1600    0.0064
    9.1700    0.0063
    9.1800    0.0060
    9.1900    0.0049
    9.2000    0.0040
    9.2100    0.0032
    9.2200    0.0028
    9.2300    0.0036
    9.2400    0.0038
    9.2500    0.0037
    9.2600    0.0034
    9.2700    0.0040
    9.2800    0.0051
    9.2900    0.0053
    9.3000    0.0051
    9.3100    0.0047
    9.3200    0.0043
    9.3300    0.0047
    9.3400    0.0053
    9.3500    0.0049
    9.3600    0.0045
    9.3700    0.0044
    9.3800    0.0037
    9.3900    0.0039
    9.4000    0.0043
    9.4100    0.0042
    9.4200    0.0042
    9.4300    0.0051
    9.4400    0.0055
    9.4500    0.0046
    9.4600    0.0036
    9.4700    0.0028
    9.4800    0.0021
    9.4900    0.0022
    9.5000    0.0016
    9.5100    0.0008
    9.5200    0.0006
    9.5300    0.0007
    9.5400    0.0008
    9.5500    0.0003
    9.5600    0.0000
    9.5700   -0.0006
    9.5800   -0.0010
    9.5900   -0.0012
    9.6000   -0.0015
    9.6100   -0.0013
    9.6200   -0.0008
    9.6300    0.0001
    9.6400    0.0006
    9.6500    0.0009
    9.6600    0.0005
    9.6700   -0.0003
    9.6800    0.0003
    9.6900    0.0001
    9.7000    0.0002
    9.7100    0.0008
    9.7200    0.0014
    9.7300    0.0019
    9.7400    0.0023
    9.7500    0.0023
    9.7600    0.0015
    9.7700    0.0010
    9.7800    0.0009
    9.7900    0.0014
    9.8000    0.0015
    9.8100    0.0007
    9.8200    0.0018
    9.8300    0.0026
    9.8400    0.0029
    9.8500    0.0041
    9.8600    0.0041
    9.8700    0.0038
    9.8800    0.0037
    9.8900    0.0037
    9.9000    0.0045
    9.9100    0.0043
    9.9200    0.0043
    9.9300    0.0055
    9.9400    0.0055
    9.9500    0.0051
    9.9600    0.0052
    9.9700    0.0054
    9.9800    0.0059
    9.9900    0.0068
   10.0000    0.0071
    };

==> Data/Oscillator/sigma3/kf_varn_vel.tex <==
    \addplot[
    thick,
    dotted,
    black
    ]
    table {
         0         0
    0.0100   -0.0099
    0.0200   -0.0196
    0.0300   -0.0291
    0.0400   -0.0384
    0.0500   -0.0475
    0.0600   -0.0565
    0.0700   -0.0652
    0.0800   -0.0738
    0.0900   -0.0822
    0.1000   -0.0904
    0.1100   -0.0984
    0.1200   -0.1064
    0.1300   -0.1142
    0.1400   -0.1219
    0.1500   -0.1295
    0.1600   -0.1369
    0.1700   -0.1441
    0.1800   -0.1512
    0.1900   -0.1582
    0.2000   -0.1650
    0.2100   -0.1716
    0.2200   -0.1781
    0.2300   -0.1846
    0.2400   -0.1910
    0.2500   -0.1971
    0.2600   -0.2032
    0.2700   -0.2091
    0.2800   -0.2150
    0.2900   -0.2207
    0.3000   -0.2263
    0.3100   -0.2319
    0.3200   -0.2372
    0.3300   -0.2425
    0.3400   -0.2477
    0.3500   -0.2529
    0.3600   -0.2581
    0.3700   -0.2631
    0.3800   -0.2680
    0.3900   -0.2727
    0.4000   -0.2773
    0.4100   -0.2818
    0.4200   -0.2861
    0.4300   -0.2904
    0.4400   -0.2947
    0.4500   -0.2989
    0.4600   -0.3029
    0.4700   -0.3068
    0.4800   -0.3108
    0.4900   -0.3146
    0.5000   -0.3184
    0.5100   -0.3222
    0.5200   -0.3258
    0.5300   -0.3293
    0.5400   -0.3327
    0.5500   -0.3361
    0.5600   -0.3393
    0.5700   -0.3426
    0.5800   -0.3457
    0.5900   -0.3487
    0.6000   -0.3517
    0.6100   -0.3546
    0.6200   -0.3575
    0.6300   -0.3603
    0.6400   -0.3630
    0.6500   -0.3656
    0.6600   -0.3682
    0.6700   -0.3707
    0.6800   -0.3732
    0.6900   -0.3756
    0.7000   -0.3779
    0.7100   -0.3802
    0.7200   -0.3824
    0.7300   -0.3845
    0.7400   -0.3865
    0.7500   -0.3885
    0.7600   -0.3904
    0.7700   -0.3923
    0.7800   -0.3941
    0.7900   -0.3959
    0.8000   -0.3977
    0.8100   -0.3993
    0.8200   -0.4009
    0.8300   -0.4024
    0.8400   -0.4039
    0.8500   -0.4053
    0.8600   -0.4066
    0.8700   -0.4079
    0.8800   -0.4092
    0.8900   -0.4104
    0.9000   -0.4115
    0.9100   -0.4126
    0.9200   -0.4136
    0.9300   -0.4146
    0.9400   -0.4156
    0.9500   -0.4165
    0.9600   -0.4173
    0.9700   -0.4181
    0.9800   -0.4188
    0.9900   -0.4195
    1.0000   -0.4201
    1.0100   -0.4207
    1.0200   -0.4212
    1.0300   -0.4217
    1.0400   -0.4221
    1.0500   -0.4225
    1.0600   -0.4229
    1.0700   -0.4232
    1.0800   -0.4234
    1.0900   -0.4236
    1.1000   -0.4238
    1.1100   -0.4239
    1.1200   -0.4240
    1.1300   -0.4241
    1.1400   -0.4240
    1.1500   -0.4240
    1.1600   -0.4239
    1.1700   -0.4238
    1.1800   -0.4237
    1.1900   -0.4236
    1.2000   -0.4234
    1.2100   -0.4231
    1.2200   -0.4228
    1.2300   -0.4225
    1.2400   -0.4223
    1.2500   -0.4220
    1.2600   -0.4216
    1.2700   -0.4213
    1.2800   -0.4208
    1.2900   -0.4204
    1.3000   -0.4199
    1.3100   -0.4195
    1.3200   -0.4189
    1.3300   -0.4184
    1.3400   -0.4179
    1.3500   -0.4172
    1.3600   -0.4166
    1.3700   -0.4160
    1.3800   -0.4154
    1.3900   -0.4147
    1.4000   -0.4140
    1.4100   -0.4133
    1.4200   -0.4125
    1.4300   -0.4117
    1.4400   -0.4109
    1.4500   -0.4101
    1.4600   -0.4092
    1.4700   -0.4084
    1.4800   -0.4076
    1.4900   -0.4067
    1.5000   -0.4058
    1.5100   -0.4049
    1.5200   -0.4040
    1.5300   -0.4030
    1.5400   -0.4019
    1.5500   -0.4009
    1.5600   -0.3999
    1.5700   -0.3989
    1.5800   -0.3978
    1.5900   -0.3967
    1.6000   -0.3956
    1.6100   -0.3944
    1.6200   -0.3931
    1.6300   -0.3920
    1.6400   -0.3908
    1.6500   -0.3896
    1.6600   -0.3884
    1.6700   -0.3872
    1.6800   -0.3860
    1.6900   -0.3847
    1.7000   -0.3834
    1.7100   -0.3822
    1.7200   -0.3808
    1.7300   -0.3794
    1.7400   -0.3781
    1.7500   -0.3767
    1.7600   -0.3753
    1.7700   -0.3740
    1.7800   -0.3727
    1.7900   -0.3713
    1.8000   -0.3699
    1.8100   -0.3685
    1.8200   -0.3671
    1.8300   -0.3657
    1.8400   -0.3643
    1.8500   -0.3629
    1.8600   -0.3617
    1.8700   -0.3602
    1.8800   -0.3588
    1.8900   -0.3573
    1.9000   -0.3559
    1.9100   -0.3545
    1.9200   -0.3530
    1.9300   -0.3515
    1.9400   -0.3501
    1.9500   -0.3485
    1.9600   -0.3470
    1.9700   -0.3454
    1.9800   -0.3438
    1.9900   -0.3421
    2.0000   -0.3404
    2.0100   -0.3389
    2.0200   -0.3374
    2.0300   -0.3357
    2.0400   -0.3340
    2.0500   -0.3323
    2.0600   -0.3307
    2.0700   -0.3290
    2.0800   -0.3274
    2.0900   -0.3258
    2.1000   -0.3242
    2.1100   -0.3227
    2.1200   -0.3209
    2.1300   -0.3192
    2.1400   -0.3173
    2.1500   -0.3155
    2.1600   -0.3140
    2.1700   -0.3123
    2.1800   -0.3105
    2.1900   -0.3088
    2.2000   -0.3071
    2.2100   -0.3054
    2.2200   -0.3036
    2.2300   -0.3019
    2.2400   -0.3002
    2.2500   -0.2985
    2.2600   -0.2969
    2.2700   -0.2952
    2.2800   -0.2935
    2.2900   -0.2918
    2.3000   -0.2901
    2.3100   -0.2884
    2.3200   -0.2868
    2.3300   -0.2852
    2.3400   -0.2835
    2.3500   -0.2818
    2.3600   -0.2800
    2.3700   -0.2782
    2.3800   -0.2766
    2.3900   -0.2751
    2.4000   -0.2734
    2.4100   -0.2717
    2.4200   -0.2700
    2.4300   -0.2681
    2.4400   -0.2664
    2.4500   -0.2648
    2.4600   -0.2630
    2.4700   -0.2612
    2.4800   -0.2595
    2.4900   -0.2577
    2.5000   -0.2560
    2.5100   -0.2543
    2.5200   -0.2527
    2.5300   -0.2511
    2.5400   -0.2495
    2.5500   -0.2478
    2.5600   -0.2463
    2.5700   -0.2446
    2.5800   -0.2429
    2.5900   -0.2411
    2.6000   -0.2394
    2.6100   -0.2379
    2.6200   -0.2362
    2.6300   -0.2344
    2.6400   -0.2327
    2.6500   -0.2313
    2.6600   -0.2298
    2.6700   -0.2283
    2.6800   -0.2269
    2.6900   -0.2254
    2.7000   -0.2238
    2.7100   -0.2221
    2.7200   -0.2205
    2.7300   -0.2190
    2.7400   -0.2175
    2.7500   -0.2160
    2.7600   -0.2144
    2.7700   -0.2128
    2.7800   -0.2114
    2.7900   -0.2100
    2.8000   -0.2086
    2.8100   -0.2070
    2.8200   -0.2054
    2.8300   -0.2039
    2.8400   -0.2025
    2.8500   -0.2011
    2.8600   -0.1997
    2.8700   -0.1982
    2.8800   -0.1969
    2.8900   -0.1954
    2.9000   -0.1938
    2.9100   -0.1924
    2.9200   -0.1911
    2.9300   -0.1898
    2.9400   -0.1884
    2.9500   -0.1871
    2.9600   -0.1859
    2.9700   -0.1846
    2.9800   -0.1833
    2.9900   -0.1820
    3.0000   -0.1807
    3.0100   -0.1791
    3.0200   -0.1777
    3.0300   -0.1765
    3.0400   -0.1752
    3.0500   -0.1738
    3.0600   -0.1724
    3.0700   -0.1711
    3.0800   -0.1698
    3.0900   -0.1686
    3.1000   -0.1674
    3.1100   -0.1660
    3.1200   -0.1646
    3.1300   -0.1634
    3.1400   -0.1623
    3.1500   -0.1610
    3.1600   -0.1599
    3.1700   -0.1587
    3.1800   -0.1575
    3.1900   -0.1564
    3.2000   -0.1553
    3.2100   -0.1542
    3.2200   -0.1530
    3.2300   -0.1517
    3.2400   -0.1505
    3.2500   -0.1494
    3.2600   -0.1482
    3.2700   -0.1470
    3.2800   -0.1457
    3.2900   -0.1444
    3.3000   -0.1432
    3.3100   -0.1421
    3.3200   -0.1409
    3.3300   -0.1399
    3.3400   -0.1391
    3.3500   -0.1382
    3.3600   -0.1371
    3.3700   -0.1360
    3.3800   -0.1350
    3.3900   -0.1338
    3.4000   -0.1327
    3.4100   -0.1317
    3.4200   -0.1305
    3.4300   -0.1293
    3.4400   -0.1279
    3.4500   -0.1266
    3.4600   -0.1255
    3.4700   -0.1245
    3.4800   -0.1234
    3.4900   -0.1223
    3.5000   -0.1214
    3.5100   -0.1205
    3.5200   -0.1193
    3.5300   -0.1183
    3.5400   -0.1172
    3.5500   -0.1160
    3.5600   -0.1149
    3.5700   -0.1137
    3.5800   -0.1128
    3.5900   -0.1120
    3.6000   -0.1109
    3.6100   -0.1098
    3.6200   -0.1088
    3.6300   -0.1078
    3.6400   -0.1067
    3.6500   -0.1056
    3.6600   -0.1047
    3.6700   -0.1038
    3.6800   -0.1029
    3.6900   -0.1019
    3.7000   -0.1009
    3.7100   -0.0999
    3.7200   -0.0989
    3.7300   -0.0980
    3.7400   -0.0972
    3.7500   -0.0962
    3.7600   -0.0954
    3.7700   -0.0947
    3.7800   -0.0937
    3.7900   -0.0928
    3.8000   -0.0918
    3.8100   -0.0908
    3.8200   -0.0899
    3.8300   -0.0892
    3.8400   -0.0884
    3.8500   -0.0876
    3.8600   -0.0867
    3.8700   -0.0858
    3.8800   -0.0850
    3.8900   -0.0841
    3.9000   -0.0831
    3.9100   -0.0822
    3.9200   -0.0815
    3.9300   -0.0809
    3.9400   -0.0802
    3.9500   -0.0794
    3.9600   -0.0788
    3.9700   -0.0783
    3.9800   -0.0776
    3.9900   -0.0769
    4.0000   -0.0760
    4.0100   -0.0753
    4.0200   -0.0748
    4.0300   -0.0740
    4.0400   -0.0734
    4.0500   -0.0727
    4.0600   -0.0721
    4.0700   -0.0714
    4.0800   -0.0706
    4.0900   -0.0701
    4.1000   -0.0697
    4.1100   -0.0693
    4.1200   -0.0685
    4.1300   -0.0677
    4.1400   -0.0671
    4.1500   -0.0663
    4.1600   -0.0658
    4.1700   -0.0651
    4.1800   -0.0644
    4.1900   -0.0639
    4.2000   -0.0633
    4.2100   -0.0626
    4.2200   -0.0622
    4.2300   -0.0616
    4.2400   -0.0608
    4.2500   -0.0601
    4.2600   -0.0592
    4.2700   -0.0586
    4.2800   -0.0581
    4.2900   -0.0578
    4.3000   -0.0573
    4.3100   -0.0568
    4.3200   -0.0561
    4.3300   -0.0556
    4.3400   -0.0551
    4.3500   -0.0545
    4.3600   -0.0540
    4.3700   -0.0535
    4.3800   -0.0529
    4.3900   -0.0525
    4.4000   -0.0519
    4.4100   -0.0512
    4.4200   -0.0507
    4.4300   -0.0503
    4.4400   -0.0498
    4.4500   -0.0493
    4.4600   -0.0489
    4.4700   -0.0484
    4.4800   -0.0481
    4.4900   -0.0478
    4.5000   -0.0472
    4.5100   -0.0466
    4.5200   -0.0464
    4.5300   -0.0461
    4.5400   -0.0457
    4.5500   -0.0454
    4.5600   -0.0450
    4.5700   -0.0446
    4.5800   -0.0443
    4.5900   -0.0440
    4.6000   -0.0437
    4.6100   -0.0435
    4.6200   -0.0433
    4.6300   -0.0430
    4.6400   -0.0428
    4.6500   -0.0425
    4.6600   -0.0422
    4.6700   -0.0419
    4.6800   -0.0416
    4.6900   -0.0411
    4.7000   -0.0408
    4.7100   -0.0404
    4.7200   -0.0401
    4.7300   -0.0399
    4.7400   -0.0396
    4.7500   -0.0394
    4.7600   -0.0391
    4.7700   -0.0388
    4.7800   -0.0385
    4.7900   -0.0383
    4.8000   -0.0381
    4.8100   -0.0379
    4.8200   -0.0373
    4.8300   -0.0365
    4.8400   -0.0361
    4.8500   -0.0358
    4.8600   -0.0355
    4.8700   -0.0352
    4.8800   -0.0349
    4.8900   -0.0348
    4.9000   -0.0346
    4.9100   -0.0343
    4.9200   -0.0342
    4.9300   -0.0338
    4.9400   -0.0332
    4.9500   -0.0330
    4.9600   -0.0325
    4.9700   -0.0322
    4.9800   -0.0320
    4.9900   -0.0316
    5.0000   -0.0313
    5.0100   -0.0309
    5.0200   -0.0307
    5.0300   -0.0304
    5.0400   -0.0301
    5.0500   -0.0300
    5.0600   -0.0297
    5.0700   -0.0292
    5.0800   -0.0289
    5.0900   -0.0287
    5.1000   -0.0285
    5.1100   -0.0281
    5.1200   -0.0277
    5.1300   -0.0274
    5.1400   -0.0273
    5.1500   -0.0270
    5.1600   -0.0268
    5.1700   -0.0265
    5.1800   -0.0263
    5.1900   -0.0263
    5.2000   -0.0259
    5.2100   -0.0257
    5.2200   -0.0256
    5.2300   -0.0256
    5.2400   -0.0255
    5.2500   -0.0253
    5.2600   -0.0251
    5.2700   -0.0250
    5.2800   -0.0249
    5.2900   -0.0248
    5.3000   -0.0247
    5.3100   -0.0246
    5.3200   -0.0245
    5.3300   -0.0241
    5.3400   -0.0234
    5.3500   -0.0230
    5.3600   -0.0228
    5.3700   -0.0227
    5.3800   -0.0228
    5.3900   -0.0228
    5.4000   -0.0227
    5.4100   -0.0225
    5.4200   -0.0224
    5.4300   -0.0223
    5.4400   -0.0224
    5.4500   -0.0224
    5.4600   -0.0222
    5.4700   -0.0220
    5.4800   -0.0219
    5.4900   -0.0218
    5.5000   -0.0216
    5.5100   -0.0216
    5.5200   -0.0217
    5.5300   -0.0217
    5.5400   -0.0218
    5.5500   -0.0220
    5.5600   -0.0220
    5.5700   -0.0219
    5.5800   -0.0218
    5.5900   -0.0217
    5.6000   -0.0216
    5.6100   -0.0218
    5.6200   -0.0219
    5.6300   -0.0219
    5.6400   -0.0218
    5.6500   -0.0214
    5.6600   -0.0213
    5.6700   -0.0212
    5.6800   -0.0209
    5.6900   -0.0209
    5.7000   -0.0210
    5.7100   -0.0209
    5.7200   -0.0208
    5.7300   -0.0207
    5.7400   -0.0206
    5.7500   -0.0204
    5.7600   -0.0204
    5.7700   -0.0204
    5.7800   -0.0205
    5.7900   -0.0208
    5.8000   -0.0207
    5.8100   -0.0206
    5.8200   -0.0206
    5.8300   -0.0204
    5.8400   -0.0204
    5.8500   -0.0205
    5.8600   -0.0206
    5.8700   -0.0206
    5.8800   -0.0205
    5.8900   -0.0206
    5.9000   -0.0207
    5.9100   -0.0208
    5.9200   -0.0208
    5.9300   -0.0208
    5.9400   -0.0208
    5.9500   -0.0209
    5.9600   -0.0209
    5.9700   -0.0209
    5.9800   -0.0210
    5.9900   -0.0209
    6.0000   -0.0208
    6.0100   -0.0209
    6.0200   -0.0208
    6.0300   -0.0207
    6.0400   -0.0207
    6.0500   -0.0206
    6.0600   -0.0206
    6.0700   -0.0206
    6.0800   -0.0203
    6.0900   -0.0202
    6.1000   -0.0201
    6.1100   -0.0202
    6.1200   -0.0202
    6.1300   -0.0202
    6.1400   -0.0201
    6.1500   -0.0199
    6.1600   -0.0199
    6.1700   -0.0198
    6.1800   -0.0200
    6.1900   -0.0202
    6.2000   -0.0202
    6.2100   -0.0200
    6.2200   -0.0197
    6.2300   -0.0196
    6.2400   -0.0196
    6.2500   -0.0196
    6.2600   -0.0195
    6.2700   -0.0195
    6.2800   -0.0193
    6.2900   -0.0193
    6.3000   -0.0194
    6.3100   -0.0194
    6.3200   -0.0196
    6.3300   -0.0197
    6.3400   -0.0196
    6.3500   -0.0196
    6.3600   -0.0195
    6.3700   -0.0193
    6.3800   -0.0192
    6.3900   -0.0192
    6.4000   -0.0193
    6.4100   -0.0192
    6.4200   -0.0193
    6.4300   -0.0195
    6.4400   -0.0196
    6.4500   -0.0196
    6.4600   -0.0195
    6.4700   -0.0193
    6.4800   -0.0193
    6.4900   -0.0194
    6.5000   -0.0193
    6.5100   -0.0190
    6.5200   -0.0188
    6.5300   -0.0189
    6.5400   -0.0191
    6.5500   -0.0192
    6.5600   -0.0191
    6.5700   -0.0190
    6.5800   -0.0191
    6.5900   -0.0192
    6.6000   -0.0193
    6.6100   -0.0193
    6.6200   -0.0192
    6.6300   -0.0193
    6.6400   -0.0194
    6.6500   -0.0194
    6.6600   -0.0193
    6.6700   -0.0195
    6.6800   -0.0196
    6.6900   -0.0198
    6.7000   -0.0199
    6.7100   -0.0198
    6.7200   -0.0199
    6.7300   -0.0202
    6.7400   -0.0204
    6.7500   -0.0203
    6.7600   -0.0203
    6.7700   -0.0204
    6.7800   -0.0206
    6.7900   -0.0207
    6.8000   -0.0206
    6.8100   -0.0206
    6.8200   -0.0205
    6.8300   -0.0205
    6.8400   -0.0206
    6.8500   -0.0205
    6.8600   -0.0204
    6.8700   -0.0204
    6.8800   -0.0205
    6.8900   -0.0202
    6.9000   -0.0201
    6.9100   -0.0203
    6.9200   -0.0202
    6.9300   -0.0203
    6.9400   -0.0204
    6.9500   -0.0205
    6.9600   -0.0202
    6.9700   -0.0202
    6.9800   -0.0202
    6.9900   -0.0202
    7.0000   -0.0201
    7.0100   -0.0199
    7.0200   -0.0200
    7.0300   -0.0200
    7.0400   -0.0200
    7.0500   -0.0199
    7.0600   -0.0199
    7.0700   -0.0200
    7.0800   -0.0201
    7.0900   -0.0200
    7.1000   -0.0200
    7.1100   -0.0202
    7.1200   -0.0201
    7.1300   -0.0202
    7.1400   -0.0204
    7.1500   -0.0203
    7.1600   -0.0202
    7.1700   -0.0203
    7.1800   -0.0204
    7.1900   -0.0204
    7.2000   -0.0204
    7.2100   -0.0203
    7.2200   -0.0203
    7.2300   -0.0202
    7.2400   -0.0201
    7.2500   -0.0203
    7.2600   -0.0204
    7.2700   -0.0204
    7.2800   -0.0203
    7.2900   -0.0203
    7.3000   -0.0203
    7.3100   -0.0201
    7.3200   -0.0201
    7.3300   -0.0204
    7.3400   -0.0204
    7.3500   -0.0205
    7.3600   -0.0204
    7.3700   -0.0203
    7.3800   -0.0204
    7.3900   -0.0204
    7.4000   -0.0204
    7.4100   -0.0204
    7.4200   -0.0205
    7.4300   -0.0206
    7.4400   -0.0208
    7.4500   -0.0209
    7.4600   -0.0210
    7.4700   -0.0211
    7.4800   -0.0211
    7.4900   -0.0213
    7.5000   -0.0215
    7.5100   -0.0217
    7.5200   -0.0219
    7.5300   -0.0218
    7.5400   -0.0216
    7.5500   -0.0216
    7.5600   -0.0217
    7.5700   -0.0216
    7.5800   -0.0215
    7.5900   -0.0214
    7.6000   -0.0212
    7.6100   -0.0212
    7.6200   -0.0211
    7.6300   -0.0209
    7.6400   -0.0209
    7.6500   -0.0208
    7.6600   -0.0205
    7.6700   -0.0204
    7.6800   -0.0205
    7.6900   -0.0205
    7.7000   -0.0204
    7.7100   -0.0203
    7.7200   -0.0203
    7.7300   -0.0203
    7.7400   -0.0202
    7.7500   -0.0201
    7.7600   -0.0201
    7.7700   -0.0202
    7.7800   -0.0204
    7.7900   -0.0206
    7.8000   -0.0208
    7.8100   -0.0209
    7.8200   -0.0210
    7.8300   -0.0209
    7.8400   -0.0206
    7.8500   -0.0207
    7.8600   -0.0209
    7.8700   -0.0210
    7.8800   -0.0210
    7.8900   -0.0212
    7.9000   -0.0210
    7.9100   -0.0209
    7.9200   -0.0208
    7.9300   -0.0209
    7.9400   -0.0209
    7.9500   -0.0210
    7.9600   -0.0209
    7.9700   -0.0208
    7.9800   -0.0207
    7.9900   -0.0205
    8.0000   -0.0202
    8.0100   -0.0201
    8.0200   -0.0201
    8.0300   -0.0201
    8.0400   -0.0201
    8.0500   -0.0199
    8.0600   -0.0198
    8.0700   -0.0198
    8.0800   -0.0197
    8.0900   -0.0195
    8.1000   -0.0194
    8.1100   -0.0195
    8.1200   -0.0193
    8.1300   -0.0193
    8.1400   -0.0191
    8.1500   -0.0190
    8.1600   -0.0190
    8.1700   -0.0190
    8.1800   -0.0188
    8.1900   -0.0188
    8.2000   -0.0186
    8.2100   -0.0186
    8.2200   -0.0187
    8.2300   -0.0189
    8.2400   -0.0190
    8.2500   -0.0189
    8.2600   -0.0189
    8.2700   -0.0186
    8.2800   -0.0184
    8.2900   -0.0183
    8.3000   -0.0183
    8.3100   -0.0183
    8.3200   -0.0181
    8.3300   -0.0180
    8.3400   -0.0180
    8.3500   -0.0178
    8.3600   -0.0177
    8.3700   -0.0177
    8.3800   -0.0174
    8.3900   -0.0173
    8.4000   -0.0173
    8.4100   -0.0173
    8.4200   -0.0170
    8.4300   -0.0168
    8.4400   -0.0165
    8.4500   -0.0164
    8.4600   -0.0163
    8.4700   -0.0162
    8.4800   -0.0161
    8.4900   -0.0162
    8.5000   -0.0160
    8.5100   -0.0158
    8.5200   -0.0156
    8.5300   -0.0152
    8.5400   -0.0151
    8.5500   -0.0150
    8.5600   -0.0148
    8.5700   -0.0147
    8.5800   -0.0144
    8.5900   -0.0141
    8.6000   -0.0140
    8.6100   -0.0140
    8.6200   -0.0139
    8.6300   -0.0136
    8.6400   -0.0132
    8.6500   -0.0128
    8.6600   -0.0126
    8.6700   -0.0125
    8.6800   -0.0124
    8.6900   -0.0124
    8.7000   -0.0123
    8.7100   -0.0122
    8.7200   -0.0123
    8.7300   -0.0123
    8.7400   -0.0122
    8.7500   -0.0125
    8.7600   -0.0125
    8.7700   -0.0125
    8.7800   -0.0126
    8.7900   -0.0126
    8.8000   -0.0125
    8.8100   -0.0125
    8.8200   -0.0124
    8.8300   -0.0124
    8.8400   -0.0125
    8.8500   -0.0126
    8.8600   -0.0127
    8.8700   -0.0125
    8.8800   -0.0124
    8.8900   -0.0123
    8.9000   -0.0121
    8.9100   -0.0119
    8.9200   -0.0116
    8.9300   -0.0115
    8.9400   -0.0115
    8.9500   -0.0114
    8.9600   -0.0114
    8.9700   -0.0112
    8.9800   -0.0109
    8.9900   -0.0107
    9.0000   -0.0106
    9.0100   -0.0105
    9.0200   -0.0104
    9.0300   -0.0104
    9.0400   -0.0104
    9.0500   -0.0103
    9.0600   -0.0101
    9.0700   -0.0099
    9.0800   -0.0096
    9.0900   -0.0096
    9.1000   -0.0096
    9.1100   -0.0095
    9.1200   -0.0095
    9.1300   -0.0094
    9.1400   -0.0092
    9.1500   -0.0089
    9.1600   -0.0087
    9.1700   -0.0087
    9.1800   -0.0087
    9.1900   -0.0088
    9.2000   -0.0089
    9.2100   -0.0090
    9.2200   -0.0089
    9.2300   -0.0087
    9.2400   -0.0085
    9.2500   -0.0085
    9.2600   -0.0084
    9.2700   -0.0082
    9.2800   -0.0079
    9.2900   -0.0078
    9.3000   -0.0078
    9.3100   -0.0078
    9.3200   -0.0078
    9.3300   -0.0076
    9.3400   -0.0074
    9.3500   -0.0074
    9.3600   -0.0074
    9.3700   -0.0074
    9.3800   -0.0074
    9.3900   -0.0073
    9.4000   -0.0072
    9.4100   -0.0071
    9.4200   -0.0070
    9.4300   -0.0068
    9.4400   -0.0067
    9.4500   -0.0068
    9.4600   -0.0069
    9.4700   -0.0070
    9.4800   -0.0070
    9.4900   -0.0069
    9.5000   -0.0070
    9.5100   -0.0070
    9.5200   -0.0070
    9.5300   -0.0068
    9.5400   -0.0067
    9.5500   -0.0067
    9.5600   -0.0067
    9.5700   -0.0067
    9.5800   -0.0066
    9.5900   -0.0066
    9.6000   -0.0065
    9.6100   -0.0063
    9.6200   -0.0061
    9.6300   -0.0058
    9.6400   -0.0056
    9.6500   -0.0055
    9.6600   -0.0055
    9.6700   -0.0055
    9.6800   -0.0053
    9.6900   -0.0053
    9.7000   -0.0052
    9.7100   -0.0050
    9.7200   -0.0047
    9.7300   -0.0046
    9.7400   -0.0044
    9.7500   -0.0044
    9.7600   -0.0045
    9.7700   -0.0045
    9.7800   -0.0044
    9.7900   -0.0043
    9.8000   -0.0042
    9.8100   -0.0043
    9.8200   -0.0040
    9.8300   -0.0038
    9.8400   -0.0037
    9.8500   -0.0034
    9.8600   -0.0033
    9.8700   -0.0034
    9.8800   -0.0033
    9.8900   -0.0033
    9.9000   -0.0031
    9.9100   -0.0031
    9.9200   -0.0031
    9.9300   -0.0028
    9.9400   -0.0028
    9.9500   -0.0029
    9.9600   -0.0029
    9.9700   -0.0028
    9.9800   -0.0027
    9.9900   -0.0025
   10.0000   -0.0025
    };

==> Data/Oscillator/sigma3/x_tr_pos.tex <==
    \addplot[
    thick,
    red
    ]
    table {
    0         0.7884
    0.0100    0.7871
    0.0200    0.7858
    0.0300    0.7845
    0.0400    0.7831
    0.0500    0.7817
    0.0600    0.7802
    0.0700    0.7787
    0.0800    0.7771
    0.0900    0.7756
    0.1000    0.7742
    0.1100    0.7726
    0.1200    0.7711
    0.1300    0.7696
    0.1400    0.7681
    0.1500    0.7665
    0.1600    0.7649
    0.1700    0.7633
    0.1800    0.7617
    0.1900    0.7601
    0.2000    0.7585
    0.2100    0.7568
    0.2200    0.7552
    0.2300    0.7535
    0.2400    0.7518
    0.2500    0.7501
    0.2600    0.7484
    0.2700    0.7467
    0.2800    0.7450
    0.2900    0.7432
    0.3000    0.7415
    0.3100    0.7397
    0.3200    0.7379
    0.3300    0.7360
    0.3400    0.7341
    0.3500    0.7321
    0.3600    0.7301
    0.3700    0.7282
    0.3800    0.7262
    0.3900    0.7242
    0.4000    0.7221
    0.4100    0.7201
    0.4200    0.7180
    0.4300    0.7159
    0.4400    0.7139
    0.4500    0.7118
    0.4600    0.7097
    0.4700    0.7076
    0.4800    0.7054
    0.4900    0.7033
    0.5000    0.7013
    0.5100    0.6992
    0.5200    0.6970
    0.5300    0.6949
    0.5400    0.6927
    0.5500    0.6906
    0.5600    0.6884
    0.5700    0.6862
    0.5800    0.6841
    0.5900    0.6819
    0.6000    0.6798
    0.6100    0.6776
    0.6200    0.6754
    0.6300    0.6732
    0.6400    0.6711
    0.6500    0.6690
    0.6600    0.6668
    0.6700    0.6647
    0.6800    0.6625
    0.6900    0.6603
    0.7000    0.6582
    0.7100    0.6560
    0.7200    0.6539
    0.7300    0.6517
    0.7400    0.6496
    0.7500    0.6474
    0.7600    0.6453
    0.7700    0.6431
    0.7800    0.6409
    0.7900    0.6387
    0.8000    0.6365
    0.8100    0.6343
    0.8200    0.6321
    0.8300    0.6300
    0.8400    0.6279
    0.8500    0.6257
    0.8600    0.6236
    0.8700    0.6215
    0.8800    0.6194
    0.8900    0.6173
    0.9000    0.6152
    0.9100    0.6131
    0.9200    0.6109
    0.9300    0.6088
    0.9400    0.6067
    0.9500    0.6047
    0.9600    0.6026
    0.9700    0.6005
    0.9800    0.5984
    0.9900    0.5963
    1.0000    0.5942
    1.0100    0.5920
    1.0200    0.5899
    1.0300    0.5877
    1.0400    0.5856
    1.0500    0.5835
    1.0600    0.5813
    1.0700    0.5792
    1.0800    0.5771
    1.0900    0.5751
    1.1000    0.5730
    1.1100    0.5709
    1.1200    0.5688
    1.1300    0.5667
    1.1400    0.5646
    1.1500    0.5626
    1.1600    0.5605
    1.1700    0.5585
    1.1800    0.5564
    1.1900    0.5544
    1.2000    0.5523
    1.2100    0.5503
    1.2200    0.5483
    1.2300    0.5463
    1.2400    0.5444
    1.2500    0.5424
    1.2600    0.5404
    1.2700    0.5385
    1.2800    0.5365
    1.2900    0.5346
    1.3000    0.5326
    1.3100    0.5307
    1.3200    0.5287
    1.3300    0.5267
    1.3400    0.5247
    1.3500    0.5227
    1.3600    0.5207
    1.3700    0.5188
    1.3800    0.5168
    1.3900    0.5148
    1.4000    0.5129
    1.4100    0.5110
    1.4200    0.5090
    1.4300    0.5071
    1.4400    0.5051
    1.4500    0.5031
    1.4600    0.5011
    1.4700    0.4991
    1.4800    0.4971
    1.4900    0.4951
    1.5000    0.4931
    1.5100    0.4911
    1.5200    0.4891
    1.5300    0.4871
    1.5400    0.4852
    1.5500    0.4832
    1.5600    0.4813
    1.5700    0.4794
    1.5800    0.4774
    1.5900    0.4756
    1.6000    0.4737
    1.6100    0.4718
    1.6200    0.4698
    1.6300    0.4679
    1.6400    0.4661
    1.6500    0.4643
    1.6600    0.4625
    1.6700    0.4607
    1.6800    0.4588
    1.6900    0.4570
    1.7000    0.4552
    1.7100    0.4534
    1.7200    0.4515
    1.7300    0.4497
    1.7400    0.4478
    1.7500    0.4460
    1.7600    0.4441
    1.7700    0.4423
    1.7800    0.4405
    1.7900    0.4387
    1.8000    0.4370
    1.8100    0.4352
    1.8200    0.4334
    1.8300    0.4316
    1.8400    0.4298
    1.8500    0.4281
    1.8600    0.4264
    1.8700    0.4246
    1.8800    0.4229
    1.8900    0.4212
    1.9000    0.4196
    1.9100    0.4179
    1.9200    0.4162
    1.9300    0.4146
    1.9400    0.4129
    1.9500    0.4113
    1.9600    0.4097
    1.9700    0.4081
    1.9800    0.4065
    1.9900    0.4050
    2.0000    0.4034
    2.0100    0.4019
    2.0200    0.4003
    2.0300    0.3988
    2.0400    0.3973
    2.0500    0.3958
    2.0600    0.3943
    2.0700    0.3929
    2.0800    0.3914
    2.0900    0.3899
    2.1000    0.3884
    2.1100    0.3869
    2.1200    0.3855
    2.1300    0.3840
    2.1400    0.3825
    2.1500    0.3811
    2.1600    0.3796
    2.1700    0.3781
    2.1800    0.3766
    2.1900    0.3751
    2.2000    0.3737
    2.2100    0.3722
    2.2200    0.3708
    2.2300    0.3694
    2.2400    0.3680
    2.2500    0.3666
    2.2600    0.3651
    2.2700    0.3637
    2.2800    0.3623
    2.2900    0.3609
    2.3000    0.3595
    2.3100    0.3581
    2.3200    0.3567
    2.3300    0.3553
    2.3400    0.3539
    2.3500    0.3525
    2.3600    0.3510
    2.3700    0.3496
    2.3800    0.3481
    2.3900    0.3466
    2.4000    0.3452
    2.4100    0.3437
    2.4200    0.3423
    2.4300    0.3409
    2.4400    0.3395
    2.4500    0.3381
    2.4600    0.3367
    2.4700    0.3353
    2.4800    0.3339
    2.4900    0.3325
    2.5000    0.3312
    2.5100    0.3298
    2.5200    0.3285
    2.5300    0.3271
    2.5400    0.3258
    2.5500    0.3245
    2.5600    0.3232
    2.5700    0.3219
    2.5800    0.3206
    2.5900    0.3193
    2.6000    0.3181
    2.6100    0.3168
    2.6200    0.3156
    2.6300    0.3143
    2.6400    0.3131
    2.6500    0.3118
    2.6600    0.3106
    2.6700    0.3093
    2.6800    0.3080
    2.6900    0.3068
    2.7000    0.3055
    2.7100    0.3043
    2.7200    0.3031
    2.7300    0.3019
    2.7400    0.3007
    2.7500    0.2996
    2.7600    0.2984
    2.7700    0.2972
    2.7800    0.2960
    2.7900    0.2948
    2.8000    0.2936
    2.8100    0.2925
    2.8200    0.2914
    2.8300    0.2903
    2.8400    0.2892
    2.8500    0.2881
    2.8600    0.2870
    2.8700    0.2860
    2.8800    0.2849
    2.8900    0.2839
    2.9000    0.2828
    2.9100    0.2817
    2.9200    0.2806
    2.9300    0.2795
    2.9400    0.2784
    2.9500    0.2774
    2.9600    0.2763
    2.9700    0.2752
    2.9800    0.2741
    2.9900    0.2730
    3.0000    0.2718
    3.0100    0.2707
    3.0200    0.2695
    3.0300    0.2683
    3.0400    0.2672
    3.0500    0.2661
    3.0600    0.2650
    3.0700    0.2638
    3.0800    0.2628
    3.0900    0.2617
    3.1000    0.2606
    3.1100    0.2596
    3.1200    0.2586
    3.1300    0.2576
    3.1400    0.2565
    3.1500    0.2555
    3.1600    0.2545
    3.1700    0.2534
    3.1800    0.2523
    3.1900    0.2513
    3.2000    0.2502
    3.2100    0.2492
    3.2200    0.2482
    3.2300    0.2471
    3.2400    0.2461
    3.2500    0.2451
    3.2600    0.2441
    3.2700    0.2430
    3.2800    0.2420
    3.2900    0.2410
    3.3000    0.2399
    3.3100    0.2389
    3.3200    0.2378
    3.3300    0.2368
    3.3400    0.2357
    3.3500    0.2346
    3.3600    0.2336
    3.3700    0.2326
    3.3800    0.2316
    3.3900    0.2305
    3.4000    0.2295
    3.4100    0.2285
    3.4200    0.2275
    3.4300    0.2264
    3.4400    0.2254
    3.4500    0.2244
    3.4600    0.2235
    3.4700    0.2225
    3.4800    0.2216
    3.4900    0.2206
    3.5000    0.2197
    3.5100    0.2188
    3.5200    0.2180
    3.5300    0.2171
    3.5400    0.2161
    3.5500    0.2152
    3.5600    0.2144
    3.5700    0.2135
    3.5800    0.2126
    3.5900    0.2117
    3.6000    0.2109
    3.6100    0.2100
    3.6200    0.2091
    3.6300    0.2083
    3.6400    0.2074
    3.6500    0.2066
    3.6600    0.2058
    3.6700    0.2050
    3.6800    0.2041
    3.6900    0.2033
    3.7000    0.2024
    3.7100    0.2016
    3.7200    0.2007
    3.7300    0.1998
    3.7400    0.1990
    3.7500    0.1981
    3.7600    0.1973
    3.7700    0.1964
    3.7800    0.1955
    3.7900    0.1947
    3.8000    0.1938
    3.8100    0.1930
    3.8200    0.1922
    3.8300    0.1915
    3.8400    0.1907
    3.8500    0.1899
    3.8600    0.1892
    3.8700    0.1885
    3.8800    0.1878
    3.8900    0.1871
    3.9000    0.1864
    3.9100    0.1857
    3.9200    0.1849
    3.9300    0.1842
    3.9400    0.1835
    3.9500    0.1827
    3.9600    0.1820
    3.9700    0.1812
    3.9800    0.1804
    3.9900    0.1796
    4.0000    0.1789
    4.0100    0.1781
    4.0200    0.1774
    4.0300    0.1767
    4.0400    0.1759
    4.0500    0.1751
    4.0600    0.1744
    4.0700    0.1736
    4.0800    0.1729
    4.0900    0.1722
    4.1000    0.1715
    4.1100    0.1708
    4.1200    0.1702
    4.1300    0.1695
    4.1400    0.1688
    4.1500    0.1681
    4.1600    0.1674
    4.1700    0.1668
    4.1800    0.1661
    4.1900    0.1654
    4.2000    0.1647
    4.2100    0.1640
    4.2200    0.1633
    4.2300    0.1626
    4.2400    0.1619
    4.2500    0.1612
    4.2600    0.1605
    4.2700    0.1599
    4.2800    0.1593
    4.2900    0.1587
    4.3000    0.1581
    4.3100    0.1575
    4.3200    0.1569
    4.3300    0.1564
    4.3400    0.1558
    4.3500    0.1552
    4.3600    0.1546
    4.3700    0.1539
    4.3800    0.1533
    4.3900    0.1527
    4.4000    0.1521
    4.4100    0.1515
    4.4200    0.1509
    4.4300    0.1503
    4.4400    0.1497
    4.4500    0.1491
    4.4600    0.1486
    4.4700    0.1480
    4.4800    0.1475
    4.4900    0.1470
    4.5000    0.1464
    4.5100    0.1459
    4.5200    0.1453
    4.5300    0.1448
    4.5400    0.1442
    4.5500    0.1436
    4.5600    0.1431
    4.5700    0.1425
    4.5800    0.1419
    4.5900    0.1413
    4.6000    0.1407
    4.6100    0.1401
    4.6200    0.1395
    4.6300    0.1390
    4.6400    0.1384
    4.6500    0.1378
    4.6600    0.1372
    4.6700    0.1366
    4.6800    0.1360
    4.6900    0.1354
    4.7000    0.1349
    4.7100    0.1343
    4.7200    0.1338
    4.7300    0.1332
    4.7400    0.1327
    4.7500    0.1322
    4.7600    0.1317
    4.7700    0.1312
    4.7800    0.1307
    4.7900    0.1302
    4.8000    0.1297
    4.8100    0.1292
    4.8200    0.1286
    4.8300    0.1281
    4.8400    0.1276
    4.8500    0.1271
    4.8600    0.1267
    4.8700    0.1262
    4.8800    0.1257
    4.8900    0.1252
    4.9000    0.1248
    4.9100    0.1243
    4.9200    0.1239
    4.9300    0.1234
    4.9400    0.1230
    4.9500    0.1226
    4.9600    0.1221
    4.9700    0.1217
    4.9800    0.1212
    4.9900    0.1208
    5.0000    0.1204
    5.0100    0.1199
    5.0200    0.1195
    5.0300    0.1191
    5.0400    0.1187
    5.0500    0.1183
    5.0600    0.1179
    5.0700    0.1176
    5.0800    0.1172
    5.0900    0.1169
    5.1000    0.1165
    5.1100    0.1161
    5.1200    0.1156
    5.1300    0.1152
    5.1400    0.1147
    5.1500    0.1143
    5.1600    0.1138
    5.1700    0.1134
    5.1800    0.1130
    5.1900    0.1126
    5.2000    0.1123
    5.2100    0.1119
    5.2200    0.1115
    5.2300    0.1111
    5.2400    0.1106
    5.2500    0.1102
    5.2600    0.1098
    5.2700    0.1094
    5.2800    0.1090
    5.2900    0.1086
    5.3000    0.1082
    5.3100    0.1078
    5.3200    0.1074
    5.3300    0.1070
    5.3400    0.1066
    5.3500    0.1062
    5.3600    0.1058
    5.3700    0.1053
    5.3800    0.1049
    5.3900    0.1044
    5.4000    0.1040
    5.4100    0.1036
    5.4200    0.1032
    5.4300    0.1028
    5.4400    0.1024
    5.4500    0.1020
    5.4600    0.1017
    5.4700    0.1013
    5.4800    0.1009
    5.4900    0.1005
    5.5000    0.1001
    5.5100    0.0997
    5.5200    0.0993
    5.5300    0.0989
    5.5400    0.0985
    5.5500    0.0981
    5.5600    0.0977
    5.5700    0.0974
    5.5800    0.0970
    5.5900    0.0966
    5.6000    0.0963
    5.6100    0.0959
    5.6200    0.0956
    5.6300    0.0953
    5.6400    0.0950
    5.6500    0.0947
    5.6600    0.0944
    5.6700    0.0941
    5.6800    0.0938
    5.6900    0.0935
    5.7000    0.0932
    5.7100    0.0930
    5.7200    0.0927
    5.7300    0.0925
    5.7400    0.0923
    5.7500    0.0921
    5.7600    0.0918
    5.7700    0.0916
    5.7800    0.0913
    5.7900    0.0910
    5.8000    0.0907
    5.8100    0.0905
    5.8200    0.0902
    5.8300    0.0899
    5.8400    0.0896
    5.8500    0.0893
    5.8600    0.0889
    5.8700    0.0886
    5.8800    0.0883
    5.8900    0.0879
    5.9000    0.0876
    5.9100    0.0872
    5.9200    0.0868
    5.9300    0.0865
    5.9400    0.0861
    5.9500    0.0858
    5.9600    0.0855
    5.9700    0.0851
    5.9800    0.0848
    5.9900    0.0846
    6.0000    0.0843
    6.0100    0.0840
    6.0200    0.0838
    6.0300    0.0836
    6.0400    0.0834
    6.0500    0.0832
    6.0600    0.0830
    6.0700    0.0828
    6.0800    0.0826
    6.0900    0.0824
    6.1000    0.0823
    6.1100    0.0821
    6.1200    0.0820
    6.1300    0.0818
    6.1400    0.0817
    6.1500    0.0815
    6.1600    0.0813
    6.1700    0.0811
    6.1800    0.0810
    6.1900    0.0808
    6.2000    0.0807
    6.2100    0.0806
    6.2200    0.0806
    6.2300    0.0805
    6.2400    0.0804
    6.2500    0.0803
    6.2600    0.0802
    6.2700    0.0801
    6.2800    0.0800
    6.2900    0.0798
    6.3000    0.0797
    6.3100    0.0796
    6.3200    0.0795
    6.3300    0.0793
    6.3400    0.0792
    6.3500    0.0790
    6.3600    0.0788
    6.3700    0.0786
    6.3800    0.0784
    6.3900    0.0781
    6.4000    0.0778
    6.4100    0.0775
    6.4200    0.0772
    6.4300    0.0768
    6.4400    0.0764
    6.4500    0.0760
    6.4600    0.0756
    6.4700    0.0752
    6.4800    0.0749
    6.4900    0.0745
    6.5000    0.0741
    6.5100    0.0737
    6.5200    0.0733
    6.5300    0.0730
    6.5400    0.0726
    6.5500    0.0723
    6.5600    0.0719
    6.5700    0.0716
    6.5800    0.0712
    6.5900    0.0709
    6.6000    0.0705
    6.6100    0.0702
    6.6200    0.0698
    6.6300    0.0694
    6.6400    0.0690
    6.6500    0.0686
    6.6600    0.0682
    6.6700    0.0678
    6.6800    0.0674
    6.6900    0.0670
    6.7000    0.0667
    6.7100    0.0663
    6.7200    0.0660
    6.7300    0.0656
    6.7400    0.0654
    6.7500    0.0651
    6.7600    0.0649
    6.7700    0.0647
    6.7800    0.0645
    6.7900    0.0642
    6.8000    0.0640
    6.8100    0.0638
    6.8200    0.0635
    6.8300    0.0633
    6.8400    0.0630
    6.8500    0.0627
    6.8600    0.0624
    6.8700    0.0622
    6.8800    0.0619
    6.8900    0.0616
    6.9000    0.0613
    6.9100    0.0610
    6.9200    0.0608
    6.9300    0.0605
    6.9400    0.0603
    6.9500    0.0600
    6.9600    0.0597
    6.9700    0.0594
    6.9800    0.0591
    6.9900    0.0588
    7.0000    0.0585
    7.0100    0.0583
    7.0200    0.0580
    7.0300    0.0578
    7.0400    0.0575
    7.0500    0.0573
    7.0600    0.0571
    7.0700    0.0569
    7.0800    0.0567
    7.0900    0.0564
    7.1000    0.0561
    7.1100    0.0558
    7.1200    0.0555
    7.1300    0.0552
    7.1400    0.0549
    7.1500    0.0545
    7.1600    0.0542
    7.1700    0.0539
    7.1800    0.0536
    7.1900    0.0533
    7.2000    0.0530
    7.2100    0.0528
    7.2200    0.0525
    7.2300    0.0522
    7.2400    0.0519
    7.2500    0.0517
    7.2600    0.0514
    7.2700    0.0511
    7.2800    0.0508
    7.2900    0.0505
    7.3000    0.0502
    7.3100    0.0499
    7.3200    0.0496
    7.3300    0.0493
    7.3400    0.0489
    7.3500    0.0485
    7.3600    0.0480
    7.3700    0.0476
    7.3800    0.0472
    7.3900    0.0467
    7.4000    0.0463
    7.4100    0.0459
    7.4200    0.0455
    7.4300    0.0451
    7.4400    0.0447
    7.4500    0.0442
    7.4600    0.0438
    7.4700    0.0434
    7.4800    0.0430
    7.4900    0.0426
    7.5000    0.0422
    7.5100    0.0418
    7.5200    0.0415
    7.5300    0.0411
    7.5400    0.0408
    7.5500    0.0405
    7.5600    0.0402
    7.5700    0.0398
    7.5800    0.0395
    7.5900    0.0392
    7.6000    0.0389
    7.6100    0.0385
    7.6200    0.0382
    7.6300    0.0379
    7.6400    0.0376
    7.6500    0.0373
    7.6600    0.0370
    7.6700    0.0368
    7.6800    0.0365
    7.6900    0.0363
    7.7000    0.0361
    7.7100    0.0358
    7.7200    0.0356
    7.7300    0.0353
    7.7400    0.0351
    7.7500    0.0348
    7.7600    0.0345
    7.7700    0.0343
    7.7800    0.0340
    7.7900    0.0338
    7.8000    0.0335
    7.8100    0.0333
    7.8200    0.0331
    7.8300    0.0329
    7.8400    0.0327
    7.8500    0.0324
    7.8600    0.0322
    7.8700    0.0321
    7.8800    0.0319
    7.8900    0.0318
    7.9000    0.0316
    7.9100    0.0314
    7.9200    0.0312
    7.9300    0.0310
    7.9400    0.0308
    7.9500    0.0307
    7.9600    0.0305
    7.9700    0.0304
    7.9800    0.0303
    7.9900    0.0301
    8.0000    0.0300
    8.0100    0.0300
    8.0200    0.0298
    8.0300    0.0297
    8.0400    0.0296
    8.0500    0.0295
    8.0600    0.0294
    8.0700    0.0293
    8.0800    0.0292
    8.0900    0.0290
    8.1000    0.0289
    8.1100    0.0288
    8.1200    0.0286
    8.1300    0.0285
    8.1400    0.0283
    8.1500    0.0282
    8.1600    0.0280
    8.1700    0.0279
    8.1800    0.0277
    8.1900    0.0275
    8.2000    0.0274
    8.2100    0.0272
    8.2200    0.0270
    8.2300    0.0268
    8.2400    0.0266
    8.2500    0.0264
    8.2600    0.0261
    8.2700    0.0259
    8.2800    0.0257
    8.2900    0.0254
    8.3000    0.0252
    8.3100    0.0250
    8.3200    0.0248
    8.3300    0.0246
    8.3400    0.0244
    8.3500    0.0243
    8.3600    0.0241
    8.3700    0.0239
    8.3800    0.0238
    8.3900    0.0236
    8.4000    0.0234
    8.4100    0.0232
    8.4200    0.0230
    8.4300    0.0229
    8.4400    0.0227
    8.4500    0.0225
    8.4600    0.0223
    8.4700    0.0220
    8.4800    0.0218
    8.4900    0.0216
    8.5000    0.0213
    8.5100    0.0211
    8.5200    0.0208
    8.5300    0.0206
    8.5400    0.0204
    8.5500    0.0202
    8.5600    0.0199
    8.5700    0.0196
    8.5800    0.0193
    8.5900    0.0191
    8.6000    0.0188
    8.6100    0.0186
    8.6200    0.0183
    8.6300    0.0181
    8.6400    0.0178
    8.6500    0.0175
    8.6600    0.0172
    8.6700    0.0169
    8.6800    0.0166
    8.6900    0.0163
    8.7000    0.0159
    8.7100    0.0156
    8.7200    0.0153
    8.7300    0.0150
    8.7400    0.0147
    8.7500    0.0145
    8.7600    0.0142
    8.7700    0.0139
    8.7800    0.0135
    8.7900    0.0132
    8.8000    0.0130
    8.8100    0.0127
    8.8200    0.0125
    8.8300    0.0122
    8.8400    0.0119
    8.8500    0.0117
    8.8600    0.0115
    8.8700    0.0112
    8.8800    0.0109
    8.8900    0.0107
    8.9000    0.0104
    8.9100    0.0101
    8.9200    0.0099
    8.9300    0.0097
    8.9400    0.0095
    8.9500    0.0093
    8.9600    0.0090
    8.9700    0.0088
    8.9800    0.0086
    8.9900    0.0084
    9.0000    0.0082
    9.0100    0.0080
    9.0200    0.0078
    9.0300    0.0076
    9.0400    0.0074
    9.0500    0.0072
    9.0600    0.0071
    9.0700    0.0069
    9.0800    0.0067
    9.0900    0.0065
    9.1000    0.0063
    9.1100    0.0061
    9.1200    0.0060
    9.1300    0.0058
    9.1400    0.0056
    9.1500    0.0054
    9.1600    0.0052
    9.1700    0.0050
    9.1800    0.0047
    9.1900    0.0045
    9.2000    0.0043
    9.2100    0.0042
    9.2200    0.0040
    9.2300    0.0039
    9.2400    0.0038
    9.2500    0.0037
    9.2600    0.0036
    9.2700    0.0035
    9.2800    0.0034
    9.2900    0.0033
    9.3000    0.0032
    9.3100    0.0032
    9.3200    0.0030
    9.3300    0.0030
    9.3400    0.0029
    9.3500    0.0027
    9.3600    0.0026
    9.3700    0.0026
    9.3800    0.0025
    9.3900    0.0024
    9.4000    0.0024
    9.4100    0.0023
    9.4200    0.0023
    9.4300    0.0023
    9.4400    0.0023
    9.4500    0.0022
    9.4600    0.0022
    9.4700    0.0022
    9.4800    0.0022
    9.4900    0.0021
    9.5000    0.0021
    9.5100    0.0020
    9.5200    0.0020
    9.5300    0.0019
    9.5400    0.0018
    9.5500    0.0018
    9.5600    0.0018
    9.5700    0.0017
    9.5800    0.0017
    9.5900    0.0018
    9.6000    0.0018
    9.6100    0.0019
    9.6200    0.0019
    9.6300    0.0019
    9.6400    0.0019
    9.6500    0.0020
    9.6600    0.0020
    9.6700    0.0020
    9.6800    0.0021
    9.6900    0.0022
    9.7000    0.0022
    9.7100    0.0023
    9.7200    0.0023
    9.7300    0.0024
    9.7400    0.0024
    9.7500    0.0025
    9.7600    0.0026
    9.7700    0.0027
    9.7800    0.0028
    9.7900    0.0029
    9.8000    0.0031
    9.8100    0.0032
    9.8200    0.0034
    9.8300    0.0035
    9.8400    0.0037
    9.8500    0.0039
    9.8600    0.0041
    9.8700    0.0043
    9.8800    0.0044
    9.8900    0.0046
    9.9000    0.0047
    9.9100    0.0048
    9.9200    0.0049
    9.9300    0.0049
    9.9400    0.0050
    9.9500    0.0051
    9.9600    0.0053
    9.9700    0.0054
    9.9800    0.0055
    9.9900    0.0057
    10.0000    0.0058
};


==> Data/Oscillator/sigma3/x_tr_vel.tex <==
    \addplot[
    thick,
    red
    ]
    table {
    0   -0.1266
    0.0100   -0.1280
    0.0200   -0.1324
    0.0300   -0.1378
    0.0400   -0.1401
    0.0500   -0.1448
    0.0600   -0.1501
    0.0700   -0.1535
    0.0800   -0.1523
    0.0900   -0.1484
    0.1000   -0.1501
    0.1100   -0.1514
    0.1200   -0.1504
    0.1300   -0.1529
    0.1400   -0.1552
    0.1500   -0.1576
    0.1600   -0.1609
    0.1700   -0.1621
    0.1800   -0.1617
    0.1900   -0.1613
    0.2000   -0.1617
    0.2100   -0.1650
    0.2200   -0.1681
    0.2300   -0.1679
    0.2400   -0.1681
    0.2500   -0.1688
    0.2600   -0.1693
    0.2700   -0.1712
    0.2800   -0.1735
    0.2900   -0.1762
    0.3000   -0.1782
    0.3100   -0.1805
    0.3200   -0.1849
    0.3300   -0.1888
    0.3400   -0.1946
    0.3500   -0.1977
    0.3600   -0.1971
    0.3700   -0.1990
    0.3800   -0.1995
    0.3900   -0.2012
    0.4000   -0.2043
    0.4100   -0.2058
    0.4200   -0.2067
    0.4300   -0.2070
    0.4400   -0.2085
    0.4500   -0.2103
    0.4600   -0.2113
    0.4700   -0.2116
    0.4800   -0.2104
    0.4900   -0.2087
    0.5000   -0.2092
    0.5100   -0.2107
    0.5200   -0.2127
    0.5300   -0.2158
    0.5400   -0.2175
    0.5500   -0.2162
    0.5600   -0.2157
    0.5700   -0.2166
    0.5800   -0.2168
    0.5900   -0.2161
    0.6000   -0.2164
    0.6100   -0.2178
    0.6200   -0.2174
    0.6300   -0.2158
    0.6400   -0.2132
    0.6500   -0.2117
    0.6600   -0.2135
    0.6700   -0.2163
    0.6800   -0.2184
    0.6900   -0.2170
    0.7000   -0.2152
    0.7100   -0.2152
    0.7200   -0.2146
    0.7300   -0.2140
    0.7400   -0.2139
    0.7500   -0.2164
    0.7600   -0.2195
    0.7700   -0.2203
    0.7800   -0.2198
    0.7900   -0.2200
    0.8000   -0.2184
    0.8100   -0.2164
    0.8200   -0.2157
    0.8300   -0.2135
    0.8400   -0.2126
    0.8500   -0.2126
    0.8600   -0.2108
    0.8700   -0.2100
    0.8800   -0.2100
    0.8900   -0.2109
    0.9000   -0.2133
    0.9100   -0.2142
    0.9200   -0.2130
    0.9300   -0.2090
    0.9400   -0.2067
    0.9500   -0.2071
    0.9600   -0.2068
    0.9700   -0.2089
    0.9800   -0.2112
    0.9900   -0.2133
    1.0000   -0.2139
    1.0100   -0.2135
    1.0200   -0.2139
    1.0300   -0.2138
    1.0400   -0.2136
    1.0500   -0.2133
    1.0600   -0.2129
    1.0700   -0.2110
    1.0800   -0.2077
    1.0900   -0.2056
    1.1000   -0.2077
    1.1100   -0.2105
    1.1200   -0.2093
    1.1300   -0.2084
    1.1400   -0.2080
    1.1500   -0.2062
    1.1600   -0.2039
    1.1700   -0.2040
    1.1800   -0.2058
    1.1900   -0.2067
    1.2000   -0.2042
    1.2100   -0.1995
    1.2200   -0.1966
    1.2300   -0.1958
    1.2400   -0.1971
    1.2500   -0.1974
    1.2600   -0.1960
    1.2700   -0.1946
    1.2800   -0.1937
    1.2900   -0.1948
    1.3000   -0.1969
    1.3100   -0.1976
    1.3200   -0.1997
    1.3300   -0.2001
    1.3400   -0.1985
    1.3500   -0.1975
    1.3600   -0.1982
    1.3700   -0.1977
    1.3800   -0.1953
    1.3900   -0.1946
    1.4000   -0.1942
    1.4100   -0.1938
    1.4200   -0.1953
    1.4300   -0.1967
    1.4400   -0.1971
    1.4500   -0.1983
    1.4600   -0.1997
    1.4700   -0.2006
    1.4800   -0.2024
    1.4900   -0.2024
    1.5000   -0.1997
    1.5100   -0.1981
    1.5200   -0.1971
    1.5300   -0.1970
    1.5400   -0.1957
    1.5500   -0.1937
    1.5600   -0.1937
    1.5700   -0.1920
    1.5800   -0.1898
    1.5900   -0.1898
    1.6000   -0.1898
    1.6100   -0.1901
    1.6200   -0.1913
    1.6300   -0.1887
    1.6400   -0.1831
    1.6500   -0.1801
    1.6600   -0.1804
    1.6700   -0.1820
    1.6800   -0.1823
    1.6900   -0.1807
    1.7000   -0.1805
    1.7100   -0.1836
    1.7200   -0.1868
    1.7300   -0.1870
    1.7400   -0.1851
    1.7500   -0.1831
    1.7600   -0.1817
    1.7700   -0.1806
    1.7800   -0.1800
    1.7900   -0.1786
    1.8000   -0.1782
    1.8100   -0.1782
    1.8200   -0.1776
    1.8300   -0.1779
    1.8400   -0.1767
    1.8500   -0.1739
    1.8600   -0.1731
    1.8700   -0.1720
    1.8800   -0.1690
    1.8900   -0.1675
    1.9000   -0.1670
    1.9100   -0.1666
    1.9200   -0.1664
    1.9300   -0.1659
    1.9400   -0.1650
    1.9500   -0.1632
    1.9600   -0.1598
    1.9700   -0.1569
    1.9800   -0.1560
    1.9900   -0.1549
    2.0000   -0.1535
    2.0100   -0.1538
    2.0200   -0.1533
    2.0300   -0.1513
    2.0400   -0.1503
    2.0500   -0.1490
    2.0600   -0.1477
    2.0700   -0.1479
    2.0800   -0.1486
    2.0900   -0.1484
    2.1000   -0.1486
    2.1100   -0.1468
    2.1200   -0.1454
    2.1300   -0.1464
    2.1400   -0.1471
    2.1500   -0.1486
    2.1600   -0.1495
    2.1700   -0.1493
    2.1800   -0.1472
    2.1900   -0.1452
    2.2000   -0.1460
    2.2100   -0.1448
    2.2200   -0.1410
    2.2300   -0.1394
    2.2400   -0.1408
    2.2500   -0.1424
    2.2600   -0.1425
    2.2700   -0.1417
    2.2800   -0.1411
    2.2900   -0.1403
    2.3000   -0.1388
    2.3100   -0.1392
    2.3200   -0.1410
    2.3300   -0.1422
    2.3400   -0.1429
    2.3500   -0.1430
    2.3600   -0.1426
    2.3700   -0.1452
    2.3800   -0.1482
    2.3900   -0.1463
    2.4000   -0.1452
    2.4100   -0.1445
    2.4200   -0.1422
    2.4300   -0.1410
    2.4400   -0.1400
    2.4500   -0.1407
    2.4600   -0.1417
    2.4700   -0.1391
    2.4800   -0.1364
    2.4900   -0.1355
    2.5000   -0.1356
    2.5100   -0.1357
    2.5200   -0.1347
    2.5300   -0.1332
    2.5400   -0.1324
    2.5500   -0.1324
    2.5600   -0.1297
    2.5700   -0.1293
    2.5800   -0.1286
    2.5900   -0.1252
    2.6000   -0.1232
    2.6100   -0.1234
    2.6200   -0.1253
    2.6300   -0.1257
    2.6400   -0.1249
    2.6500   -0.1257
    2.6600   -0.1263
    2.6700   -0.1265
    2.6800   -0.1270
    2.6900   -0.1255
    2.7000   -0.1237
    2.7100   -0.1215
    2.7200   -0.1186
    2.7300   -0.1177
    2.7400   -0.1176
    2.7500   -0.1179
    2.7600   -0.1198
    2.7700   -0.1197
    2.7800   -0.1180
    2.7900   -0.1175
    2.8000   -0.1160
    2.8100   -0.1138
    2.8200   -0.1123
    2.8300   -0.1100
    2.8400   -0.1073
    2.8500   -0.1056
    2.8600   -0.1059
    2.8700   -0.1070
    2.8800   -0.1061
    2.8900   -0.1062
    2.9000   -0.1077
    2.9100   -0.1094
    2.9200   -0.1100
    2.9300   -0.1074
    2.9400   -0.1060
    2.9500   -0.1057
    2.9600   -0.1082
    2.9700   -0.1098
    2.9800   -0.1110
    2.9900   -0.1154
    3.0000   -0.1171
    3.0100   -0.1173
    3.0200   -0.1171
    3.0300   -0.1151
    3.0400   -0.1126
    3.0500   -0.1117
    3.0600   -0.1113
    3.0700   -0.1100
    3.0800   -0.1083
    3.0900   -0.1062
    3.1000   -0.1041
    3.1100   -0.1027
    3.1200   -0.1025
    3.1300   -0.1011
    3.1400   -0.1019
    3.1500   -0.1043
    3.1600   -0.1057
    3.1700   -0.1069
    3.1800   -0.1059
    3.1900   -0.1036
    3.2000   -0.1033
    3.2100   -0.1043
    3.2200   -0.1040
    3.2300   -0.1036
    3.2400   -0.1029
    3.2500   -0.1015
    3.2600   -0.1015
    3.2700   -0.1022
    3.2800   -0.1041
    3.2900   -0.1045
    3.3000   -0.1032
    3.3100   -0.1045
    3.3200   -0.1054
    3.3300   -0.1065
    3.3400   -0.1072
    3.3500   -0.1070
    3.3600   -0.1044
    3.3700   -0.0999
    3.3800   -0.1008
    3.3900   -0.1023
    3.4000   -0.1026
    3.4100   -0.1037
    3.4200   -0.1029
    3.4300   -0.1011
    3.4400   -0.0998
    3.4500   -0.0977
    3.4600   -0.0958
    3.4700   -0.0953
    3.4800   -0.0936
    3.4900   -0.0922
    3.5000   -0.0906
    3.5100   -0.0887
    3.5200   -0.0888
    3.5300   -0.0912
    3.5400   -0.0905
    3.5500   -0.0886
    3.5600   -0.0886
    3.5700   -0.0874
    3.5800   -0.0862
    3.5900   -0.0866
    3.6000   -0.0876
    3.6100   -0.0878
    3.6200   -0.0857
    3.6300   -0.0846
    3.6400   -0.0842
    3.6500   -0.0825
    3.6600   -0.0821
    3.6700   -0.0831
    3.6800   -0.0841
    3.6900   -0.0840
    3.7000   -0.0853
    3.7100   -0.0862
    3.7200   -0.0863
    3.7300   -0.0867
    3.7400   -0.0858
    3.7500   -0.0859
    3.7600   -0.0866
    3.7700   -0.0859
    3.7800   -0.0870
    3.7900   -0.0872
    3.8000   -0.0827
    3.8100   -0.0784
    3.8200   -0.0773
    3.8300   -0.0768
    3.8400   -0.0771
    3.8500   -0.0757
    3.8600   -0.0723
    3.8700   -0.0701
    3.8800   -0.0700
    3.8900   -0.0704
    3.9000   -0.0704
    3.9100   -0.0711
    3.9200   -0.0718
    3.9300   -0.0733
    3.9400   -0.0750
    3.9500   -0.0758
    3.9600   -0.0775
    3.9700   -0.0782
    3.9800   -0.0771
    3.9900   -0.0760
    4.0000   -0.0744
    4.0100   -0.0732
    4.0200   -0.0738
    4.0300   -0.0762
    4.0400   -0.0773
    4.0500   -0.0771
    4.0600   -0.0751
    4.0700   -0.0737
    4.0800   -0.0722
    4.0900   -0.0698
    4.1000   -0.0676
    4.1100   -0.0659
    4.1200   -0.0662
    4.1300   -0.0683
    4.1400   -0.0694
    4.1500   -0.0679
    4.1600   -0.0670
    4.1700   -0.0676
    4.1800   -0.0682
    4.1900   -0.0693
    4.2000   -0.0706
    4.2100   -0.0709
    4.2200   -0.0706
    4.2300   -0.0701
    4.2400   -0.0690
    4.2500   -0.0678
    4.2600   -0.0653
    4.2700   -0.0626
    4.2800   -0.0600
    4.2900   -0.0586
    4.3000   -0.0586
    4.3100   -0.0581
    4.3200   -0.0576
    4.3300   -0.0561
    4.3400   -0.0578
    4.3500   -0.0615
    4.3600   -0.0642
    4.3700   -0.0650
    4.3800   -0.0625
    4.3900   -0.0609
    4.4000   -0.0601
    4.4100   -0.0583
    4.4200   -0.0586
    4.4300   -0.0591
    4.4400   -0.0592
    4.4500   -0.0581
    4.4600   -0.0562
    4.4700   -0.0542
    4.4800   -0.0528
    4.4900   -0.0525
    4.5000   -0.0518
    4.5100   -0.0540
    4.5200   -0.0571
    4.5300   -0.0573
    4.5400   -0.0564
    4.5500   -0.0575
    4.5600   -0.0591
    4.5700   -0.0592
    4.5800   -0.0596
    4.5900   -0.0593
    4.6000   -0.0586
    4.6100   -0.0569
    4.6200   -0.0558
    4.6300   -0.0565
    4.6400   -0.0577
    4.6500   -0.0598
    4.6600   -0.0608
    4.6700   -0.0606
    4.6800   -0.0586
    4.6900   -0.0569
    4.7000   -0.0566
    4.7100   -0.0558
    4.7200   -0.0537
    4.7300   -0.0524
    4.7400   -0.0514
    4.7500   -0.0501
    4.7600   -0.0506
    4.7700   -0.0506
    4.7800   -0.0503
    4.7900   -0.0515
    4.8000   -0.0517
    4.8100   -0.0516
    4.8200   -0.0518
    4.8300   -0.0510
    4.8400   -0.0490
    4.8500   -0.0479
    4.8600   -0.0476
    4.8700   -0.0473
    4.8800   -0.0472
    4.8900   -0.0463
    4.9000   -0.0463
    4.9100   -0.0465
    4.9200   -0.0454
    4.9300   -0.0445
    4.9400   -0.0424
    4.9500   -0.0412
    4.9600   -0.0426
    4.9700   -0.0453
    4.9800   -0.0461
    4.9900   -0.0440
    5.0000   -0.0430
    5.0100   -0.0420
    5.0200   -0.0407
    5.0300   -0.0402
    5.0400   -0.0397
    5.0500   -0.0391
    5.0600   -0.0385
    5.0700   -0.0354
    5.0800   -0.0337
    5.0900   -0.0372
    5.1000   -0.0405
    5.1100   -0.0429
    5.1200   -0.0445
    5.1300   -0.0450
    5.1400   -0.0452
    5.1500   -0.0446
    5.1600   -0.0434
    5.1700   -0.0420
    5.1800   -0.0391
    5.1900   -0.0357
    5.2000   -0.0359
    5.2100   -0.0399
    5.2200   -0.0414
    5.2300   -0.0423
    5.2400   -0.0441
    5.2500   -0.0437
    5.2600   -0.0410
    5.2700   -0.0385
    5.2800   -0.0391
    5.2900   -0.0393
    5.3000   -0.0387
    5.3100   -0.0383
    5.3200   -0.0388
    5.3300   -0.0407
    5.3400   -0.0416
    5.3500   -0.0425
    5.3600   -0.0449
    5.3700   -0.0443
    5.3800   -0.0430
    5.3900   -0.0434
    5.4000   -0.0423
    5.4100   -0.0414
    5.4200   -0.0404
    5.4300   -0.0395
    5.4400   -0.0386
    5.4500   -0.0366
    5.4600   -0.0361
    5.4700   -0.0372
    5.4800   -0.0392
    5.4900   -0.0405
    5.5000   -0.0411
    5.5100   -0.0418
    5.5200   -0.0409
    5.5300   -0.0399
    5.5400   -0.0387
    5.5500   -0.0379
    5.5600   -0.0372
    5.5700   -0.0366
    5.5800   -0.0369
    5.5900   -0.0355
    5.6000   -0.0348
    5.6100   -0.0356
    5.6200   -0.0338
    5.6300   -0.0305
    5.6400   -0.0300
    5.6500   -0.0298
    5.6600   -0.0295
    5.6700   -0.0292
    5.6800   -0.0269
    5.6900   -0.0272
    5.7000   -0.0280
    5.7100   -0.0253
    5.7200   -0.0238
    5.7300   -0.0221
    5.7400   -0.0202
    5.7500   -0.0217
    5.7600   -0.0258
    5.7700   -0.0287
    5.7800   -0.0283
    5.7900   -0.0273
    5.8000   -0.0265
    5.8100   -0.0268
    5.8200   -0.0274
    5.8300   -0.0291
    5.8400   -0.0318
    5.8500   -0.0335
    5.8600   -0.0337
    5.8700   -0.0330
    5.8800   -0.0342
    5.8900   -0.0353
    5.9000   -0.0359
    5.9100   -0.0372
    5.9200   -0.0368
    5.9300   -0.0354
    5.9400   -0.0347
    5.9500   -0.0331
    5.9600   -0.0318
    5.9700   -0.0309
    5.9800   -0.0294
    5.9900   -0.0274
    6.0000   -0.0256
    6.0100   -0.0236
    6.0200   -0.0221
    6.0300   -0.0223
    6.0400   -0.0207
    6.0500   -0.0196
    6.0600   -0.0204
    6.0700   -0.0196
    6.0800   -0.0186
    6.0900   -0.0172
    6.1000   -0.0148
    6.1100   -0.0137
    6.1200   -0.0146
    6.1300   -0.0152
    6.1400   -0.0165
    6.1500   -0.0181
    6.1600   -0.0172
    6.1700   -0.0163
    6.1800   -0.0154
    6.1900   -0.0126
    6.2000   -0.0097
    6.2100   -0.0089
    6.2200   -0.0085
    6.2300   -0.0078
    6.2400   -0.0094
    6.2500   -0.0118
    6.2600   -0.0113
    6.2700   -0.0105
    6.2800   -0.0104
    6.2900   -0.0113
    6.3000   -0.0128
    6.3100   -0.0125
    6.3200   -0.0137
    6.3300   -0.0152
    6.3400   -0.0154
    6.3500   -0.0170
    6.3600   -0.0183
    6.3700   -0.0207
    6.3800   -0.0253
    6.3900   -0.0289
    6.4000   -0.0312
    6.4100   -0.0335
    6.4200   -0.0364
    6.4300   -0.0377
    6.4400   -0.0388
    6.4500   -0.0400
    6.4600   -0.0386
    6.4700   -0.0373
    6.4800   -0.0369
    6.4900   -0.0368
    6.5000   -0.0385
    6.5100   -0.0398
    6.5200   -0.0383
    6.5300   -0.0349
    6.5400   -0.0332
    6.5500   -0.0352
    6.5600   -0.0365
    6.5700   -0.0355
    6.5800   -0.0350
    6.5900   -0.0362
    6.6000   -0.0348
    6.6100   -0.0349
    6.6200   -0.0377
    6.6300   -0.0393
    6.6400   -0.0409
    6.6500   -0.0407
    6.6600   -0.0397
    6.6700   -0.0399
    6.6800   -0.0393
    6.6900   -0.0372
    6.7000   -0.0354
    6.7100   -0.0347
    6.7200   -0.0337
    6.7300   -0.0314
    6.7400   -0.0277
    6.7500   -0.0236
    6.7600   -0.0211
    6.7700   -0.0197
    6.7800   -0.0212
    6.7900   -0.0230
    6.8000   -0.0242
    6.8100   -0.0256
    6.8200   -0.0254
    6.8300   -0.0253
    6.8400   -0.0268
    6.8500   -0.0281
    6.8600   -0.0285
    6.8700   -0.0280
    6.8800   -0.0284
    6.8900   -0.0288
    6.9000   -0.0281
    6.9100   -0.0264
    6.9200   -0.0250
    6.9300   -0.0252
    6.9400   -0.0265
    6.9500   -0.0291
    6.9600   -0.0300
    6.9700   -0.0297
    6.9800   -0.0291
    6.9900   -0.0292
    7.0000   -0.0278
    7.0100   -0.0253
    7.0200   -0.0239
    7.0300   -0.0228
    7.0400   -0.0232
    7.0500   -0.0225
    7.0600   -0.0210
    7.0700   -0.0216
    7.0800   -0.0244
    7.0900   -0.0271
    7.1000   -0.0297
    7.1100   -0.0308
    7.1200   -0.0308
    7.1300   -0.0313
    7.1400   -0.0329
    7.1500   -0.0331
    7.1600   -0.0313
    7.1700   -0.0305
    7.1800   -0.0291
    7.1900   -0.0286
    7.2000   -0.0288
    7.2100   -0.0276
    7.2200   -0.0266
    7.2300   -0.0267
    7.2400   -0.0269
    7.2500   -0.0268
    7.2600   -0.0281
    7.2700   -0.0301
    7.2800   -0.0298
    7.2900   -0.0293
    7.3000   -0.0300
    7.3100   -0.0311
    7.3200   -0.0324
    7.3300   -0.0358
    7.3400   -0.0400
    7.3500   -0.0420
    7.3600   -0.0439
    7.3700   -0.0445
    7.3800   -0.0442
    7.3900   -0.0416
    7.4000   -0.0393
    7.4100   -0.0395
    7.4200   -0.0408
    7.4300   -0.0423
    7.4400   -0.0435
    7.4500   -0.0440
    7.4600   -0.0422
    7.4700   -0.0400
    7.4800   -0.0396
    7.4900   -0.0414
    7.5000   -0.0408
    7.5100   -0.0361
    7.5200   -0.0331
    7.5300   -0.0335
    7.5400   -0.0326
    7.5500   -0.0314
    7.5600   -0.0321
    7.5700   -0.0310
    7.5800   -0.0311
    7.5900   -0.0342
    7.6000   -0.0353
    7.6100   -0.0337
    7.6200   -0.0326
    7.6300   -0.0313
    7.6400   -0.0290
    7.6500   -0.0263
    7.6600   -0.0254
    7.6700   -0.0248
    7.6800   -0.0233
    7.6900   -0.0234
    7.7000   -0.0249
    7.7100   -0.0251
    7.7200   -0.0244
    7.7300   -0.0244
    7.7400   -0.0248
    7.7500   -0.0270
    7.7600   -0.0281
    7.7700   -0.0274
    7.7800   -0.0257
    7.7900   -0.0231
    7.8000   -0.0207
    7.8100   -0.0201
    7.8200   -0.0217
    7.8300   -0.0238
    7.8400   -0.0243
    7.8500   -0.0202
    7.8600   -0.0161
    7.8700   -0.0160
    7.8800   -0.0157
    7.8900   -0.0159
    7.9000   -0.0186
    7.9100   -0.0191
    7.9200   -0.0189
    7.9300   -0.0192
    7.9400   -0.0170
    7.9500   -0.0148
    7.9600   -0.0132
    7.9700   -0.0139
    7.9800   -0.0148
    7.9900   -0.0116
    8.0000   -0.0086
    8.0100   -0.0097
    8.0200   -0.0117
    8.0300   -0.0124
    8.0400   -0.0124
    8.0500   -0.0115
    8.0600   -0.0105
    8.0700   -0.0105
    8.0800   -0.0115
    8.0900   -0.0128
    8.1000   -0.0124
    8.1100   -0.0134
    8.1200   -0.0156
    8.1300   -0.0153
    8.1400   -0.0156
    8.1500   -0.0156
    8.1600   -0.0149
    8.1700   -0.0159
    8.1800   -0.0166
    8.1900   -0.0165
    8.2000   -0.0170
    8.2100   -0.0180
    8.2200   -0.0184
    8.2300   -0.0201
    8.2400   -0.0222
    8.2500   -0.0229
    8.2600   -0.0241
    8.2700   -0.0239
    8.2800   -0.0235
    8.2900   -0.0233
    8.3000   -0.0212
    8.3100   -0.0199
    8.3200   -0.0194
    8.3300   -0.0181
    8.3400   -0.0172
    8.3500   -0.0164
    8.3600   -0.0170
    8.3700   -0.0169
    8.3800   -0.0165
    8.3900   -0.0193
    8.4000   -0.0195
    8.4100   -0.0177
    8.4200   -0.0170
    8.4300   -0.0166
    8.4400   -0.0178
    8.4500   -0.0221
    8.4600   -0.0243
    8.4700   -0.0234
    8.4800   -0.0235
    8.4900   -0.0228
    8.5000   -0.0234
    8.5100   -0.0253
    8.5200   -0.0243
    8.5300   -0.0219
    8.5400   -0.0222
    8.5500   -0.0256
    8.5600   -0.0281
    8.5700   -0.0278
    8.5800   -0.0259
    8.5900   -0.0242
    8.6000   -0.0248
    8.6100   -0.0252
    8.6200   -0.0256
    8.6300   -0.0273
    8.6400   -0.0285
    8.6500   -0.0299
    8.6600   -0.0308
    8.6700   -0.0314
    8.6800   -0.0319
    8.6900   -0.0320
    8.7000   -0.0321
    8.7100   -0.0323
    8.7200   -0.0307
    8.7300   -0.0279
    8.7400   -0.0265
    8.7500   -0.0274
    8.7600   -0.0302
    8.7700   -0.0334
    8.7800   -0.0318
    8.7900   -0.0271
    8.8000   -0.0250
    8.8100   -0.0252
    8.8200   -0.0269
    8.8300   -0.0269
    8.8400   -0.0239
    8.8500   -0.0235
    8.8600   -0.0252
    8.8700   -0.0252
    8.8800   -0.0268
    8.8900   -0.0274
    8.9000   -0.0262
    8.9100   -0.0239
    8.9200   -0.0216
    8.9300   -0.0211
    8.9400   -0.0214
    8.9500   -0.0228
    8.9600   -0.0242
    8.9700   -0.0244
    8.9800   -0.0219
    8.9900   -0.0205
    9.0000   -0.0202
    9.0100   -0.0198
    9.0200   -0.0197
    9.0300   -0.0177
    9.0400   -0.0159
    9.0500   -0.0165
    9.0600   -0.0181
    9.0700   -0.0188
    9.0800   -0.0187
    9.0900   -0.0194
    9.1000   -0.0196
    9.1100   -0.0175
    9.1200   -0.0159
    9.1300   -0.0160
    9.1400   -0.0183
    9.1500   -0.0210
    9.1600   -0.0229
    9.1700   -0.0242
    9.1800   -0.0234
    9.1900   -0.0205
    9.2000   -0.0162
    9.2100   -0.0140
    9.2200   -0.0141
    9.2300   -0.0131
    9.2400   -0.0114
    9.2500   -0.0097
    9.2600   -0.0077
    9.2700   -0.0083
    9.2800   -0.0091
    9.2900   -0.0084
    9.3000   -0.0091
    9.3100   -0.0105
    9.3200   -0.0095
    9.3300   -0.0088
    9.3400   -0.0108
    9.3500   -0.0116
    9.3600   -0.0089
    9.3700   -0.0064
    9.3800   -0.0059
    9.3900   -0.0064
    9.4000   -0.0054
    9.4100   -0.0033
    9.4200   -0.0025
    9.4300   -0.0029
    9.4400   -0.0030
    9.4500   -0.0015
    9.4600   -0.0024
    9.4700   -0.0035
    9.4800   -0.0039
    9.4900   -0.0042
    9.5000   -0.0042
    9.5100   -0.0046
    9.5200   -0.0059
    9.5300   -0.0072
    9.5400   -0.0065
    9.5500   -0.0036
    9.5600   -0.0028
    9.5700   -0.0014
    9.5800    0.0029
    9.5900    0.0047
    9.6000    0.0044
    9.6100    0.0031
    9.6200    0.0031
    9.6300    0.0032
    9.6400    0.0018
    9.6500    0.0022
    9.6600    0.0036
    9.6700    0.0049
    9.6800    0.0063
    9.6900    0.0062
    9.7000    0.0050
    9.7100    0.0051
    9.7200    0.0051
    9.7300    0.0055
    9.7400    0.0075
    9.7500    0.0084
    9.7600    0.0085
    9.7700    0.0086
    9.7800    0.0126
    9.7900    0.0160
    9.8000    0.0136
    9.8100    0.0136
    9.8200    0.0159
    9.8300    0.0154
    9.8400    0.0171
    9.8500    0.0200
    9.8600    0.0203
    9.8700    0.0191
    9.8800    0.0165
    9.8900    0.0128
    9.9000    0.0100
    9.9100    0.0080
    9.9200    0.0073
    9.9300    0.0074
    9.9400    0.0087
    9.9500    0.0120
    9.9600    0.0135
    9.9700    0.0129
    9.9800    0.0134
    9.9900    0.0130
   10.0000    0.0120 
};
